Fragmentation and optimal liquidity supply on decentralized exchanges

We investigate how liquidity providers (LPs) choose between high- and low-fee trading venues, in the face of a fixed common gas cost. Analyzing Uniswap data, we find that high-fee pools attract 58% of liquidity supply yet execute only 21% of volume. Large LPs dominate low-fee pools, frequently adjusting out-of-range positions in response to informed order flow. In contrast, small LPs converge to high-fee pools, accepting lower execution probabilities to mitigate adverse selection and liquidity management costs. Fragmented liquidity dominates a single-fee market, as it encourages more liquidity providers to enter the market, while fostering LP competition on the low-fee pool.

==> Old/data_202307.tex <==
\subsection{Sample construction \label{sec:sample}}
We obtain data from Kaiko on all trades, liquidity deposits (``mints''), and liquidity withdrawals (``burns'') on 1,361 Uniswap v3 pools from the launch of the protocol on May 4, 2021 until September 15, 2022 -- that is, the date when the Ethereum blockchain replaced its proof-of-work protocol with a proof-of-stake one. Our data includes a transaction hash that identifies each trade and liquidity update on the Ethereum blockchain; trade price, direction, and quantity; as well as quantities and price range for each liquidity update.

Further, we collect data from Blockchair on the wallet addresses that initiate each transaction (i.e., akin to an anonymous trader id), the position of each transaction in its block, as well as the gas price limit set by the trader and the amount of gas used -- in Ether as well as US dollars. Finally, we use the Kaiko ``Cross-Price'' API to collect token prices in US dollars. For each token, we obtain the volume-weighted average price at minute and day frequencies, using data from all major centralized and decentralized exchanges. If a particular token does not directly trade against U.S. dollars, Kaiko computes the benchmark price across the most liquid trading path (usually first converting the token to BTC or ETH, and then to U.S. dollars). 

% We obtain data from Kaiko on all trades and liquidity updates on 1,361 Uniswap v3 pools in 881 asset pairs from May 4, 2021 to September 15, 2022 -- that is, from the launch of the platform until Ethereum's transition to a Proof-of-Stake protocol.\footnote{There are virtually no restrictions to create a liquidity pool on Uniswap for any pair of ERC-20 tokens. Throughout our sample, a total of 8,167 Uniswap v3 pools were created for 6,535 asset pairs. Kaiko filters out most of these pools in their trade data set -- either because the trading volume is zero, or because tokens are labelled as untrustworthy (including scams or clones).}

There are no restrictions to list a token pair on Uniswap. Some pools might therefore be used for experiments, or they might include untrustworthy tokens. Following \citet{LeharParlour2021}, we remove pools that are either very small or that are not attracting an economically meaningful trading volume. We retain liquidity pools that fulfill the following four criteria: (i) have at least one interaction in more than 30 days in the sample, (ii) have more than 100 liquidity interactions throughout the sample, (iii) have an average daily liquidity balance in excess of US\$100,000, and (iv) capture more than 1\% of trading volume for a particular asset pair.

These basic screens give us a baseline sample of 262 liquidity pools covering 224 asset pairs, with combined daily dollar volume of \$1.32 billion and total value locked (i.e., aggregate liquidity supply) of \$3.07 billion as of September 15, 2022. We capture 13,006,390 interactions with liquidity pool smart contracts (accounting for 87.56\% of the entire universe of trades and liquidity updates). Trading and liquidity provision on Uniswap is heavily concentrated: the five largest pairs (USDC-WETH, WETH-USDT, WBTC-WETH, USDC-USDT, and DAI-WETH) account on average for 81\% of trading volume and 52\% of supplied liquidity.\footnote{WETH and WBTC stand for ``wrapped'' Bitcoin and Ether. Plain vanilla Bitcon and Ether are not compliant with the ERC-20 standard for tokens, and therefore cannot be directly used on decentralized exchanges' smart contracts. USDC (USD Coin), USDT (Tether), and DAI are stablecoins meant to closely track the US dollar.}


\subsection{Liquidity fragmentation patterns}

For 37 out of the 224 asset pairs in our baseline sample, liquidity supply is fragmented across two pools with different fees -- either with 1 and 5 bps fees (7 pairs), 5 and 30 bps fees (8 pairs), or 30 and 100 bps fees (22 pairs).\footnote{In some cases, more than two pools are created for a pair -- e.g., for USDC-WETH there are four pools with 1, 5, 30, and 100 bps liquidity fees. In all but one case however, two pools heavily dominate the others. As described in Section \ref{sec:sample} we filter out small pools with less than 1\% volume share or less than \$100,000 liquidity deposits. The exception is FEI-USDC, for which three pools attract significant volume throughout the sample. However, on any given day two pools remain dominant: either the 5 and 30 bps fee pools before the launch of the 1 bps pool, and the 1 and 5 bps fee pool afterwards.} Despite being fewer in number, fragmented pairs are economically important: they account on average for 84\% of the capital committed to Uniswap v3 and for 94\% of its dollar trading volume. All major token pairs such as WETH-USDC, WETH-USDT, or WBTC-WETH trade on fragmented pools.

For each fragmented liquidity pair, we label the \emph{low} and the \emph{high} fee liquidity pool to facilitate analysis across assets. For example, the low and high liquidity fees for USDC-WETH are 5 and 30 bps, respectively, but only 1 and 5 bps for a lower volatility pair such as USDC-USDT. We refer to non-fragmented pools as \emph{single} (i.e., the unique pool for an asset pair).

We aggregate all interactions with Uniswap smart contracts into a panel across days and liquidity pools. To compute the end-of-day pool size, we account for all changes in token balances, across all price ranges. There are three possible interactions: A deposit or ``mint'' adds tokens to the pool, a withdrawal or ``burn'' removes tokens, whereas a trade or ``swap'' adds one token and removes the other. We track these changes across to obtain daily variation in the quantity of tokens on each pool. We compute the end-of-day pool size as the cumulative sum of daily changes in token balance, marked to market in US dollars at end-of-day prices.\footnote{Since we track all pools since inception, the initial balance is set to zero.} Intra-day trades and liquidity mint volumes are converted in US dollars using the price of the corresponding minute. 

Table \ref{tab:sumstat} reports summary statistics across pools with different fee levels. High-fee pools attract on average more liquidity than their low-fee counterparts (\$43.42 million and \$31.35 million, respectively), but only capture 36.66\% percent of the trading volume. Consistent with our theoretical predictions, low-fee pools attract five times as many trades as high-fee competitors (577 versus 111 average trade count per day).  At the same time, the average trade on a high-fee pool is twice as large (\$22,460) than on a low-fee pool (\$9,890). 

The distribution of mint sizes is heavily skewed to the right, with 6.5\% of deposits exceeding \$1 million. There are large differences across pools -- the median $\LP$ deposit on the low-fee pool is \$22,780, twice as much as the median deposit on the high-fee pool (\$10,590). At the same time, the number of liquidity providers on high-fee pools is 91\% higher than on low-fee pools (12.48 unique addresses per day on high-fee pools versus only 6.52 unique address on high-fee pools).




% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: Fri, Oct 21, 2022 - 4:01:40 PM
\begin{table}[H] \centering 
\caption{Descriptive statistics} 
  \label{tab:sumstat} 

\begin{minipage}[t]{1\columnwidth}%
\footnotesize
This table reports descriptive statistics for variables used in the empirical analysis. \emph{Pool size} is defined as the total value locked in the pool's smart contract at the end of each day. We compute the balance on day $t$ as follows: we take the balance at day $t-1$ and add (subtract) liquidity deposits (withdrawals) on day $t$, as well as accounting for token balance changes due to trades. The liquidity balance on the first day of the pool is taken to be zero. End of day balances are finally converted to US dollars. \emph{Daily volume} is computed as the sum of US dollar volume for all trades in a given pool and day. \emph{Liquidity share} (\emph{Volume share}) is computed as the ratio between a pool size (trading volume) for a given fee level and the aggregate size of all pools (trading volumes) for the same pair in a given day. \emph{Trade size} and \emph{Mint size} are the median trade and liquidity deposit size on a given pool and day, denominated in US dollars. \emph{Trade count} represents the number of trades in a given pool and day. \emph{\textbf{LP} wallets} counts the unique number of wallet addresses interacting with a given pool in a day.  The \emph{liquidity yield} is computed as the ratio between the daily trading volume and end-of-day TVL, multiplied by the fee tier. The \emph{price range} for every mint is computed as the difference between the top and bottom of the range, normalized by the range midpoint -- a measure that naturally lies between zero and two. The \emph{impermanent loss} is computed as in \citet{Heimbach2023} for a position in the range of 99\% to 101\% of the current pool price, with a forward-looking horizon of 200 blocks. Finally, \emph{mint-to-burn} and \emph{burn-to-mint} times are defined as the time between a mint (burn) and a subsequent burn (mint) by the same address in the same pool, measured in hours. \emph{Mint-to-burn} and \emph{burn-to-mint} are recorded on the day of the final interaction with the pool. 
\end{minipage}

\vspace{0.05in}
\resizebox{0.95\textwidth}{!}{

\small
\begin{tabular}{@{\extracolsep{5pt}}llrrrrrr} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
Statistic & Pool fee & \multicolumn{1}{c}{Mean} & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{St. Dev.} & \multicolumn{1}{c}{Pctl(25)} & \multicolumn{1}{c}{Pctl(75)} & \multicolumn{1}{c}{N} \\ 
\hline \\[-1.8ex] 

Pool size (\$M) & Low & 31.35 & 1.87 & 96.74 & 0.21 & 14.12 & 12,334 \\   
& High & 43.42 & 2.78 & 96.92 & 0.32 & 23.54 & 13,252 \\ 
& Single & 4.56 & 0.60 & 16.91 & 0.18 & 2.15 & 88,269 \\ 

Liquidity share (\%) & Low & 38.82 & 23.95 & 34.82 & 6.94 & 75.37 & 12,334 \\ 
 & High & 48.29 & 49.66 & 36.30 & 10.81 & 82.87 & 13,252 \\ 

 
Daily volume (\$000) & Low & 36,405.67 & 586.66 & 130,441.30 & 6.29 & 8,752.90 & 12,334 \\ 
& High & 10,317.39 & 72.41 & 36,160.20 & 0.62 & 2,605.98 & 13,252 \\  
& Single & 867.11 & 32.68 & 4,628.82 & 0.89 & 267.78 & 88,405 \\   

Volume share & Low & 64.64 & 80.11 & 37.35 & 32.64 & 97.76 & 10,546 \\ 
& High & 36.66 & 21.54 & 37.96 & 2.43 & 72.72 & 10,660 \\ 

Trade size (\$000) & Low & 9.89 & 3.68 & 18.03 & 0.94 & 10.00 & 10,546 \\
& High & 22.46 & 4.49 & 45.05 & 0.90 & 21.34 & 10,660 \\  
& Single   & 6.79 & 2.30 & 23.30 & 0.84 & 6.00 & 72,404 \\ 

Mint size (\$000) & Low & 1,134.84 & 22.78 & 15,770.57 & 5.20 & 88.24 & 6,076 \\ 
& High & 1,086.86 & 10.59 & 14,313.54 & 2.53 & 40.87 & 5,911 \\
& Single & 193.34 & 13.97 & 1,077.82 & 3.05 & 61.64 & 21,189 \\ 

Trade count & Low & 577.91 & 76 & 1,404.21 & 10 & 410 & 12,334 \\ 
& High & 111.26 & 20 & 478.30 & 2 & 84 & 13,252 \\ 
& Single & 42.45 & 12 & 125.46 & 2 & 36 & 88,405 \\  

$\LP$ wallets & Low & 6.52 & 1 & 16.19 & 0 & 5 & 12,334 \\   
& High & 12.48 & 1 & 45.63 & 0 & 6 & 13,252 \\  
& Single  & 1.28 & 0 & 4.05 & 0 & 1 & 88,405 \\ 

Liquidity yield (bps) & Low & 12.84 & 3.39 & 63.36 & 0.20 & 10.68 & 12,308 \\ 
& High & 11.79 & 2.18 & 62.94 & 0.05 & 7.99 & 13,075 \\ 
& Single & 11.76 & 1.76 & 57.93 & 0.11 & 7.50 & 87,852 \\

Price range & Low &  0.46 & 0.36 & 0.42 & 0.17 & 0.66 & 7,394 \\ 
& High & 0.60 & 0.54 & 0.43 & 0.32 & 0.82 & 7,209 \\  
& Single & 0.68 & 0.58 & 0.55 & 0.23 & 1.06 & 32,833 \\ 

Impermanent loss (bps) & Low  & 16.06 & 7.74 & 29.68 & 0.51 & 19.25 & 11,981 \\  
& High & 12.52 & 4.17 & 35.06 & 0.0005 & 13.72 & 13,112 \\  
& Single & 17.51 & 6.24 & 55.70 & 0.01 & 19.72 & 87,149 \\ 

Mint-to-burn (hrs) & Low & 458.20 & 60.35 & 1,253.01 & 18.72 & 256.80 & 6,233 \\
& High & 693.84 & 119.98 & 1,526.30 & 30.94 & 468.60 & 6,110 \\  
& Single & 629.24 & 135.39 & 1,343.18 & 31.99 & 508.04 & 22,900 \\ 

Burn-to-mint (hrs) & Low & 75.26 & 0.17 & 430.05 & 0.07 & 1.11 & 4,973 \\
& High & 107.81 & 0.18 & 589.12 & 0.06 & 1.58 & 4,985 \\  
& Single & 105.48 & 0.17 & 507.14 & 0.06 & 4.07 & 15,897 \\ 

\hline \\[-1.8ex] 

\end{tabular} 
}
\end{table} 

One concern with measuring average mint size is just-in-time liquidity provision (JIT). JIT liquidity providers submit very large and short-lived deposits to the pool to dilute competitors on an incoming large trade; they immediately withdraw the balance in the same block after executing the trade. In our sample, JIT liquidity provision is not economically significant, accounting for less than 1\% of aggregate trading volume. However, it has the potential to skew mint sizes to the right, particularly in low-fee pools, without providing liquidity to the market at large. We address this issue by (i) filtering out JIT mints using the algorithm in Appendix \ref{sec:app-jit} and (ii) taking the median liquidity mint size at day-pool level rather than the mean. 

Further, we follow \citet{augustin2022reaching} to compute the daily liquidity fee yield as the product between pool's fee tier and the ratio between trading volume and the lagged total value locked (TVL). That is,
\begin{equation}
    \text{Liquidity yield}=\text{liquidity fee}_i \times \frac{\text{Volume}_{i,t}}{\text{TVL}_{i,t-1}},
\end{equation}
for pool $i$ and day $t$. The average daily yield is about 12 basis points, with slightly more elevated figures for low-fee pools.


A salient observation in Table \ref{tab:sumstat} is that non-fragmented pairs (``single'' pools) are significantly smaller -- on average less than 5\% of the pool size and trading volume of fragmented pairs. Average trade and mint sizes are correspondingly lower as well. The evidence suggests that pairs for which there is significant trading interest, and therefore potentially a broader cross-section of potential liquidity providers, are more likely to become fragmented.

Figure \ref{fig:stat_liq} plots the distributions of our empirical measures across low- and high-fee liquidity pools. It suggest a sharp segmentation of liquidity supply and trading across pools. High-fee pools attract a large number of small liquidity providers, and end up with a larger \emph{aggregate} size than their low-fee counterparts. Trading volume is similarly segmented: most small value trades are executed on the cheaper low-fee pools, making up the majority of daily volume for a given pair. High-value trades, of which there are fewer, are more likely to (also) execute on high-fee pools.

\begin{figure}[H]
\caption{\label{fig:stat_liq} Liquidity supply on decentralized exchanges}
\begin{minipage}[t]{1\columnwidth}%
\footnotesize
This figure plots the empirical distributions of variables in the pool-day panel, across low and high fee pools (for fragmented pairs) as well as single pools in pairs that are not fragmented. In each box plot, the median is marked as a vertical line; the box extends to the quartiles of the data set, whereas the whiskers extend to an additional 1.5 times the inter-quartile range.
\end{minipage}

\vspace{0.05in}

\begin{centering}

\subfloat[Pool size and trading volume]{
\includegraphics[width=\textwidth]{Figures/sumstat_TVL_volume.png}
}

\subfloat[Average liquidity mint and trade size]{
\includegraphics[width=\textwidth]{Figures/sumstat_mint_trade.png}
}

\subfloat[Number of liquidity providers and trades]{
\includegraphics[width=\textwidth]{Figures/sumstat_wallets.png}
}
\par\end{centering}

\end{figure}




Our theoretical framework in Section \ref{sec:model} implies that liquidity suppliers manage their positions more actively in the low- than the high-fee pool. Figure \ref{fig:liq_cycles} provides suggestive evidence for liquidity cycles of different lengths in the cross-section of pools. Liquidity on decentralized exchanges is significantly more passive than on traditional equity markets. That is, liquidity providers do not often manage their positions at high frequencies. The median time from a mint (deposit) to a subsequent burn (withdrawal) from the same wallet on the same pool ranges from 2.48 days on low-fee pools to 4.97 days on high-fee pools. 

When do $\LP$s re-balance their positions? In 67\% of cases, liquidity providers only withdraw tokens from the pool when their position exits the price range that allows them to collect fees. Concretely, $\LP$s specified price range for liquidity provision does not straddle the most recent reference price of the pool. The scenario mirrors a limit order market where a liquidity provider's outstanding limit orders are deep in the book, such that she doesn't stand to earn the spread on the marginal incoming trade. In this case, a rational market maker might want to cancel their outstanding order and place a new one at the top of the book. This is exactly the pattern we observe on Uniswap: the subsequent mint following a burn straddles the new price 81\% of the time -- $\LP$s reposition
their liquidity around the current prices to keep earning fees on incoming trades. Moreover, re-balancing is swift -- the median time between a burn and a subsequent mint is just 10 minutes (0.17 hours).

The empirical pattern in Figure \ref{fig:liq_cycles} echoes liquidity cycles as described in Section \ref{sec:model}. Liquidity deposit tokens in Uniswap pools and then patiently wait for days until incoming order flow exhausts their position (i.e., posted liquidity no longer earns fees). Once this happens, $\LP$s quickly re-balance their position in a matter of minutes -- by removing stale liquidity and adding a new position around the current price. The cycle is longer on high-fee pools for which trading volume is lower and liquidity takes longer to deplete.

Importantly, $\LP$s do not seem to ``race'' to update liquidity upon information arrival as in \citet{Budish2015TheResponse}. First, they very rarely manage their position intraday. Second, $\LP$s on Uniswap typically do not remove in-range liquidity that stands to trade first against incoming order flow and therefore bears the highest adverse selection risk. Our results are consistent with \citet{CapponiJia2021} who theoretically argue that $\LP$s have low incentives to manage liquidity on news arrival, as well as with \citet{CapponiJiaYu2022} who find no evidence of traders racing to trade on information on Uniswap v2.


\begin{figure}[H]
\caption{\label{fig:liq_cycles} Liquidity cycles on high- and low-fee pools}
\begin{minipage}[t]{1\columnwidth}%
\footnotesize
The top panel plots the distribution of liquidity cycle times from mint to subsequent burn (left) and from burn to subsequent mint (right) for the same $\LP$ wallet address in the same pool. In each box plot, the median is marked as a vertical line; the box extends to the quartiles of the data set, whereas the whiskers extend to an additional 1.5 times the inter-quartile range. The bottom panel plots the probability that the $\LP$ position is out of range and therefore does not earn fees. A position is considered to be ``out of range'' when the minimum and maximum prices at which the $\LP$ is willing to provide liquidity do no straddle the current price on the pool. We plot the probability separately for low- and high- fees, as well as conditional on whether the event is a burn (liquidity withdrawal) or mint (liquidity deposit).
\end{minipage}

\vspace{0.05in}

\begin{centering}

\includegraphics[width=\textwidth]{Figures/time_elapsed_distribution.png}
\includegraphics[width=\textwidth]{Figures/out_of_range_distribution.png}

\par\end{centering}

\end{figure}

\paragraph{Measuring gas prices.} Each interaction with smart contracts on the Ethereum blockchain requires computational resources, measured in units of ``gas.'' Upon submitting a mint or burn transaction to the decentralized exchange, each liquidity provider specifies their willingness to pay per unit of gas, that is they bid a  ``gas price.'' Traders are likely to bid higher prices for more complex transactions or if they require a faster execution. To generate a conservative daily benchmark for the gas price, we compute the average of the lowest 100 user gas bids for mint and burn interactions on day $t$, across all liquidity pools in the benchmark sample. These transactions are more likely to be plain vanilla deposits or withdrawals of liquidity, capturing the cost of a simple interaction with the decentralized exchange smart contract.

Figure \ref{fig:gascosts} showcases the significant fluctuation in gas costs for Uniswap liquidity transactions over time. 
Gas costs denominated in USD are influenced by two primary factors: network congestion, which leads to variations in gas prices measured in Ether, and the fluctuation of Ether's value relative to the US dollar. On a monthly average, gas costs peaked at US\$195 in November 2021 and have since plummeted to US\$6 in August and September 2022.

\begin{figure}[H]
\caption{\label{fig:gascosts} Gas costs for Uniswap v3 mint/burn transactions}
\begin{minipage}[t]{1\columnwidth}%
\footnotesize
The figure illustrates the daily average gas cost on mint/burn transactions in Uniswap v3 pools. The gas cost is computed as the average of the lowest 100 user gas bids for mint and burn interactions on each day, across all liquidity pools in the benchmark sample.
\end{minipage}

\vspace{0.05in}

\begin{centering}

\includegraphics[width=\textwidth]{Figures/gas_timeline.png}


\par\end{centering}

\end{figure}


==> Old/empirics_202307.tex <==
\subsection{Liquidity supply on high- and low-fee pools}

To formally test the model predictions and quantify the differences in liquidity supply across fragmented pools, we build a panel data set for the 37 fragmented pairs in our sample where the unit of observation is pool-day. We estimate linear regressions of liquidity and volume measures on liquidity fees and gas costs:
\begin{equation}
    y_{ijt}=\alpha + \beta_0 d_\emph{low-fee, ij} + \beta_1 \text{GasPrice}_{jt} + \beta_2 \text{GasPrice}_{jt} \times d_\emph{low-fee, ij} + \sum \beta_k \emph{Controls}_{ijt} + \theta_j + \delta_w + \varepsilon_{ijt},
\end{equation}
where $y$ is a variable of interest, $i$ indexes liquidity pools, $j$ runs over asset pairs, and $t$ and $w$ indicates days and weeks, respectively. The dummy $d_\emph{low-fee, ij}$ takes the value one for the pool with the lowest fee in pair $j$ and zero else. 



Further, our set of controls includes pair and week fixed effects, the log aggregate trading volume and log liquidity supply (i.e., total value locked) for day $t$ across all pools $i$. Volume and liquidity are measured in US dollars. We also control for return volatility, computed as the 20-day rolling standard deviation of daily pair returns. Daily returns are obtained from the Kaiko Cross-Price data set, which measures the daily volume-weighted average price across all exchanges where the pair is traded. Therefore, our measure of returns and volatility is less likely to be affected by attempts to manipulate prices on any particular exchange.

Consistent with Figure \ref{fig:stat_liq}, most of the capital deployed to provide liquidity for a given pair is locked in high-fee pools. At the same time, low-fee pools attract much larger trading volume. Models (1) and (5) show that low-fee pools attract 44.2\% of liquidity supply for the average pair (that is, equal to $\nicefrac{(100-11.57)}{2}$) while they execute 64.5\% (i.e., $\nicefrac{(100+29.01)}{2}$) of the total trading volume. At a first glance, it would seem that a majority of capital on decentralized exchanges is inefficiently deployed in pools with low execution probability. We will show that, in line with our model, the difference is driven by heterogeneous liquidity cycles across pools, leading to the formation of $\LP$ clienteles. 

The regression results in Table \ref{tab:markeshare} support Prediction \ref{pred:comp_stat_Gamma}, stating that market share differences between pools are linked to variation in fixed transaction costs on the blockchain. A one-standard deviation increase in gas prices leads to a 2.29 percentage point increase in the high-fee liquidity share. The results suggests that blockchain transaction costs have an economically meaningful and statistically significant impact on liquidity fragmentation. In line with the theoretical model in Section \ref{sec:model}, a jump in gas prices leads to a reshuffling of liquidity supply from low- to high-fee pools. 

Evidence suggests that a higher gas price leads to a larger volume share for the high-fee pool, but the correlation is noisier, and the effect is not statistically significant at conventional levels. The weak link between gas prices and volume is consistent with our model assumption that incoming order flow is inelastic with respect to transaction costs. 


% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: Tue, Oct 25, 2022 - 8:34:54 PM

\begin{table}[H] 
  \caption{Liquidity pool market shares and gas prices}   \label{tab:markeshare}
\begin{minipage}[t]{1\columnwidth}%
\footnotesize
			This table reports the coefficients of the following regression:
	\begin{align*}
    \text{MarketShare}_{ijt}=\alpha + \beta_0 d_\emph{low-fee, ij} + \beta_1 \text{GasPrice}_{jt} + \beta_2 \text{GasPrice}_{jt} \times d_\emph{low-fee, ij} + \sum \beta_k \emph{Controls}_{ijt} + \theta_j + \varepsilon_{ijt}
    \end{align*}
	where the dependent variable is the liquidity or trading volume market share for pool $i$ in asset pair $j$ on day $t$. $d_\emph{low-fee, ij}$ is a dummy that takes the value one for the pool with the lowest fee in pair $j$ and zero else. $\emph{GasPrice}_{jt}$ is the average of the lowest 100 bids on liquidity provision events across all pairs on day $t$, standardized to have a zero mean and unit variance. \emph{Volume} is the natural logarithm of the sum of all swap amounts on day $t$, expressed in thousands of US dollars. \emph{Total value locked} is the natural logarithm of the total value locked on Uniswap v3 pools on day $t$, expressed in millions of dollars. \emph{Volatility} is 20-day rolling standard deviation of daily returns, using the volume-weighted average price for each day across all exchanges where the pair is traded. All regressions include pair and week fixed-effects. Robust standard errors in parenthesis are clustered by week and ***, **, and * denote the statistical significance at the 1, 5, and 10\% level, respectively.  The sample period is from May 4, 2021 to September 15, 2022. 
\end{minipage}
\small
\begin{center}
\resizebox{\textwidth}{!}{
\begin{tabular}{lcccc@{\hskip 0.3in}cccc}
\toprule
 & \multicolumn{4}{c}{Liquidity market share (\%)} & \multicolumn{4}{c}{Volume market share (\%)} \\ 
 & (1) & (2) & (3) & (4) & (5) & (6) & (7) & (8) \\
 \cmidrule{1-9}

$ d_\text{low-fee}$ & -11.57*** & -11.82*** & -11.57*** & -11.57*** & 29.01*** & 28.49*** & 29.01*** & 29.01*** \\
 & (-16.82) & (-16.18) & (-16.82) & (-16.82) & (25.95) & (23.43) & (25.92) & (25.92) \\
Gas price $\times$ $ d_\text{low-fee}$ & -2.30*** & -2.02** & -2.30*** & -2.30*** & -2.30* & -1.37 & -2.30* & -2.30* \\
 & (-3.19) & (-2.64) & (-3.19) & (-3.19) & (-1.77) & (-0.99) & (-1.77) & (-1.77) \\
Gas price & 1.26*** & 1.09*** & 1.30*** & 1.30*** & 1.28* & 0.80 & 1.50** & 1.50** \\
 & (3.32) & (2.68) & (3.43) & (3.43) & (1.95) & (1.14) & (2.23) & (2.23) \\
Volume & -0.28** & -0.31** & -0.34** & -0.34** & -0.54*** & -0.58*** & -0.91* & -0.91* \\
Total value locked & -0.77* & -1.10** &  &  & -4.56*** & -5.11*** &  &  \\
 & (-1.74) & (-2.45) &  &  & (-3.54) & (-4.10) &  &  \\
Volatility & 0.06** &  & 0.06** & 0.06** & 0.02 &  & 0.02 & 0.02 \\
 & (2.54) &  & (2.53) & (2.53) & (0.87) &  & (0.78) & (0.78) \\
Constant & 65.84*** & 68.95*** & 60.58*** & 60.58*** & 79.44*** & 84.64*** & 48.53*** & 48.53*** \\
 & (15.85) & (15.87) & (24.95) & (24.95) & (7.21) & (7.72) & (6.44) & (6.44) \\
Pair FE & Yes & Yes & Yes & Yes & Yes & Yes & Yes & Yes \\
Week FE & Yes & Yes & Yes & Yes & Yes & Yes & Yes & Yes \\
Observations & 20,454 & 21,097 & 20,454 & 20,454 & 20,454 & 21,097 & 20,454 & 20,454 \\
 R-squared & 0.03 & 0.03 & 0.03 & 0.03 & 0.13 & 0.13 & 0.13 & 0.13 \\ \hline
\bottomrule
\multicolumn{9}{l}{Robust t-statistics in parentheses. Standard errors are clustered at week level.  *** p$<$0.01, ** p$<$0.05, * p$<$0.1} \\
\end{tabular}
}
\end{center}
\end{table} 

What drives the market share gap across fragmented pools? In Table \ref{tab:ordersize} we document stark differences between the characteristics of individual orders supplying or demanding liquidity on pools with low and high fees. On the liquidity supply side, model (1) in Table \ref{tab:ordersize} shows that the average liquidity mint is 91.5\% larger on low-fee pools, which supports Prediction \ref{pred:clienteles} of the model.\footnote{Since all dependent variables are measured in natural logs, the marginal impact of a dummy coefficient $\beta$ is computed $\left(e^\beta-1\right) \times 100$ percent.} At the same time, there are 18\% fewer $\LP$ wallets (Model 5) and 16\% fewer liquidity events on the low-fee pool (Model 6).

\begin{table}[H] 
\caption{Fragmentation and order flow characteristics}  \label{tab:ordersize}
\begin{minipage}[t]{1\columnwidth}%
\footnotesize
			This table reports the coefficients of the following regression:
	\begin{align*}
    y_{ijt}=\alpha + \beta_0 d_\emph{low-fee, ij} + \beta_1 \text{GasPrice}_{jt} d_\emph{low-fee, ij} + \beta_2 \text{GasPrice}_{jt} \times d_\emph{high-fee, ij} + \sum \beta_k \emph{Controls}_{ijt} + \theta_j + \varepsilon_{ijt}
    \end{align*}
	where the dependent variable $y_{ijt}$ can be (i) the log median mint size, (ii) the log median trade size, (iii) the log trading volume, (iv) the log trade count $\log(1+\# trades)$, (v) the log count of unique $\LP$ wallets interacting with a pool in a given day, or (vi) the log count of interactions with a liquidity pool, for pool $i$ in asset $j$ on day $t$for pool $i$ in asset $j$ on day $t$. $d_\emph{low-fee, ij}$ is a dummy that takes the value one for the pool with the lowest fee in pair $j$ and zero else. $d_\emph{high-fee, ij}$ is defined as $1-d_\emph{low-fee, ij}$. $\emph{GasPrice}_{jt}$ is the average of the lowest 100 bids on liquidity provision events across all pairs on day $t$, standardized to have a zero mean and unit variance. \emph{Volume} is the natural logarithm of the sum of all swap amounts on day $t$, expressed in thousands of US dollars. \emph{Total value locked} is the natural logarithm of the total value locked on Uniswap v3 pools on day $t$, expressed in millions of dollars. \emph{Volatility} is 20-day rolling standard deviation of daily returns, using the volume-weighted average price for each day across all exchanges where the pair is traded. All regressions include pair and week fixed-effects. Robust standard errors in parenthesis are clustered by week and ***, **, and * denote the statistical significance at the 1, 5, and 10\% level, respectively.  The sample period is from May 4, 2021 to September 15, 2022. 
\end{minipage}
\begin{center}
\resizebox{1\textwidth}{!}{  
\begin{tabular}{lccccccc}
\toprule
 & \multicolumn{1}{c}{Mint size} &  \multicolumn{1}{c}{Trade size} & \multicolumn{1}{c}{Volume} & \multicolumn{1}{c}{\# Trades}  & \multicolumn{1}{c}{\# Wallets} & \multicolumn{1}{c}{$\LP$ interactions} & \multicolumn{1}{c}{Price range} \\
 & (1) & (2) & (3) & (4) & (5) & (6) & (7) \\
\cmidrule{1-8}
$ d_\text{low-fee}$ & 0.65*** & -0.32*** & 1.08*** & 1.19*** & -0.20*** & -0.18*** & -0.14*** \\
 & (9.76) & (-14.48) & (19.85) & (47.69) & (-7.71) & (-5.91) & (-24.80) \\
Gas price $\times$ $ d_\text{low-fee}$ & 0.38*** & 0.12*** & -0.03 & -0.15*** & -0.21*** & -0.24*** & -0.00 \\
 & (4.03) & (4.21) & (-0.80) & (-5.64) & (-10.07) & (-9.76) & (-0.57) \\
Gas price $\times$ $ d_\text{high-fee}$ & 0.54*** & 0.16*** & 0.21*** & -0.01 & -0.12*** & -0.11*** & -0.03*** \\
 & (5.85) & (6.75) & (4.06) & (-0.28) & (-4.19) & (-3.38) & (-4.21) \\
Volume & 0.69*** & 0.30*** & 0.73*** & 0.38*** & 0.06*** & 0.11*** & -0.04*** \\
 & (8.13) & (14.84) & (15.88) & (12.89) & (3.44) & (5.09) & (-4.14) \\
Total value locked & -0.58* & -0.03 & -0.07 & -0.28*** & -0.08 & -0.15** & 0.08** \\
 & (-1.97) & (-0.16) & (-0.34) & (-3.38) & (-1.33) & (-2.23) & (2.28) \\
Volatility & -0.00 & -0.03*** & 0.05 & 0.11** & 0.01 & 0.02 & 0.01 \\
 & (-0.03) & (-3.39) & (0.62) & (2.58) & (0.65) & (1.38) & (1.59) \\
Constant & -2.68 & -2.01 & -4.08*** & 0.54 & 1.15** & 1.24*** & 0.53** \\
 & (-1.08) & (-1.50) & (-2.72) & (1.01) & (2.62) & (2.69) & (2.15) \\
 &  &  &  &  &  &  \\
Pair FE & Yes & Yes & Yes & Yes & Yes & Yes & Yes  \\
Week FE & Yes & Yes & Yes & Yes & Yes & Yes  & Yes \\
Observations & 11,695 & 20,454 & 20,454 & 20,454 & 20,454 & 20,454 & 13,920 \\
R-squared & 0.26 & 0.55 & 0.59 & 0.67 & 0.62 & 0.60 & 0.48 \\ 
\bottomrule
\multicolumn{7}{l}{Robust t-statistics in parentheses. Standard errors are clustered at week level.} \\
\multicolumn{7}{l}{*** p$<$0.01, ** p$<$0.05, * p$<$0.1} \\
\end{tabular}
}
\end{center}
\end{table}



On the liquidity supply side, trades on the low-fee pool are 27.3\% smaller (Model 2), consistent with Prediction \ref{pred:trade_size_volume}. However, the low-fee pool executes more than three times the number of trades (i.e., trade count is 228\% higher from Model 4) and has 194\% higher volume than the high-fee pool (Model 3).

Our findings (Model 7) indicate that liquidity providers on low-fee pools select price ranges that are 26\% (=0.14/0.53) narrower when minting liquidity compared to those on high-fee pools. This pattern aligns with the capability of large LPs to adjust their liquidity positions frequently, enabling more efficient capital concentration. Similarly, \citet{caparros2023blockchain} report a higher concentration of liquidity in pools on alternative blockchains like Polygon, known for lower transaction costs than Ethereum.

The results point to an asymmetric match between liquidity supply and demand across pools. On low-fee pools, a few $\LP$s provide large chunks of liquidity for the vast majority of incoming small trades. Conversely, on high-fee pools there is a sizeable mass of small liquidity providers that mostly trade against a few large incoming trades. 

How does variation in fixed transaction costs impact the gap between individual order size across pools? We find that increasing the gas price by one standard deviation leads to higher liquidity deposits on both the low- and the high-fee pools (54\% and 67\% higher, respectively). The result supports Prediction \ref{pred:clienteles_cs} of the model. Our theoretical framework implies that a larger gas price leads to some (marginal) $\LP$s switching from the low- to the high-fee pool. The switching $\LP$s have low capital endowments relative to their low-fee pool peers, but higher than $\LP$s on the high-fee pool. Therefore, the gas-driven reshuffle of liquidity leads to a higher average endowment on both high- and low-fee pools. Consistent with the model, a higher gas price leads to fewer active liquidity providers, particularly on low-fee pools. A one-standard increase in gas costs is associated with an 18\% and 11\% drop in the number of $\LP$ wallets interacting daily with the low- and high-fee pools, respectively (Model 5).

While a higher gas price is correlated with a shift in liquidity supply, it has a muted impact on liquidity demand on low-fee pools. A higher gas cost is associated with 12.7\% larger trades (Model 2), likely as traders aim to achieve better economies of scale. At the same time, the number of trades on the low-fee pool drops by 13.9\% (Model 4) -- since small traders might be driven out of the market. The net of gas prices effect on aggregate volume on the low-fee pool is small and not statistically significant (Model 3). The result matches our model assumption that the aggregate order flow on low-fee pool is not sensitive to gas prices.\footnote{Formally, one could extend the model to assume that small $\LT$s arrive at the market at rate $\tilde{\theta}\left(\Gamma\right) \diff t$ and demand $f\left(\Gamma\right)$ units each, where $\tilde{\theta}\left(\Gamma\right)$ decreases in $\Gamma$ and $f\left(\Gamma\right)$ increases in $\Gamma$ such that $\tilde{\theta}\left(\Gamma\right)f\left(\Gamma\right) =\theta$.} 

\begin{table}[H] 
\caption{Liquidity flows and gas costs on fragmented pools} \label{tab:flows}
\begin{minipage}[t]{1\columnwidth}%
\footnotesize
			This table reports the coefficients of the following regression:
	\begin{align*}
    y_{ijt}=\alpha + \beta_0 d_\emph{low-fee, ij} + \beta_1 \text{GasPrice}_{jt} d_\emph{low-fee, ij} + \beta_2 \text{GasPrice}_{jt} \times d_\emph{high-fee, ij} + \sum \beta_k \emph{Controls}_{ijt} + \theta_j + \varepsilon_{ijt}
    \end{align*}
	where the dependent variable $y_{ijt}$ can be (i) the aggregate dollar value of mints (in logs), or (vi) a dummy variable taking value one hundred if there is at least one mint on liquidity pool $i$ in asset $j$ on day $t$. $d_\emph{low-fee, ij}$ is a dummy that takes the value one for the pool with the lowest fee in pair $j$ and zero else. $d_\emph{high-fee, ij}$ is defined as $1-d_\emph{low-fee, ij}$. $\emph{GasPrice}_{jt}$ is the average of the lowest 100 bids on liquidity provision events across all pairs on day $t$, standardized to have a zero mean and unit variance. \emph{Volume} is the natural logarithm of the sum of all swap amounts on day $t$, expressed in thousands of US dollars. \emph{Total value locked} is the natural logarithm of the total value locked on Uniswap v3 pools on day $t$, expressed in millions of dollars. \emph{Volatility} is 20-day rolling standard deviation of daily returns, using the volume-weighted average price for each day across all exchanges where the pair is traded. All regressions include pair and week fixed-effects. Robust standard errors in parenthesis are clustered by week and ***, **, and * denote the statistical significance at the 1, 5, and 10\% level, respectively.  The sample period is from May 4, 2021 to September 15, 2022. 
\end{minipage}
\begin{center}
\begin{tabular}{lcccccc}
\toprule
 & \multicolumn{3}{c}{Daily mints (log US\$)} &  \multicolumn{3}{c}{$\text{Prob}\left(\text{at least one mint}\right)$} \\
 & (1) & (2) & (3) & (4) & (5) & (6) \\
\cmidrule{1-7}
$ d_\text{low-fee}$ & 0.15* & 0.16** & 0.15* & 1.33* & 1.30* & 1.33* \\
 & (1.94) & (2.03) & (1.94) & (1.82) & (1.85) & (1.82) \\
Gas price $\times$ $ d_\text{low-fee}$ & -0.36*** & -0.36*** & -0.39*** & -7.60*** & -7.63*** & -5.68*** \\
 & (-6.66) & (-6.43) & (-5.22) & (-9.36) & (-9.09) & (-8.22) \\
Gas price $\times$ $ d_\text{high-fee}$ & 0.03 & 0.00 &  & -1.92*** & -2.14*** &  \\
 & (0.33) & (0.00) &  & (-2.74) & (-2.85) &  \\
Volume & 0.45*** & 0.44*** & 0.45*** & 1.19 & 1.17 & 1.19 \\
 & (7.16) & (7.04) & (7.16) & (1.33) & (1.25) & (1.33) \\
Total value locked & -0.45*** & -0.52*** & -0.45*** & -5.31** & -5.56** & -5.31** \\
 & (-2.75) & (-3.34) & (-2.75) & (-2.43) & (-2.52) & (-2.43) \\
Volatility & 0.02 &  & 0.02 & 1.50* &  & 1.50* \\
 & (0.73) &  & (0.73) & (1.80) &  & (1.80) \\
Gas price &  &  & 0.03 &  &  & -1.92*** \\
 &  &  & (0.33) &  &  & (-2.74) \\
Constant & 0.55 & 1.14 & 0.55 & 81.06*** & 82.73*** & 81.06*** \\
 & (0.60) & (1.36) & (0.60) & (6.12) & (5.72) & (6.12) \\
 &  &  &  &  &  &  \\
Pair FE & Yes & Yes & Yes & Yes & Yes & Yes  \\
Week FE & Yes & Yes & Yes & Yes & Yes & Yes  \\
Observations & 20,454 & 21,097 & 20,454 & 21,097 & 20,454 & 20,454 \\
 R-squared & 0.51 & 0.51 & 0.51 & 0.61 & 0.62 & 0.62 \\ \hline
\bottomrule
\multicolumn{7}{l}{Robust t-statistics in parentheses. Standard errors are clustered at week level.} \\
\multicolumn{7}{l}{*** p$<$0.01, ** p$<$0.05, * p$<$0.1} \\
\end{tabular}
\end{center}
\end{table}


On the high-fee pool, a higher gas price is also associated with a higher trade size, but does not lead to a change in the number of trades. The implication is that large-size traders who typically route orders to the high-fee pool are unlikely to be deterred by an increase in fixed costs, while they do adjust quantities to achieve better economies of scale. In the context of our model, the large $\LT$ arrival rate $\lambda$ does not depend on the gas price $\Gamma$.




In Table \ref{tab:flows}, we shift the analysis from individual orders to aggregate daily liquidity flows to Uniswap pools. We find that higher gas prices lead to a decrease in liquidity inflows, but only on the low fee pools. A one standard deviation increase in gas prices leads to a 30\% drop in new liquidity deposits by volume (Model 1) and an 7.60\% drop in probability of having at least one mint (Model 4) on the low-fee pool. However, the slow-down in liquidity inflows is less evident in high fee pools. While an increase in gas prices reduce the probability of liquidity inflows by 1.92\%, it has a negligible impact on the daily dollar inflow to the pool. Together with the result in Table \ref{tab:ordersize} that the size of individual mints increases with gas prices, our evidence is consistent with the model implication that higher fixed transaction costs change the composition of liquidity supply on the high-fee pool, with small $\LP$ being substituted by larger $\LP$s switching over from the low-fee pool.

\subsection{Liquidity cycles on high- and low-fee pools}

Next, we test Predictions \ref{pred:updates} and \ref{pred:updates_gas} on the duration of liquidity cycles on fragmented pools. Since the descriptive statistics in Table \ref{tab:sumstat} suggest that $\LP$s manage their positions over multiple days, we cannot accurately measure liquidity cycles in a pool-day panel. Instead, we use intraday data on liquidity events (either mints or burns) to measure the duration between two consecutive opposite-sign interactions by the same Ethereum wallet with a liquidity pool: either a mint followed by a burn, or vice-versa. 


\begin{table}[H] 
\caption{Liquidity cycles on fragmented pools} \label{tab:cycles}
\begin{minipage}[t]{1\columnwidth}%
\footnotesize
			This table reports the coefficients of the following regression:
	\begin{align*}
    y_{ijtk}=\alpha + \beta_0 d_\emph{low-fee, ij} + \beta_1 \text{GasPrice}_{jt} d_\emph{low-fee, ij} + \beta_2 \text{GasPrice}_{jt} \times d_\emph{high-fee, ij} + \sum \beta_k \emph{Controls}_{ijt} + \theta_j + \varepsilon_{ijt}
    \end{align*}
	where the dependent variable $y_{ijt}$ can be (i) the mint-to-burn time, (ii) the burn-to-mint time, measured in hours, for a transaction initiated by wallet $k$ on day $t$ and pool $i$ trading asset $j$. The mint-to-burn and burn-to-mint times are computed for consecutive interactions of the same wallet address with the liquidity pool. $d_\emph{low-fee, ij}$ is a dummy that takes the value one for the pool with the lowest fee in pair $j$ and zero else. $d_\emph{high-fee, ij}$ is defined as $1-d_\emph{low-fee, ij}$. $\emph{GasPrice}_{jt}$ is the average of the lowest 100 bids on liquidity provision events across all pairs on day $t$, standardized to have a zero mean and unit variance. \emph{Volume} is the natural logarithm of the sum of all swap amounts on day $t$, expressed in thousands of US dollars. \emph{Total value locked} is the natural logarithm of the total value locked on Uniswap v3 pools on day $t$, expressed in millions of dollars. \emph{Volatility} is 20-day rolling standard deviation of daily returns, using the volume-weighted average price for each day across all exchanges where the pair is traded. $d_\text{out-range}$ is a dummy taking value one if the position being burned or minted is out of range, that is if the price range selected by the $\LP$ does not straddle the current pool price. All variables are measured as of the time of the second leg of the cycle (i.e., the burn of a mint-burn cycle). All regressions include pair, week, and trader wallet fixed-effects. Robust standard errors in parenthesis are clustered by day and ***, **, and * denote the statistical significance at the 1, 5, and 10\% level, respectively.  The sample period is from May 4, 2021 to September 15, 2022. 
\end{minipage}
\begin{center}
\begin{tabular}{lcccccc}
\toprule
 & \multicolumn{3}{c}{Mint-burn time} & \multicolumn{3}{c}{Burn-mint time} \\
 & (1) & (2) & (3) & (4) & (5) & (6)  \\
\cmidrule{1-7}
$ d_\text{low-fee}$ & -77.26*** & -95.74*** & -99.63*** & -117.18*** & -132.22*** & -132.65*** \\
 & (-8.53) & (-10.46) & (-11.01) & (-9.76) & (-10.49) & (-10.53) \\
Gas price $\times$ $ d_\text{low-fee}$ & -30.43*** & -33.90*** & -33.62*** & -10.03 & -13.01* & -12.93* \\
 & (-3.76) & (-4.04) & (-4.02) & (-1.61) & (-1.88) & (-1.86) \\
Gas price $\times$ $ d_\text{high-fee}$ & -16.84*** & -9.75* & -9.13 & -1.08 & 0.45 & 0.53 \\
 & (-2.99) & (-1.77) & (-1.67) & (-0.20) & (0.07) & (0.08) \\
Volume &  & 1.46 & -1.04 &  & -6.54 & -7.01 \\
 &  & (0.18) & (-0.13) &  & (-0.76) & (-0.82) \\
Total value locked &  & 73.87 & 80.68 &  & -74.14* & -73.89* \\
 &  & (1.05) & (1.18) &  & (-1.72) & (-1.71) \\
Volatility &  & 3.37 & 2.70 &  & -50.19*** & -50.23*** \\
 &  & (0.17) & (0.14) &  & (-5.57) & (-5.59) \\
Position out-of-range &  &  & 46.80*** &  &  & 14.39** \\
 &  &  & (8.60) &  &  & (2.27) \\
Constant & 389.08*** & -174.79 & -222.32 & 150.80*** & 831.58** & 833.67** \\
 & (110.18) & (-0.30) & (-0.39) & (29.01) & (2.39) & (2.40) \\
 &  &  &  &  &  &  \\
 Pair FE & Yes & Yes & Yes & Yes & Yes & Yes  \\
 Week FE & Yes & Yes & Yes & Yes & Yes & Yes  \\
 Trader wallet FE & Yes & Yes & Yes & Yes & Yes & Yes \\
Observations & 287,505 & 265,182 & 265,182 & 196,145 & 182,581 & 182,581 \\
 R-squared & 0.82 & 0.82 & 0.82 & 0.37 & 0.38 & 0.38 \\ \hline
\bottomrule
\multicolumn{7}{l}{Robust t-statistics in parentheses. Standard errors are clustered at week level.} \\
\multicolumn{7}{l}{*** p$<$0.01, ** p$<$0.05, * p$<$0.1} \\
\end{tabular}

\end{center}
\end{table}

To complement our previous analysis, we additionally control for whether each liquidity position is out of range (i.e., the price range set by the $\LP$ does not straddle the current price and therefore the $\LP$ does not earn fees). We further introduce wallet fixed effects to soak up variation in reaction times across traders.

Table \ref{tab:cycles} presents the results. Liquidity updates on decentralized exchanges are very infrequent, as times elapsed between consecutive interactions are measured in days or even weeks. In line with Prediction \ref{pred:updates}, we find evidence for shorter liquidity cycles on low-fee pools. The average time between consecutive mint and burn orders is 19.85\% shorter on the low-fee pool (from Model 1, the relative difference is 77.26 hours/389.08 hours).

Liquidity cycles are in part driven by fixed Blockchain transaction costs. A one standard deviation increase in gas prices speeds up the liquidity cycle on low-fee pools by a further 33.6 hours (Model 3), without significantly changing the average mint-to-burn time on high-fee pools. The result supports the intuition behind Prediction \ref{pred:updates_gas}. When the gas price spikes, the liquidity supply on the low-fee pool decreases at a higher rate than the liquidity demand. As a result, liquidity deposits deplete faster (i.e., they move outside the fee-earning range), triggering the need for more frequent updates. We do not see a similar impact on the high-fee pool, for which the duration of liquidity cycles is not sensitive to gas prices (Models 2 and 3). The result is intuitive, since neither aggregate liquidity supply (measured as mint inflows in Table \ref{tab:flows}) or liquidity demand (i.e., corresponding to trade volume in Table \ref{tab:ordersize}) on the high-fee pool change significantly with gas prices.

The reaction time of a trader may depend on capital constraints, network congestion, and other confounding factors that can correlate with gas prices. As a robustness check, we repeat the analysis above with burn-to-mint times as the dependent variables. The burn-to-mint time measures the speed at which $\LP$s deposit liquidity at updated prices after removing (out-of-range) positions, and should not depend on the rate at which liquidity is consumed. Consistent with the theory, we find no significant relationship between gas price and the burn-to-mint duration (Models 4 through 6).

\subsection{Adverse selection costs across low- and high-fee pools}

Our findings indicate that larger aggressive orders tend to execute on high-fee liquidity pools. Given that, at least in equity markets, larger incoming orders tend to be better informed \citep{Hasbrouck1991}, a natural question is whether liquidity providers on high-fee pools face higher adverse selection. 

A widely-used measure for gauging informational costs for liquidity providers on decentralized exchanges employing automated market makers (AMMs) is the ``impermanent loss,'' the equivalent of adverse selection measures in traditional limit order markets  \citep[see, for example,][]{aoyagi2020,BarbonRanaldo2021}. The impermanent loss (IL) is defined as the negative return from providing liquidity as opposed to holding the assets outside the exchange and marking them to market as the price evolves. Intuitively, if the fundamental value of the asset changes, an arbitrageur trades at the stale price in the direction of the price change, thus minimizing the value of the liquidity pool \citep{zhang2023amm}. 

To illustrate, let's consider a straightforward example. At some initial time $t_0$, a liquidity provider deposits 1 ETH (i.e., a token quantity of $T_0=1$) and 3000 USDC (i.e., a numeraire $N_0=3000$) into a liquidity pool, establishing a token price of $p_0=3000$.  If at the next time interval ($t=1$), the intrinsic value surges to $v_1=3500$, an arbitrager has the incentive to remove ETH from the pool and deposit USDC until the price reflects the intrinsic value, or $\frac{N_1}{T_1}=3500$.

Given that the AMM requires the product of token and numeraire quantities to be constant ($T_0 N_0 = T_1 N_1$), this leads to $T_1 = 0.926$ and $N_1=3240.37$. In terms of the numeraire equivalent, the liquidity provider's position is valued at $V_\text{pos}=\$3500 \times 0.926 + \$3240.37 = \$6480.74$.  Had the liquidity provider not deposited their tokens on the exchange and instead held it in its own account, the value would be $V_\text{hold}=\$3500 \times 1 + \$3000 = \$6500$ (that is, equal to $T_0 \times p_1 + N_0$).

Hence, disregarding gas cost and liquidity fees, the impermanent loss can be calculated as:
\begin{equation}
    \text{ImpermanentLoss}=\frac{V_\text{hold}-V_\text{pos}}{V_\text{hold}}=29 \text{ bps}.
\end{equation}

However, liquidity providers on Uniswap V3 pools can set a price range for their orders. While this feature caps the potential adverse selection cost, it simultaneously introduces a new layer of computational complexity. In Appendix \ref{app:IL}, we present the exact formulas for calculating impermanent loss on Uniswap V3, based on the methodology described by \citet{Heimbach2023}. 

We obtain block-by-block liquidity snapshots from Kaiko, which allow us to calculate the impermanent loss for symmetric liquidity positions within a price range of $\left[\frac{1}{\alpha} p, \alpha p\right]$ centered around the current pool price $p$. We consider different ranges of $\alpha$, specifically $\alpha\in\left\{1.01, 1.05, 1.1, 1.25\right\}$. The liquidity management horizon, which represents the time delay between measuring $p_0$ and $p_1$, is set to 200 blocks or approximately 45 minutes.

Table \ref{tab:il} presents the empirical results. In Models 1, 3, 5, and 7, where we exclude control variables, the impermanent loss appears to be higher in low-fee pools. However, the link is mechanical: since high-fee pools exhibit lower trading activity, the price updates less frequently leading to a lower measured impermanent loss. Once we account for trading activity in our analysis (Models 2, 4, 6, and 8), we find no significant difference in the impermanent loss between high-fee and low-fee pools. This finding suggests that liquidity providers in same-asset pools with different fees do not encounter substantially different informational costs, which aligns with the assumptions of our theoretical framework.

\begin{table}[H] 
\scriptsize
\caption{Impermanent loss across high- and low-fee pools}\label{tab:il}
\begin{minipage}[t]{1\columnwidth}%
\footnotesize
This table reports the coefficients of the following regression:
	\begin{align*}
    \text{Impermanent Loss}_{ijt}=\alpha + \beta_0 d_\emph{low-fee, ij}  + \sum \beta_k \emph{Controls}_{ijt} + \theta_j + \varepsilon_{ijt}
    \end{align*}
	where the dependent variable is the daily average impermanent loss for a liquidity position with price range $\left[\frac{p}{\alpha}, \alpha p\right]$ around the current pool price $p$, for $\alpha\in\left\{1.01, 1.05, 1.1., 1.25\right\}$. The average impermanent loss is computed across all Ethereum blocks mined within the day. To compute the impermanent loss, we use a liquidity provider horizon of 200 blocks: that is, we compare the current pool price with the pool price 200 blocks later. $d_\emph{low-fee, ij}$ is a dummy that takes the value one for the pool with the lowest fee in pair $j$ and zero else. $\emph{GasPrice}_{jt}$ is the average of the lowest 100 bids on liquidity provision events across all pairs on day $t$, standardized to have a zero mean and unit variance. $\emph{TradeCount}_{jt}$ is number of trades on pool $j$ and day $t$, standardized to have a zero mean and unit variance. \emph{Volume} is the natural logarithm of the sum of all swap amounts on day $t$, expressed in thousands of US dollars. \emph{Total value locked} is the natural logarithm of the total value locked on Uniswap v3 pools on day $t$, expressed in millions of dollars. \emph{Volatility} is the 20-day rolling standard deviation of daily returns, using the volume-weighted average price for each day across all exchanges where the pair is traded. All regressions include pair and week fixed-effects. Robust standard errors in parenthesis are clustered by week and ***, **, and * denote the statistical significance at the 1, 5, and 10\% level, respectively.  The sample period is from May 4, 2021 to September 15, 2022. 
\end{minipage}

\begin{center}
\resizebox{1\textwidth}{!}{  
\begin{tabular}{lcccccccc}
\toprule
& \multicolumn{8}{c}{Impermanent loss for a liquidity position with range $\left[\frac{p}{\alpha}, \alpha p\right]$ around price $p$} \\
\cmidrule{1-9} 
& \multicolumn{2}{c}{$\alpha=1.01$} & \multicolumn{2}{c}{$\alpha=1.05$} & \multicolumn{2}{c}{$\alpha=1.1$} & \multicolumn{2}{c}{$\alpha=1.25$} \\
 & (1) & (2) & (3) & (4) & (5) & (6) & (7) & (8) \\
\cmidrule{1-9}
$ d_\text{low-fee}$ & 3.41*** & 0.72 & 1.23*** & -0.61 & 0.64*** & -0.66 & 0.20 & -0.49 \\
 & (9.56) & (0.87) & (4.52) & (-0.84) & (2.65) & (-1.10) & (0.90) & (-1.25) \\
Gas price &  & 3.04*** &  & 2.27*** &  & 1.68*** &  & 1.02*** \\
 &  & (3.09) &  & (3.07) &  & (3.03) &  & (2.77) \\
Trade count &  & 2.39*** &  & 1.64** &  & 1.21** &  & 0.68* \\
 &  & (2.96) &  & (2.31) &  & (2.07) &  & (1.94) \\
Volume &  & 7.85*** &  & 3.63*** &  & 2.17*** &  & 0.95*** \\
 &  & (7.37) &  & (5.04) &  & (4.13) &  & (2.74) \\
Total value locked &  & -15.46*** &  & -6.46* &  & -3.18 &  & -1.09 \\
 &  & (-3.41) &  & (-1.87) &  & (-1.18) &  & (-0.64) \\
Volatility &  & 6.39*** &  & 3.79*** &  & 2.45*** &  & 1.25*** \\
 &  & (5.21) &  & (4.92) &  & (4.59) &  & (4.22) \\
Constant & 12.62*** & 26.06 & 5.97*** & 6.42 & 3.84*** & -1.30 & 2.13*** & -2.65 \\
 & (73.61) & (0.88) & (45.69) & (0.27) & (32.98) & (-0.07) & (19.91) & (-0.21) \\
 &  &  &  &  &  &  \\
Pair FE & Yes & Yes & Yes & Yes & Yes & Yes & Yes  \\
Week FE & Yes & Yes & Yes & Yes & Yes & Yes  & Yes \\
Observations & 24,937 & 20,449 & 24,937 & 20,449 & 24,937 & 20,449 & 24,937 & 20,449 \\
 R-squared & 0.14 & 0.28 & 0.07 & 0.17 & 0.04 & 0.12 & 0.02 & 0.07 \\ \hline
\bottomrule
\multicolumn{9}{l}{Robust t-statistics in parentheses. Standard errors are clustered at week level.} \\
\multicolumn{9}{l}{*** p$<$0.01, ** p$<$0.05, * p$<$0.1} \\
\end{tabular}
}
\end{center}
\end{table}








 



==> Old/empirics_202404.tex <==
subsection{Liquidity supply on high- and low-fee pools}

To formally test the model predictions and quantify the differences in liquidity supply across fragmented pools, we build a panel data set for the 32 fragmented pairs in our sample where the unit of observation is pool-day. We estimate linear regressions of liquidity and volume measures on liquidity fees and gas costs:
\begin{equation}
    y_{ijt}=\alpha + \beta_0 d_\emph{low-fee, ij} + \beta_1 \text{GasPrice}_{jt} + \beta_2 \text{GasPrice}_{jt} \times d_\emph{low-fee, ij} + \sum \beta_k \emph{Controls}_{ijt} + \theta_j + \delta_w + \varepsilon_{ijt},
\end{equation}
where $y$ is a variable of interest, $i$ indexes liquidity pools, $j$ runs over asset pairs, and $t$ and $w$ indicates days and weeks, respectively. The dummy $d_\emph{low-fee, ij}$ takes the value one for the pool with the lowest fee in pair $j$ and zero else. 

Further, our set of controls includes pair and week fixed effects, the log aggregate trading volume and log liquidity supply (i.e., total value locked) for day $t$ across all pools $i$. Volume and liquidity are measured in US dollars. We also control for daily return volatility, computed as the range between the daily high and low prices for a given pair $j$ \citep[following][]{Alizadeh2002}: 
\begin{equation}
    \text{Volatility}_{jt}=\frac{1}{2\sqrt{\log 2}} \log\left(\frac{\text{High}_{jt}}{\text{Low}_{jt}}\right).
\end{equation}
To measure volatility for fragmented pairs that actively trade in multiple pools, we select the pool with the highest trading volume for a given day.

Consistent with Figure \ref{fig:stat_liq}, most of the capital deployed to provide liquidity for a given pair is locked in high-fee pools. At the same time, low-fee pools attract much larger trading volume. Models (1) and (5) show that the average low-fee pool attracts 39.5\% of liquidity supply for the average pair (that is, equal to $\nicefrac{(100-20.92)}{2}$) while it executes 62\% (i.e., $\nicefrac{(100+24.62)}{2}$) of the total trading volume. At a first glance, it would seem that a majority of capital on decentralized exchanges is inefficiently deployed in pools with low execution probability. We will show that, in line with our model, the difference is driven by heterogeneous liquidity cycles across pools, leading to the formation of $\LP$ clienteles. 

The regression results in Table \ref{tab:markeshare} support Prediction \ref{pred:comp_stat_Gamma}, stating that market share differences between pools are linked to variation in fixed transaction costs on the blockchain. A one-standard deviation increase in gas prices leads to a 4.63 percentage point increase in the high-fee liquidity share. The results suggests that blockchain transaction costs have an economically meaningful and statistically significant impact on liquidity fragmentation. In line with the theoretical model in Section \ref{sec:model}, a jump in gas prices leads to a reshuffling of liquidity supply from low- to high-fee pools. 

Evidence suggests that a higher gas price leads to a 6.52\% lower volume share for the low-fee pool. This outcome is natural, as the incoming order flow is optimally routed to the high-fee pool, following the liquidity providers.


% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: Tue, Oct 25, 2022 - 8:34:54 PM

\begin{table}
  \caption{Liquidity pool market shares and gas prices}   \label{tab:markeshare}
\begin{minipage}[t]{1\columnwidth}%
\footnotesize
			This table reports the coefficients of the following regression:
	\begin{align*}
    \text{MarketShare}_{ijt}=\alpha + \beta_0 d_\emph{low-fee, ij} + \beta_1 \text{GasPrice}_{jt} + \beta_2 \text{GasPrice}_{jt} \times d_\emph{low-fee, ij} + \sum \beta_k \emph{Controls}_{ijt} + \theta_j + \varepsilon_{ijt}
    \end{align*}
 	where the dependent variable is the liquidity or trading volume market share for pool $i$ in asset pair $j$ on day $t$. $d_\emph{low-fee, ij}$ is a dummy that takes the value one for the pool with the lowest fee in pair $j$ and zero else. $\emph{GasPrice}_{jt}$ is the average of the lowest 100 bids on liquidity provision events across all pairs on day $t$, standardized to have a zero mean and unit variance. \emph{Volume} is the natural logarithm of the sum of all swap amounts on day $t$, expressed in thousands of US dollars. \emph{Total value locked} is the natural logarithm of the total value locked on Uniswap v3 pools on day $t$, expressed in millions of dollars.\emph{Volatility} is computed as the daily range between high and low prices on the most active pool for a given pair.All regressions include pair and week fixed-effects. Robust standard errors in parenthesis are clustered by week and ***, **, and * denote the statistical significance at the 1, 5, and 10\% level, respectively.  The sample period is from May 4, 2021 to July 15, 2023. 
\end{minipage}
\small
\begin{center}
\resizebox{\textwidth}{!}{
\begin{tabular}{lcccc@{\hskip 0.3in}cccc}
\toprule
 & \multicolumn{4}{c}{Liquidity market share (\%)} & \multicolumn{4}{c}{Volume market share (\%)} \\ 
 & (1) & (2) & (3) & (4) & (5) & (6) & (7) & (8) \\
 \cmidrule{1-9}

$ d_\text{low-fee}$ & -20.92*** & -20.92*** & -20.92*** & -20.94*** & 24.62*** & 24.63*** & 24.62*** & 24.71*** \\
 & (-27.42) & (-27.41) & (-27.42) & (-23.95) & (20.55) & (20.56) & (20.55) & (18.54) \\
Gas price $\times$ $ d_\text{low-fee}$ & -4.63*** & -4.62*** & -4.63*** &  & -6.52*** & -6.52*** & -6.52*** &  \\
 & (-7.32) & (-7.32) & (-7.32) &  & (-5.92) & (-5.92) & (-5.92) &  \\
Gas price & 2.31*** & 2.31*** & 2.31*** &  & 3.63*** & 3.61*** & 3.61*** &  \\
 & (7.32) & (7.32) & (7.32) &  & (7.33) & (7.30) & (7.26) &  \\
Volume & 0.00 & 0.00 & 0.00 & 0.00 & -0.19** & -0.20** & -0.19** & -0.12 \\
 & (0.65) & (1.33) & (0.65) & (0.66) & (-2.54) & (-2.61) & (-2.50) & (-1.56) \\
Total value locked & -0.00 & -0.00 &  & -0.00 & 0.58 & 0.58 &  & 0.44 \\
 & (-0.58) & (-0.06) &  & (-0.64) & (1.44) & (1.44) &  & (1.10) \\
Volatility & -0.29 &  & -0.29 & -0.28 & -1.15*** &  & -1.15*** & -1.13** \\
 & (-0.90) &  & (-0.90) & (-0.82) & (-2.74) &  & (-2.74) & (-2.56) \\
Constant & 60.45*** & 60.46*** & 60.45*** & 60.46*** & 41.96*** & 41.99*** & 41.96*** & 41.96*** \\
 & (158.00) & (158.46) & (158.00) & (137.54) & (69.99) & (70.22) & (70.02) & (62.81) \\
Pair FE & Yes & Yes & Yes & Yes & Yes & Yes & Yes & Yes \\
Week FE & Yes & Yes & Yes & Yes & Yes & Yes & Yes & Yes \\
Observations & 40,288 & 40,288 & 40,288 & 40,288 & 36,059 & 36,059 & 36,059 & 36,059 \\
 R-squared & 0.10 & 0.10 & 0.10 & 0.09 & 0.13 & 0.13 & 0.13 & 0.12 \\ \hline
\bottomrule
\multicolumn{9}{l}{Robust t-statistics in parentheses. Standard errors are clustered at week level.  *** p$<$0.01, ** p$<$0.05, * p$<$0.1} \\
\end{tabular}
}
\end{center}
\end{table} 

What drives the market share gap across fragmented pools? In Table \ref{tab:ordersize} we document stark differences between the characteristics of individual orders supplying or demanding liquidity on pools with low and high fees. On the liquidity supply side, model (1) in Table \ref{tab:ordersize} shows that the average liquidity mint is 107.5\% larger on low-fee pools, which supports Prediction \ref{pred:clienteles} of the model.\footnote{Since all dependent variables are measured in natural logs, the marginal impact of a dummy coefficient $\beta$ is computed $\left(e^\beta-1\right) \times 100$ percent.} At the same time, there are 3.40 fewer unique wallets (Model 5) providing liquidity on the low-fee pool -- that is, a 34\% relative difference between high- and low-fee pools.

\begin{table}
\caption{Fragmentation and order flow characteristics}  \label{tab:ordersize}
\begin{minipage}[t]{1\columnwidth}%
\footnotesize
			This table reports the coefficients of the following regression:
	\begin{align*}
    y_{ijt}=\alpha + \beta_0 d_\emph{low-fee, ij} + \beta_1 \text{GasPrice}_{jt} d_\emph{low-fee, ij} + \beta_2 \text{GasPrice}_{jt} \times d_\emph{high-fee, ij} + \sum \beta_k \emph{Controls}_{ijt} + \theta_j + \varepsilon_{ijt}
    \end{align*}
	where the dependent variable $y_{ijt}$ can be (i) the log median mint size, (ii) the log median trade size, (iii) the log trading volume, (iv) the log trade count $\log(1+\# trades)$, (v) count of unique $\LP$ wallets interacting with a pool in a given day, (vi) the liquidity yield in bps for pool $i$ in asset $j$ on day $t$, computed as in equation \eqref{eq:liq_yield}, and (vii) the average liquidity mint price range for pool $i$ in asset $j$ on day $t$. Price range is computed as the difference between the top and bottom of the range, normalized by the range midpoint -- a measure that naturally lies between zero and two. $d_\emph{low-fee, ij}$ is a dummy that takes the value one for the pool with the lowest fee in pair $j$ and zero else. $d_\emph{high-fee, ij}$ is defined as $1-d_\emph{low-fee, ij}$. $\emph{GasPrice}_{jt}$ is the average of the lowest 100 bids on liquidity provision events across all pairs on day $t$, standardized to have a zero mean and unit variance. \emph{Volume} is the natural logarithm of the sum of all swap amounts on day $t$, expressed in thousands of US dollars. \emph{Total value locked} is the natural logarithm of the total value locked on Uniswap v3 pools on day $t$, expressed in millions of dollars. \emph{Volatility} is computed as the daily range between high and low prices on the most active pool for a given pair. All regressions include pair and week fixed-effects. Robust standard errors in parenthesis are clustered by week and ***, **, and * denote the statistical significance at the 1, 5, and 10\% level, respectively.  The sample period is from May 4, 2021 to July 15, 2023. 
\end{minipage}
\begin{center}
\resizebox{1\textwidth}{!}{  
\begin{tabular}{lccccccc}
\toprule
 & \multicolumn{1}{c}{Mint size} &  \multicolumn{1}{c}{Trade size} & \multicolumn{1}{c}{Volume} & \multicolumn{1}{c}{\# Trades}  & \multicolumn{1}{c}{\# Wallets} & \multicolumn{1}{c}{Liquidity yield} & \multicolumn{1}{c}{Price range} \\
 & (1) & (2) & (3) & (4) & (5) & (6) & (7) \\
\cmidrule{1-8}
$ d_\text{low-fee}$ & 0.73*** & -0.30*** & 0.89*** & 1.02*** & -3.40*** & 2.03*** & -0.18*** \\
 & (12.27) & (-10.05) & (14.23) & (32.95) & (-5.00) & (3.60) & (-41.84) \\
Gas price $\times$ $ d_\text{low-fee}$ & 0.37*** & 0.08*** & -0.03 & -0.22*** & -3.00*** & 3.57** & -0.00 \\
 & (4.96) & (3.75) & (-0.95) & (-7.29) & (-3.43) & (2.30) & (-0.47) \\
Gas price $\times$ $ d_\text{high-fee}$ & 0.58*** & 0.17*** & 0.24*** & 0.07** & -2.89*** & 5.57*** & -0.03*** \\
 & (7.52) & (8.81) & (5.95) & (2.46) & (-3.15) & (2.83) & (-4.65) \\
Volume & 0.37*** & 0.16*** & 0.43*** & 0.20*** & 1.22*** & 1.01 & -0.01** \\
 & (8.68) & (21.38) & (15.27) & (13.85) & (6.56) & (0.81) & (-2.56) \\
Total value locked & -0.16 & 0.11*** & 0.23** & -0.01 & -1.86 & -13.42 & -0.02 \\
 & (-1.30) & (3.54) & (1.99) & (-0.18) & (-0.99) & (-1.09) & (-0.99) \\
Volatility & -0.04 & -0.01 & -0.07 & 0.01 & -0.09 & 1.18** & 0.02*** \\
 & (-1.11) & (-1.34) & (-1.38) & (0.88) & (-1.03) & (2.21) & (3.98) \\
Constant & 1.88*** & 1.64*** & 5.27*** & 3.26*** & 10.12*** & 10.01*** & 0.59*** \\
 & (58.27) & (111.47) & (168.58) & (209.84) & (28.65) & (26.04) & (184.91) \\
 &  &  &  &  &  &  \\
Pair FE & Yes & Yes & Yes & Yes & Yes & Yes & Yes  \\
Week FE & Yes & Yes & Yes & Yes & Yes & Yes  & Yes \\
Observations & 21,000 & 36,059 & 36,059 & 40,288 & 40,288 & 40,252 & 24,058 \\
 R-squared & 0.26 & 0.53 & 0.55 & 0.52 & 0.37 & 0.09 & 0.42 \\ \hline
\bottomrule
\multicolumn{7}{l}{Robust t-statistics in parentheses. Standard errors are clustered at week level.} \\
\multicolumn{7}{l}{*** p$<$0.01, ** p$<$0.05, * p$<$0.1} \\
\end{tabular}
}
\end{center}
\end{table}


On the liquidity demand side, trades on the low-fee pool are 25.91\% smaller (Model 2), consistent with Prediction \ref{pred:trade_size_volume}. However, the low-fee pool executes almost three times the number of trades (i.e., trade count is 177\% higher from Model 4) and has 143\% higher volume than the high-fee pool (Model 3). On average, liquidity providers on low-fee pools earn 2.03 basis points higher revenue than their counterparts on high-fee pools (Model 6), indicating significant positive returns resulting from economies of scale.

Our findings (Model 7) indicate that liquidity providers on low-fee pools select price ranges that are 30\% (=0.18/0.59) narrower when minting liquidity compared to those on high-fee pools. This pattern aligns with the capability of large LPs to adjust their liquidity positions frequently, enabling more efficient capital concentration. Similarly, \citet{caparros2023blockchain} report a higher concentration of liquidity in pools on alternative blockchains like Polygon, known for lower transaction costs than Ethereum.

The results point to an asymmetric match between liquidity supply and demand across pools. On low-fee pools, a few $\LP$s provide large chunks of liquidity for the vast majority of incoming small trades. Conversely, on high-fee pools there is a sizeable mass of small liquidity providers that mostly trade against a few large incoming trades. 

How does variation in fixed transaction costs impact the gap between individual order size across pools? We find that increasing the gas price by one standard deviation leads to higher liquidity deposits on both the low- and the high-fee pools (14.2\% and 30.1\% higher, respectively).\footnote{The relative effects are computed as $\nicefrac{0.37}{(1.88+0.73)}=13.8\%$ for low pools and $\nicefrac{0.58}{1.88}=30.85\%$ for high-fee pools, respectively.} The result supports Prediction \ref{pred:clienteles_cs} of the model. Our theoretical framework implies that a larger gas price leads to some (marginal) $\LP$s switching from the low- to the high-fee pool. The switching $\LP$s have low capital endowments relative to their low-fee pool peers, but higher than $\LP$s on the high-fee pool. Therefore, the gas-driven reshuffle of liquidity leads to a higher average endowment on both high- and low-fee pools. Consistent with the model, a higher gas price leads to fewer active liquidity providers, particularly on low-fee pools. Specifically, a one-standard increase in gas costs leads to a significant decrease in the number of $\LP$ wallets interacting daily with low- and high-fee pools, respectively (Model 5). 

While a higher gas price is correlated with a shift in liquidity supply, it has a muted impact on liquidity demand on low-fee pools. A higher gas cost is associated with 6\% larger trades (Model 2), likely as traders aim to achieve better economies of scale. At the same time, the number of trades on the low-fee pool drops by 5.1\% (Model 4) -- since small traders might be driven out of the market. The net of gas prices effect on aggregate volume on the low-fee pool is small and not statistically significant (Model 3). The result matches our model assumption that the aggregate order flow on low-fee pool is not sensitive to gas prices.\footnote{Formally, one could extend the model to assume that small $\LT$s arrive at the market at rate $\tilde{\theta}\left(\Gamma\right) \diff t$ and demand $f\left(\Gamma\right)$ units each, where $\tilde{\theta}\left(\Gamma\right)$ decreases in $\Gamma$ and $f\left(\Gamma\right)$ increases in $\Gamma$ such that $\tilde{\theta}\left(\Gamma\right)f\left(\Gamma\right) =\theta$.} 

On the high-fee pool, a higher gas price is also associated with a higher trade size, but a much smaller relative increase in the number of trades. The implication is that large-size traders who typically route orders to the high-fee pool are unlikely to be deterred by an increase in fixed costs, while they do adjust quantities to achieve better economies of scale. In the context of our model, the large $\LT$ arrival rate $\lambda$ does not depend on the gas price $\Gamma$.



In Table \ref{tab:flows}, we shift the analysis from individual orders to aggregate daily liquidity flows to Uniswap pools. We find that higher gas prices lead to a decrease in liquidity inflows, but only on the low fee pools. A one standard deviation increase in gas prices leads to a 29.5\% drop in new liquidity deposits by volume (Model 1) and an 6.02\% drop in probability of having at least one mint (Model 4) on the low-fee pool. However, the slow-down in liquidity inflows is less evident in high fee pools. While an increase in gas prices reduce the probability of liquidity inflows by 1.43\%, it actually leads to a 11.6\% increase in the daily dollar inflow to the pool. Together with the result in Table \ref{tab:ordersize} that the size of individual mints increases with gas prices, our evidence is consistent with the model implication that higher fixed transaction costs change the composition of liquidity supply on the high-fee pool, with small $\LP$ being substituted by larger $\LP$s switching over from the low-fee pool.


\begin{table}
\caption{Liquidity flows and gas costs on fragmented pools} \label{tab:flows}
\begin{minipage}[t]{1\columnwidth}%
\footnotesize
			This table reports the coefficients of the following regression:
	\begin{align*}
    y_{ijt}=\alpha + \beta_0 d_\emph{low-fee, ij} + \beta_1 \text{GasPrice}_{jt} d_\emph{low-fee, ij} + \beta_2 \text{GasPrice}_{jt} \times d_\emph{high-fee, ij} + \sum \beta_k \emph{Controls}_{ijt} + \theta_j + \varepsilon_{ijt}
    \end{align*}
	where the dependent variable $y_{ijt}$ can be (i) the aggregate dollar value of mints (in logs), or (vi) a dummy variable taking value one hundred if there is at least one mint on liquidity pool $i$ in asset $j$ on day $t$. $d_\emph{low-fee, ij}$ is a dummy that takes the value one for the pool with the lowest fee in pair $j$ and zero else. $d_\emph{high-fee, ij}$ is defined as $1-d_\emph{low-fee, ij}$. $\emph{GasPrice}_{jt}$ is the average of the lowest 100 bids on liquidity provision events across all pairs on day $t$, standardized to have a zero mean and unit variance. \emph{Volume} is the natural logarithm of the sum of all swap amounts on day $t$, expressed in thousands of US dollars. \emph{Total value locked} is the natural logarithm of the total value locked on Uniswap v3 pools on day $t$, expressed in millions of dollars.\emph{Volatility} is computed as the daily range between high and low prices on the most active pool for a given pair.All regressions include pair and week fixed-effects. Robust standard errors in parenthesis are clustered by week and ***, **, and * denote the statistical significance at the 1, 5, and 10\% level, respectively.  The sample period is from May 4, 2021 to July 15, 2023. 
\end{minipage}
\begin{center}
\begin{tabular}{lcccccc}
\toprule
 & \multicolumn{3}{c}{Daily mints (log US\$)} &  \multicolumn{3}{c}{$\text{Prob}\left(\text{at least one mint}\right)$} \\
 & (1) & (2) & (3) & (4) & (5) & (6) \\
\cmidrule{1-7}
$ d_\text{low-fee}$ & 0.43*** & 0.43*** & 0.43*** & 1.38* & 1.37* & 1.38* \\
 & (6.07) & (6.07) & (6.07) & (1.71) & (1.71) & (1.71) \\
Gas price $\times$ $ d_\text{low-fee}$ & -0.35*** & -0.35*** & -0.46*** & -6.02*** & -6.01*** & -4.58*** \\
 & (-8.50) & (-8.50) & (-7.14) & (-9.13) & (-9.13) & (-6.76) \\
Gas price $\times$ $ d_\text{high-fee}$ & 0.11** & 0.11** &  & -1.43** & -1.43** &  \\
 & (2.15) & (2.15) &  & (-2.57) & (-2.57) &  \\
Volume & 0.26*** & 0.26*** & 0.26*** & 0.96*** & 0.96*** & 0.96*** \\
 & (14.78) & (14.77) & (14.78) & (3.93) & (3.93) & (3.93) \\
Total value locked & -0.07 & -0.07 & -0.07 & 1.47 & 1.47 & 1.47 \\
 & (-0.78) & (-0.78) & (-0.78) & (1.01) & (1.00) & (1.01) \\
Volatility & -0.01 &  & -0.01 & 0.26 &  & 0.26 \\
 & (-0.68) &  & (-0.68) & (0.59) &  & (0.59) \\
Gas price &  &  & 0.11** &  &  & -1.43** \\
 &  &  & (2.15) &  &  & (-2.57) \\
Constant & 2.61*** & 2.61*** & 2.61*** & 51.44*** & 51.43*** & 51.44*** \\
 & (73.46) & (73.49) & (73.46) & (126.67) & (127.28) & (126.67) \\
 &  &  &  &  &  &  \\
Pair FE & Yes & Yes & Yes & Yes & Yes & Yes  \\
Week FE & Yes & Yes & Yes & Yes & Yes & Yes  \\
Observations & 40,288 & 40,288 & 40,288 & 40,288 & 40,288 & 40,288 \\
 R-squared & 0.47 & 0.47 & 0.47 & 0.28 & 0.28 & 0.28 \\ \hline
\bottomrule
\multicolumn{7}{l}{Robust t-statistics in parentheses. Standard errors are clustered at week level.} \\
\multicolumn{7}{l}{*** p$<$0.01, ** p$<$0.05, * p$<$0.1} \\
\end{tabular}
\end{center}
\end{table}



\subsection{Liquidity cycles on high- and low-fee pools}
Next, we test Predictions \ref{pred:updates} and \ref{pred:updates_gas} on the duration of liquidity cycles on fragmented pools. Since the descriptive statistics in Table \ref{tab:sumstat} suggest that $\LP$s manage their positions over multiple days, we cannot accurately measure liquidity cycles in a pool-day panel. Instead, we use intraday data on liquidity events (either mints or burns) to measure the duration between two consecutive opposite-sign interactions by the same Ethereum wallet with a liquidity pool: either a mint followed by a burn, or vice-versa. 

To complement our previous analysis, we additionally control for whether each liquidity position is out of range (i.e., the price range set by the $\LP$ does not straddle the current price and therefore the $\LP$ does not earn fees). We further introduce wallet fixed effects to soak up variation in reaction times across traders.

Table \ref{tab:cycles} presents the results. Liquidity updates on decentralized exchanges are very infrequent, as times elapsed between consecutive interactions are measured in days or even weeks. In line with Prediction \ref{pred:updates}, we find evidence for shorter liquidity cycles on low-fee pools. The average time between consecutive mint and burn orders is 20.06\% shorter on the low-fee pool (from Model 1, the relative difference is 99.74 hours/497.18 hours).

Liquidity cycles are in part driven by fixed Blockchain transaction costs. A one standard deviation increase in gas prices speeds up the liquidity cycle on low-fee pools by a further 15.80 hours, a result which supports the intuition behind Prediction \ref{pred:updates_gas}. When the gas price spikes, the liquidity supply on the low-fee pool decreases at a higher rate than the liquidity demand. As a result, liquidity deposits deplete faster (i.e., they move outside the fee-earning range), triggering the need for more frequent updates. At the same time, a higher gas fee speeds up the liquidity cycle on the high-fee pool as well. The result is consistent with small liquidity providers on the high-fee pool being crowded out by the high fixed costs, leading to a lower liquidity supply.



\begin{table}
\caption{Liquidity cycles on fragmented pools} \label{tab:cycles}
\begin{minipage}[t]{1\columnwidth}%
\footnotesize
			This table reports the coefficients of the following regression:
	\begin{align*}
    y_{ijtk}=\alpha + \beta_0 d_\emph{low-fee, ij} + \beta_1 \text{GasPrice}_{jt} d_\emph{low-fee, ij} + \beta_2 \text{GasPrice}_{jt} \times d_\emph{high-fee, ij} + \sum \beta_k \emph{Controls}_{ijt} + \theta_j + \varepsilon_{ijt}
    \end{align*}
	where the dependent variable $y_{ijt}$ can be (i) the mint-to-burn time, (ii) the burn-to-mint time, measured in hours, for a transaction initiated by wallet $k$ on day $t$ and pool $i$ trading asset $j$. The mint-to-burn and burn-to-mint times are computed for consecutive interactions of the same wallet address with the liquidity pool. $d_\emph{low-fee, ij}$ is a dummy that takes the value one for the pool with the lowest fee in pair $j$ and zero else. $d_\emph{high-fee, ij}$ is defined as $1-d_\emph{low-fee, ij}$. $\emph{GasPrice}_{jt}$ is the average of the lowest 100 bids on liquidity provision events across all pairs on day $t$, standardized to have a zero mean and unit variance. \emph{Volume} is the natural logarithm of the sum of all swap amounts on day $t$, expressed in thousands of US dollars. \emph{Total value locked} is the natural logarithm of the total value locked on Uniswap v3 pools on day $t$, expressed in millions of dollars. \emph{Volatility} is computed as the daily range between high and low prices on the most active pool for a given pair. \emph{Position out-of-range} is a dummy taking value one if the position being burned or minted is out of range, that is if the price range selected by the $\LP$ does not straddle the current pool price. All variables are measured as of the time of the second leg of the cycle (i.e., the burn of a mint-burn cycle). All regressions include pair, week, and trader wallet fixed-effects. Robust standard errors in parenthesis are clustered by day and ***, **, and * denote the statistical significance at the 1, 5, and 10\% level, respectively.  The sample period is from May 4, 2021 to July 15, 2023. 
\end{minipage}
\begin{center}
\begin{tabular}{lcccccc}
\toprule
 & \multicolumn{3}{c}{Mint-burn time} & \multicolumn{3}{c}{Burn-mint time} \\
 & (1) & (2) & (3) & (4) & (5) & (6)  \\
\cmidrule{1-7}
$ d_\text{low-fee}$ & -99.74*** & -100.17*** & -104.09*** & -157.95*** & -159.71*** & -159.69*** \\
 & (-8.86) & (-8.94) & (-9.22) & (-10.59) & (-10.81) & (-10.80) \\
Gas price $\times$ $ d_\text{low-fee}$ & -16.65** & -15.41* & -15.80** & -11.29 & 2.95 & 2.94 \\
 & (-2.13) & (-1.98) & (-2.02) & (-1.65) & (0.40) & (0.39) \\
Gas price $\times$ $ d_\text{high-fee}$ & -14.44** & -13.42* & -13.98* & -10.52* & 1.96 & 1.95 \\
 & (-2.04) & (-1.89) & (-1.96) & (-1.69) & (0.32) & (0.32) \\
Volume &  & -5.87 & -7.45 &  & -24.84*** & -24.82*** \\
 &  & (-1.15) & (-1.41) &  & (-4.10) & (-4.09) \\
Total value locked &  & -53.17* & -51.72* &  & -12.71 & -12.71 \\
 &  & (-1.70) & (-1.66) &  & (-0.52) & (-0.52) \\
Volatility &  & -2.11*** & -2.26*** &  & -2.99*** & -2.98*** \\
 &  & (-2.75) & (-2.86) &  & (-3.36) & (-3.36) \\
Position out-of-range &  &  & 37.09*** &  &  & -1.53 \\
 &  &  & (6.43) &  &  & (-0.22) \\
Constant & 497.18*** & 497.00*** & 479.22*** & 248.00*** & 250.13*** & 250.47*** \\
 & (91.65) & (90.60) & (82.13) & (29.91) & (30.27) & (30.32) \\
 &  &  &  &  &  &  \\
 Pair FE & Yes & Yes & Yes & Yes & Yes & Yes  \\
 Week FE & Yes & Yes & Yes & Yes & Yes & Yes  \\
 Trader wallet FE & Yes & Yes & Yes & Yes & Yes & Yes \\
Observations & 405,586 & 405,584 & 405,584 & 265,848 & 265,848 & 265,848 \\
 R-squared & 0.82 & 0.82 & 0.82 & 0.37 & 0.37 & 0.37 \\ \hline
\bottomrule
\multicolumn{7}{l}{Robust t-statistics in parentheses. Standard errors are clustered at week level.} \\
\multicolumn{7}{l}{*** p$<$0.01, ** p$<$0.05, * p$<$0.1} \\
\end{tabular}

\end{center}
\end{table}


The reaction time of a trader may depend on capital constraints, network congestion, and other confounding factors that can correlate with gas prices. As a robustness check, we repeat the analysis above with burn-to-mint times as the dependent variables. The burn-to-mint time measures the speed at which $\LP$s deposit liquidity at updated prices after removing (out-of-range) positions, and should not depend on the rate at which liquidity is consumed. Consistent with the theory, we find no significant relationship between gas price and the burn-to-mint duration (Models 4 through 6).



\subsection{Adverse selection costs across low- and high-fee pools}

In our model, the first-order friction driving liquidity fragmentation is the fixed gas cost, which leads to heterogeneous rebalancing costs for small and large market makers respectively. Thus, pool fees in our setup simply offset liquidity providers' costs to manage their position. An alternative channel driving fragmentation might be adverse selection: The rationale is that liquidity providers gravitate towards high-fee pools as they provide superior protection against informed traders \citep[following the arguments in][]{milionis2023automated}. 

For example, consider a token pair traded in the 5 (low) and 30 (high) basis point fee pools. If an arbitrage opportunity is worth 50 basis points and the relative gas cost is 15 basis points, arbitrageurs would optimally execute swaps on both pools since the trade value surpasses total cost, but obtain lower profits on the high-fee pool. However, if gas cost rises to 25 basis points, arbitrageurs would only trade in the low fee pool. Thus, large gas costs might make the high-fee pool more appealing to liquidity providers, as it offers added protection against adverse selection. The mechanism could provide an alternative explanation for the result in Table \ref{tab:markeshare} showing that market makers shift to high-fee pools when gas prices rise. In this section, we investigate differences in adverse selection across low- and high-fee pools, as well as the role of asymmetric information costs in driving liquidity fragmentation.

Our main metric for informational costs is the \emph{loss-versus-rebalancing} (LVR), as defined in \citet{zhang2023amm}. The measure is equivalent to the adverse selection component of the bid-ask spread in equity markets. To calculate it, for each swap \(j\) exchanging \(\Delta x_j\) for \(\Delta y_j\) in a pool with assets \(x\) and \(y\), we use:
\begin{equation}
      \text{LVR}_{j}=d_j \times \Delta x_j (p_{\text{swap},j}-p^\prime_j),
\end{equation}
where \(d_j\) is one for a ``buy'' trade (\(\Delta x_j<0\)) and minus one for a ``sell'' trade (\(\Delta x_j>0\)). The effective swap price is \(p_{\text{swap},j}=-\frac{\Delta y_j}{\Delta x_j}\), and \(p^\prime_j\) represents a benchmark price.

We use two benchmark prices \(p^\prime_j\) in our analysis. The first, \(p^\prime_j=p_{j}^{\Delta t=0}\), is the pool's equilibrium price immediately after a swap. The resulting LVR metric captures both temporary and permanent price impact, driven by uninformed and informed trades, respectively, and represents an upper bound for $\LP$'s adverse selection cost. 

The second benchmark is the liquidity-weighted average price across Uniswap v3 pools, measured with a one-hour delay after the swap (\(p^\prime_j=p_{j}^{\Delta t=1h}\)). This approach assumes that any price deviations caused by uninformed liquidity trades are corrected by arbitrageurs within an hour, as supported by \citet{LeharParlour2021}. Thus, the LVR metric derived using this benchmark captures only the permanent price impact, a more precise measure of adverse selection cost for liquidity providers.\footnote{Our methodology is equivalent to the one in \citet{zhang2023amm} under two assumptions. First, liquidity providers can re-balance their position following each swap. Second, we assume that our two benchmarks for $p^\prime_j$, derived from decentralized exchange data, closely track the fundamental value of the token. This perspective aligns with \citet{han2022trust}, who also note that centralized exchange prices are subject to manipulative practices such as wash trading. Further, our selection of benchmarks reflects the fact that our sample includes several token pairs not traded on major centralized exchanges such as Binance.}

To compute LVR for each day $t$ and liquidity pool $i$, we aggregate the loss-versus-balancing for each swap within a day. We subsequently winsorize our measures at the 0.5\% and 99.5\% quantiles to remove extreme outliers. The resulting sum is normalized by dividing it by the total value locked (TVL) in the pool at day's end:
\begin{equation}\label{eq:LVR}
      \text{LVR}_{i,t}=\frac{\sum_j \text{LVR}_{j, i,t}}{\text{TVL}_{i,t}},  
\end{equation}
which ensures that the LVR metric is comparable across pools trading different token pairs.

We complement our analysis with the calculation of \emph{impermanent loss} (IL), an additional metric for assessing adverse selection costs. Impermanent loss is defined as the negative return from providing liquidity compared to simply holding the assets outside the exchange and marking them to market as prices change \citep[see, for example,][]{aoyagi2020,BarbonRanaldo2021}.

The key distinction between IL and loss-versus-rebalancing (LVR) measures lies in their assumptions about liquidity providers' strategies \citep{zhang2023amm}. While LVR assumes that providers actively re-balance their holdings by mirroring decentralized exchange trades on centralized exchanges at the fundamental value to hedge market risk, IL is based on a more passive approach where providers maintain their positions without active re-balancing. Loss-versus-rebalancing is a function of the entire price path, reflecting constant rebalancing by liquidity providers. In contrast, impermanent loss is determined solely by the initial and final prices of the assets.

We obtain hourly liquidity snapshots from the Uniswap V3 Subgraph to calculate impermanent loss for a theoretical symmetric liquidity position. This position is set within a price range of \(\left[\frac{1}{\alpha} p, \alpha p\right]\), centered around the current pool price \(p\), with \(\alpha\) set to 1.05. We set a one-hour horizon to measure changes in position value, aligning with the time horizon used for the LVR metric. In Appendix \ref{app:IL}, we present the exact formulas for calculating impermanent loss on Uniswap V3, based on the methodology described by \citet{Heimbach2023}. 



\begin{table}
\scriptsize
\caption{Adverse selection costs on high- and low-fee pools}\label{tab:lvr}
\begin{minipage}[t]{1\columnwidth}%
\footnotesize
This table presents regression results that analyze adverse selection costs in fragmented Uniswap v3 pools. For columns (1) through (4), the dependent variable is loss-versus-rebalancing (LVR), as defined in equation \eqref{eq:LVR}. We use the one-hour horizon benchmark (\(p_j^{\Delta t=1h}\)) in models (1) and (2) to measure permanent price impact, and the immediate, same-block price benchmark (\(p_j^{\Delta t=0}\)) in models (3) and (4) to measure total price impact. For columns (5) and (6), the dependent variable is the impermanent loss for a symmetric liquidity position at $\pm 5\%$ centered around the current pool price. The average impermanent loss is calculated for each day, based on Ethereum blocks mined within that day. The impermanent loss computation uses a one-hour liquidity provider horizon, comparing current pool prices with those one hour later. For columns (7) and (8), the dependent variables are the liquidity (TVL) and volume share of the pool, measured in percent. Finally, in columns (9) and (10) the dependent variable is the absolute deviation of the Uniswap pool price from Binance prices, sampled hourly, and measured in percent.
$d_\emph{low-fee, ij}$ is a dummy that takes the value one for the pool with the lowest fee in pair $j$ and zero else. $\emph{GasPrice}_{jt}$ is the average of the lowest 100 bids on liquidity provision events across all pairs on day $t$, standardized to have a zero mean and unit variance.  \emph{Volume} is the natural logarithm of the sum of all swap amounts on day $t$, expressed in thousands of US dollars. \emph{Total value locked} is the natural logarithm of the total value locked on Uniswap v3 pools on day $t$, expressed in millions of dollars.  When LVR is an explanatory variable, it is calculated using the one-hour ahead benchmark price.  \emph{Volatility} is computed as the daily range between high and low prices on the most active pool for a given pair. All regressions include pair and week fixed-effects. Robust standard errors in parenthesis are clustered by week, and ***, **, and * denote the statistical significance at the 1, 5, and 10\% level, respectively.  The sample period is from May 4, 2021 to July 15, 2023. 
\end{minipage}

\begin{center}
\resizebox{1\textwidth}{!}{  
\begin{tabular}{lcccccccccc}
\toprule
& \multicolumn{2}{c}{LVR (1h horizon)} & \multicolumn{2}{c}{LVR (after swap)} & \multicolumn{2}{c}{Impermanent loss} & TVL share & Volume share & \multicolumn{2}{c}{CEX price deviation} \\
& \multicolumn{2}{c}{Permanent price impact} & \multicolumn{2}{c}{Total price impact} \\
\cmidrule{1-11} 
 & (1) & (2) & (3) & (4) & (5) & (6) & (7) & (8) & (9) & (10) \\
\cmidrule{1-11}
$ d_\text{low-fee}$ & 6.39*** & 6.39*** & 29.78*** & 29.67*** & 1.08*** & 1.13*** & -21.00*** & 24.43*** & 0.06 & -0.00 \\
 & (16.57) & (17.05) & (14.86) & (14.95) & (5.72) & (6.18) & (-26.45) & (19.79) & (1.51) & (-0.06) \\
Gas price $\times$ $ d_\text{low-fee}$ &  & -0.75** &  & 3.51** &  & -0.01 & -4.41*** & -6.16*** &  & 0.09 \\
 &  & (-2.05) &  & (2.10) &  & (-0.05) & (-6.52) & (-5.64) &  & (0.95) \\
Gas price $\times$ $ d_\text{low-fee}$ $\times$ LVR &  &  &  &  &  &  & -0.38* & -0.48 &  & -0.10* \\
 &  &  &  &  &  &  & (-1.88) & (-1.45) &  & (-1.68) \\
Gas price &  & 2.61*** &  & 6.16** &  & 3.71*** & 1.53*** & 2.82*** &  & -0.09 \\
 &  & (2.74) &  & (2.53) &  & (3.76) & (4.73) & (5.23) &  & (-0.83) \\
Gas price $\times$ LVR &  &  &  &  &  &  & 0.59*** & 0.56*** &  & 0.11** \\
 &  &  &  &  &  &  & (4.26) & (2.80) &  & (2.17) \\
Loss-versus-rebalancing (LVR) &  &  &  &  &  &  & 0.41*** & 0.67*** &  & 0.11*** \\
 &  &  &  &  &  &  & (2.72) & (3.86) &  & (6.05) \\
Volume &  & 3.22*** &  & 8.67*** &  & 1.81*** & -0.02 & -0.30*** &  & 0.18*** \\
 &  & (8.15) &  & (6.61) &  & (6.22) & (-0.56) & (-3.18) &  & (3.82) \\
Total value locked &  & 0.53 &  & -2.12 &  & 1.93 & -0.13 & 0.46 &  & -0.33*** \\
 &  & (0.14) &  & (-0.34) &  & (0.74) & (-0.52) & (0.77) &  & (-4.00) \\
Volatility &  & 1.85*** &  & 4.23*** &  & 6.69** & -0.36 & -1.27*** &  & 0.77*** \\
 &  & (2.87) &  & (3.17) &  & (2.61) & (-1.16) & (-3.13) &  & (3.16) \\
Constant & 7.85*** & 7.86*** & 8.88*** & 8.97*** & 7.37*** & 7.51*** & 60.22*** & 41.59*** & 0.60*** & 0.64*** \\
 & (40.71) & (36.89) & (8.87) & (8.88) & (77.84) & (61.32) & (162.17) & (71.02) & (30.71) & (38.64) \\
 &  &  &  &  &  &  \\
Pair FE & Yes & Yes & Yes & Yes & Yes & Yes & Yes & Yes & Yes & Yes  \\
Week FE & Yes & Yes & Yes & Yes & Yes & Yes & Yes & Yes & Yes & Yes \\
Observations & 40,302 & 40,288 & 40,302 & 40,288 & 40,250 & 40,248 & 40,288 & 36,059 & 5,207 & 5,207 \\
 R-squared & 0.14 & 0.15 & 0.09 & 0.10 & 0.09 & 0.11 & 0.10 & 0.13 & 0.10 & 0.11 \\ \hline
\bottomrule
\multicolumn{11}{l}{Robust t-statistics in parentheses. Standard errors are clustered at week level.} \\
\multicolumn{11}{l}{*** p$<$0.01, ** p$<$0.05, * p$<$0.1} \\
\end{tabular}
}
\end{center}
\end{table}

Table \ref{tab:lvr} presents our empirical results. In line with \citet{milionis2023automated}, all price impact measures --- that is, the immediate and one-hour horizon LVR and the impermanent loss --- are significantly larger in low-fee pools. This indicates that a higher liquidity fee indeed acts as barrier to arbitrageurs. Specifically, the permanent price impact, measured by the one-hour horizon LVR, is 6.85 basis points or 81\% larger in low-fee pools. The total price impact, represented by the after-swap LVR metric, is 3.5 times larger in low-fee pools. The wide gap between permanent and total price impact highlights the substantially higher volume of uninformed trading in low-fee pools. Further, an increase in gas prices leads to a 3.51 wider gap in total price impact but a 0.75 bps narrower gap in permanent price impact between the high- and low-fee pools. The result suggests that a higher gas price primarily discourages uninformed traders, rather than arbitrageurs, from trading on high-fee pools. 

The findings in Table \ref{tab:markeshare} reveal that a higher gas cost translates to a lower liquidity and volume market share for low-fee pools. We attribute this effect primarily to the fixed costs associated with re-balancing. To examine whether the impact of gas prices on market share is driven by adverse selection, in Models (7) and (8) we add an interaction between our permanent price impact measure (one-hour horizon LVR), a dummy variable for low-fee pools, and the standardized gas price. The analysis reveals that adverse selection contributes only 8\% (computed as $\nicefrac{0.38}{4.41+0.38}$) to the effect of gas prices on liquidity market shares. Moreover, this coefficient is only marginally statistically significant. A similar pattern is observed for trading volume shares in Model 8.

Finally, in Models (9) and (10) of Table \ref{tab:lvr} we explore whether various arbitrage frictions lead to price discrepancies between high- and low-fee pools. For this purpose, we collect hourly price data from Binance for the largest four pairs by trading volume: WBTC-WETH, USDC-WETH, WETH-USDT, and USDT-USDC. We subsequently compute daily averages of hourly price deviations between centralized and decentralized exchanges. The analysis reveals that the average hourly price deviation across centralized and decentralized exchanges is 0.60\%. Notably, there is no significant difference in price deviations between low- and high-fee pools. The result suggests that arbitrage activities remain efficient despite the differences in trading costs between these pools.

\begin{figure}[H]
\caption{\label{fig:lvr} Price impact and price deviations across high- and low-fee pools}
\begin{minipage}[t]{1\columnwidth}%
\footnotesize
This figure plots the average total and permanent price impact, liquidity yield, and price deviation from centralized exchanges across low and high fee pools for fragmented pairs.
\end{minipage}

\vspace{0.05in}

\begin{centering}

\includegraphics[width=\textwidth]{Figures/Empirics_202308/lvr.png}


\par\end{centering}

\end{figure}

Figure \ref{fig:lvr} graphically illustrates the result, contrasting permanent price impact measures against the liquidity yield, as calculated in equation \eqref{eq:liq_yield}. Notably, before accounting for gas costs, we observe that liquidity providers in low-fee pools experience losses on average: the average daily permanent price impact in these pools is 14.21 basis points, which exceeds the fee revenue of 11.71 bps.  In contrast, liquidity providers in high-fee pools approximately break even before considering gas costs: the fee revenue amounts to 9.69 bps, which is slightly higher than the permanent price impact of 7.85 bps. One should keep in mind, however, that the magnitude of losses from adverse selection depends on the horizon at which we measure the loss-versus-rebalancing.

==> Old/introduction.tex <==
Uniswap V3 offers liquidity providers two instruments to manage adverse selection risk:
\begin{itemize}
    \item A menu of liquidity fees (currently set to either 0.01\%, 0.05\%, 0.3\%, or 1\% of the incoming trade value), analogous to a tick size that pins down a fixed spread \citep{LeharParlour2021}. 
    \item ``Concentrated liquidity:'' the possibility to set up a (narrow) price band for providing liquidity, akin to a limit order in traditional markets.
\end{itemize}

\mz{(To confirm with model!)} To an extent, the two instruments are substitutes. Adjusting the liquidity provision price band is a more flexible and precise tool to manage adverse selection risk. At the same time, it is more costly since it requires frequent adjustment of the price band as the reference price moves. Managing liquidity on Uniswap is costly since every interaction with the decentralized exchange requires paying a gas fee. Importantly, the gas fee is (to a first approximation) a fixed cost as does not scale with the dollar value of the order.

In an environment with heterogeneous liquidity provider (LP) capital, liquidity becomes segmented across pools with different fees. High-capital LPs commit large chunks of liquidity to the market and manage it frequently: gas fees are small relative to order size. The ability to frequently adjust their liquidity position allows high-capital LPs to participate in markets with a smaller fixed liquidity fee. On the other hand, low-capital LPs cannot manage liquidity at high frequency and rely on a large liquidity fee to protect them against adverse selection risk. In equilibrium, the low-fee market captures most of the liquidity and trading volume. Liquidity is provided in large chunks by high-capital accounts, is concentrated in a smaller price range, and actively managed. The high-fee market captures liquidity provided in smaller amounts by low-capital accounts and is less actively managed.

\paragraph{Implications/hypotheses}
\begin{enumerate}
    \item Time variation in gas fees can be used to test the model implications. A lower gas fee reduces constraints for low-capital investors, yielding higher liquidity share for the low fee exchange. 
    \item What drives the emergence of multiple active pools for the same share? The volatility of the pair is a factor. For pairs like USDC/USDT, where information asymmetries are low, everyone converges to the low-fee 0.01\% pair.
    \item Informational content on trades on the two markets? Low-capital LPs might be exposed to large informed trades that have already consumed the liquidity on low-fee pools. Is the liquidity fee sufficient compensation? Is there an optimal liquidity fee menu? Or, is it better to have a single fee as on Uniswap V2?
\end{enumerate}

\begin{figure}[H]
\caption{Liquidity provision in Uniswap v3. Stylized facts \mz{To be updated w/ all pairs.} \label{fig:stylized}} 
\begin{minipage}[t]{1\columnwidth}%
\footnotesize
We plot stylized facts on liquidity minting and trading activity in the most active Uniswap v3 pairs (\texttt{USDC-WETH},\texttt{WETH-USDT}, \texttt{DAI-WETH}, and \texttt{USDC-USDT}) across pools with different fees. All variables are computed as monthly average. Liquidity events are scraped from the Ethereum blockchain as interactions with the \texttt{Uniswap V3 Positions NFT} contract. Liquidity is computed as the parameter $L$ in the Uniswap v3 \href{https://uniswap.org/whitepaper-v3.pdf}{whitepaper}. The price range size for a particular liquidity mint is computed as $\frac{\text{Upper}-\text{Lower}}{0.5\left(\text{Upper}+\text{Lower}\right)}$, where the \emph{Upper} and \emph{Lower} prices are inferred from the tick parameters $i_u$ and $i_l$, respectively, submitted to the \texttt{Uniswap V3 Positions NFT} smart contract. The average liquidity mint (bottom-left panel) is measured in standard deviations at pair level across all pools. We refer to a liquidity mint as \emph{two-sided} if the liquidity provider deposits non-zero amounts of both tokens in a given pair.

\end{minipage}

\vspace{0.1in}
    \centering
    \includegraphics[width=0.9\textwidth]{Figures/stylized_facts.png}
\end{figure}

==> Old/introduction_202307.tex <==
In 1971, Fischer Black explored the concept of computer-driven ``automated exchanges'' that could streamline intermediation in financial markets \citep{Black1971}. One important argument was that broadening the group of traders who provide liquidity would alleviate the limitations imposed by a specialist's inventory size. Over the following half-century, markets progressively moved in this direction, with the majority of exchanges now operating as limit order books, theoretically enabling any trader to supply liquidity. However, in practice, the rise of algorithmic and high-frequency trading made liquidity provision in limit order markets a technology-intensive affair, necessitating low-latency connectivity and active management of quotes. Some trader categories, such as retail investors, struggle to competitively supply liquidity in this environment.

Decentralized exchanges (DEXs), which function as fully automated trading platforms implemented as smart contracts on public blockchains, offer a novel passive liquidity supply mechanism which requires significantly fewer quote updates. Market makers can deposit and withdraw funds into a ``liquidity pool,'' and trade prices are determined by an Automated Market Maker algorithm \citep[see, e.g.,][]{park2022} as a function of the available funds in the pool. They receive compensation through liquidity fees, computed as a fixed percentage of trading volume charged to traders seeking immediate execution, as opposed to bid-ask spreads. Uniswap, the leading decentralized exchange, allows for the fragmentation of trading for each token pair across multiple pools with varying liquidity fees.  In Appendix \ref{sec:app-dex}, we discuss in depth the trading mechanics on Uniswap.

The passive nature of liquidity supply in DEXs was initially designed to minimize interactions with blockchain smart contracts, as these interactions incur gas costs to compensate the decentralized network for spent computational power. Nevertheless, passive liquidity supply is particularly well-suited for small retail liquidity providers, who face their own time and effort fixed costs. Can the mechanisms used by decentralized exchanges have a comparable impact on liquidity supply as ETFs had on transforming portfolio management in recent decades?

Our paper shows that fixed costs translate to significant economies of scale on decentralized exchanges, which lead to market fragmentation and the emergence of liquidity provider clienteles. Specifically, our findings reveal that a small number of highly active large liquidity providers, potentially institutional investors and hedge funds, primarily trade against numerous small incoming trades on pools with low fees. In contrast, high-fee pools involve less frequent trading between a substantial number of capital-constrained passive liquidity providers (e.g., retail market makers) on one side and a few sizeable incoming orders on the other. The underlying economic mechanism is that smaller liquidity providers strategically trades off a lower execution probability against higher liquidity fee and less frequent fixed costs, such as gas fees.



% Market makers on decentralized exchanges are primarily compensated by liquidity fees: a fixed percentage of trading volume levied on traders who demand immediacy. If the current price (i.e., the pool ``mid-point'') drifts outside of the liquidity providers' price range, the position stops earning fees.\footnote{In a limit order market, the situation corresponds to a limit order being filled and then immediately re-posted at the old price which is deeper in the book.} To be able to earn fees again, liquidity providers need to cancel (``burn'') the old position and deposit (``mint'') tokens specifying a new price range that straddles the current benchmark price. While such re-balancing is trivial on centralized exchanges, liquidity providers on DEXs have to pay a significant fixed cost each time they interact with the liquidity pool's smart contract. For the Ethereum blockchain, the fixed cost corresponds to the price of ``gas'' needed to compensate the decentralized network for spent computational power.

% We find that low-fee pools are very active and match a handful of large liquidity providers (such as institutional investors and hedge funds) with many small incoming trades. In contrast, trading on high-fee pools involves infrequent trades between a large number of capital-constrained passive liquidity providers (e.g., retail market makers) on the one side and a few sizeable incoming orders, on the other. 


% Thirty years ago, \citet{Glosten1994} conjectured that the limit order book is an ``inevitable'' equilibrium market design for trading financial securities. The recent evolution of decentralized exchanges (DEXs), fully automated trading platforms built as smart contracts on top of public blockchains, lends further weight to this argument. 

% Early iterations of decentralized exchange protocols (such the 2018 version of Uniswap) allowed market makers to deposit and withdraw funds to a ``liquidity pool,'' but not to set price limits beyond which they do not want to provide liquidity -- i.e., akin to bid and ask prices in traditional markets. Instead, trade prices are exogenously determined by an Automated Market Maker algorithm \citep[see, e.g.,][]{park2022}. Modern implementations alleviate the rigidity of automated market makers and bring the DEX design closer to that of limit order books. Uniswap v3, the world's leading DEX with a 40\% volume share as of November 2022, distinguishes itself from its predecessors and competitors by effectively allowing traders to submit limit orders. Liquidity providers can specify a maximum (minimum) price at which they are willing to buy (sell) the asset. With a fine enough tick size, depth on Uniswap v3 can therefore replicate any arbitrary price schedule on a limit order book.\footnote{Uniswap Labs refers to these orders as ``concentrated liquidity'' or ``range orders'' -- see, for example, \url{https://docs.uniswap.org/protocol/concepts/V3-overview/range-orders}. Liquidity providers can set prices on a relatively fine price grid -- the tick size for liquid pairs ranges from 1 to 10 basis points. Prices inside the grid are set exogenously by the same AMM constant product logic as described, for example, in \citet{LeharParlour2021}. We provide an in-depth discussion of trading mechanics on Uniswap v3 in Appendix \ref{sec:app-dex}.}

% Our paper shows, both theoretically and empirically, that the ability to deploy limit orders on decentralized exchanges may lead to fragmented markets. The rationale is that liquidity providers submitting limit orders need to frequently manage their position as the market price drifts outside the pre-set range. While such re-balancing is trivial on centralized exchanges, liquidity providers on DEXs have to pay a significant fixed cost each time they interact with the liquidity pool's smart contract. For the Ethereum blockchain, the fixed cost corresponds to the price of ``gas'' needed to compensate the decentralized network for spent computational power.

% Market makers on decentralized exchanges are primarily compensated by liquidity fees: a fixed percentage of trading volume levied on traders who demand immediacy. If the current price (i.e., the pool ``mid-point'') drifts outside of the liquidity providers' price range, the position stops earning fees.\footnote{In a limit order market, the situation corresponds to a limit order being filled and then immediately re-posted at the old price which is deeper in the book.} To be able to earn fees again, liquidity providers need to cancel (``burn'') the old position and deposit (``mint'') tokens specifying a new price range that straddles the current benchmark price. We show that high enough gas prices drive the emergence of heterogeneous market maker clienteles across pools with different fees. Low-fee pools are very active and match a handful of large liquidity providers (such as institutional investors and hedge funds) with many small incoming trades. In contrast, trading on high-fee pools involves infrequent trades between a large number of capital-constrained passive liquidity providers (e.g., retail market makers) on the one side and a few sizeable incoming orders, on the other. 


Our first contribution is a theoretical model of liquidity provision on decentralized exchanges. A continuum of liquidity providers ($\LP$s) choose to deposit their token endowments in either a high- or a low-fee pool; that is, they \emph{mint} liquidity. The liquidity providers have heterogeneous token endowments, which map to different capital constraints --- low-endowment $\LP$s are akin to retail traders, whereas high-endowment $\LP$s may stand in for large institutional investors or quantitative funds. Further, liquidity providers incur a fixed cost (i.e., gas price) each time they update their position.

Traders demanding liquidity route their orders first to the low-fee pool to minimize transaction costs. The high-fee pool executes the residual order flow from large traders who exhaust all liquidity at the cheaper venue. As a result, low-fee markets are actively traded and require frequent liquidity updates whereas high-fee pools have a longer liquidity update cycle since they absorb fewer trades. 

Both pools can attract a positive market share if the gas price is large enough due to economies of scale. Liquidity providers trade off a higher revenue per unit of time in the low-fee pool (driven by the larger trading volume) against the additional gas cost required for active liquidity management. As a result, market maker clienteles emerge in equilibrium. Liquidity providers with large endowments gravitate towards low-fee markets, as they are best positioned to frequently update their position. In contrast, smaller market makers choose to passively provide liquidity on high-fee markets where they only trade against large orders being routed there. They optimally trade off a lower execution probability against higher fees per unit of volume and a lower liquidity management cost per unit of time. 

Using the model for guidance, we analyze a data set comprising of more than 13 million interactions with Uniswap v3 liquidity pools -- that is, all liquidity updates and trades from May 2021 until September 2022. Uniswap v3 launched in May 2021 and quickly established itself as the leading decentralized exchange. Daily trading volume on Uniswap v3 typically exceeds US \$1 billion, whereas the total liquidity supply varies between US \$3-5 billion in our sample, across hundreds of cryptocurrencies. For major pairs such as Ether against USD stablecoins, Uniswap boasts twice or three times better liquidity than centralized exchanges such as Binance.\footnote{See \href{https://uniswap.org/blog/uniswap-v3-dominance}{The Dominance of Uniswap v3 Liquidity}; May 5, 2022.} 

The market design explicitly allows for fragmentation. Each asset pair to be traded on up to four liquidity pools that only differ in the compensation for liquidity providers: in particular, liquidity fees can be equal to 1, 5, 30, or 100 basis points and the corresponding tick sizes are 1, 10, 60, or 200 basis points. The liquidity pools are otherwise identical and, importantly, they share the common infrastructure of the Ethereum blockchain -- i.e., they are similarly impacted by variation in gas prices due to, say, network congestion. At launch, Uniswap Labs conjectured that trading and liquidity should consolidate in equilibrium on a single ``canonical'' pool for which the liquidity fee is just enough to compensate the marginal market maker for adverse selection and inventory costs. That is, activity in low-volatility pairs such as stablecoin-to-stablecoin trades should naturally gravitate to low fee liquidity pools, whereas speculative trading in more volatile pairs will consolidate on high fee markets.\footnote{See \emph{Flexible fees} paragraph at \url{https://uniswap.org/blog/uniswap-v3}; accessed September 14, 2022.}

We document significant liquidity fragmentation in 37 out of 217 asset pairs in our sample, which account for 84\% of liquidity committed to Uniswap v3 smart contracts and 94\% of trading volume. For each of the fragmented pairs, trading consolidates on two pools with adjacent fee levels: either 1 and 5 basis points (e.g., USDC-USDT), 5 and 30 basis points (ETH-USDC), or 30 and 100 basis points (USDC-CRV).

High-fee pools are on average larger -- with aggregate end-of-day liquidity of \$43.42 million relative to \$31.35 million, the average size of low-fee pools. Nevertheless, two thirds of trading volume executes on low-fee pools. In line with the model predictions, low-fee pools are more active as they capture many small trades. There are five times as many trades on low- than on high-fee pools (577 versus 111). However, the average trade on the high fee pool is twice as large: \$22,460 relative to \$9,890. Unsurprisingly, liquidity cycles -- measured as the time between the submission and update of an order -- are 19.85\% shorter on the highly active low-fee pool. 

We find evidence of market maker clienteles across pools. The average liquidity deposit is 91.5\% larger on the low-fee pool, after controlling for daily volume and return volatility. At the same time, there are 18\% fewer liquidity providers on low-fee pools. The results point to an asymmetric match between liquidity supply and demand: large $\LP$s are matched with small trader on low-fee pools, whereas a sizeable mass of small $\LP$s trade with a few large orders on the high-fee pool. 

The degree of market fragmentation depends on the magnitude of gas costs on the Ethereum blockchain. In the model, a higher gas price leads to a shift in liquidity supply from the low- to the high-fee pool as active position management becomes relatively more costly for the marginal $\LP$. We find that a one standard deviation increase in gas prices corresponds to a 2.30 percentage points decrease in the low-fee pool market share, and a 36\% drop in liquidity inflows on days when gas costs are elevated. As $\LP$s leave the low-fee pool, the time between position updates becomes 10\% shorter since incoming order flow depletes liquidity at a faster pace. The effect reinforces the expected gas cost difference between the two pools, leading to more $\LP$s switching to the high-fee venue.

Our paper relates to a nascent and fast-growing literature on the economics of decentralized exchanges. Many studies \citep[e.g.,][]{aoyagi2020,aoyagiito2021,park2022} focus on the economics of constant-function automated market makers, which do not allow liquidity providers to set price limits. In this restrictive environment, \citet{CapponiJia2021} argue that market makers have little incentives to update their position upon the arrival of news to avoid adverse selection, since pro-rata clearing gives an advantage to arbitrageurs. \citet{LeharParlour2021} solve for the equilibrium pool size in a setting where liquidity providers fully internalize information costs without rushing to withdraw positions at risk of being sniped. We argue that on exchanges that allow for limit or range orders, the cost of actively managing positions becomes a first-order concern, as $\LP$s need to re-set the price limits once posted liquidity no longer earns fees. Our empirical result on economies of scale echoes the argument in \citet{BarbonRanaldo2021}, who compare transaction costs on centralized and decentralized exchanges and find that high gas prices imply that the latter only become competitive for transactions over US\$100,000. \citet{HasbrouckRiveraSaleh2022} argue that higher liquidity fees on decentralized exchanges stimulate liquidity supply and lead to an increase in the equilibrium trading volume. We complement the argument by stating that high fees might be \emph{necessary} for some liquidity providers to cover the fixed costs of managing their position. In line with our theoretical predictions, \citet{caparros2023blockchain} find that liquidity providers reposition their quotes more often on Uniswap V3 pools built on Polygon, which features substantially lower gas fees. Finally, \citet{Heimbach2023} document that after accounting for price impact, concentrated liquidity on Uniswap v3 pools results in increased returns for sophisticated participants but losses for retail traders. 


Despite higher gas costs, decentralized exchanges may hold advantages over centralized venues. \citet{han2022trust} demonstrate Uniswap frequently leads price discovery compared to centralized exchanges such as Binance, despite the latter having higher trading volume. \citet{capponi2023price} find that the fee paid traders to establish execution priority unveils their private information, and therefore contributes to price discovery. \citet{ASPRIS2021101845} argue that decentralized exchanges offer better security than their centralized counterparts since assets are never transferred to the custody of a third party such as an exchange wallet. In turn, \citet{BrolleyZoican2022b} make the point that decentralized exchanges may be able to reduce overall computational costs associated with latency arbitrage races, as they eliminate long-term co-location subscriptions.

We also relate to a rich literature on market fragmentation and differential fees. Closest to our paper, \citet{Battalio2016} and \citet{Cimon2021} study the trade-off between order execution risk and compensation for liquidity provision in the context of make-take fee exchanges. However, \citet{Battalio2016} specifically addresses the issue of the broker-customer agency problem, whereas our study focuses on liquidity providers who trade on their own behalf. In traditional securities markets, make-take fees are contingent on trade execution and proportional to the size of the order.  On the other hand, gas costs on decentralized exchanges are independent of order execution, highlighting the significance of economies of scale (lower proportional costs for larger liquidity provision orders) and dynamic liquidity cycles (managing the frequency of fixed cost payments). Strategic brokers in \citet{Cimon2021} examines strategic brokers who provide liquidity alongside exogenous market-makers in a static setting. We complement this approach by modelling network externalities inherent in the coordination problem of heterogeneous liquidity suppliers. In our dynamic setup, this allows us to pin down the equilibrium duration of liquidity cycles and the relative importance of gas fixed costs.

Fixed costs for order submission are uncommon in traditional markets. However, in 2012, the Canadian regulator IIROC implemented an ``integrated fee model'' that charged traders for all messages sent to Canadian marketplaces. \citet{KorajczykMurphy2018} document that this measure disproportionately affected high-frequency traders, resulting in wider bid-ask spreads but lower implementation shortfall for large traders, possibly due to a reduction in back-running activity. Our study contributes additional insights by highlighting that the introduction of a fixed cost, even when applied across exchanges, can lead to market fragmentation.

The classical study of \citet{pagano1989trading} shows that if an asset is traded on two identical exchanges with equal transaction costs, in equilibrium market participants gravitate to a single exchange due to network effects. In practice, exchanges are rarely identical: fragmentation can emerge between fast and slow exchanges \citep{pagnotta2018competing, brocim:20} or between lit and dark markets \citep{Zhu2014}. In our model, fragmentation on decentralized exchanges is driven by variation in liquidity fees as well as different economies of scale due to heterogeneity in liquidity provider capital. We find that liquidity fragmentation driven by high gas fees implies larger transaction costs on incoming orders. We note that there is no time priority on decentralized exchanges, which clear in a pro rata fashion. On markets with time priority, \citet{FoucaultMenkveld2008} and \citet{Ohara2011market} find that market segmentation in equity markets improves liquidity (by allowing queue jumping) and price discovery.


==> Old/model.tex <==
% A model of AMM liquidity provision \citep[potentially as in][]{LeharParlour2021}, with a clientele effect due to investor heterogeneity \citep[maybe along the lines of][]{KhomynPutninsZoican2022}. Among key parameters are heterogeneous investor capital (or aversion to transaction fees) and network transaction fees.

\subsection{Model primitives}

\paragraph{Assets.} Consider a three-period economy, where time is indexed by $t\in\left\{0,1,2\right\}$. There are two assets: a risky token $\T$ and a riskless num\'{e}raire $\C$. At $t=2$, the risky token $\T$ pays a stochastic dividend $\tilde{v}$ (denominated in units of $\C$). At the start of the game, the expected token value is $\mathbb{E}_0 \tilde{v}=v>1$. 

The asset $\C$ stands in for cryptocurrencies typically used as num\'{e}raire on decentralized exchanges -- for example Ether (the native currency of the Ethereum blockchain) or stablecoins such as Tether or USD~Coin. The num\'{e}raire pays a risk-free rate of return $r$, which we normalize to zero without loss of generality.

\paragraph{Trading environment.} The risky token is traded on two liquidity pools: $L$ (a low-fee pool) and $H$ (a high-fee pool). The asset quantities in each pool $k\in\left\{L,K\right\}$ must satisfy at all times the following linear bonding curve:
\begin{equation}\label{eq:bond_curve}
    v \T_k + \C_k = \text{constant}.
\end{equation}
The bonding curve \eqref{eq:bond_curve} implies that the token price is constant and equal to $v$ units of the num\'{e}raire, since $-\frac{\diff T}{\diff C}=v$. To fix intuition behind the mechanics of the market, suppose a trader wishes to buy $t$ units of the token. This reduces the token amount in the pool to $\T_k-t$. In return, the trader needs to add $\Delta$ units of the num\'{e}raire, where $\Delta$ is such that the new asset quantities remain on the bonding curve, that is:
\begin{equation}
    v \left(\T_k-t\right) + \left(\C_k+\Delta\right) = v \T_k + \C_k,
\end{equation}
which is equivalent to having $\Delta = v t$. The slope of the bonding curve is equal to the expected value of the asset to ensure there are no arbitrage opportunities at the start of the game. 

The two liquidity pools charge different fees on liquidity-removing trades. Fees are expressed in units of num\'{e}raire and are distributed to all liquidity providers in a given pool, proportional to the amount of liquidity provided.  The low-fee pool $L$ charges a fee of $f~\C$ where $f<1$, and the high-fee pool $H$ charges a fee of $1~\C$ per token traded. That is, to purchase $t$ units of the token, the total cost of an investor is $t\left(v+f\right)$.

\paragraph{Events.} At $t=1$, two types of exogenous events can occur. With probability $\eta<1$, the common value of the token changes to $v+1$ (good news) or to $v-1$ (bad news); good and bad news are equally likely. With probability $\left(1-\eta\right)$ -- that is if news does not occur -- a liquidity trader ($\LT$) receives a private value shock and needs to trade $\tilde{\theta}$ units of the token, where $\tilde{\theta}\sim\text{Uniform}\left[0,1\right]$. The liquidity trader is equally likely to buy or sell the token. We assume the $\LT$s private value is large enough to cover transaction costs on either liquidity pool.

\paragraph{Liquidity providers and arbitrageurs.} In addition to liquidity traders, the token is traded by two types of agents: risk-neutral liquidity providers ($\LP$) and arbitrageurs ($\A$). There is a continuum of liquidity providers indexed by $i$, endowed with heterogeneous amounts of the token $T$. Liquidity provider $i$ is endowed with $t_i= \log\left(2\right) q_i$ units of the token. Following \citet{KhomynPutninsZoican2022}, we assume that $q_i$ is distributed with density
\begin{equation}\label{eq:density}
    \phi\left(q\right)=\log^{-1}\left(2\right)\frac{1}{q},\text{ for }q\in\left[1,2\right].
\end{equation}
The choice of density ensures that the aggregate token endowment of liquidity providers $\T_\text{agg}$ is normalized to one, since
\begin{equation}\label{eq:aggliq}
    \T_\text{agg}=\int_1^2 \underbrace{\log\left(2\right) q_i}_{\equiv t_i} \phi\left(q_i\right)\diff q_i = 1.
\end{equation}
Further, the density is chosen to match key features of the empirical distribution of $\LP$s: there are many low-endowment liquidity providers (e.g., retail traders) and a long tail of high-capital investors who provide liquidity to decentralized exchange -- for example, quantitative institutional investors. Figure \ref{fig:distribution} illustrates the distribution of $\LP$s endowments.

\begin{figure}[H]
\caption{\label{fig:distribution} Liquidity provider endowment (scaled) $q_i$}
\begin{minipage}[t]{1\columnwidth}%
\footnotesize
This figure illustrates the probability density of liquidity provider token endowments, $\phi\left(\cdot\right)$, as defined in equation \eqref{eq:density}.
\end{minipage}

\vspace{0.05in}

\begin{centering}
\includegraphics[width=0.7\textwidth]{Figures/model_density.png}
\par\end{centering}

\end{figure}

The arbitrageurs $\A$ are risk-neutral speculative traders as in \citet{Budish2015TheResponse} or \citet{Menkveld2017NeedLiquidity}, and have zero private value for the token. Upon observing a common value innovation, arbitrageurs can submit a trade against liquidity providers if (i) liquidity is being offered at a stale price and (ii) it is profitable to take liquidity after taking into account gas costs and pool fees.

\paragraph{Gas fee (order execution cost).} Orders submitted at $t=1$ to trade against pool liquidity or to withdraw existing liquidity incur a fixed execution cost $\Gamma \times \log\left(2\right) \diff i$, where $\Gamma>0$. The execution cost can be interpreted as a gas fee on the Ethereum blockchain as in \citet{CapponiJia2021}. In contrast to \citet{CapponiJia2021}, we assume traders on the decentralized exchanges are price takers on the gas market and their orders do not impact the gas cost. A natural interpretation is that message volume at any time in a particular asset pair traded on decentralized exchanges is small relative to the aggregate transaction flow on the entire blockchain.


\paragraph{Timing.} Figure \ref{fig:timing} summarizes the sequence of events at each time $t$. At $t=0$, liquidity providers arrive at the market and choose to deposit their tokens (and corresponding num\'{e}raire) on either the high- or low-fee liquidity pool. At $t=1$, an exogenous trigger event happens: either news, that is a common value innovation, or a private value shock to liquidity traders. With probability $1-\eta$, a liquidity trader arrives and trades a random quantity $\tilde{\theta}$. Conversely, with probability $\eta$, news arrives which moves the asset value to either $v+1$ or $v-1$. In this case, liquidity providers have a first-mover advantage: they can pay the fixed gas fee $\Gamma$ and withdraw liquidity from the pool to avoid being adversely selected. Following the $\LP$s' choice, arbitrageurs may trade in the direction of the news if profitable to do so. Finally, at $t=2$ all payoffs are realized. 

\begin{figure}[H]
\caption{\label{fig:timing} \textbf{Model timing}}

\vspace{0.1in}
\begin{centering}
\includegraphics[width=0.9\textwidth]{Figures/timing_dex_v1.pdf}
\par\end{centering}

\end{figure}

\subsection{Equilibrium \label{sec:eq}}

We solve the game by backward induction. First, we discuss the optimal strategy of arbitrageurs and liquidity traders at $t=1$, taking equilibrium liquidity provision as given. Next, we solve for the optimal liquidity pool choices of $\LP$s at $t=0$. 

\subsubsection{Optimal strategies at \texorpdfstring{$t=1$}{t=1}}

The linear pricing curve ensures that the liquidity trader $\LT$ always trades at the fundamental token value $v$, regardless of the trade size. In contrast to markets with convex bonding curves as described in \citet{LeharParlour2021} or \citet{CapponiJia2021}, there is no price impact on the constant price market, which implies there is no impermanent loss for liquidity providers from uninformed trading, and further that no arbitrage trade is needed to restore the fundamental value. However, the liquidity trader faces a difference in the constant per-unit liquidity fee across the two pools. 

Let $T^\star_L$ and $T^\star_H$ be the equilibrium supply of tokens on liquidity pools $L$ and $H$, respectively. To minimize trading cost, the liquidity trader first submits an order on the low-fee pool. If liquidity on pool $L$ is sufficient to accommodate the demand, that is if $\theta\leq T^\star_L$, then the $\LT$ executes its entire order on $L$. Conversely, if $\theta>T^\star_L$, the liquidity trader exhaust the liquidity supply on $L$ and trades the residual quantity $\theta-T^\star_L$ against liquidity on pool $H$. From equation \eqref{eq:aggliq}, the aggregate liquidity supply is $T^\star_L+T^\star_H=1$, which implies that $T^\star_k \leq 1$, for $k\in\left\{L,H\right\}$. Since $\theta<1$, the liquidity trader executes her entire order with probability one and incurs a net cost of $f \times T_L^\star + 1 \times T_H^\star$.

If news occurs and $\LP$s do not withdraw liquidity from the pool, arbitrageurs can trade in the direction on the news to obtain a gross profit of $1~\C$ per token traded (i.e., the size of the news). Concretely, upon good news an arbitrageur deposits $q_{\text{arb},k} v$ units of num\'{e}raire into liquidity pool $k$ and removes $q_{\text{arb},k}$ tokens with a value of $q_{\text{arb},k} \left(v+1\right)$. Further, the arbitrageurs pays the pool fee $f_k$ and the gas fee equal to $\Gamma\log\left(2\right) \diff i$. The net profit from trading $q_{\text{arb},k}$ on liquidity pool $k$ is therefore:
\begin{equation}\label{eq:pi_arb}
    \Pi_\A = q_{\text{arb},k}\left(1-f_k\right)-\Gamma\log\left(2\right) \diff i
\end{equation}

\begin{ass}\label{ass:gamma}
\begin{leftbar} \setlength{\parskip}{0ex}
The gas fee is low enough such that it does not prevent arbitrageurs from trading on any opportunities, that is $\Gamma < 1-f$.
\end{leftbar}
\end{ass}

Assumption \ref{ass:gamma} guarantees that the arbitrageur profit as defined in \eqref{eq:pi_arb} is always positive on liquidity pool $L$, as long as the pool is non-empty. That is, arbitrageurs are willing to trade upon news even if only the lowest-endowment $\LP$ with $\tau_i=\log\left(2\right) \times 1 \diff i$ submits liquidity on pool $L$. Further, since the arbitrageur profit increases in the quantity traded, $\A$ optimally removes the entire liquidity from pool $L$. Finally, since the fee on pool $H$ is equal to the size of the news, the arbitrageur never consumes liquidity from pool $H$ for any positive gas fee. The mechanism is similar to the one in \citet{FoucaultMoinasTheissen2007}, where the size of news and the tick size are such that arbitrageurs consume only the liquidity at the best bid or ask. 

When do liquidity providers withdraw their liquidity? On pool $H$, withdrawing is never optimal since the fee is high enough to deter arbitrageurs and push adverse selection risk to zero. On pool $L$, liquidity providers with endowment $q_i$ compare the adverse selection cost and the gas fee and withdraw liquidity if and only if
\begin{equation}
    q_i \log\left(2\right)\left(1-f\right)>\Gamma \log\left(2\right),
\end{equation}
which is always true under Assumption \ref{ass:gamma}. Lemma \ref{lem:t1} summarizes the optimal strategies for all agents at $t=1$.

\begin{lem}\label{lem:t1}
\begin{leftbar} \setlength{\parskip}{0ex}
At $t=1$, the optimal strategies are as follows:
\begin{enumerate}
    \item[(i)] arbitrageurs buy (sell) $T^\dagger_L$ tokens on pool $L$ upon a positive (negative) common value innovation, where $T^\dagger_L$ is the size of pool $L$ at $t=1$, after the liquidity providers' decision to withdraw or not. The arbitrageur does not trade otherwise.
    \item[(ii)] a liquidity trader with a private value shock of size $\theta$ trades $\min\left\{T_L^\star,\theta\right\}$ on pool $L$ and $\max\left\{0,T_L^\star-\theta\right\}$ on pool $H$. 
    \item[(iii)] Liquidity providers on pool $L$ pay the gas fee and withdraw their liquidity. In contrast, liquidity providers on pool $H$ do not attempt to withdraw liquidity.
\end{enumerate}

\end{leftbar}
\end{lem}

\subsubsection{Liquidity provision at \texorpdfstring{$t=0$}{t=0} \label{sec:liqprov}}

We turn next to the liquidity providers' choice of pool at $t=0$. Let $T_L$ and $T_H$ denote the size of liquidity pools $L$ and $H$, expressed in token units. The expected profit of an $\LP$ with endowment $\tau_i=q_i \log 2$ posting liquidity on pool $L$ is
\begin{align}\label{eq:lp_L}
    \pi^\LP_L &= q_i \log 2 \left(1-\eta\right)\mathbb{E}\left[\min\left\{\frac{\theta}{T_L},1\right\}\right] f  - \eta \Gamma \log 2 \nonumber \\
    &=q_i \log 2 \left[\left(1-\eta\right)\left(1-\frac{T_L}{2}\right) f\right] - \eta \Gamma \log 2,
\end{align}
since
\begin{align}
    \mathbb{E}\left[\min\left\{\frac{\theta}{T_L},1\right\}\right] &= \mathbb{P}\left(\theta\leq T_L\right) \times \mathbb{E}\left[\frac{\theta}{T_L} \mid \theta\leq T_L\right] + \mathbb{P}\left(\theta > T_L\right) \times 1 \nonumber \\
    & = T_L \times \frac{1}{2} + \left(1-T_L\right) = 1 - \frac{T_L}{2},
\end{align}
where the last equality follows from the fact that $\theta$ is uniformly distributed over $\left[0,1\right]$. With probability $1-\eta$, a liquidity trader arrives at $t=1$ and trades $\theta$. If $\theta>T_L$, then the liquidity trader consumes the entire pool and the $\LP$ receives the fee $f$ for each unit of liquidity posted. Conversely, if $\theta\leq T_L$, then the liquidity provider receives a share $\frac{q_i}{T_L}$ of the aggregate fees $\theta f$. With probability $\eta$, news occurs: from Lemma \ref{lem:t1}, the liquidity provider pays the gas fee $\Gamma \log 2$ and withdraws $q_i$ from the pool. 

Alternatively, the $\LP$ can deposit liquidity on pool $H$ and earn expected profit
\begin{align}\label{eq:lp_H}
    \pi^\LP_H &= q_i \log 2 \left(1-\eta\right) \mathbb{E}\left[\max\left\{0,\frac{\theta-T_L}{T_H}\right\}\right] \nonumber \\
    & = q_i \log 2 \left(1-\eta\right) \left(1-T_L\right) \frac{1-T_L}{2 T_H},
\end{align}
where the second line follows from explicitly computing the expectation
\begin{align}
    \mathbb{E}\left[\max\left\{0,\frac{\theta-T_L}{T_H}\right\}\right] &= \mathbb{P}\left(\theta\leq T_L\right) \times 0 + \mathbb{P}\left(\theta > T_L\right) \times \frac{\frac{1+T_L}{2}-T_L}{T_H} \nonumber \\
    & = \left(1-T_L\right) \frac{1-T_L}{2 T_H}.
\end{align}
If the liquidity trader demand is low enough, that is if $\theta\leq T_L$, then the entire trade is filled on pool $L$ and liquidity providers on $H$ earn nothing. However, if $\theta>T_L$, the residual liquidity demand $\theta-T_L$ is routed to pool $H$ and liquidity providers earn a share proportional to their deposit, i.e., $\frac{q_i}{T_H}$. If news occurs, $\LP$s on $H$ do not incur an adverse selection cost since from Lemma \ref{lem:t1} arbitrageurs do not submit orders to the high-fee pool.

Liquidity providers in the low-fee pool absorb a larger share of the uninformed order flow, since the $\LT$ order is first routed to pool $L$. On the other hand, they need to pay gas fees $\Gamma$ to update their liquidity if token value changes to avoid being adversely selected. At the same, $\LP$s in the high-fee pool face no adverse selection, receive a larger fee per unit traded, but volume is limited as they only fill the residual demand from uninformed $\LT$s after liquidity on the low-fee pool is exhausted. From equations \eqref{eq:lp_L} and \eqref{eq:lp_H}, liquidity provider $i$ chooses the low-fee pool $L$ if and only if
\begin{equation}\label{eq:cost_comparison}
    \pi^\LP_L>\pi^\LP_H \Longleftrightarrow q_i \frac{\left(1-\eta\right)\left(\left(1-T_L\right)^2-f T_H \left(2-T_L\right)\right)}{2T_H} - \eta\Gamma > 0.
\end{equation}
A salient implication of equation \eqref{eq:cost_comparison} is that $\LP$s with larger endowments are more likely to choose the low-fee pool, keeping liquidity shares constant. The rationale is that gas fees are a fixed cost, and larger $\LP$s are more likely to achieve economies of scale. The expected fee revenue scales linearly with a liquidity provider's share in the liquidity pool (proportional to $q_i$), better compensating $\LP$s for the gas fee paid upon news arrival at $t=1$. 

We follow \citet{KatzShapiro1985} and conjecture that there exists a marginal liquidity provider $\qmg$ such that all $\LP$s with $q_i>\qmg$ post liquidity on the low-fee pool and all $\LP$s with $q_i\leq \qmg$ choose the high-fee pool.\footnote{We note that there cannot be a ``reversed-sign'' equilibrium, where $\LP$s with $q_i\leq\qmg$ post liquidity on the low-fee pool and all $\LP$s with $q_i>\qmg$ choose the high-fee pool. To understand the rationale, we point out that for an $\LP$ with endowment $\tilde{q}<\qmg$, submitting liquidity to pool $L$ yields a lower expected revenue since
\begin{equation*}
    \pi^\LP_L-\pi^\LP_H=\tilde{q} \frac{\left(1-\eta\right)\left(\left(1-T_L\right)^2-f T_H \left(2-T_L\right)\right)}{2T_H} - \eta\Gamma < 0.
\end{equation*}
Therefore, it is optimal for the $\LP$ with endowment $\tilde{q}$ to post liquidity on the high-fee pool, which contradicts the conjectured equilibrium.  Importantly, since each $\LP$ is ``small'' relative to the aggregate mass of liquidity providers, individual deviations do not impact aggregate pool sizes $T_L$ and $T_H$.} The conjectured equilibrium pins down the pool sizes $T_L$ and $T_H$ as a function of the endowment for the marginal $\LP$:
\begin{align}\label{eq:liquidity_levels}
    T_L&=\int_{\qmg}^2 \log\left(2\right) q_i \phi\left(q_i\right) \diff i = 2 - \qmg \text{ and }\nonumber \\
    T_H&=\int_1^{\qmg} \log\left(2\right) q_i \phi\left(q_i\right) \diff i = \qmg -1. 
\end{align}
From equations \eqref{eq:cost_comparison} and \eqref{eq:liquidity_levels} it follows that the expected profit difference between the low- and high-fee pools can be written as a linear decreasing function of the marginal $\LP$'s endowment, that is
\begin{equation}\label{eq:pi_diff}
    \pi^\LP_L-\pi^\LP_H = \frac{1}{2}q_i \left(1-\eta\right) \left(1-\left(1-f\right)\qmg\right) - \eta \Gamma.
\end{equation}
We search for fulfilled expectation equilibria \citep[following the definition of][]{KatzShapiro1985}, where the beliefs of $\LP$s at $t=0$ about the size of liquidity pools are consistent with the outcome of their choices. We solve \eqref{eq:pi_diff} on the support for $q_i$ -- the interval $\left[1,2\right]$ to obtain the $\LP$ reaction function
\begin{equation}\label{eq:reaction}
    \tilde{q}\left(\qmg\right)=\begin{cases}
    1, & \text{ for } \qmg \leq \frac{1-\eta - 2\Gamma \eta}{\left(1-f\right)\left(1-\eta\right)}\\
    \frac{2\eta\Gamma}{ \left(1-\eta\right) \left(1-\left(1-f\right)\qmg\right)}, & \text{ for } \qmg \in \left(\frac{1-\eta - 2\Gamma \eta}{\left(1-f\right)\left(1-\eta\right)}, \frac{1-\eta\left(1+\Gamma\right)}{\left(1-f\right)\left(1-\eta\right)}\right] \\
    2, & \text{ for } \qmg > \frac{1-\eta\left(1+\Gamma\right)}{\left(1-f\right)\left(1-\eta\right)}.
    \end{cases}
\end{equation}
In any fulfilled expectation equilibrium, the equilibrium endowment of the marginal $\LP$ is a fixed point of equation \eqref{eq:reaction}. Figure \ref{fig:reaction} plots the $\LP$ reaction function $\tilde{q}\left(\cdot\right)$ to graphically illustrate the different possible equilibria. Let $q^\star_1$ and $q^\star_2$ be the interior roots of the reaction function \eqref{eq:reaction}, that is the solutions of the quadratic form
\begin{equation}
    q-\frac{2\eta\Gamma}{ \left(1-\eta\right) \left(1-\left(1-f\right)q\right)}=0.
\end{equation}
that is, 
\begin{equation}\label{eq:roots}
    q^\star_{\left\{1,2\right\}} = \frac{1}{2\left(1-f\right)} \pm \frac{1}{2\left(1-f\right)}\sqrt{1-\eta\frac{1+8\left(1-f\right)\Gamma}{1-\eta}}.
\end{equation}
In the top left panel, we illustrate a parameter combination for which are three equilibria, at $\qmg\in\left\{q^\star_1, q^\star_2, 2\right\}$. However, $q^\star_2$ is an unstable equilibrium -- a tipping point \citep{Jullien2011} at which small perturbation in beliefs cause the $\LP$s to spiral away from the postulated equilibrium (we refer the reader to the proof of Proposition \ref{prop:equilibria} for a more formal discussion). The top right panel illustrates a parameter combination for which there is a unique and stable interior equilibrium at $\qmg=q^\star_1$. Finally, the bottom panels illustrate scenarios for which $\LP$s only deposit liquidity on a single pool -- we distinguish between a multiple equilibria case (bottom left) where either pool having a 100\% market share is an equilibrium and a unique equilibrium case (bottom right) for which the pool attracting the entire liquidity is unambiguous. 

\begin{figure}[H]
\caption{\label{fig:reaction} Liquidity provider reaction function and equilibria}
\begin{minipage}[t]{1\columnwidth}%
\footnotesize
This figure illustrates equilibrium $\LP$ liquidity pool choices as fixed points of the reaction function $\tilde{q}\left(\qmg\right)=\qmg$. We consider four distinct cases that may arise. Stable equilibria are marked with green circles, whereas unstable equilibria are market with magenta squares. Parameter values are $f=0.64$, $G=0.14$, $\eta=0.71$ (top left), $f=0.69$, $G=0.15$, $\eta=0.71$ (top right), $f=0.51$, $G=0.24$, $\eta=0.46$ (bottom left), $f=0.51$, $G=0.35$, $\eta=0.46$ (bottom right, blue line), $f=0.56$, $G=0.30$, $\eta=0.27$ (bottom right, green line).
\end{minipage}

\vspace{0.05in}

\begin{centering}
\includegraphics[width=0.9\textwidth]{Figures/model_reactions.png}
\par\end{centering}

\end{figure}



\begin{prop}\label{prop:equilibria}
\begin{leftbar} \setlength{\parskip}{0ex}
For ease of notation, we define and tabulate below three gas fee thresholds $\bar{\Gamma}_k$, $k\in\left\{1,2,3\right\}$.

\begin{center}
    \begin{tabular}{ccc}
    \toprule
    $\bar{\Gamma}_1$ & $\bar{\Gamma}_2$ & $\bar{\Gamma}_3$ \\
    \cmidrule{1-3}
    $f\frac{1-\eta}{2\eta}$     &  $\frac{\left(2f-1\right)\left(1-\eta\right)}{\eta}$ & $\frac{1-\eta}{8\left(1-f\right)\eta}$\\
    \bottomrule
    \end{tabular}
\end{center}

It follows there are has either one, two, or three stable fulfilled expectation equilibria at $t=0$, corresponding to the following $\LP$ liquidity pool choices:
\begin{enumerate}
    \item[(i)] An interior equilibrium with marginal $\LP$ characterized by endowment $\qmg^\star=q^\star_1$, such that all $\LP$s with endowment $q>q^\star_1$ add liquidity to the low-fee pool and the rest choose the high-fee pool. The equilibrium emerges for $f\in\left[\frac{1}{2},\frac{3}{4}\right)$ and $\Gamma\in\left(\bar{\Gamma}_1, \bar{\Gamma}_3\right]$ and $f>\frac{3}{4}$ and $\Gamma\in\left(\bar{\Gamma}_1, \bar{\Gamma}_2\right]$. Moreover, the interior equilibrium is unique for $f>\frac{2}{3}$ and $\Gamma\in\left(\bar{\Gamma}_1, \bar{\Gamma}_2\right]$.
    \item[(ii)] A corner equilibrium where $\qmg^\star=1$, such that all $\LP$s post liquidity on the low-fee pool. The equilibrium emerges for $\Gamma\leq\bar{\Gamma}_1$ and is further unique if $f>\frac{1}{2}$ and $\Gamma\leq\min\left\{\bar{\Gamma}_1,\bar{\Gamma}_2\right\}$.
    \item[(iii)] A corner equilibrium where $\qmg^\star=2$, such that all $\LP$s post liquidity on the high-fee pool. The equilibrium emerges for $\Gamma>\bar{\Gamma}_2$ and is further unique if $f>\frac{3}{4}$ and $\Gamma>\bar{\Gamma}_2$, $f>\frac{1}{2}$ and $\Gamma>\bar{\Gamma}_3$, or $f\leq\frac{1}{2}$ and $\Gamma>\bar{\Gamma}_1$.
\end{enumerate}

\end{leftbar}
\end{prop}

Proposition \ref{prop:equilibria} establishes existence conditions for each possible equilibrium. In particular, an interior equilibrium for which both the $L$ and $H$ pool attract a positive market share emerges for moderate gas fee $\Gamma$ and a small enough difference between liquidity fees on the two pools (i.e., a large $f$). The interior equilibrium is unique if the liquidity fees are close enough across the two pools. Figure \ref{fig:regions} highlights the parameter region where multiple liquidity pools coexist with positive market share. 

The remaining results in Proposition \ref{prop:equilibria} are intuitive: a small gas fee $\Gamma$ reduces the $\LP$s' costs to manage stale liquidity upon news and stimulates competition on the low-fee pool. In other words, the cost of updating liquidity is lower than the opportunity cost of not capturing uninformed trades. In contrast, a large enough $\Gamma$ incentivizes liquidity providers to deposit tokens on the high-fee pool, since managing liquidity on pool $L$ is too costly. 

\begin{figure}[H]
\caption{\label{fig:regions} The emergence of two-pool equilibria}
\begin{minipage}[t]{1\columnwidth}%
\footnotesize
This figure illustrates the emergence of two-pool equilibria for different values of the liquidity fee $f$ and gas fee $\Gamma$. We set the probability of informed trading at $\eta=0.85$. We highlight the parameter region for which a two-pool equilibria emerges and is unique (in red) as well as the region for which a two-pool equilibria emerges but is not unique (in blue). 
\end{minipage}

\vspace{0.05in}

\begin{centering}
\includegraphics[width=0.9\textwidth]{Figures/model_int_eq_region.png}
\par\end{centering}

\end{figure}

\subsection{Implications and empirical predictions}

In this section, we zoom in on the properties of the interior equilibrium, that is, the most interesting case featuring segmented liquidity across multiple pools. From Proposition \ref{prop:equilibria}, the only possible interior equilibrium in the liquidity provision game is for a marginal $\LP$ with endowment $\qmg=q_1^\star$, the smallest root of \eqref{eq:reaction}.

\begin{pred}\label{pred:clienteles}
\emph{If an interior equilibrium exists where liquidity is segmented across multiple pools, the average liquidity deposit in the low-fee pool is larger than for the high-fee pool.}
\end{pred}

Prediction \ref{pred:clienteles} follows from the discussion in Section \ref{sec:liqprov}. Liquidity providers with large token endowments ($q_i>\qmg$) deposit them in the low-fee pool since they have stronger incentives to pay the gas fee and actively manage the liquidity. Conversely, $\LP$s with lower endowments ($q_i\leq\qmg$) gravitate towards the high-fee pool, accepting a lower trade probability in exchange for reducing adverse selection costs without active liquidity management and paying gas fees.

\begin{pred}\label{pred:updates}
\emph{Liquidity providers on the low-fee pool are more likely to actively manage liquidity.}
\end{pred}
In equilibrium, the $\LP$s on the low-fee pool update their liquidity upon news arrival to avoid adverse selection, unlike their counterparts on the high-fee pool.


\begin{pred}\label{pred:comp_stat_Gamma}
\emph{The liquidity share of the low-fee pool $L$ decreases in the gas fee $\Gamma$.}
\end{pred}
\begin{pred}\label{pred:comp_stat_eta}
\emph{The liquidity share of the low-fee pool $L$ decreases in the probability of informed trading $\eta$.}
\end{pred}

Predictions \ref{pred:comp_stat_Gamma} and \ref{pred:comp_stat_eta} state that the low-fee pool becomes less attractive for liquidity providers if the gas fee increases (higher $\Gamma$) -- making active liquidity management less profitable -- or if the probability of informed trading is higher ($\eta$ increases) which leads to \emph{more frequent} liquidity management. Formally, we can show that $q_1^\star$ increases in both $\Gamma$ and $\eta$ -- leading to a lower value of $T_L^\star$:
\begin{align}
    \frac{\partial q_1^\star}{\partial \Gamma}&=\frac{2 \eta }{\sqrt{(1-\eta ) (\eta  (8 \Gamma  (f-1)-1)+1)}}>0 \text{ and } \nonumber \\
    \frac{\partial q_1^\star}{\partial \eta}&=\frac{2 \Gamma }{(1-\eta) \sqrt{(1-\eta ) (\eta  (8 \Gamma  (f-1)-1)+1)}}.
\end{align}

\begin{pred}\label{pred:trade_volume}
\emph{If an interior equilibrium exists, the trading volume share of the low-fee pool is higher than its liquidity share.}
\end{pred}

The intuition is that $\LP$s on the low-fee pool deposit large token quantities and they absorb a disproportionate amount of incoming trades -- it is possible that $\LP$s on the high-fee pool do not trade at all against incoming orders, despite providing positive liquidity in equilibrium. To formally see the result, we first note that there is no informed trade in equilibrium on either pool. The average $\LT$ trade size on the low-fee pool is
\begin{align}
    \mathbb{E}\left[\min\left\{\theta,T_L^\star\right\}\right]&=\mathbb{P}\left(\theta\leq T_L\right) \mathbb{E}\left[\theta\mid \theta<T_L^\star\right] + \left(1-\mathbb{P}\left(\theta\leq T_L\right)\right) T_L^\star \nonumber \\
    &= T_L^\star\frac{T_L^\star}{2} + \left(1-T_L^\star\right) T_L^\star= T_L^\star-\frac{\left(T_L^\star\right)^2}{2}.
\end{align}
The average $\LT$ trade size on the high-fee pool is
\begin{align}
    \mathbb{E}\left[\max\left\{0,\theta-T_L^\star\right\}\right]& + \left(1-\mathbb{P}\left(\theta\leq T_L\right)\right) \left(\mathbb{E}\left[\theta\mid \theta>T_L^\star\right]-T_L^\star\right] \nonumber \\
    &= \left(1-T_L^\star\right) \frac{\left(1-T_L^\star\right)}{2}=\frac{1}{2}-T_L^\star+\frac{\left(T_L^\star\right)^2}{2}.
\end{align}
We note that the trade share of pool $L$ is equal to $2T_L^\star-\left(T_L^\star\right)^2$ which is larger than its liquidity share $T_L^\star$ since $T_L^\star<1$. Figure \ref{fig:liqshares} illustrates this result.




\begin{figure}[H]
\caption{\label{fig:liqshares} Liquidity and volume shares}
\begin{minipage}[t]{1\columnwidth}%
\footnotesize
This figure illustrates the relative liquidity and trade volume on the two pools, as a function of the gas fee $\Gamma$. Parameters: $\eta=0.36$ and $f=0.8$.
\end{minipage}

\vspace{0.05in}

\begin{centering}
\includegraphics[width=0.9\textwidth]{Figures/model_compstatics.png}
\par\end{centering}

\end{figure}


\begin{pred}\label{pred:liq_shares}
\emph{The low-fee pool is larger than the high-fee pool (in terms of aggregate deposits) only if the gas fee is low enough, that is if}
\begin{equation}
    \Gamma < \Gamma^\star \equiv \frac{3 (3 f-1) (1-\eta)}{8 \eta }
\end{equation}
\end{pred}

From equation \eqref{eq:liquidity_levels}, if the marginal $\LP$ has endowment $q_1^\star$, then the equilibrium sizes of the two liquidity pools are, respectively,
\begin{align}
    T_L^\star&=2- \frac{1}{2\left(1-f\right)} \left(1- \sqrt{1-\eta\frac{1+8\left(1-f\right)\Gamma}{1-\eta}}\right) \text{ and } \nonumber \\
    T_H^\star&=\frac{1}{2\left(1-f\right)} \left(1- \sqrt{1-\eta\frac{1+8\left(1-f\right)\Gamma}{1-\eta}}\right)-1.
\end{align}


Prediction \ref{pred:liq_shares} translates to stating that $T_L^\star>T_H^\star$, or equivalently to $q_1^\star\leq \frac{3}{2}$, where the latter inequality is true for any $\Gamma\leq\Gamma^\star$. Therefore, even though the low-fee pool attracts the $\LP$s with large token endowments, it is not necessarily the largest pool if the gas fee exceeds a certain threshold. 






==> Old/model_rebalance_old.tex <==
\subsection{Primitives}

\paragraph{Token and traders.} A single token is traded in a continuous-time economy. There are two trader types in the economy: a continuum of liquidity providers ($\LP$s) and liquidity takers ($\LT$s). Both market participant types are risk neutral.  

The expected value of the token equals $v>0$, which is common knowledge. However, market participants have heterogeneous private values for the asset. In particular, liquidity takers value the token at $v\left(1+\Delta\right)$ with $\Delta>0$ whereas $\LP$s have no private value for the token. It follows that there are gains from trade if $\LT$s buy the token from $\LP$s \citep[we follow, e.g.,][in that we focus on a one-sided market where liquidity providers only act as sellers]{foucault2013liquidity}.

Liquidity providers have heterogeneous capital constraints: at any time $\LP$ $i$ can supply liquidity for at most $q_i$ units of the token, where $q_i$ has a log-uniform distribution on $\left[1,Q\right]$:
\begin{equation}
    \varphi\left(q\right)=\frac{1}{\log Q} \frac{1}{q} \text{ for } q\in\left[1,Q\right].
\end{equation}
Our choice of density implies that there are many low-endowment liquidity providers (e.g., retail traders) and a long tail of high-capital investors who provide liquidity to decentralized exchange -- for example, quantitative institutional investors. On aggregate, $\LP$s can provide at most
\begin{equation}
    \int_1^Q q \varphi\left(q\right) \diff q = \frac{Q-1}{\log Q}
\end{equation}
units of liquidity.

There are two types of liquidity takers: small and large. Small $\LT$s arrive at the market at rate $\theta$ per unit of time and demand one unit of the token. Further, a large $\LT$ demands $\Theta$ units of the token, where $\Theta>\frac{Q-1}{\log Q}$. That is, we assume that the large $\LT$ liquidity demand exceeds the maximum liquidity supply. The large $\LT$ arrival time follows a Poisson process with rate $\lambda>0$. The aggregate liquidity demand from small and large $\LT$s evolves over time as
\begin{equation}
    \diff \emph{LiquidityDemand}_t = \theta \diff t + \Theta \diff J_t\left(\lambda\right),
\end{equation}
where $J_t\left(\lambda\right)$ stands in for a Poisson process with rate $\lambda$.

\paragraph{Trading environment.} The token is traded on two liquidity pools that charge liquidity fees proportional to the value of the trade. The token and numeraire quantities ($T$ and $N$, respecitvely) in each pool must satisfy at all times the following linear bonding curve:
\begin{equation}\label{eq:bond_curve}
    v \times T_k + N_k = \text{constant}, \forall k\in\left\{L,K\right\}
\end{equation}
The bonding curve \eqref{eq:bond_curve} implies that the token price is constant and equal to $v$ units of the num\'{e}raire, since $-\frac{\diff T_k}{\diff N_k}=v$.\footnote{In practice, most decentralized exchanges use convex bonding curve, for example constant product pricing. While the choice of bonding curve is of first order importance for liquidity takers who need to split trades to optimize price impact, we argue it is less important for liquidity suppliers. For tractability, we assume a linear bonding curve which implies that liquidity traders only care about pool fees -- the focus of our model. In a richer model with convex pricing, we would expect to see relatively more fragmentation since minimizing price impact might require further splitting trades.} The low-fee pool $L$ charges a fee of $\ell$ and the high-fee pool $H$ charges a fee of $h$ per token traded, where $\ell<h$. For example, to purchase $t$ units of the token on the $L$ pool, the total cost of an investor is $t\left(v+\ell\right)$. Incoming trades are matched with $\LP$s on a pro rata basis, that is all liquidity providers receive fees proportional to their outstanding deposits.

\paragraph{Gas costs.} Any interaction with a liquidity pool (for example, to add or remove liquidity)  incurs a fixed execution cost $\Gamma>0$. The execution cost can be interpreted as the gas price on the Ethereum blockchain as in \citet{CapponiJia2021}. In contrast to \citet{CapponiJia2021}, we assume traders on the decentralized exchanges are price takers on the gas market and their orders do not impact the gas cost. A natural interpretation is that message volume at any time in a particular asset pair traded on decentralized exchanges is small relative to the aggregate transaction flow on the entire blockchain.

Gas fees on decentralized exchanges differ from trading fees on traditional exchanges in a number of ways. First, they are not set by individual exchanges to compete with each other, but are a common transaction cost \emph{across} exchanges. Second, they are levied on a per-order rather than per-share basis: this implies economies of scale for larger orders. Third, there is significant time variation in gas fees which allows us to better empirically identify the impact of transaction costs on liquidity pool market shares.

To ensure that both small and large liquidity traders participate in the market, we assume that the gains from trade are larger than the aggregate transaction cost, including the pool fee and the gas price:
\begin{equation}
    v\left(1+\Delta\right)-v > v\left(1+h\right) + \Gamma \Rightarrow \Delta > h + \frac{\Gamma}{v}.
\end{equation}

To rule out trivial cases, we further assume that $Q\ell-\Gamma>0$. The condition ensures that there are at least some liquidity providers who can earn positive expected profit on pool $L$; otherwise, pool $L$ never attracts any deposits.

\paragraph{Timing.} We follow \citet{foucault2013liquidity} and partition time between liquidity cycles. A liquidity cycle starts with an empty pool and $\LP$ deposits and ends when incoming trades deplete the liquidity supply, returning the pool to an empty state. The first cycle starts at $t=0$ when each liquidity provider $i$ selects a pool $k\in\left\{L,H\right\}$, pays the gas cost $\Gamma$, and deposits their token endowment $q_i$. Liquidity providers also have the option to not provide any liquidity, that is $k=\emptyset$. Following the initial liquidity deposit, $\LP$s do not further interact with the pool until the cycle ends at some random time $\tilde{\tau}$. The liquidity cycle restarts at $\tilde{\tau}$: $\LP$s use the sales cash proceeds to borrow or purchase $q_i$ tokens and refill liquidity on decentralized exchange pools.

\subsection{Equilibrium analysis}\label{sec:liqprov}

An equilibrium in our trading game is a mapping from the $\LP$ endowment $q_i$ to a liquidity pool $k\in\left\{L,H, \emptyset \right\}$ such that no liquidity provider is better off by deviating and choosing either to deposit liquidity in another pool or to not provide liquidity at all. Conditional on making a deposit, liquidity providers choose the pool $k^\star$ that maximizes their expected profit per unit of time, that is
\begin{equation}\label{eq:optimal_pool}
    k^\star\left(q_i\right) \coloneqq \arg\max_{k} \left(q_i f_k - \Gamma\right) \frac{1}{d_k}, 
\end{equation}
where $f_k$ is the liquidity fee on pool $k$, and $d_k$ is the duration of a liquidity cycle on pool $k$. The revenue per liquidity cycle is equal to the pool liquidity fee times the deposit $q_i$, net of the gas cost to submit the order.

Let $\Omega_k$ denote the set of $\LP$s who choose pool $k$ in equilibrium, that is $\Omega_k\coloneqq\left\{i \mid k^\star\left(q_i\right)=k\right\}$. We can define total liquidity on pool $k$ at $t=0$ as the aggregate deposit from all liquidity providers in $\Omega_k$:
\begin{equation}
    \mathcal{L}_k=\int_{i\in\Omega_k} q_i \varphi(q_i) \diff i.
\end{equation}

Before solving for the equilibrium $\LP$ pool choice, we first analyze the liquidity traders' decisions. A large $\LT$'s liquidity demand exceeds the aggregate $\LP$ token endowment: upon arrival, the large $\LT$ therefore consumes the entire liquidity on both pools and triggers the end of the liquidity cycle. In contrast, small $\LT$s trade smoothly over time and consume liquidity from the cheaper pool $L$ at rate $\frac{\theta}{\mathcal{L}_L} \diff t$. Once the low-fee pool is empty, liquidity providers immediately refill it and restart the cycle.

\begin{lem}\label{lem:duration}
\begin{leftbar} \setlength{\parskip}{0ex}
The duration of a liquidity cycle is lower in pool $L$ than in pool $H$. Formally, $d_L<d_H$.
\end{leftbar}
\end{lem}

Lemma \ref{lem:duration} states that liquidity cycles in pool $L$ are shorter than in pool $H$. The result is intuitive: From the discussion above, a liquidity cycle on pool $H$ only ends with the arrival of a large liquidity trader: from the properties of Poisson processes, the expected cycle duration $d_H$ equals $\frac{1}{\lambda}$. Conversely, a liquidity cycle on pool $L$ ends either upon the large $\LT$ arrival or when small $\LT$s exhaust the pool liquidity. Formally,
\begin{align}
    d_L &=\exp\left(-\lambda \frac{\LL}{\theta}\right) \frac{\LL}{\theta}+\int_{0}^{\frac{\LL}{\theta}} t\lambda\exp\left(-\lambda t\right)\diff t \nonumber \\
    &=\frac{1}{\lambda}-\frac{1}{\lambda}\exp\left(-\frac{\LL}{\theta}\lambda\right)<\frac{1}{\lambda}=d_H.
\end{align}

Liquidity providers on pool $L$ absorb a larger share of the order flow, as they trade with both small and large $\LT$s. However, they earn a lower fee per traded volume than they would on pool $H$. Furthermore, they need to manage their liquidity more often, which implies larger gas costs per unit of time. From equation \eqref{eq:optimal_pool}, liquidity provider $i$ chooses the low-fee pool $L$ if and only if
\begin{equation}\label{eq:cost_comparison}
    \pi_\ell-\pi_h=\frac{1}{d_h d_\ell}\left[\left(d_h \ell - d_\ell h\right) q_i - \Gamma \left(d_h-d_\ell\right)\right]>0
\end{equation}
A salient implication of equation \eqref{eq:cost_comparison} is that $\LP$s with larger endowments are more likely to choose the low-fee pool, keeping liquidity shares constant. The rationale is that gas fees are a fixed cost, and larger $\LP$s are more likely to achieve economies of scale. The expected fee revenue scales linearly with a liquidity provider's share in the liquidity pool (proportional to $q_i$), better compensating $\LP$s for the gas fee paid at the start of the liquidity cycle. 

We follow \citet{KatzShapiro1985} and conjecture that there exists a marginal liquidity provider $\qmg$ such that all $\LP$s with $q_i>\qmg$ post liquidity on the low-fee pool and all $\LP$s with $q_i\leq \qmg$ choose the high-fee pool.\footnote{We note that there cannot be a ``reversed-sign'' equilibrium, where $\LP$s with $q_i\leq\qmg$ post liquidity on the low-fee pool and all $\LP$s with $q_i>\qmg$ choose the high-fee pool. To understand the rationale, we point out that for an $\LP$ with endowment $\tilde{q}<\qmg$, submitting liquidity to pool $L$ yields a lower expected revenue since
\begin{equation*}
    \pi_\ell-\pi_h=\frac{1}{d_h d_\ell}\left[\left(d_h \ell - d_\ell h\right) \tilde{q} - \Gamma \left(d_h-d_\ell\right)\right] < 0.
\end{equation*}
Therefore, it is optimal for the $\LP$ with endowment $\tilde{q}$ to post liquidity on the high-fee pool, which contradicts the conjectured equilibrium.  Importantly, since each $\LP$ is ``small'' relative to the aggregate mass of liquidity providers, individual deviations do not impact aggregate pool sizes $\LL$ and $\LH$.} To provide liquidity, $\LP$s need to earn positive expected profits per unit of time, at least in the high-fee pool. From equation \eqref{eq:optimal_pool}, the $\LP$ participation constraint becomes
\begin{equation}\label{eq:pc}
    q_i h - \Gamma =\geq 0 \Rightarrow q_i>\underline{q}\coloneqq \max\left\{\frac{\Gamma}{h},1\right\}.
\end{equation}
If $\frac{\Gamma}{h}>1$, then liquidity providers are competitive since the marginal $\LP$ earns zero profit in expectation. 

The conjectured equilibrium pins down the pool sizes $\LL$ and $\LH$ as a function of the endowment for the marginal $\LP$:
\begin{align}\label{eq:liquidity_levels}
    \LL&=\int_{\qmg}^Q q_i \varphi\left(q_i\right) \diff i = \frac{1}{\log Q}\left(Q - \qmg \right)  \text{ and }\nonumber \\
    \LH&=\int_{\underline{q}}^{\qmg}  q_i \varphi\left(q_i\right) \diff i = \frac{1}{\log Q}\left(\qmg -  \underline{q}\right)
\end{align}
From equations \eqref{eq:cost_comparison} through \eqref{eq:liquidity_levels} it follows that the expected profit difference between the low- and high-fee pools can be written as an increasing function of the marginal $\LP$'s endowment, that is
\begin{align}\label{eq:pi_diff}
    \pi_\ell-\pi_h &=\frac{1}{\lambda d_h d_\ell}\left[\exp\left(-\frac{\lambda}{\theta} \LL\right) \underbrace{\left(q_i h - \Gamma\right)}_{>0} - q_i\left(h-\ell\right)\right] \nonumber \\
        &=\frac{1}{\lambda d_h d_\ell}\left[\exp\left(-\frac{\lambda}{\theta \log Q}\left(Q-\qmg\right)\right) \underbrace{\left(q_i h - \Gamma\right)}_{>0}- q_i\left(h-\ell\right)\right]. 
\end{align}
We search for fulfilled expectation equilibria \citep[following the definition of][]{KatzShapiro1985}, where the beliefs of $\LP$s at $t=0$ about the size of liquidity pools are consistent with the outcome of their choices. Proposition \ref{prop:equilibria} characterizes the equilibrium liquidity provision.

\begin{prop}\label{prop:equilibria}
\begin{leftbar} \setlength{\parskip}{0ex}
If $\frac{h-l}{h} \exp\left(-\frac{\lambda}{\theta \log Q}\left(Q-1\right)\right)<1$ and $\frac{\Gamma}{h}<1-\exp\left(-\frac{\lambda}{\theta \log Q}\left(Q-1\right)\right)$, then there exists a unique corner equilibrium where all $\LP$s deposit liquidity on pool $L$. Otherwise, there exists a unique fragmented equilibrium characterized by marginal trader $\qmg^\star$ which solves
\begin{equation}\label{eq:mg_eq}
    \qmg = \Gamma \frac{\exp\left(-\frac{\lambda}{\theta \log Q}\left(Q-\qmg\right)\right)}{h\exp\left(-\frac{\lambda}{\theta \log Q}\left(Q-\qmg\right)\right)-\left(h-\ell\right)} \in \left[\underline{q},Q\right]
\end{equation}
such that all $\LP$s with $q_i\leq \qmg^\star$ deposit liquidity in pool $H$ and all $\LP$s with $q_i>\qmg^\star$ choose pool $L$.
\end{leftbar}    
\end{prop}

\begin{cor}\label{cor:comp_stat}
\begin{leftbar} \setlength{\parskip}{0ex}
In equilibrium, the endowment marginal trader $\qmg^\star$:
\begin{itemize}
    \item[(i)] increases in the gas cost ($\Gamma$), the fee on pool $H$ ($h$), the arrival rate of large trades ($\lambda$), and the liquidity distribution parameter $Q$.
    \item[(ii)] decreases in the fee on pool $L$ ($\ell$) and the arrival rate of small trades ($\theta$).
\end{itemize}
\end{leftbar}    
\end{cor}

From equation \eqref{eq:liquidity_levels}, we can compute the market share of the low-fee pool as
\begin{equation}
w_L=\frac{\LL}{\LL+\LH}=\frac{Q - \qmg^\star}{Q - \underline{q}}.
\end{equation}

\begin{cor}\label{cor:comp_stat_ms}
\begin{leftbar} \setlength{\parskip}{0ex}
In equilibrium, the market share of the low fee pool $w_L$
\begin{itemize}
    \item[(i)] increases in the fee on pool $L$ ($\ell$) and the arrival rate of small trades ($\theta$).
    \item[(ii)] decreases in the arrival rate of large trades ($\lambda$) and the fee on pool $H$ (h).
\end{itemize}
\end{leftbar}    
\end{cor}


\subsection{Empirical predictions}

\begin{pred}\label{pred:clienteles}
\emph{$\LP$s on the low-fee pool make larger liquidity deposits than $\LP$s on the high-fee pool.}
\end{pred}

Prediction \ref{pred:clienteles} follows from the discussion in Section \ref{sec:liqprov}. Liquidity providers with large token endowments ($q_i>\qmg$) deposit them in the low-fee pool since they have stronger incentives to pay the gas fee and actively manage the liquidity. Conversely, $\LP$s with lower endowments ($q_i\leq\qmg$) gravitate towards the high-fee pool, accepting a lower trade probability in exchange for reducing adverse selection costs without active liquidity management and paying gas fees.

\begin{pred}\label{pred:updates}
\emph{$\LP$s on the low-fee pool update liquidity more often than $\LP$s on the high-fee pool.}
\end{pred}

\begin{pred}\label{pred:trade_size}
\emph{The average trade on the high-fee pool is larger than the average trade on the low-fee pool.}
\end{pred}


\begin{pred}\label{pred:trade_volume}
\emph{The trading volume on the low-fee pool is larger than the trading volume on the high-fee pool.}
\end{pred}

\begin{pred}\label{pred:dispersion_trades}
\emph{The liquidity share of the low-fee pool $L$ decreases in the trade size heterogeneity for the pair.}
\end{pred}
We proxy trade size heterogeneity by $\frac{\lambda}{\theta}$, i.e., the ratio between the likelihood of a large trade and the size of small trades.

\begin{pred}\label{pred:comp_stat_Gamma}
\emph{The liquidity share of the low-fee pool $L$ decreases in the gas fee $\Gamma$.}
\end{pred}

\begin{pred}\label{pred:frag_exist}
\emph{A fragmented market equilibrium is more likely if the average liquidity deposit, the trade size heterogeneity, and gas fees are larger.}
\end{pred}



==> Old/model_v2.tex <==

\subsection{Model primitives}

\paragraph{Assets.} Consider a three-period economy, where time is indexed by $t\in\left\{0,1,2\right\}$. There are two assets: a risky token $\T$ and a riskless num\'{e}raire $\C$. At $t=2$, the risky token $\T$ pays a stochastic dividend $\tilde{v}$ (denominated in units of $\C$). At the start of the game, the expected token value is $\mathbb{E}_0 \tilde{v}=v>1$. 

The asset $\C$ stands in for cryptocurrencies typically used as num\'{e}raire on decentralized exchanges -- for example Ether (the native currency of the Ethereum blockchain) or stablecoins such as Tether or USD~Coin. The num\'{e}raire pays a risk-free rate of return $r$, which we normalize to zero without loss of generality.

\paragraph{Trading environment.} The risky token is traded on two liquidity pools: $L$ (a low-fee pool) and $H$ (a high-fee pool). The asset quantities in each pool $k\in\left\{L,K\right\}$ must satisfy at all times the following linear bonding curve:
\begin{equation}\label{eq:bond_curve}
    v \T_k + \C_k = \text{constant}.
\end{equation}
The bonding curve \eqref{eq:bond_curve} implies that the token price is constant and equal to $v$ units of the num\'{e}raire, since $-\frac{\diff T}{\diff C}=v$.\footnote{In practice, most decentralized exchanges use convex bonding curve, for example constant product pricing. While the choice of bonding curve is of first order importance for liquidity demanders who need to split trades to optimize price impact, we argue it is less important for liquidity suppliers. For tractability, we assume a linear bonding curve which implies that liquidity traders only care about pool fees -- the focus of our model. In a richer model with convex pricing, we would expect to see relatively more fragmentation since minimzing price impact might require further splitting trades.} To fix intuition behind the mechanics of the market, suppose a trader wishes to buy $t$ units of the token. This reduces the token amount in the pool to $\T_k-t$. In return, the trader needs to add $\Delta$ units of the num\'{e}raire, where $\Delta$ is such that the new asset quantities remain on the bonding curve, that is:
\begin{equation}
    v \left(\T_k-t\right) + \left(\C_k+\Delta\right) = v \T_k + \C_k,
\end{equation}
which is equivalent to having $\Delta = v t$. The slope of the bonding curve is equal to the expected value of the asset to ensure there are no arbitrage opportunities at the start of the game. 

The two liquidity pools charge different fees on liquidity-removing trades. Fees are expressed in units of num\'{e}raire and are distributed to all liquidity providers in a given pool, proportional to the amount of liquidity provided.  The low-fee pool $L$ charges a fee of $f~\C$ where $f<1$, and the high-fee pool $H$ charges a fee of $1~\C$ per token traded. That is, to purchase $t$ units of the token on the $L$ pool, the total cost of an investor is $t\left(v+f\right)$.

\paragraph{Events.} At $t=1$, two types of exogenous events can occur. With probability $\eta<1$, the common value of the token changes to $v+1$ (good news) or to $v-1$ (bad news); good and bad news are equally likely. With probability $\left(1-\eta\right)$ -- that is if news does not occur -- a liquidity trader ($\LT$) receives a private value shock and needs to trade $\tilde{\theta}$ units of the token, where $\tilde{\theta}\sim\text{Uniform}\left[0,\log^{-1}\left(2\right)\right]$. The liquidity trader is equally likely to buy or sell the token. We assume the $\LT$s private value is large enough to cover transaction costs on either liquidity pool.

\paragraph{Liquidity providers and arbitrageurs.} In addition to liquidity traders, the token is traded by two types of agents: risk-neutral liquidity providers ($\LP$) and arbitrageurs ($\A$). There is a continuum of liquidity providers indexed by $i$, endowed with heterogeneous amounts of the token $T$. Liquidity provider $i$ is endowed with $q_i$ units of the token. Following \citet{KhomynPutninsZoican2022}, we assume that $q_i$ is distributed with density
\begin{equation}\label{eq:density}
    \phi\left(q\right)=\log^{-1}\left(2\right)\frac{1}{q},\text{ for }q\in\left[1,2\right].
\end{equation}
The choice of density ensures that the aggregate token endowment of liquidity providers $\T_\text{agg}$ is normalized to a constant, since
\begin{equation}\label{eq:aggliq}
    \T_\text{agg}=\int_1^2 q_i \phi\left(q_i\right)\diff q_i = \log^{-1} \left(2\right).
\end{equation}
Further, the density is chosen to match key features of the empirical distribution of $\LP$s: there are many low-endowment liquidity providers (e.g., retail traders) and a long tail of high-capital investors who provide liquidity to decentralized exchange -- for example, quantitative institutional investors. Figure \ref{fig:distribution} illustrates the theoretical distribution of $\LP$s endowments.

\begin{figure}[H]
\caption{\label{fig:distribution} Liquidity provider endowment (scaled) $q_i$}
\begin{minipage}[t]{1\columnwidth}%
\footnotesize
This figure illustrates the probability density of liquidity provider token endowments, $\phi\left(\cdot\right)$, as defined in equation \eqref{eq:density}.
\end{minipage}

\vspace{0.05in}

\begin{centering}
\includegraphics[width=0.8\textwidth]{Figures/model_density.png}
\par\end{centering}

\end{figure}

The arbitrageurs $\A$ are risk-neutral speculative traders as in \citet{Budish2015TheResponse} or \citet{Menkveld2017NeedLiquidity}, and have zero private value for the token. Upon observing a common value innovation, arbitrageurs can submit a trade against liquidity providers if (i) liquidity is being offered at a stale price and (ii) it is profitable to take liquidity after taking into account gas costs and pool fees.

\paragraph{Gas fee (order execution cost).} Orders submitted at $t=1$ to trade against pool liquidity or to withdraw existing liquidity incur a fixed execution cost $\Gamma>0$. The execution cost can be interpreted as the gas price on the Ethereum blockchain as in \citet{CapponiJia2021}. In contrast to \citet{CapponiJia2021}, we assume traders on the decentralized exchanges are price takers on the gas market and their orders do not impact the gas cost. A natural interpretation is that message volume at any time in a particular asset pair traded on decentralized exchanges is small relative to the aggregate transaction flow on the entire blockchain.

Gas fees on decentralized exchanges differ from trading fees on traditional exchanges in a number of ways. First, they are not set by individual exchanges to compete with each other, but are a common transaction cost \emph{across} exchanges. Second, they are levied on a per-order rather than per-share basis: this implies economies of scale for larger orders. Third, there is significant time variation in gas fees which allows us to better empirically identify the impact of transaction costs on liquidity pool market shares.

\paragraph{Timing.} Figure \ref{fig:timing} summarizes the sequence of events at each time $t$. At $t=0$, liquidity providers arrive at the market and choose to deposit their tokens (and corresponding num\'{e}raire) on either the high- or low-fee liquidity pool. At $t=1$, an exogenous trigger event happens: either news, that is a common value innovation, or a private value shock to liquidity traders. With probability $1-\eta$, a liquidity trader arrives and trades a random quantity $\tilde{\theta}$. Conversely, with probability $\eta$, news arrives which moves the asset value to either $v+1$ or $v-1$. In this case, liquidity providers have a first-mover advantage: they can pay the fixed gas fee $\Gamma$ and withdraw liquidity from the pool to avoid being adversely selected. Following the $\LP$s' choice, arbitrageurs may trade in the direction of the news if profitable to do so. Finally, at $t=2$ all payoffs are realized. 

\begin{figure}[H]
\caption{\label{fig:timing} \textbf{Model timing}}

\vspace{0.1in}
\begin{centering}
\includegraphics[width=0.9\textwidth]{Figures/timing_dex_v2.pdf}
\par\end{centering}

\end{figure}

\subsection{Equilibrium \label{sec:eq}}

We solve the game by backward induction. First, we discuss the optimal strategy of arbitrageurs and liquidity traders at $t=1$, taking equilibrium liquidity provision as given. Next, we solve for the optimal liquidity pool choices of $\LP$s at $t=0$. 

\subsubsection{Optimal strategies at \texorpdfstring{$t=1$}{t=1}}

The linear pricing curve ensures that the liquidity trader $\LT$ always trades at the fundamental token value $v$, regardless of the trade size. In contrast to markets with convex bonding curves as described in \citet{LeharParlour2021} or \citet{CapponiJia2021}, there is no price impact on the constant price market. In turn, this implies there is no impermanent loss for liquidity providers following a liquidity trader arrival, and also that no subsequent arbitrage trade is needed to restore prices to the fundamental value. However, even in the absence of price impact, the liquidity trader needs to take into account the liquidity fee difference across the two pools. 

Let $T^\star_L$ and $T^\star_H$ be the equilibrium supply of tokens on liquidity pools $L$ and $H$, respectively. To minimize trading cost, the liquidity trader first submits an order on the low-fee pool. If liquidity on pool $L$ is sufficient to accommodate the demand, that is if $\theta\leq T^\star_L$, then the $\LT$ executes its entire order on $L$. Conversely, if $\theta>T^\star_L$, the liquidity trader exhaust the liquidity supply on $L$ and trades the residual quantity $\theta-T^\star_L$ against liquidity on pool $H$. From equation \eqref{eq:aggliq}, the aggregate liquidity supply is $T^\star_L+T^\star_H=\log^{-1}\left(2\right)$. Since $\theta<\log^{-1}\left(2\right)$, the liquidity trader executes her entire order with probability one and incurs a net cost of $f \times T_L^\star + 1 \times T_H^\star$.

If news occurs and $\LP$s do not withdraw liquidity from the pool, arbitrageurs can trade in the direction on the news to obtain a gross profit of $1~\C$ per token traded (i.e., the size of the news). Concretely, upon good news an arbitrageur deposits $q_{\text{arb},k} v$ units of num\'{e}raire into liquidity pool $k$ and removes $q_{\text{arb},k}$ tokens with a value of $q_{\text{arb},k} \left(v+1\right)$. Further, the arbitrageurs pays the pool fee $f_k$ and the gas fee equal to $\Gamma \diff i$. The net profit from trading $q_{\text{arb},k}$ on liquidity pool $k$ is therefore:
\begin{equation}\label{eq:pi_arb}
    \Pi_\A = q_{\text{arb},k}\left(1-f_k\right)-\Gamma \diff i>0.
\end{equation}
Since the arbitrageur can trade against a mass of liquidity providers and pay an infinitesimal gas price,  $\A$ optimally removes the entire liquidity from pool $L$. However, since the fee on pool $H$ is equal to the size of the news, the arbitrageur never consumes liquidity from pool $H$ for any positive gas fee. The mechanism is similar to the one in \citet{FoucaultMoinasTheissen2007}, where the size of news and the tick size are such that arbitrageurs consume only the liquidity at the best bid or ask. 

% \begin{ass}\label{ass:gamma}
% \begin{leftbar} \setlength{\parskip}{0ex}
% The gas fee is low enough such that it does not prevent arbitrageurs from trading on any opportunities, that is $\Gamma < 1-f$.
% \end{leftbar}
% \end{ass}

% Assumption \ref{ass:gamma} guarantees that the arbitrageur profit as defined in \eqref{eq:pi_arb} is always positive on liquidity pool $L$, as long as the pool is non-empty. That is, arbitrageurs are willing to trade upon news even if only the lowest-endowment $\LP$ with $\tau_i=\log\left(2\right) \times 1 \diff i$ submits liquidity on pool $L$. Further, since the arbitrageur profit increases in the quantity traded, $\A$ optimally removes the entire liquidity from pool $L$. Finally, since the fee on pool $H$ is equal to the size of the news, the arbitrageur never consumes liquidity from pool $H$ for any positive gas fee. The mechanism is similar to the one in \citet{FoucaultMoinasTheissen2007}, where the size of news and the tick size are such that arbitrageurs consume only the liquidity at the best bid or ask. 

When do liquidity providers withdraw their liquidity? On pool $H$, withdrawing is never optimal since the fee is high enough to deter arbitrageurs which implies adverse selection risk is zero. On pool $L$, liquidity providers with endowment $q_i$ compare the adverse selection cost and the gas fee and withdraw liquidity upon news if and only if
\begin{equation}
    q_i \left(1-f\right)>\Gamma.
\end{equation}
Lemma \ref{lem:t1} summarizes the optimal strategies for all agents at $t=1$.

\begin{lem}\label{lem:t1}
\begin{leftbar} \setlength{\parskip}{0ex}
At $t=1$, the optimal strategies are as follows:
\begin{enumerate}
    \item[(i)] a liquidity trader with a private value shock of size $\theta$ trades $\min\left\{T_L^\star,\theta\right\}$ on pool $L$ and $\max\left\{0,T_L^\star-\theta\right\}$ on pool $H$.
    \item[(ii)] upon news arrival, liquidity providers on pool $L$ pay the gas price and withdraw their liquidity if $\Gamma\leq q_i \left(1-f\right)$. In contrast, liquidity providers on pool $H$ do not attempt to withdraw liquidity upon news.
    \item[(iii)] upon news, arbitrageurs buy (sell) on pool $L$ an amount of tokens equal to the size of the pool. The arbitrageurs does not trade on pool $H$.
\end{enumerate}

\end{leftbar}
\end{lem}

\subsubsection{Liquidity provision at \texorpdfstring{$t=0$}{t=0} \label{sec:liqprov}}

We turn next to the liquidity providers' choice of pool at $t=0$. Let $T_L$ and $T_H$ denote the size of liquidity pools $L$ and $H$, expressed in token units. The expected profit of an $\LP$ with endowment $q_i$ posting liquidity on pool $L$ is
\begin{align}\label{eq:lp_L}
    \pi^\LP_L &= q_i \left(1-\eta\right)\mathbb{E}\left[\min\left\{\frac{\theta}{T_L},1\right\}\right] f  - \eta \min\left\{\Gamma, q_i\left(1-f\right)\right\} \nonumber \\
    &=q_i \left[\left(1-\eta\right)\left(1 - \log 2\frac{T_L}{2}\right) f\right] -\eta \min\left\{\Gamma, q_i\left(1-f\right)\right\},
\end{align}
since
\begin{align}
    \mathbb{E}\left[\min\left\{\frac{\theta}{T_L},1\right\}\right] &= \mathbb{P}\left(\theta\leq T_L\right) \times \mathbb{E}\left[\frac{\theta}{T_L} \mid \theta\leq T_L\right] + \mathbb{P}\left(\theta > T_L\right) \times 1 \nonumber \\
    & = T_L \log 2 \times \frac{1}{2} + \left(1-T_L \log 2\right) = 1 - \log 2\frac{T_L}{2},
\end{align}
where the last equality follows from the fact that $\theta$ is uniformly distributed over $\left[0,\log^{-1} 2\right]$. With probability $1-\eta$, a liquidity trader arrives at $t=1$ and trades $\theta$. If $\theta>T_L$, then the liquidity trader consumes the entire pool and the $\LP$ receives the fee $f$ for each unit of liquidity posted. Conversely, if $\theta\leq T_L$, then the liquidity provider receives a share $\frac{q_i}{T_L}$ of the aggregate fees $\theta f$. With probability $\eta$, news occurs: from Lemma \ref{lem:t1}, the liquidity provider either pays the gas fee $\Gamma$ and withdraws $q_i$ from the pool or does nothing and incurs a loss $q_i\left(1-f\right)$ on the subsequent arbitrage trade.

Alternatively, the $\LP$ can deposit liquidity on pool $H$ and earn expected profit
\begin{align}\label{eq:lp_H}
    \pi^\LP_H &= q_i \left(1-\eta\right) \mathbb{E}\left[\max\left\{0,\frac{\theta-T_L}{T_H}\right\}\right] \nonumber \\
    & = q_i \left(1-\eta\right) \left(1-T_L \log 2\right) \frac{1-T_L \log 2}{2 T_H \log 2},
\end{align}
where the second line follows from explicitly computing the expectation
\begin{align}
    \mathbb{E}\left[\max\left\{0,\frac{\theta-T_L}{T_H}\right\}\right] &= \mathbb{P}\left(\theta\leq T_L\right) \times 0 + \mathbb{P}\left(\theta > T_L\right) \times \frac{\frac{\log^{-1} 2+T_L}{2}-T_L}{T_H} \nonumber \\
    & = \left(1-T_L \log 2\right) \frac{1-T_L \log 2}{2 T_H \log 2}.
\end{align}
If the liquidity trader demand is low enough, that is if $\theta\leq T_L$, then the entire trade is filled on pool $L$ and liquidity providers on $H$ earn nothing. However, if $\theta>T_L$, the residual liquidity demand $\theta-T_L$ is routed to pool $H$ and liquidity providers earn a share proportional to their deposit, i.e., $\frac{q_i}{T_H}$. If news occurs, $\LP$s on $H$ do not incur an adverse selection cost since from Lemma \ref{lem:t1} arbitrageurs do not submit orders to the high-fee pool.


Liquidity providers in the low-fee pool absorb a larger share of the uninformed order flow, since the $\LT$ order is first routed to pool $L$. On the other hand, they face adverse selection costs and may need to pay gas fees $\Gamma$ upon the realization of news to withdraw liquidity. At the same, $\LP$s in the high-fee pool face no adverse selection, receive a larger fee per unit traded, but volume is limited as they only fill the residual demand from uninformed $\LT$s after liquidity on the low-fee pool is exhausted. From equations \eqref{eq:lp_L} and \eqref{eq:lp_H}, liquidity provider $i$ chooses the low-fee pool $L$ if and only if
\begin{equation}\label{eq:cost_comparison}
    \pi^\LP_L>\pi^\LP_H \Longleftrightarrow q_i \frac{\left(1-\eta\right)\left(\left(1-T_L \log 2\right)^2-f T_H \log 2 \left(2-T_L\log 2\right)\right)}{2\log2 T_H} - \eta\min\left\{\Gamma,q_i\left(1-f\right)\right\} > 0.
\end{equation}
A salient implication of equation \eqref{eq:cost_comparison} is that $\LP$s with larger endowments are more likely to choose the low-fee pool, keeping liquidity shares constant. The rationale is that gas fees are a fixed cost, and larger $\LP$s are more likely to achieve economies of scale. The expected fee revenue scales linearly with a liquidity provider's share in the liquidity pool (proportional to $q_i$), better compensating $\LP$s for the gas fee paid upon news arrival at $t=1$. 

We follow \citet{KatzShapiro1985} and conjecture that there exists a marginal liquidity provider $\qmg$ such that all $\LP$s with $q_i>\qmg$ post liquidity on the low-fee pool and all $\LP$s with $q_i\leq \qmg$ choose the high-fee pool.\footnote{We note that there cannot be a ``reversed-sign'' equilibrium, where $\LP$s with $q_i\leq\qmg$ post liquidity on the low-fee pool and all $\LP$s with $q_i>\qmg$ choose the high-fee pool. To understand the rationale, we point out that for an $\LP$ with endowment $\tilde{q}<\qmg$, submitting liquidity to pool $L$ yields a lower expected revenue since
\begin{equation*}
    \pi^\LP_L-\pi^\LP_H=\tilde{q} \frac{\left(1-\eta\right)\left(\left(1-T_L\right)^2-f T_H \left(2-T_L\right)\right)}{2T_H} - \eta\min\left\{\Gamma,q_i\left(1-f\right)\right\} < 0.
\end{equation*}
Therefore, it is optimal for the $\LP$ with endowment $\tilde{q}$ to post liquidity on the high-fee pool, which contradicts the conjectured equilibrium.  Importantly, since each $\LP$ is ``small'' relative to the aggregate mass of liquidity providers, individual deviations do not impact aggregate pool sizes $T_L$ and $T_H$.} The conjectured equilibrium pins down the pool sizes $T_L$ and $T_H$ as a function of the endowment for the marginal $\LP$:
\begin{align}\label{eq:liquidity_levels}
    T_L&=\int_{\qmg}^2 q_i \phi\left(q_i\right) \diff i = \log^{-1}\left(2\right) \left(2 - \qmg\right) \text{ and }\nonumber \\
    T_H&=\int_1^{\qmg}  q_i \phi\left(q_i\right) \diff i = \log^{-1}\left(2\right)\left(\qmg -1\right). 
\end{align}
From equations \eqref{eq:cost_comparison} and \eqref{eq:liquidity_levels} it follows that the expected profit difference between the low- and high-fee pools can be written as a linear decreasing function of the marginal $\LP$'s endowment, that is
\begin{equation}\label{eq:pi_diff}
    \pi^\LP_L-\pi^\LP_H = q_i \left[\frac{1}{2} \left(1-\eta\right) \left(1-\left(1-f\right)\qmg\right)\right] - \eta \min\left\{q_i\left(1-f\right),\Gamma\right\}.
\end{equation}
We search for fulfilled expectation equilibria \citep[following the definition of][]{KatzShapiro1985}, where the beliefs of $\LP$s at $t=0$ about the size of liquidity pools are consistent with the outcome of their choices. We solve \eqref{eq:pi_diff} on the support for $q_i$ -- the interval $\left[1,2\right]$ to obtain the $\LP$ reaction function
\begin{equation}\label{eq:reaction_main}
    \tilde{q}\left(\qmg\right)=\begin{cases}
    1, & \text{ for } \qmg \leq \frac{1-\eta\left(1+2\min\left\{\Gamma,1-f\right\}\right)}{\left(1-f\right)\left(1-\eta\right)}\\
    \frac{2\eta\Gamma}{ \left(1-\eta\right) \left(1-\left(1-f\right)\qmg\right)}, & \text{ for } \qmg \in \left(\frac{1-\eta\left(1+2\min\left\{\Gamma,1-f\right\}\right)}{\left(1-f\right)\left(1-\eta\right)}, \frac{1-\eta\left(1+\Gamma\right)}{\left(1-f\right)\left(1-\eta\right)}\right] \\
    2, & \text{ for } \qmg > \frac{1-\eta\left(1+\Gamma\right)}{\left(1-f\right)\left(1-\eta\right)}.
    \end{cases}
\end{equation}
In any fulfilled expectation equilibrium, the equilibrium endowment of the marginal $\LP$ is a fixed point of equation \eqref{eq:reaction_main}. Figure \ref{fig:reaction} plots the $\LP$ reaction function $\tilde{q}\left(\cdot\right)$ to graphically illustrate equilibrium formation for two parameter choices. Let $q^\star_1$ and $q^\star_2$ be the interior roots of the reaction function \eqref{eq:reaction_main}, that is the solutions of the quadratic form
\begin{equation}
    q-\frac{2\eta\Gamma}{ \left(1-\eta\right) \left(1-\left(1-f\right)q\right)}=0.
\end{equation}
In the top left panel, we illustrate a parameter combination for which are three equilibria, at $\qmg\in\left\{q^\star_1, q^\star_2, 2\right\}$. However, $q^\star_2$ is an unstable equilibrium -- a tipping point \citep[as in][]{Jullien2011} at which small perturbation in beliefs cause the $\LP$s to spiral away from the postulated equilibrium (we refer the reader to the proof of Proposition \ref{prop:equilibria} for a more formal discussion). Consequently, the stable interior equilibrium co-exists with an equilibrium in which all $\LP$s choose pool $H$; this is the case for $f\leq\frac{2}{3}$. The top right panel illustrates a parameter combination for which the stable interior equilibrium coexists with an equilibrium where all $\LP$s provide liquidity on the low-fee pool (for $f>\frac{2\eta}{1+\eta}$).  Finally, the bottom panel illustrates a parameter combination for which there is a unique and stable interior equilibrium at $\qmg=q^\star_1$. 

\begin{figure}[H]
\caption{\label{fig:reaction} Liquidity provider reaction function and equilibria}
\begin{minipage}[t]{1\columnwidth}%
\footnotesize
This figure illustrates equilibrium $\LP$ liquidity pool choices as fixed points of the reaction function $\tilde{q}\left(\qmg\right)=\qmg$. We consider three distinct cases for which a stable interior equilibrium may arise. Stable equilibria are marked with green circles, whereas unstable equilibria are market with magenta squares. Parameter values are $f=0.64$, $G=0.14$, $\eta=0.71$ (top left), $f=0.69$, $G=0.15$, $\eta=0.71$ (top right), $f=0.792$, $G=0.26$, $\eta=0.65$ (bottom).
\end{minipage}

\vspace{0.05in}

\begin{centering}
\includegraphics[width=\textwidth]{Figures/model_reaction_stable.png}
\par\end{centering}

\end{figure}


Proposition \ref{prop:equilibria} establishes conditions under which a fragmented equilibrium exists, wherein both liquidity pools have positive market share. 

\begin{prop}\label{prop:equilibria}
\begin{leftbar} \setlength{\parskip}{0ex}
A stable fragmented equilibrium, in which both liquidity pools have positive market share, exists for $\Gamma\in\left[\underline{\Gamma},\bar{\Gamma}\right)$, where
\begin{align}
    \underline{\Gamma}&=\max\left\{f\frac{1-\eta}{2\eta},\frac{1+\eta(2f-3)}{1-\eta}\right\} \text{ and }     \bar{\Gamma}=\begin{cases} \frac{1-\eta}{8\eta(1-f)} & f \leq 0.75 \\
                           \frac{(2f-1)(1-\eta)}{\eta} & f>0.75 \end{cases}.
\end{align}
The fragmented equilibrium is further unique if $f\in\left[\frac{2}{3},\frac{2\eta}{1+\eta}\right)$ and $\Gamma\in\left[f\frac{1-\eta}{2\eta},\frac{(2f-1)(1-\eta)}{\eta}\right)$. 
In any fragmented equilibrium, the token endowment of the marginal liquidity provider is 
\begin{equation}
    \qmg^\star=\frac{1}{2\left(1-f\right)}-\frac{1}{2\left(1-f\right)}\sqrt{1-\eta\frac{1+8\left(1-f\right)\Gamma}{1-\eta}},
\end{equation}
such that all liquidity providers with $q_i\leq \qmg^\star$ post liquidity on pool $H$, and all liquidity providers with $q_i> \qmg^\star$ post liquidity on pool $L$.
\end{leftbar}    
\end{prop}

Figure \ref{fig:region_gamma} highlights the parameter region where multiple liquidity pools coexist in equilibrium with positive market share.\footnote{We note that the interior equilibrium is not necessarily the unique one. For low fees on pool $L$ ($f\leq\frac{2}{3}$), the interior equilibrium coexists with a corner equilibrium where all traders choose platform $H$. Conversely, for $f>\frac{2\eta}{1+\eta}$, the interior equilibrium coexists with an equilibrium where all traders choose platform $L$.} In particular, an interior equilibrium for which both the $L$ and $H$ pool attract a positive market share emerges for moderate gas fee $\Gamma$ and a small enough difference between liquidity fees on the two pools (i.e., a large $f$). For low values of the gas fee ($\Gamma\leq\underline{\Gamma}$), managing liquidity is cheap: competition effects are strong and all $\LP$s post liquidity on the low-fee pool. For high values of the gas fee ($\Gamma>\bar{\Gamma}$), withdrawing liquidity upon the realization of news is prohibitively expensive and $\LP$s cluster on the high-fee pool where they are protected from adverse selection. For very large gas fees $\Gamma>2\left(1-f\right)$, no $\LP$ optimally reacts upon news -- in this case, multiple single-pool equilibria may emerge where liquidity either clusters on pool $L$ or on pool $H$. 

\begin{cor}\label{cor:monitoring}
\begin{leftbar} \setlength{\parskip}{0ex}
In any interior equilibrium, \emph{all} liquidity providers on $L$ withdraw liquidity upon news.
\end{leftbar}  
\end{cor}

Corollary \ref{cor:monitoring} establishes that there are no $\LP$s in a fragmented equilibrium that do not actively manage liquidity. All low-endowment $\LP$s for whom reacting upon news is not profitable provide liquidity on platform $H$. In contrast, on single-pool equilibria and for $\Gamma>1-f$, only a fraction of liquidity providers withdraw liquidity upon news. Empirically, we would expect a higher share of $\LP$s actively managing liquidity on pool $L$ when multiple pools co-exist in equilibrium than when all trading concentrates on pool $L$.

\begin{figure}[H]
\caption{\label{fig:region_gamma} Parameter regions for which a two-pool equilibrium exists}
\begin{minipage}[t]{1\columnwidth}%
\footnotesize
This figure illustrates the parameter regions for which a fragmented stable equilibrium emerges, in which both pools attract positive market share. The top panel focuses on the case where $\eta=0.65$. We further highlight (in red) the region for which the equilibrium is unique. In the bottom panel, we plot fragmented equilibrium regions for multiple values of $\eta$.
\end{minipage}

\vspace{0.05in}

\begin{centering}
\includegraphics[width=\textwidth]{Figures/region_interior.png}
\par\end{centering}

\end{figure}





% \begin{prop}\label{prop:equilibria}
% \begin{leftbar} \setlength{\parskip}{0ex}
% For ease of notation, we define and tabulate below three gas fee thresholds $\bar{\Gamma}_k$, $k\in\left\{1,2,3\right\}$.

% \begin{center}
%     \begin{tabular}{ccc}
%     \toprule
%     $\bar{\Gamma}_1$ & $\bar{\Gamma}_2$ & $\bar{\Gamma}_3$ \\
%     \cmidrule{1-3}
%     $f\frac{1-\eta}{2\eta}$     &  $\frac{\left(2f-1\right)\left(1-\eta\right)}{\eta}$ & $\frac{1-\eta}{8\left(1-f\right)\eta}$\\
%     \bottomrule
%     \end{tabular}
% \end{center}

% It follows there are has either one, two, or three stable fulfilled expectation equilibria at $t=0$, corresponding to the following $\LP$ liquidity pool choices:
% \begin{enumerate}
%     \item[(i)] An interior equilibrium with marginal $\LP$ characterized by endowment $\qmg^\star=q^\star_1$, such that all $\LP$s with endowment $q>q^\star_1$ add liquidity to the low-fee pool and the rest choose the high-fee pool. The equilibrium emerges for $f\in\left[\frac{1}{2},\frac{3}{4}\right)$ and $\Gamma\in\left(\bar{\Gamma}_1, \bar{\Gamma}_3\right]$ and $f>\frac{3}{4}$ and $\Gamma\in\left(\bar{\Gamma}_1, \bar{\Gamma}_2\right]$. Moreover, the interior equilibrium is unique for $f>\frac{2}{3}$ and $\Gamma\in\left(\bar{\Gamma}_1, \bar{\Gamma}_2\right]$.
%     \item[(ii)] A corner equilibrium where $\qmg^\star=1$, such that all $\LP$s post liquidity on the low-fee pool. The equilibrium emerges for $\Gamma\leq\bar{\Gamma}_1$ and is further unique if $f>\frac{1}{2}$ and $\Gamma\leq\min\left\{\bar{\Gamma}_1,\bar{\Gamma}_2\right\}$.
%     \item[(iii)] A corner equilibrium where $\qmg^\star=2$, such that all $\LP$s post liquidity on the high-fee pool. The equilibrium emerges for $\Gamma>\bar{\Gamma}_2$ and is further unique if $f>\frac{3}{4}$ and $\Gamma>\bar{\Gamma}_2$, $f>\frac{1}{2}$ and $\Gamma>\bar{\Gamma}_3$, or $f\leq\frac{1}{2}$ and $\Gamma>\bar{\Gamma}_1$.
% \end{enumerate}

% \end{leftbar}
% \end{prop}

% Proposition \ref{prop:equilibria} establishes existence conditions for each possible equilibrium. In particular, an interior equilibrium for which both the $L$ and $H$ pool attract a positive market share emerges for moderate gas fee $\Gamma$ and a small enough difference between liquidity fees on the two pools (i.e., a large $f$). The interior equilibrium is unique if the liquidity fees are close enough across the two pools. Figure \ref{fig:regions} highlights the parameter region where multiple liquidity pools coexist with positive market share. 

% The remaining results in Proposition \ref{prop:equilibria} are intuitive: a small gas fee $\Gamma$ reduces the $\LP$s' costs to manage stale liquidity upon news and stimulates competition on the low-fee pool. In other words, the cost of updating liquidity is lower than the opportunity cost of not capturing uninformed trades. In contrast, a large enough $\Gamma$ incentivizes liquidity providers to deposit tokens on the high-fee pool, since managing liquidity on pool $L$ is too costly. 

% \begin{figure}[H]
% \caption{\label{fig:regions} The emergence of two-pool equilibria}
% \begin{minipage}[t]{1\columnwidth}%
% \footnotesize
% This figure illustrates the emergence of two-pool equilibria for different values of the liquidity fee $f$ and gas fee $\Gamma$. We set the probability of informed trading at $\eta=0.85$. We highlight the parameter region for which a two-pool equilibria emerges and is unique (in red) as well as the region for which a two-pool equilibria emerges but is not unique (in blue). 
% \end{minipage}

% \vspace{0.05in}

% \begin{centering}
% \includegraphics[width=0.9\textwidth]{Figures/model_int_eq_region.png}
% \par\end{centering}

% \end{figure}

\subsection{Implications and empirical predictions}

In this section, we zoom in on the properties of the interior equilibrium, that is, the most interesting case featuring segmented liquidity across multiple pools. From Proposition \ref{prop:equilibria}, the only possible interior equilibrium in the liquidity provision game is for a marginal $\LP$ with endowment $\qmg=q_1^\star$.

\begin{pred}\label{pred:clienteles}
\emph{If an interior equilibrium exists where liquidity is segmented across multiple pools, the average liquidity deposit in the low-fee pool is larger than for the high-fee pool.}
\end{pred}

Prediction \ref{pred:clienteles} follows from the discussion in Section \ref{sec:liqprov}. Liquidity providers with large token endowments ($q_i>\qmg$) deposit them in the low-fee pool since they have stronger incentives to pay the gas fee and actively manage the liquidity. Conversely, $\LP$s with lower endowments ($q_i\leq\qmg$) gravitate towards the high-fee pool, accepting a lower trade probability in exchange for reducing adverse selection costs without active liquidity management and paying gas fees.

\begin{pred}\label{pred:updates}
\emph{Liquidity providers on the low-fee pool are more likely to actively manage liquidity.}
\end{pred}
\begin{pred}\label{pred:monitoring_shares}
\emph{Liquidity providers on the low-fee pool are more likely to actively manage liquidity in a fragmented market than in a consolidated market.}
\end{pred}

The two predictions follow from Corollary \ref{cor:monitoring}. In equilibrium, the $\LP$s on the low-fee pool update their liquidity upon news arrival to avoid adverse selection, unlike their counterparts on the high-fee pool. 


\begin{pred}\label{pred:comp_stat_Gamma}
\emph{The liquidity share of the low-fee pool $L$ decreases in the gas fee $\Gamma$.}
\end{pred}
\begin{pred}\label{pred:comp_stat_eta}
\emph{The liquidity share of the low-fee pool $L$ decreases in the probability of informed trading $\eta$.}
\end{pred}

Predictions \ref{pred:comp_stat_Gamma} and \ref{pred:comp_stat_eta} state that the low-fee pool becomes less attractive for liquidity providers if the gas fee increases (higher $\Gamma$) -- making active liquidity management less profitable -- or if the probability of informed trading is higher ($\eta$ increases) which leads to \emph{more frequent} liquidity management. Formally, we can show that $q_1^\star$ increases in both $\Gamma$ and $\eta$ -- leading to a lower value of $T_L^\star$:
\begin{align}
    \frac{\partial q_1^\star}{\partial \Gamma}&=\frac{2 \eta }{\sqrt{(1-\eta ) (\eta  (8 \Gamma  (f-1)-1)+1)}}>0 \text{ and } \nonumber \\
    \frac{\partial q_1^\star}{\partial \eta}&=\frac{2 \Gamma }{(1-\eta) \sqrt{(1-\eta ) (\eta  (8 \Gamma  (f-1)-1)+1)}}.
\end{align}

\begin{pred}\label{pred:trade_volume}
\emph{If an interior equilibrium exists, the trading volume share of the low-fee pool is higher than its liquidity share.}
\end{pred}
The intuition is that $\LP$s on the low-fee pool deposit large token quantities and they absorb a disproportionate amount of incoming trades -- it is possible that $\LP$s on the high-fee pool do not trade at all against incoming orders, despite providing positive liquidity in equilibrium. To formally see the result, we first note that there is no informed trade in equilibrium on either pool. The average $\LT$ trade size on the low-fee pool is
\begin{align}
    \mathbb{E}\left[\min\left\{\theta,T_L^\star\right\}\right]&=\mathbb{P}\left(\theta\leq T_L\right) \mathbb{E}\left[\theta\mid \theta<T_L^\star\right] + \left(1-\mathbb{P}\left(\theta\leq T_L\right)\right) T_L^\star \nonumber \\
    &= T_L^\star\log 2\frac{T_L^\star}{2} + \left(1-T_L^\star\log 2\right) T_L^\star= T_L^\star-\frac{\left(T_L^\star\right)^2}{2}\log 2.
\end{align}
The average $\LT$ trade size on the high-fee pool is
\begin{align}
    \mathbb{E}\left[\max\left\{0,\theta-T_L^\star\right\}\right]& = \left(1-\mathbb{P}\left(\theta\leq T_L\right)\right) \left(\mathbb{E}\left[\theta\mid \theta>T_L^\star\right]-T_L^\star\right)\nonumber \\
    &= \left(1-T_L^\star\log 2\right) \frac{\left(\log^{-1} 2-T_L^\star\right)}{2}=\frac{\log^{-1} 2}{2}-T_L^\star+\frac{\left(T_L^\star\right)^2}{2}\log 2.
\end{align}
We note that the trade share of pool $L$ is equal to $2T_L^\star\log 2-\left(T_L^\star\log 2\right)^2$ which is larger than its liquidity share $T_L^\star\log 2$ since $T_L^\star\log 2<1$. Figure \ref{fig:liqshares} illustrates this result.




\begin{figure}[H]
\caption{\label{fig:liqshares} Liquidity and volume shares}
\begin{minipage}[t]{1\columnwidth}%
\footnotesize
This figure illustrates the relative liquidity and trade volume on the two pools, as a function of the gas fee $\Gamma$. Parameters: $\eta=0.36$ and $f=0.8$.
\end{minipage}

\vspace{0.05in}

\begin{centering}
\includegraphics[width=0.9\textwidth]{Figures/model_compstatics.png}
\par\end{centering}

\end{figure}


\begin{pred}\label{pred:liq_shares}
\emph{The low-fee pool is larger than the high-fee pool (in terms of aggregate deposits) only if the gas fee is low enough, that is if}
\begin{equation}
    \Gamma < \Gamma^\star \equiv \frac{3 (3 f-1) (1-\eta)}{8 \eta }
\end{equation}
\end{pred}

From equation \eqref{eq:liquidity_levels}, if the marginal $\LP$ has endowment $q_1^\star$, then the equilibrium sizes of the two liquidity pools are, respectively,
\begin{align}
    T_L^\star&=\log^{-1}\left(2\right)\left[2- \frac{1}{2\left(1-f\right)} \left(1- \sqrt{1-\eta\frac{1+8\left(1-f\right)\Gamma}{1-\eta}}\right)\right] \text{ and } \nonumber \\
    T_H^\star&=\log^{-1}\left(2\right)\left[\frac{1}{2\left(1-f\right)} \left(1- \sqrt{1-\eta\frac{1+8\left(1-f\right)\Gamma}{1-\eta}}\right)-1\right].
\end{align}


Prediction \ref{pred:liq_shares} translates to stating that $T_L^\star>T_H^\star$, or equivalently to $q_1^\star\leq \frac{3}{2}$, where the latter inequality is true for any $\Gamma\leq\Gamma^\star$. Therefore, even though the low-fee pool attracts the $\LP$s with large token endowments, it is not necessarily the largest pool if the gas fee exceeds a certain threshold. 

\section{Stylized facts}

To understand liquidity provision and trading on Uniswap v3, I describe below some stylized facts pertaining to the USDC-WETH pair (the most widely traded).

\begin{enumerate}
    \item 86.4\% of all new mints by volume (and 6.2\% by mint count) come from JIT liquidity provision events (i.e., mints and burns that happen in the same block, by same address, exactly 2 positions apart and which sandwich a trade in the same pool).
        \begin{itemize}
            \item Out of the subset of JIT mints, 87.74\% are relayed through Flashbots (presumably the others are relayed through different private mempools) and 97.92\% are executed through a MEV contract as labeled by Etherscan.
            \item For non-JIT mints, 99.02\% are lit (i.e., not relayed through Flashbots) and 99.16\% are not executed through MEV smart contracts.
            \item JIT seems to be the main ``game in town'' for sophisticated or dark liquidity provision.
        \end{itemize}
        \item 66.27\% of non-JIT mints by count occur in the 30bps pool, whereas 56.86\% of new mints by volume happen in the 5bps pool.
        \item The median non-JIT liquidity mint in the 5bps pool is \$47,646, that is 10 times larger than for the 30bps pool (median mint is \$4,181).
        \item On aggregate, 81.4\% of traded volume is in the 5bps pool and 18.3\% in the 30bps pool.
            \begin{itemize}
                \item Flow to the 5bps seems more sophisticated. 61\% of volume (20.9\% of trades) is dark -- relayed through Flashbots, compared to only 38.6\% (21.64\% of trades) of volume on the 30bps pool.
                \item Similarly, 57.9\% of volume (17.46\% of trades) on the 5bps pool comes from MEV contracts, copared to 49\% on the 30bps pool (30.7\% of trades).
            \end{itemize}
        \item The average trade on the 30bps pool is much larger than on the 5bps pool (mean is twice as large \$189,166 versus \$94,215, median 8x as large: \$78,200 versus \$9,000). Only 9\% of trades occur on the 30bps pool, but they are large so amount for 18\% of volume. The difference comes from non-MEV trades primarily.
        \item About half of trades use a router in either pool (48\% in the 5bps pool, 44\% in the 30bps pool).
        \item Not many trades seem to be routed (same initiator and direction, same block). Just 1.1\% on the 5bps pool and 6.5\% on the 30bps pool. Why submit directly to the 30bps pool? Avoid gas fee from splitting.
\item The time from mint to burn (i.e., from opening a new position to removing or re-balancing it) is much larger on the 30 bps pool:
    \begin{enumerate}
        \item Median: 19h31m (5 bps pool) versus 37h36m (30 bps pool).
        \item Average: 6 days 12h (5 bps pool) versus 13 days 17h (30 bps pool).
    \end{enumerate}
\item The time from burn to mint is much shorter -- conditional on re-balancing, LPs do so fast:
    \begin{enumerate}
        \item Median: 9 min 1 second (5 bps pool) versus 8 minute 33 seconds (30 bps pool).
        \item Average: 3 days 9h (5 bps pool) versus 5 days 8h (30 bps pool) -- driven by some large outliers.
    \end{enumerate}
\item A majority of time when they burn liquidity, LPs do so because their positions are out of range (72\% of the time on the 5bps pool, 64\% on the 30 bps pool; 67\% on aggregate). 
\item However, when they mint liquidity, LPs include the current price in the range 80\% of the time.S
\end{enumerate}





==> Old/model_v2_Comments.tex <==

\subsection{Model primitives}

\paragraph{Assets.} Consider a three-period economy, where time is indexed by $t\in\left\{0,1,2\right\}$. There are two assets, a risky token $\T$ and a riskless num\'{e}raire $\C$. At $t=2$, the risky token $\T$ pays a stochastic dividend $\tilde{v}$ (denominated in units of $\C$). At the start of the game, the expected token value is $\mathbb{E}_0 \tilde{v}=v>1$. 

\cp{Why dividend as opposed to terminal value?  Why is one token riskless?  Why isn't this just a relative price?}

The asset $\C$ stands in for cryptocurrencies typically used as num\'{e}raire on decentralized exchanges -- for example Ether (the native currency of the Ethereum blockchain) or stablecoins such as Tether or USD~Coin. The num\'{e}raire pays a risk-free rate of return $r$, which we normalize to zero without loss of generality.

\cp{I think the para above can just be nuked.}

\paragraph{Trading environment.} The risky token is traded on two liquidity pools: $L$ (a low-fee pool) and $H$ (a high-fee pool). \cp{The type of fee has not been defined, i.e., fixed, proportional.} The asset quantities in each pool $k\in\left\{L,K\right\}$ must satisfy at all times the following linear bonding curve:
\begin{equation}\label{eq:bond_curve}
    v \T_k + \C_k = \text{constant}.
\end{equation}
The bonding curve \eqref{eq:bond_curve} implies that the token price is constant and equal to $v$ units of the num\'{e}raire, since $-\frac{\diff T}{\diff C}=v$.\footnote{In practice, most decentralized exchanges use convex bonding curve, for example constant product pricing. While the choice of bonding curve is of first order importance for liquidity demanders who need to split trades to optimize price impact, we argue it is less important for liquidity suppliers. For tractability, we assume a linear bonding curve which implies that liquidity traders only care about pool fees -- the focus of our model. In a richer model with convex pricing, we would expect to see relatively more fragmentation since minimzing price impact might require further splitting trades.} To fix intuition behind the mechanics of the market, suppose a trader wishes to buy $t$ units of the token. This reduces the token amount in the pool to $\T_k-t$. In return, the trader needs to add $\Delta$ units of the num\'{e}raire, where $\Delta$ is such that the new asset quantities remain on the bonding curve, that is:
\begin{equation}
    v \left(\T_k-t\right) + \left(\C_k+\Delta\right) = v \T_k + \C_k,
\end{equation}
which is equivalent to having $\Delta = v t$. The slope of the bonding curve is equal to the expected value of the asset to ensure there are no arbitrage opportunities at the start of the game. 

The two liquidity pools charge different fees on liquidity-removing trades. Fees are expressed in units of num\'{e}raire and are distributed to all liquidity providers in a given pool, proportional to the amount of liquidity provided.  The low-fee pool $L$ charges a fee of $f~\C$ where $f<1$, and the high-fee pool $H$ charges a fee of $1~\C$ per token traded. That is, to purchase $t$ units of the token on the $L$ pool, the total cost of an investor is $t\left(v+f\right)$.

\cp{I'm not sure that the notation is fabulous. Maybe $\ell$ and $h$. Everything will be in terms of $h-\ell$.} \mz{Agreed. What's really key here is the relation between the fees and the size of news.}

\paragraph{Events.} At $t=1$, two types of exogenous events can occur. With probability $\eta<1$, the common value of the token changes to $v+1$ (good news) or to $v-1$ (bad news); good and bad news are equally likely. With probability $\left(1-\eta\right)$ -- that is if news does not occur -- a liquidity trader ($\LT$) receives a private value shock and needs to trade $\tilde{\theta}$ units of the token, where $\tilde{\theta}\sim\text{Uniform}\left[0,\log^{-1}\left(2\right)\right]$. The liquidity trader is equally likely to buy or sell the token. We assume the $\LT$s private value is large enough to cover transaction costs on either liquidity pool.

\cp{This upper bound is ugly. How far can one go with a generic upper bound....The uniform is already quite specific. Also, up and down by an amount $\delta$?.  Maybe for each parameterization find the private value assumption needed.} \mz{The upper bound was chosen to match the aggregate liquidity provision (in an earlier version I had both the upper bound \& aggregate liquidity normalized to one). If $\theta$ can be higher than that, it weakens competition between $\LP$s: if everyone's liquidity executed for sure, then $\LP$s prefer the high-fee pool. So I set the upper bound such that there's always someone who does not get executed.}

\paragraph{Liquidity providers and arbitrageurs.} In addition to liquidity traders, the token is traded by two types of agents: risk-neutral liquidity providers ($\LP$) and arbitrageurs ($\A$). There is a continuum of liquidity providers indexed by $i$, endowed with heterogeneous amounts of the token $T$. Liquidity provider $i$ is endowed with $q_i$ units of the token. Following \citet{KhomynPutninsZoican2022}, we assume that $q_i$ is distributed with density
\begin{equation}\label{eq:density}
    \phi\left(q\right)=\log^{-1}\left(2\right)\frac{1}{q},\text{ for }q\in\left[1,2\right].
\end{equation}
The choice of density ensures that the aggregate token endowment of liquidity providers $\T_\text{agg}$ is normalized to a constant, since
\begin{equation}\label{eq:aggliq}
    \T_\text{agg}=\int_1^2 q_i \phi\left(q_i\right)\diff q_i = \log^{-1} \left(2\right).
\end{equation}
Further, the density is chosen to match key features of the empirical distribution of $\LP$s: there are many low-endowment liquidity providers (e.g., retail traders) and a long tail of high-capital investors who provide liquidity to decentralized exchange -- for example, quantitative institutional investors. Figure \ref{fig:distribution} illustrates the theoretical distribution of $\LP$s endowments.


\cp{Does something like a pareto distribution work or have their liquidity supply as 1+ RV drawn from an exponential?}
\mz{I am not sure. The point here was to have market shares that are linear in the marginal trader's $\qmg$ -- otherwise we don't get a closed form when solving for the fulfilled expectation equilibrium. To have linear market shares, I need $q_i\phi(q_i)$ to be a constant, which means $\phi(\cdot)$ needs to be proportional to $\frac{1}{q_i}$. The ugly log constant term just ensures the density integrates out to one.

$\int_1^{\qmg} q_i \phi\left(q_i\right)\diff q_i = a + b \qmg $}

\begin{figure}[H]
\caption{\label{fig:distribution} Liquidity provider endowment (scaled) $q_i$}
\begin{minipage}[t]{1\columnwidth}%
\footnotesize
This figure illustrates the probability density of liquidity provider token endowments, $\phi\left(\cdot\right)$, as defined in equation \eqref{eq:density}.
\end{minipage}

\vspace{0.05in}

\begin{centering}
\includegraphics[width=0.8\textwidth]{Figures/model_density.png}
\par\end{centering}

\end{figure}

The arbitrageurs $\A$ are risk-neutral speculative traders as in \citet{Budish2015TheResponse} or \citet{Menkveld2017NeedLiquidity}, and have zero private value for the token. Upon observing a common value innovation, arbitrageurs can submit a trade against liquidity providers if (i) liquidity is being offered at a stale price and (ii) it is profitable to take liquidity after taking into account gas costs and pool fees.

\cp{Every arbitrageur since the 1980s has been risk neutral and profit maximizing.  I don't think this warrants citations. }

\paragraph{Gas fee (order execution cost).} Orders submitted at $t=1$ to trade against pool liquidity or to withdraw existing liquidity incur a fixed execution cost $\Gamma>0$. The execution cost can be interpreted as the gas price on the Ethereum blockchain as in \citet{CapponiJia2021}. In contrast to \citet{CapponiJia2021}, we assume traders on the decentralized exchanges are price takers on the gas market and their orders do not impact the gas cost. A natural interpretation is that message volume at any time in a particular asset pair traded on decentralized exchanges is small relative to the aggregate transaction flow on the entire blockchain.

Gas fees on decentralized exchanges differ from trading fees on traditional exchanges in a number of ways. First, they are not set by individual exchanges to compete with each other, but are a common transaction cost \emph{across} exchanges. Second, they are levied on a per-order rather than per-share basis: this implies economies of scale for larger orders. Third, there is significant time variation in gas fees which allows us to better empirically identify the impact of transaction costs on liquidity pool market shares.

\paragraph{Timing.} Figure \ref{fig:timing} summarizes the sequence of events at each time $t$. At $t=0$, liquidity providers arrive at the market and choose to deposit their tokens (and corresponding num\'{e}raire) on either the high- or low-fee liquidity pool. At $t=1$, an exogenous trigger event happens: either news, that is a common value innovation, or a private value shock to liquidity traders. With probability $1-\eta$, a liquidity trader arrives and trades a random quantity $\tilde{\theta}$. Conversely, with probability $\eta$, news arrives which moves the asset value to either $v+1$ or $v-1$. In this case, liquidity providers have a first-mover advantage: they can pay the fixed gas fee $\Gamma$ and withdraw liquidity from the pool to avoid being adversely selected. Following the $\LP$s' choice, arbitrageurs may trade in the direction of the news if profitable to do so. Finally, at $t=2$ all payoffs are realized. 

\begin{figure}[H]
\caption{\label{fig:timing} \textbf{Model timing}}

\vspace{0.1in}
\begin{centering}
\includegraphics[width=0.9\textwidth]{Figures/timing_dex_v2.pdf}
\par\end{centering}

\end{figure}

\cp{Useful to have a variable that captures the extent to which LP can withdraw?  Something like an attention variable. After a news event, they can probabilistically withdraw liquidity if optimal. }

\subsection{Equilibrium \label{sec:eq}}

We solve the game by backward induction. First, we discuss the optimal strategy of arbitrageurs and liquidity traders at $t=1$, taking equilibrium liquidity provision as given. Next, we solve for the optimal liquidity pool choices of $\LP$s at $t=0$. 

\subsubsection{Optimal strategies at \texorpdfstring{$t=1$}{t=1}}

The linear pricing curve ensures that the liquidity trader $\LT$ always trades at the fundamental token value $v$, regardless of the trade size. In contrast to markets with convex bonding curves as described in \citet{LeharParlour2021} or \citet{CapponiJia2021}, there is no price impact on the constant price market. In turn, this implies there is no impermanent loss for liquidity providers following a liquidity trader arrival, and also that no subsequent arbitrage trade is needed to restore prices to the fundamental value. However, even in the absence of price impact, the liquidity trader needs to take into account the liquidity fee difference across the two pools. 

Let $T^\star_L$ and $T^\star_H$ be the equilibrium supply of tokens on liquidity pools $L$ and $H$, respectively. To minimize trading cost, the liquidity trader first submits an order on the low-fee pool. If liquidity on pool $L$ is sufficient to accommodate the demand, that is if $\theta\leq T^\star_L$, then the $\LT$ executes its entire order on $L$. Conversely, if $\theta>T^\star_L$, the liquidity trader exhaust the liquidity supply on $L$ and trades the residual quantity $\theta-T^\star_L$ against liquidity on pool $H$. From equation \eqref{eq:aggliq}, the aggregate liquidity supply is $T^\star_L+T^\star_H=\log^{-1}\left(2\right)$. Since $\theta<\log^{-1}\left(2\right)$, the liquidity trader executes her entire order with probability one and incurs a net cost of $f \times T_L^\star + 1 \times T_H^\star$.
\cp{Where is the gas fee?  How does that work here?} \mz{The implicit assumption is that liquidity traders have a very large private value for $\theta$ units of the asset such that they are willing to pay two gas fees if needed.}

If news occurs and $\LP$s do not withdraw liquidity from the pool, arbitrageurs can trade in the direction on the news to obtain a gross profit of $1~\C$ per token traded (i.e., the size of the news). Concretely, upon good news an arbitrageur deposits $q_{\text{arb},k} v$ units of num\'{e}raire into liquidity pool $k$ and removes $q_{\text{arb},k}$ tokens with a value of $q_{\text{arb},k} \left(v+1\right)$. Further, the arbitrageurs pays the pool fee $f_k$ and the gas fee equal to $\Gamma \diff i$. The net profit from trading $q_{\text{arb},k}$ on liquidity pool $k$ is therefore:
\begin{equation}\label{eq:pi_arb}
    \Pi_\A = q_{\text{arb},k}\left(1-f_k\right)-\Gamma \diff i>0.
\end{equation}
Since the arbitrageur can trade against a mass of liquidity providers and pay an infinitesimal gas price,  $\A$ optimally removes the entire liquidity from pool $L$. However, since the fee on pool $H$ is equal to the size of the news, the arbitrageur never consumes liquidity from pool $H$ for any positive gas fee. The mechanism is similar to the one in \citet{FoucaultMoinasTheissen2007}, where the size of news and the tick size are such that arbitrageurs consume only the liquidity at the best bid or ask. 

\cp{This is worth discussing.  a) Would it make sense to have some sort of inventory costs for arbitrageurs?  This would prevent them from draining one pool completely.  b) Also, why is it important to have no adverse selection on the high fee pool? It would be interesting to have lower, but not no AS.}  \mz{No AS on the high-fee pool is more of a normalization than anything else to simplify the exposition and monitoring choices. Under Christine's notation, it boils down to $\ell<\delta<h$. We can also have $\ell<h<\delta$ (AS on both pools), but I'm not sure if it adds much to consider both cases separately. }

% \begin{ass}\label{ass:gamma}
% \begin{leftbar} \setlength{\parskip}{0ex}
% The gas fee is low enough such that it does not prevent arbitrageurs from trading on any opportunities, that is $\Gamma < 1-f$.
% \end{leftbar}
% \end{ass}

% Assumption \ref{ass:gamma} guarantees that the arbitrageur profit as defined in \eqref{eq:pi_arb} is always positive on liquidity pool $L$, as long as the pool is non-empty. That is, arbitrageurs are willing to trade upon news even if only the lowest-endowment $\LP$ with $\tau_i=\log\left(2\right) \times 1 \diff i$ submits liquidity on pool $L$. Further, since the arbitrageur profit increases in the quantity traded, $\A$ optimally removes the entire liquidity from pool $L$. Finally, since the fee on pool $H$ is equal to the size of the news, the arbitrageur never consumes liquidity from pool $H$ for any positive gas fee. The mechanism is similar to the one in \citet{FoucaultMoinasTheissen2007}, where the size of news and the tick size are such that arbitrageurs consume only the liquidity at the best bid or ask. 

When do liquidity providers withdraw their liquidity? On pool $H$, withdrawing is never optimal since the fee is high enough to deter arbitrageurs which implies adverse selection risk is zero. On pool $L$, liquidity providers with endowment $q_i$ compare the adverse selection cost and the gas fee and withdraw liquidity upon news if and only if
\begin{equation}
    q_i \left(1-f\right)>\Gamma.
\end{equation}
Lemma \ref{lem:t1} summarizes the optimal strategies for all agents at $t=1$.

\begin{lem}\label{lem:t1}
\begin{leftbar} \setlength{\parskip}{0ex}
At $t=1$, the optimal strategies are as follows:
\begin{enumerate}
    \item[(i)] a liquidity trader with a private value shock of size $\theta$ trades $\min\left\{T_L^\star,\theta\right\}$ on pool $L$ and $\max\left\{0,T_L^\star-\theta\right\}$ on pool $H$.
    \item[(ii)] upon news arrival, liquidity providers on pool $L$ pay the gas price and withdraw their liquidity if $\Gamma\leq q_i \left(1-f\right)$. In contrast, liquidity providers on pool $H$ do not attempt to withdraw liquidity upon news.
    \item[(iii)] upon news, arbitrageurs buy (sell) on pool $L$ an amount of tokens equal to the size of the pool. The arbitrageurs does not trade on pool $H$.
\end{enumerate}

\end{leftbar}
\end{lem}

\subsubsection{Liquidity provision at \texorpdfstring{$t=0$}{t=0} \label{sec:liqprov}}

We turn next to the liquidity providers' choice of pool at $t=0$. Let $T_L$ and $T_H$ denote the size of liquidity pools $L$ and $H$, expressed in token units. The expected profit of an $\LP$ with endowment $q_i$ posting liquidity on pool $L$ is
\begin{align}\label{eq:lp_L}
    \pi^\LP_L &= q_i \left(1-\eta\right)\mathbb{E}\left[\min\left\{\frac{\theta}{T_L},1\right\}\right] f  - \eta \min\left\{\Gamma, q_i\left(1-f\right)\right\} \nonumber \\
    &=q_i \left[\left(1-\eta\right)\left(1 - \log 2\frac{T_L}{2}\right) f\right] -\eta \min\left\{\Gamma, q_i\left(1-f\right)\right\},
\end{align}
since
\begin{align}
    \mathbb{E}\left[\min\left\{\frac{\theta}{T_L},1\right\}\right] &= \mathbb{P}\left(\theta\leq T_L\right) \times \mathbb{E}\left[\frac{\theta}{T_L} \mid \theta\leq T_L\right] + \mathbb{P}\left(\theta > T_L\right) \times 1 \nonumber \\
    & = T_L \log 2 \times \frac{1}{2} + \left(1-T_L \log 2\right) = 1 - \log 2\frac{T_L}{2},
\end{align}
where the last equality follows from the fact that $\theta$ is uniformly distributed over $\left[0,\log^{-1} 2\right]$. With probability $1-\eta$, a liquidity trader arrives at $t=1$ and trades $\theta$. If $\theta>T_L$, then the liquidity trader consumes the entire pool and the $\LP$ receives the fee $f$ for each unit of liquidity posted. Conversely, if $\theta\leq T_L$, then the liquidity provider receives a share $\frac{q_i}{T_L}$ of the aggregate fees $\theta f$. With probability $\eta$, news occurs: from Lemma \ref{lem:t1}, the liquidity provider either pays the gas fee $\Gamma$ and withdraws $q_i$ from the pool or does nothing and incurs a loss $q_i\left(1-f\right)$ on the subsequent arbitrage trade.

Alternatively, the $\LP$ can deposit liquidity on pool $H$ and earn expected profit
\begin{align}\label{eq:lp_H}
    \pi^\LP_H &= q_i \left(1-\eta\right) \mathbb{E}\left[\max\left\{0,\frac{\theta-T_L}{T_H}\right\}\right] \nonumber \\
    & = q_i \left(1-\eta\right) \left(1-T_L \log 2\right) \frac{1-T_L \log 2}{2 T_H \log 2},
\end{align}
where the second line follows from explicitly computing the expectation
\begin{align}
    \mathbb{E}\left[\max\left\{0,\frac{\theta-T_L}{T_H}\right\}\right] &= \mathbb{P}\left(\theta\leq T_L\right) \times 0 + \mathbb{P}\left(\theta > T_L\right) \times \frac{\frac{\log^{-1} 2+T_L}{2}-T_L}{T_H} \nonumber \\
    & = \left(1-T_L \log 2\right) \frac{1-T_L \log 2}{2 T_H \log 2}.
\end{align}
If the liquidity trader demand is low enough, that is if $\theta\leq T_L$, then the entire trade is filled on pool $L$ and liquidity providers on $H$ earn nothing. However, if $\theta>T_L$, the residual liquidity demand $\theta-T_L$ is routed to pool $H$ and liquidity providers earn a share proportional to their deposit, i.e., $\frac{q_i}{T_H}$. If news occurs, $\LP$s on $H$ do not incur an adverse selection cost since from Lemma \ref{lem:t1} arbitrageurs do not submit orders to the high-fee pool.


Liquidity providers in the low-fee pool absorb a larger share of the uninformed order flow, since the $\LT$ order is first routed to pool $L$. On the other hand, they face adverse selection costs and may need to pay gas fees $\Gamma$ upon the realization of news to withdraw liquidity. At the same, $\LP$s in the high-fee pool face no adverse selection, receive a larger fee per unit traded, but volume is limited as they only fill the residual demand from uninformed $\LT$s after liquidity on the low-fee pool is exhausted. From equations \eqref{eq:lp_L} and \eqref{eq:lp_H}, liquidity provider $i$ chooses the low-fee pool $L$ if and only if
\begin{equation}\label{eq:cost_comparison}
    \pi^\LP_L>\pi^\LP_H \Longleftrightarrow q_i \frac{\left(1-\eta\right)\left(\left(1-T_L \log 2\right)^2-f T_H \log 2 \left(2-T_L\log 2\right)\right)}{2\log2 T_H} - \eta\min\left\{\Gamma,q_i\left(1-f\right)\right\} > 0.
\end{equation}
A salient implication of equation \eqref{eq:cost_comparison} is that $\LP$s with larger endowments are more likely to choose the low-fee pool, keeping liquidity shares constant. The rationale is that gas fees are a fixed cost, and larger $\LP$s are more likely to achieve economies of scale. The expected fee revenue scales linearly with a liquidity provider's share in the liquidity pool (proportional to $q_i$), better compensating $\LP$s for the gas fee paid upon news arrival at $t=1$. 

We follow \citet{KatzShapiro1985} and conjecture that there exists a marginal liquidity provider $\qmg$ such that all $\LP$s with $q_i>\qmg$ post liquidity on the low-fee pool and all $\LP$s with $q_i\leq \qmg$ choose the high-fee pool.\footnote{We note that there cannot be a ``reversed-sign'' equilibrium, where $\LP$s with $q_i\leq\qmg$ post liquidity on the low-fee pool and all $\LP$s with $q_i>\qmg$ choose the high-fee pool. To understand the rationale, we point out that for an $\LP$ with endowment $\tilde{q}<\qmg$, submitting liquidity to pool $L$ yields a lower expected revenue since
\begin{equation*}
    \pi^\LP_L-\pi^\LP_H=\tilde{q} \frac{\left(1-\eta\right)\left(\left(1-T_L\right)^2-f T_H \left(2-T_L\right)\right)}{2T_H} - \eta\min\left\{\Gamma,q_i\left(1-f\right)\right\} < 0.
\end{equation*}
Therefore, it is optimal for the $\LP$ with endowment $\tilde{q}$ to post liquidity on the high-fee pool, which contradicts the conjectured equilibrium.  Importantly, since each $\LP$ is ``small'' relative to the aggregate mass of liquidity providers, individual deviations do not impact aggregate pool sizes $T_L$ and $T_H$.} The conjectured equilibrium pins down the pool sizes $T_L$ and $T_H$ as a function of the endowment for the marginal $\LP$:
\begin{align}\label{eq:liquidity_levels}
    T_L&=\int_{\qmg}^2 q_i \phi\left(q_i\right) \diff i = \log^{-1}\left(2\right) \left(2 - \qmg\right) \text{ and }\nonumber \\
    T_H&=\int_1^{\qmg}  q_i \phi\left(q_i\right) \diff i = \log^{-1}\left(2\right)\left(\qmg -1\right). 
\end{align}
From equations \eqref{eq:cost_comparison} and \eqref{eq:liquidity_levels} it follows that the expected profit difference between the low- and high-fee pools can be written as a linear decreasing function of the marginal $\LP$'s endowment, that is
\begin{equation}\label{eq:pi_diff}
    \pi^\LP_L-\pi^\LP_H = q_i \left[\frac{1}{2} \left(1-\eta\right) \left(1-\left(1-f\right)\qmg\right)\right] - \eta \min\left\{q_i\left(1-f\right),\Gamma\right\}.
\end{equation}
We search for fulfilled expectation equilibria \citep[following the definition of][]{KatzShapiro1985}, where the beliefs of $\LP$s at $t=0$ about the size of liquidity pools are consistent with the outcome of their choices. We solve \eqref{eq:pi_diff} on the support for $q_i$ -- the interval $\left[1,2\right]$ to obtain the $\LP$ reaction function
\begin{equation}\label{eq:reaction_main}
    \tilde{q}\left(\qmg\right)=\begin{cases}
    1, & \text{ for } \qmg \leq \frac{1-\eta\left(1+2\min\left\{\Gamma,1-f\right\}\right)}{\left(1-f\right)\left(1-\eta\right)}\\
    \frac{2\eta\Gamma}{ \left(1-\eta\right) \left(1-\left(1-f\right)\qmg\right)}, & \text{ for } \qmg \in \left(\frac{1-\eta\left(1+2\min\left\{\Gamma,1-f\right\}\right)}{\left(1-f\right)\left(1-\eta\right)}, \frac{1-\eta\left(1+\Gamma\right)}{\left(1-f\right)\left(1-\eta\right)}\right] \\
    2, & \text{ for } \qmg > \frac{1-\eta\left(1+\Gamma\right)}{\left(1-f\right)\left(1-\eta\right)}.
    \end{cases}
\end{equation}
In any fulfilled expectation equilibrium, the equilibrium endowment of the marginal $\LP$ is a fixed point of equation \eqref{eq:reaction_main}. Figure \ref{fig:reaction} plots the $\LP$ reaction function $\tilde{q}\left(\cdot\right)$ to graphically illustrate equilibrium formation for two parameter choices. Let $q^\star_1$ and $q^\star_2$ be the interior roots of the reaction function \eqref{eq:reaction_main}, that is the solutions of the quadratic form
\begin{equation}
    q-\frac{2\eta\Gamma}{ \left(1-\eta\right) \left(1-\left(1-f\right)q\right)}=0.
\end{equation}
In the top left panel, we illustrate a parameter combination for which are three equilibria, at $\qmg\in\left\{q^\star_1, q^\star_2, 2\right\}$. However, $q^\star_2$ is an unstable equilibrium -- a tipping point \citep[as in][]{Jullien2011} at which small perturbation in beliefs cause the $\LP$s to spiral away from the postulated equilibrium (we refer the reader to the proof of Proposition \ref{prop:equilibria} for a more formal discussion). Consequently, the stable interior equilibrium co-exists with an equilibrium in which all $\LP$s choose pool $H$; this is the case for $f\leq\frac{2}{3}$. The top right panel illustrates a parameter combination for which the stable interior equilibrium coexists with an equilibrium where all $\LP$s provide liquidity on the low-fee pool (for $f>\frac{2\eta}{1+\eta}$).  Finally, the bottom panel illustrates a parameter combination for which there is a unique and stable interior equilibrium at $\qmg=q^\star_1$. 

\begin{figure}[H]
\caption{\label{fig:reaction} Liquidity provider reaction function and equilibria}
\begin{minipage}[t]{1\columnwidth}%
\footnotesize
This figure illustrates equilibrium $\LP$ liquidity pool choices as fixed points of the reaction function $\tilde{q}\left(\qmg\right)=\qmg$. We consider three distinct cases for which a stable interior equilibrium may arise. Stable equilibria are marked with green circles, whereas unstable equilibria are market with magenta squares. Parameter values are $f=0.64$, $G=0.14$, $\eta=0.71$ (top left), $f=0.69$, $G=0.15$, $\eta=0.71$ (top right), $f=0.792$, $G=0.26$, $\eta=0.65$ (bottom).
\end{minipage}

\vspace{0.05in}

\begin{centering}
\includegraphics[width=\textwidth]{Figures/model_reaction_stable.png}
\par\end{centering}

\end{figure}


Proposition \ref{prop:equilibria} establishes conditions under which a fragmented equilibrium exists, wherein both liquidity pools have positive market share. 

\begin{prop}\label{prop:equilibria}
\begin{leftbar} \setlength{\parskip}{0ex}
A stable fragmented equilibrium, in which both liquidity pools have positive market share, exists for $\Gamma\in\left[\underline{\Gamma},\bar{\Gamma}\right)$, where
\begin{align}
    \underline{\Gamma}&=\max\left\{f\frac{1-\eta}{2\eta},\frac{1+\eta(2f-3)}{1-\eta}\right\} \text{ and }     \bar{\Gamma}=\begin{cases} \frac{1-\eta}{8\eta(1-f)} & f \leq 0.75 \\
                           \frac{(2f-1)(1-\eta)}{\eta} & f>0.75 \end{cases}.
\end{align}
The fragmented equilibrium is further unique if $f\in\left[\frac{2}{3},\frac{2\eta}{1+\eta}\right)$ and $\Gamma\in\left[f\frac{1-\eta}{2\eta},\frac{(2f-1)(1-\eta)}{\eta}\right)$. 
In any fragmented equilibrium, the token endowment of the marginal liquidity provider is 
\begin{equation}
    \qmg^\star=\frac{1}{2\left(1-f\right)}-\frac{1}{2\left(1-f\right)}\sqrt{1-\eta\frac{1+8\left(1-f\right)\Gamma}{1-\eta}},
\end{equation}
such that all liquidity providers with $q_i\leq \qmg^\star$ post liquidity on pool $H$, and all liquidity providers with $q_i> \qmg^\star$ post liquidity on pool $L$.
\end{leftbar}    
\end{prop}

Figure \ref{fig:region_gamma} highlights the parameter region where multiple liquidity pools coexist in equilibrium with positive market share.\footnote{We note that the interior equilibrium is not necessarily the unique one. For low fees on pool $L$ ($f\leq\frac{2}{3}$), the interior equilibrium coexists with a corner equilibrium where all traders choose platform $H$. Conversely, for $f>\frac{2\eta}{1+\eta}$, the interior equilibrium coexists with an equilibrium where all traders choose platform $L$.} In particular, an interior equilibrium for which both the $L$ and $H$ pool attract a positive market share emerges for moderate gas fee $\Gamma$ and a small enough difference between liquidity fees on the two pools (i.e., a large $f$). For low values of the gas fee ($\Gamma\leq\underline{\Gamma}$), managing liquidity is cheap: competition effects are strong and all $\LP$s post liquidity on the low-fee pool. For high values of the gas fee ($\Gamma>\bar{\Gamma}$), withdrawing liquidity upon the realization of news is prohibitively expensive and $\LP$s cluster on the high-fee pool where they are protected from adverse selection. For very large gas fees $\Gamma>2\left(1-f\right)$, no $\LP$ optimally reacts upon news -- in this case, multiple single-pool equilibria may emerge where liquidity either clusters on pool $L$ or on pool $H$. 

\begin{cor}\label{cor:monitoring}
\begin{leftbar} \setlength{\parskip}{0ex}
In any interior equilibrium, \emph{all} liquidity providers on $L$ withdraw liquidity upon news.
\end{leftbar}  
\end{cor}

Corollary \ref{cor:monitoring} establishes that there are no $\LP$s in a fragmented equilibrium that do not actively manage liquidity. All low-endowment $\LP$s for whom reacting upon news is not profitable provide liquidity on platform $H$. In contrast, on single-pool equilibria and for $\Gamma>1-f$, only a fraction of liquidity providers withdraw liquidity upon news. Empirically, we would expect a higher share of $\LP$s actively managing liquidity on pool $L$ when multiple pools co-exist in equilibrium than when all trading concentrates on pool $L$.

\begin{figure}[H]
\caption{\label{fig:region_gamma} Parameter regions for which a two-pool equilibrium exists}
\begin{minipage}[t]{1\columnwidth}%
\footnotesize
This figure illustrates the parameter regions for which a fragmented stable equilibrium emerges, in which both pools attract positive market share. The top panel focuses on the case where $\eta=0.65$. We further highlight (in red) the region for which the equilibrium is unique. In the bottom panel, we plot fragmented equilibrium regions for multiple values of $\eta$.
\end{minipage}

\vspace{0.05in}

\begin{centering}
\includegraphics[width=\textwidth]{Figures/region_interior.png}
\par\end{centering}

\end{figure}





% \begin{prop}\label{prop:equilibria}
% \begin{leftbar} \setlength{\parskip}{0ex}
% For ease of notation, we define and tabulate below three gas fee thresholds $\bar{\Gamma}_k$, $k\in\left\{1,2,3\right\}$.

% \begin{center}
%     \begin{tabular}{ccc}
%     \toprule
%     $\bar{\Gamma}_1$ & $\bar{\Gamma}_2$ & $\bar{\Gamma}_3$ \\
%     \cmidrule{1-3}
%     $f\frac{1-\eta}{2\eta}$     &  $\frac{\left(2f-1\right)\left(1-\eta\right)}{\eta}$ & $\frac{1-\eta}{8\left(1-f\right)\eta}$\\
%     \bottomrule
%     \end{tabular}
% \end{center}

% It follows there are has either one, two, or three stable fulfilled expectation equilibria at $t=0$, corresponding to the following $\LP$ liquidity pool choices:
% \begin{enumerate}
%     \item[(i)] An interior equilibrium with marginal $\LP$ characterized by endowment $\qmg^\star=q^\star_1$, such that all $\LP$s with endowment $q>q^\star_1$ add liquidity to the low-fee pool and the rest choose the high-fee pool. The equilibrium emerges for $f\in\left[\frac{1}{2},\frac{3}{4}\right)$ and $\Gamma\in\left(\bar{\Gamma}_1, \bar{\Gamma}_3\right]$ and $f>\frac{3}{4}$ and $\Gamma\in\left(\bar{\Gamma}_1, \bar{\Gamma}_2\right]$. Moreover, the interior equilibrium is unique for $f>\frac{2}{3}$ and $\Gamma\in\left(\bar{\Gamma}_1, \bar{\Gamma}_2\right]$.
%     \item[(ii)] A corner equilibrium where $\qmg^\star=1$, such that all $\LP$s post liquidity on the low-fee pool. The equilibrium emerges for $\Gamma\leq\bar{\Gamma}_1$ and is further unique if $f>\frac{1}{2}$ and $\Gamma\leq\min\left\{\bar{\Gamma}_1,\bar{\Gamma}_2\right\}$.
%     \item[(iii)] A corner equilibrium where $\qmg^\star=2$, such that all $\LP$s post liquidity on the high-fee pool. The equilibrium emerges for $\Gamma>\bar{\Gamma}_2$ and is further unique if $f>\frac{3}{4}$ and $\Gamma>\bar{\Gamma}_2$, $f>\frac{1}{2}$ and $\Gamma>\bar{\Gamma}_3$, or $f\leq\frac{1}{2}$ and $\Gamma>\bar{\Gamma}_1$.
% \end{enumerate}

% \end{leftbar}
% \end{prop}

% Proposition \ref{prop:equilibria} establishes existence conditions for each possible equilibrium. In particular, an interior equilibrium for which both the $L$ and $H$ pool attract a positive market share emerges for moderate gas fee $\Gamma$ and a small enough difference between liquidity fees on the two pools (i.e., a large $f$). The interior equilibrium is unique if the liquidity fees are close enough across the two pools. Figure \ref{fig:regions} highlights the parameter region where multiple liquidity pools coexist with positive market share. 

% The remaining results in Proposition \ref{prop:equilibria} are intuitive: a small gas fee $\Gamma$ reduces the $\LP$s' costs to manage stale liquidity upon news and stimulates competition on the low-fee pool. In other words, the cost of updating liquidity is lower than the opportunity cost of not capturing uninformed trades. In contrast, a large enough $\Gamma$ incentivizes liquidity providers to deposit tokens on the high-fee pool, since managing liquidity on pool $L$ is too costly. 

% \begin{figure}[H]
% \caption{\label{fig:regions} The emergence of two-pool equilibria}
% \begin{minipage}[t]{1\columnwidth}%
% \footnotesize
% This figure illustrates the emergence of two-pool equilibria for different values of the liquidity fee $f$ and gas fee $\Gamma$. We set the probability of informed trading at $\eta=0.85$. We highlight the parameter region for which a two-pool equilibria emerges and is unique (in red) as well as the region for which a two-pool equilibria emerges but is not unique (in blue). 
% \end{minipage}

% \vspace{0.05in}

% \begin{centering}
% \includegraphics[width=0.9\textwidth]{Figures/model_int_eq_region.png}
% \par\end{centering}

% \end{figure}

\subsection{Implications and empirical predictions}

In this section, we zoom in on the properties of the interior equilibrium, that is, the most interesting case featuring segmented liquidity across multiple pools. From Proposition \ref{prop:equilibria}, the only possible interior equilibrium in the liquidity provision game is for a marginal $\LP$ with endowment $\qmg=q_1^\star$.

\begin{pred}\label{pred:clienteles}
\emph{If an interior equilibrium exists where liquidity is segmented across multiple pools, the average liquidity deposit in the low-fee pool is larger than for the high-fee pool.}
\end{pred}

Prediction \ref{pred:clienteles} follows from the discussion in Section \ref{sec:liqprov}. Liquidity providers with large token endowments ($q_i>\qmg$) deposit them in the low-fee pool since they have stronger incentives to pay the gas fee and actively manage the liquidity. Conversely, $\LP$s with lower endowments ($q_i\leq\qmg$) gravitate towards the high-fee pool, accepting a lower trade probability in exchange for reducing adverse selection costs without active liquidity management and paying gas fees.

\begin{pred}\label{pred:updates}
\emph{Liquidity providers on the low-fee pool are more likely to actively manage liquidity.}
\end{pred}
\begin{pred}\label{pred:monitoring_shares}
\emph{Liquidity providers on the low-fee pool are more likely to actively manage liquidity in a fragmented market than in a consolidated market.}
\end{pred}

The two predictions follow from Corollary \ref{cor:monitoring}. In equilibrium, the $\LP$s on the low-fee pool update their liquidity upon news arrival to avoid adverse selection, unlike their counterparts on the high-fee pool. 


\begin{pred}\label{pred:comp_stat_Gamma}
\emph{The liquidity share of the low-fee pool $L$ decreases in the gas fee $\Gamma$.}
\end{pred}
\begin{pred}\label{pred:comp_stat_eta}
\emph{The liquidity share of the low-fee pool $L$ decreases in the probability of informed trading $\eta$.}
\end{pred}

Predictions \ref{pred:comp_stat_Gamma} and \ref{pred:comp_stat_eta} state that the low-fee pool becomes less attractive for liquidity providers if the gas fee increases (higher $\Gamma$) -- making active liquidity management less profitable -- or if the probability of informed trading is higher ($\eta$ increases) which leads to \emph{more frequent} liquidity management. Formally, we can show that $q_1^\star$ increases in both $\Gamma$ and $\eta$ -- leading to a lower value of $T_L^\star$:
\begin{align}
    \frac{\partial q_1^\star}{\partial \Gamma}&=\frac{2 \eta }{\sqrt{(1-\eta ) (\eta  (8 \Gamma  (f-1)-1)+1)}}>0 \text{ and } \nonumber \\
    \frac{\partial q_1^\star}{\partial \eta}&=\frac{2 \Gamma }{(1-\eta) \sqrt{(1-\eta ) (\eta  (8 \Gamma  (f-1)-1)+1)}}.
\end{align}

\begin{pred}\label{pred:trade_volume}
\emph{If an interior equilibrium exists, the trading volume share of the low-fee pool is higher than its liquidity share.}
\end{pred}
The intuition is that $\LP$s on the low-fee pool deposit large token quantities and they absorb a disproportionate amount of incoming trades -- it is possible that $\LP$s on the high-fee pool do not trade at all against incoming orders, despite providing positive liquidity in equilibrium. To formally see the result, we first note that there is no informed trade in equilibrium on either pool. The average $\LT$ trade size on the low-fee pool is
\begin{align}
    \mathbb{E}\left[\min\left\{\theta,T_L^\star\right\}\right]&=\mathbb{P}\left(\theta\leq T_L\right) \mathbb{E}\left[\theta\mid \theta<T_L^\star\right] + \left(1-\mathbb{P}\left(\theta\leq T_L\right)\right) T_L^\star \nonumber \\
    &= T_L^\star\log 2\frac{T_L^\star}{2} + \left(1-T_L^\star\log 2\right) T_L^\star= T_L^\star-\frac{\left(T_L^\star\right)^2}{2}\log 2.
\end{align}
The average $\LT$ trade size on the high-fee pool is
\begin{align}
    \mathbb{E}\left[\max\left\{0,\theta-T_L^\star\right\}\right]& = \left(1-\mathbb{P}\left(\theta\leq T_L\right)\right) \left(\mathbb{E}\left[\theta\mid \theta>T_L^\star\right]-T_L^\star\right)\nonumber \\
    &= \left(1-T_L^\star\log 2\right) \frac{\left(\log^{-1} 2-T_L^\star\right)}{2}=\frac{\log^{-1} 2}{2}-T_L^\star+\frac{\left(T_L^\star\right)^2}{2}\log 2.
\end{align}
We note that the trade share of pool $L$ is equal to $2T_L^\star\log 2-\left(T_L^\star\log 2\right)^2$ which is larger than its liquidity share $T_L^\star\log 2$ since $T_L^\star\log 2<1$. Figure \ref{fig:liqshares} illustrates this result.




\begin{figure}[H]
\caption{\label{fig:liqshares} Liquidity and volume shares}
\begin{minipage}[t]{1\columnwidth}%
\footnotesize
This figure illustrates the relative liquidity and trade volume on the two pools, as a function of the gas fee $\Gamma$. Parameters: $\eta=0.36$ and $f=0.8$.
\end{minipage}

\vspace{0.05in}

\begin{centering}
\includegraphics[width=0.9\textwidth]{Figures/model_compstatics.png}
\par\end{centering}

\end{figure}


\begin{pred}\label{pred:liq_shares}
\emph{The low-fee pool is larger than the high-fee pool (in terms of aggregate deposits) only if the gas fee is low enough, that is if}
\begin{equation}
    \Gamma < \Gamma^\star \equiv \frac{3 (3 f-1) (1-\eta)}{8 \eta }
\end{equation}
\end{pred}

From equation \eqref{eq:liquidity_levels}, if the marginal $\LP$ has endowment $q_1^\star$, then the equilibrium sizes of the two liquidity pools are, respectively,
\begin{align}
    T_L^\star&=\log^{-1}\left(2\right)\left[2- \frac{1}{2\left(1-f\right)} \left(1- \sqrt{1-\eta\frac{1+8\left(1-f\right)\Gamma}{1-\eta}}\right)\right] \text{ and } \nonumber \\
    T_H^\star&=\log^{-1}\left(2\right)\left[\frac{1}{2\left(1-f\right)} \left(1- \sqrt{1-\eta\frac{1+8\left(1-f\right)\Gamma}{1-\eta}}\right)-1\right].
\end{align}


Prediction \ref{pred:liq_shares} translates to stating that $T_L^\star>T_H^\star$, or equivalently to $q_1^\star\leq \frac{3}{2}$, where the latter inequality is true for any $\Gamma\leq\Gamma^\star$. Therefore, even though the low-fee pool attracts the $\LP$s with large token endowments, it is not necessarily the largest pool if the gas fee exceeds a certain threshold. 






==> Old/model_v3.tex <==

\subsection{Model primitives}

\paragraph{Assets.} Consider a three-period economy, where time is indexed by $t\in\left\{0,1,2\right\}$. There are two traded cryptocurrencies, labelled $\T$ and $\C$; we refer to asset $\T$ as the ``token'', whereas asset $\C$ stands in as a numeraire. At $t=2$, the risky token $\T$ has a stochastic terminal value $\tilde{v}~\C$. At the start of the game, the expected token value is $\mathbb{E}_0 \tilde{v}=v>1$. 

% \cp{Why dividend as opposed to terminal value?  Why is one token riskless?  Why isn't this just a relative price?}

% The asset $\C$ stands in for cryptocurrencies typically used as num\'{e}raire on decentralized exchanges -- for example Ether (the native currency of the Ethereum blockchain) or stablecoins such as Tether or USD~Coin. The num\'{e}raire pays a risk-free rate of return $r$, which we normalize to zero without loss of generality.

% \cp{I think the para above can just be nuked.}

\paragraph{Trading environment.} The risky token is traded on two liquidity pools that charge liquidity fees proportional to the value of the trade. We label the pools $L$ (standing for a low-fee pool) and $H$ (that is, a high-fee pool). 
%\cp{The type of fee has not been defined, i.e., fixed, proportional.} 
The asset quantities in each pool $k\in\left\{L,K\right\}$ must satisfy at all times the following linear bonding curve:
\begin{equation}\label{eq:bond_curve}
    v \T_k + \C_k = \text{constant}.
\end{equation}
The bonding curve \eqref{eq:bond_curve} implies that the token price is constant and equal to $v$ units of the num\'{e}raire, since $-\frac{\diff T}{\diff C}=v$.\footnote{In practice, most decentralized exchanges use convex bonding curve, for example constant product pricing. While the choice of bonding curve is of first order importance for liquidity demanders who need to split trades to optimize price impact, we argue it is less important for liquidity suppliers. For tractability, we assume a linear bonding curve which implies that liquidity traders only care about pool fees -- the focus of our model. In a richer model with convex pricing, we would expect to see relatively more fragmentation since minimzing price impact might require further splitting trades.} To fix intuition behind the mechanics of the market, suppose a trader wishes to buy $t$ units of the token. This reduces the token amount in the pool to $\T_k-t$. In return, the trader needs to add $\Delta$ units of the num\'{e}raire, where $\Delta$ is such that the new asset quantities remain on the bonding curve, that is:
\begin{equation}
    v \left(\T_k-t\right) + \left(\C_k+\Delta\right) = v \T_k + \C_k,
\end{equation}
which is equivalent to having $\Delta = v t$. The slope of the bonding curve is equal to the expected value of the asset to ensure there are no arbitrage opportunities at the start of the game. 

The two liquidity pools charge different fees on liquidity-removing trades. Fees are expressed in units of the num\'{e}raire $\C$ and are distributed to all liquidity providers in a given pool, proportional to the amount of liquidity provided.  The low-fee pool $L$ charges a fee of $\ell~\C$ and the high-fee pool $H$ charges a fee of $h~\C$ per token traded, where $\ell<h$. For example, to purchase $t$ units of the token on the $L$ pool, the total cost of an investor is $t\left(v+\ell\right)$.

% \cp{I'm not sure that the notation is fabulous. Maybe $\ell$ and $h$. Everything will be in terms of $h-\ell$.} \mz{Agreed. What's really key here is the relation between the fees and the size of news.}

\paragraph{Events.} At $t=1$, two types of exogenous events can occur. With probability $\eta<1$, the common value of the token changes to $v+\delta$ (good news) or to $v-\delta$ (bad news); good and bad news are equally likely. If news does not occur, that is with probability $\left(1-\eta\right)$, a liquidity trader ($\LT$) receives a private value shock and needs to trade $\tilde{\theta}$ units of the token, where $\tilde{\theta}\sim\text{Uniform}\left[0,\Theta\right]$. The liquidity trader is equally likely to buy or sell the token. We assume the $\LT$s private value is large enough to cover transaction costs on either liquidity pool.

% \cp{This upper bound is ugly. How far can one go with a generic upper bound....The uniform is already quite specific. Also, up and down by an amount $\delta$?.  Maybe for each parameterization find the private value assumption needed.} \mz{The upper bound was chosen to match the aggregate liquidity provision (in an earlier version I had both the upper bound \& aggregate liquidity normalized to one). If $\theta$ can be higher than that, it weakens competition between $\LP$s: if everyone's liquidity executed for sure, then $\LP$s prefer the high-fee pool. So I set the upper bound such that there's always someone who does not get executed.}

\paragraph{Liquidity providers and arbitrageurs.} In addition to liquidity traders, the token is traded by two types of agents: risk-neutral liquidity providers ($\LP$) and arbitrageurs ($\A$). There is a continuum of liquidity providers indexed by $i$, endowed with heterogeneous amounts of the token $T$. Liquidity provider $i$ is endowed with $q_i$ units of the token. Following \citet{KhomynPutninsZoican2022}, we assume that $q_i$ is distributed with density
\begin{equation}\label{eq:density}
    \phi\left(q\right)=\log^{-1}\left(2\right)\frac{1}{q},\text{ for }q\in\left[1,2\right].
\end{equation}
The choice of density ensures that the aggregate token endowment of liquidity providers $\T_\text{agg}$ is normalized to a constant, since
\begin{equation}\label{eq:aggliq}
    \T_\text{agg}=\int_1^2 q_i \phi\left(q_i\right)\diff q_i = \log^{-1} \left(2\right).
\end{equation}
Further, the density is chosen to match key features of the empirical distribution of $\LP$s: there are many low-endowment liquidity providers (e.g., retail traders) and a long tail of high-capital investors who provide liquidity to decentralized exchange -- for example, quantitative institutional investors. Figure \ref{fig:distribution} illustrates the theoretical distribution of $\LP$s endowments.


% \cp{Does something like a pareto distribution work or have their liquidity supply as 1+ RV drawn from an exponential?}
% \mz{I am not sure. The point here was to have market shares that are linear in the marginal trader's $\qmg$ -- otherwise we don't get a closed form when solving for the fulfilled expectation equilibrium. To have linear market shares, I need $q_i\phi(q_i)$ to be a constant, which means $\phi(\cdot)$ needs to be proportional to $\frac{1}{q_i}$. The ugly log constant term just ensures the density integrates out to one.

% \textbf{Update 9/Aug}: The distribution we currently have is a log-uniform (or reciprocal), which implies the $\log\left(q_i\right)$ is uniformly distributed on $\left[0,\log(2)\right]$. Equivalently, $q_i\sim e^{\text{Uniform}\left[0,\log(2)\right]}$

% We can perhaps generalize this to $q_i\sim e^{\text{Uniform}\left[0,Q\right]}$. To still get closed form solutions though in the pool choice step, we need that the aggregate liquidity is equal to the maximum liquidity trader size. This implies that the LT order size should be uniformly distributed over $\left[0,\frac{e^Q-1}{Q}\right]$.   

% }

\begin{figure}[H]
\caption{\label{fig:distribution} Liquidity provider endowment (scaled) $q_i$}
\begin{minipage}[t]{1\columnwidth}%
\footnotesize
This figure illustrates the probability density of liquidity provider token endowments, $\phi\left(\cdot\right)$, as defined in equation \eqref{eq:density}.
\end{minipage}

\vspace{0.05in}

\begin{centering}
\includegraphics[width=0.8\textwidth]{Figures/model_density.png}
\par\end{centering}

\end{figure}

The arbitrageurs $\A$ are risk-neutral speculative traders with zero private value for the token. Upon observing a common value innovation, arbitrageurs can submit a trade against liquidity providers if (i) liquidity is being offered at a stale price and (ii) it is profitable to take liquidity after taking into account gas costs and pool fees.

% \cp{Every arbitrageur since the 1980s has been risk neutral and profit maximizing.  I don't think this warrants citations. }

\paragraph{Gas fee (order execution cost).} Orders submitted at $t=1$ to trade against pool liquidity or to withdraw existing liquidity incur a fixed execution cost $\Gamma>0$. The execution cost can be interpreted as the gas price on the Ethereum blockchain as in \citet{CapponiJia2021}. In contrast to \citet{CapponiJia2021}, we assume traders on the decentralized exchanges are price takers on the gas market and their orders do not impact the gas cost. A natural interpretation is that message volume at any time in a particular asset pair traded on decentralized exchanges is small relative to the aggregate transaction flow on the entire blockchain.

Gas fees on decentralized exchanges differ from trading fees on traditional exchanges in a number of ways. First, they are not set by individual exchanges to compete with each other, but are a common transaction cost \emph{across} exchanges. Second, they are levied on a per-order rather than per-share basis: this implies economies of scale for larger orders. Third, there is significant time variation in gas fees which allows us to better empirically identify the impact of transaction costs on liquidity pool market shares.

\paragraph{Timing.} Figure \ref{fig:timing} summarizes the sequence of events at each time $t$. At $t=0$, liquidity providers arrive at the market and choose to deposit their tokens (and corresponding num\'{e}raire) on either the high- or low-fee liquidity pool. At $t=1$, an exogenous trigger event happens: either news, that is a common value innovation, or a private value shock to liquidity traders. With probability $1-\eta$, a liquidity trader arrives and trades a random quantity $\tilde{\theta}$. Conversely, with probability $\eta$, news arrives which moves the asset value to either $v+\delta$ or $v-\delta$. In this case, liquidity providers can act before arbitrageurs with probability $\pi$: that is, they have the option to pay the fixed gas fee $\Gamma$ and withdraw liquidity from the pool to avoid being adversely selected. Following the $\LP$s' choice, arbitrageurs may trade in the direction of the news if profitable to do so. With probability $1-\pi$, however, arbitrageurs can react on news faster than liquidity providers. Finally, at $t=2$ all payoffs are realized. 
\paragraph{Timing.} Figure \ref{fig:timing} summarizes the sequence of events at each time $t$. At $t=0$, liquidity providers arrive at the market and choose to deposit their tokens (and corresponding num\'{e}raire) on either the high- or low-fee liquidity pool. At $t=1$, an exogenous trigger event happens: either news, that is a common value innovation, or a private value shock to liquidity traders. With probability $1-\eta$, a liquidity trader arrives and trades a random quantity $\tilde{\theta}$. Conversely, with probability $\eta$, news arrives which moves the asset value to either $v+\delta$ or $v-\delta$. In this case, liquidity providers can act before arbitrageurs with probability $\pi$: that is, they have the option to pay the fixed gas fee $\Gamma$ and withdraw liquidity from the pool to avoid being adversely selected. Following the $\LP$s' choice, arbitrageurs may trade in the direction of the news if profitable to do so. With probability $1-\pi$, however, arbitrageurs can react on news faster than liquidity providers. Finally, at $t=2$ all payoffs are realized. 

\begin{figure}[H]
\caption{\label{fig:timing} \textbf{Model timing}}

\vspace{0.1in}
\begin{centering}
\includegraphics[width=0.9\textwidth]{Figures/timing_dex_v3.pdf}
\par\end{centering}

\end{figure}

% \cp{Useful to have a variable that captures the extent to which LP can withdraw?  Something like an attention variable. After a news event, they can probabilistically withdraw liquidity if optimal. }

\subsection{Equilibrium \label{sec:eq}}

We solve the game by backward induction. First, we discuss the optimal strategy of arbitrageurs and liquidity traders at $t=1$, taking equilibrium liquidity provision as given. Next, we solve for the optimal liquidity pool choices of $\LP$s at $t=0$. 

\subsubsection{Optimal strategies at \texorpdfstring{$t=1$}{t=1}}

The linear pricing curve ensures that the liquidity trader $\LT$ always trades at the fundamental token value $v$, regardless of the trade size. In contrast to markets with convex bonding curves as described in \citet{LeharParlour2021} or \citet{CapponiJia2021}, there is no price impact on the constant price market. In turn, this implies there is no impermanent loss for liquidity providers following a liquidity trader arrival, and also that no subsequent arbitrage trade is needed to restore prices to the fundamental value. However, even in the absence of price impact, the liquidity trader needs to take into account the liquidity fee difference across the two pools. 

Let $T^\star_L$ and $T^\star_H$ be the equilibrium supply of tokens on liquidity pools $L$ and $H$, respectively. To minimize trading cost, the liquidity trader first submits an order on the low-fee pool. If liquidity on pool $L$ is sufficient to accommodate the demand, that is if $\theta\leq T^\star_L$, then the $\LT$ executes its entire order on $L$. Conversely, if $\theta>T^\star_L$, the liquidity trader exhaust the liquidity supply on $L$ and trades the residual quantity $\max\left\{\theta-T^\star_L,T^\star_H\right\}$ against liquidity on pool $H$. Therefore, the liquidity trader incurs a net cost of $\ell \times T_L^\star + h \times \max\left\{\theta-T^\star_L,T^\star_H\right\}$. We assume that liquidity traders have a high enough private value for the $\theta$ units of token such that they are always willing to pay liquidity and gas fees to execute their trade.

% \cp{Where is the gas fee?  How does that work here?} \mz{The implicit assumption is that liquidity traders have a very large private value for $\theta$ units of the asset such that they are willing to pay two gas fees if needed.}

If news occurs and $\LP$s do not withdraw liquidity from the pool, arbitrageurs can trade in the direction on the news to obtain a gross profit of $\delta~\C$ per token traded (i.e., the size of the news). Concretely, upon good news an arbitrageur deposits $q_{\text{arb},k} v$ units of num\'{e}raire into liquidity pool $k$ and removes $q_{\text{arb},k}$ tokens with a value of $q_{\text{arb},k} \left(v+\delta\right)$. Further, the arbitrageurs pays the pool liquidity fee $f_k\in\left\{\ell,h\right\}$ and the gas price equal to $\Gamma \diff i$. The net profit from trading $q_{\text{arb},k}$ on liquidity pool $k$ is therefore:
\begin{equation}\label{eq:pi_arb}
    \Pi_\A = q_{\text{arb},k}\left(\delta-f_k\right)-\Gamma \diff i>0.
\end{equation}
In the spirit of \citet{FoucaultMoinasTheissen2007}, where the size of news and the tick size are such that arbitrageurs consume only the liquidity at the best bid or ask, we focus on the case in which $\ell<\delta\leq h$. Since the arbitrageur can profitably trade against a mass of liquidity providers and pay an infinitesimal gas price,  $\A$ optimally removes the entire liquidity from pool $L$. However, since the fee on pool $H$ at least equal to the size of the news, the arbitrageur never consumes liquidity from pool $H$ for any positive gas fee. 

% \cp{This is worth discussing.  a) Would it make sense to have some sort of inventory costs for arbitrageurs?  This would prevent them from draining one pool completely.  b) Also, why is it important to have no adverse selection on the high fee pool? It would be interesting to have lower, but not no AS.}  \mz{No AS on the high-fee pool is more of a normalization than anything else to simplify the exposition and monitoring choices. Under Christine's notation, it boils down to $\ell<\delta<h$. We can also have $\ell<h<\delta$ (AS on both pools), but I'm not sure if it adds much to consider both cases separately. }

% \begin{ass}\label{ass:gamma}
% \begin{leftbar} \setlength{\parskip}{0ex}
% The gas fee is low enough such that it does not prevent arbitrageurs from trading on any opportunities, that is $\Gamma < 1-f$.
% \end{leftbar}
% \end{ass}

% Assumption \ref{ass:gamma} guarantees that the arbitrageur profit as defined in \eqref{eq:pi_arb} is always positive on liquidity pool $L$, as long as the pool is non-empty. That is, arbitrageurs are willing to trade upon news even if only the lowest-endowment $\LP$ with $\tau_i=\log\left(2\right) \times 1 \diff i$ submits liquidity on pool $L$. Further, since the arbitrageur profit increases in the quantity traded, $\A$ optimally removes the entire liquidity from pool $L$. Finally, since the fee on pool $H$ is equal to the size of the news, the arbitrageur never consumes liquidity from pool $H$ for any positive gas fee. The mechanism is similar to the one in \citet{FoucaultMoinasTheissen2007}, where the size of news and the tick size are such that arbitrageurs consume only the liquidity at the best bid or ask. 

When do liquidity providers withdraw their liquidity? On pool $H$, withdrawing is never optimal since the fee is high enough to deter arbitrageurs which implies adverse selection risk is zero. On pool $L$, liquidity providers with endowment $q_i$ compare the adverse selection cost and the gas fee and withdraw liquidity upon news if and only if
\begin{equation}
    q_i \left(\delta-\ell\right)>\Gamma.
\end{equation}
Lemma \ref{lem:t1} summarizes the optimal strategies for all agents at $t=1$.

\begin{lem}\label{lem:t1}
\begin{leftbar} \setlength{\parskip}{0ex}
At $t=1$, the optimal strategies are as follows:
\begin{enumerate}
    \item[(i)] a liquidity trader with a private value shock of size $\theta$ trades $\min\left\{T_L^\star,\theta\right\}$ on pool $L$ and $\max\left\{0,\min\left\{\theta-T_L^\star,T_H^\star\right\}\right\}$ on pool $H$.
    \item[(ii)] upon news arrival, liquidity providers on pool $L$ pay the gas price and withdraw their liquidity if $\Gamma\leq q_i \left(\delta-\ell\right)$. In contrast, liquidity providers on pool $H$ do not attempt to withdraw liquidity upon news.
    \item[(iii)] upon news, arbitrageurs buy (sell) on pool $L$ an amount of tokens equal to the size of the pool. The arbitrageurs does not trade on pool $H$.
\end{enumerate}

\end{leftbar}
\end{lem}

\subsubsection{Liquidity provision at \texorpdfstring{$t=0$}{t=0} \label{sec:liqprov}}

We turn next to the liquidity providers' choice of pool at $t=0$. Let $T_L$ and $T_H$ denote the size of liquidity pools $L$ and $H$, expressed in token units. The expected profit of an $\LP$ with endowment $q_i$ posting liquidity on pool $L$ is
\begin{align}\label{eq:lp_L}
    \pi^\LP_L &= q_i \left(1-\eta\right)\mathbb{E}\left[\min\left\{\frac{\theta}{T_L},1\right\}\right] \ell  - \eta \left[\pi \min\left\{\Gamma, q_i\left(\delta-\ell\right)\right\}+\left(1-\pi\right)q_i\left(\delta-\ell\right)\right] \nonumber \\
    &=q_i \left[\left(1-\eta\right)\left(1 - \frac{T_L}{2\Theta}\right) \ell\right] -\eta \left[\pi \min\left\{\Gamma, q_i\left(\delta-\ell\right)\right\}+\left(1-\pi\right)q_i\left(\delta-\ell\right)\right],
\end{align}
since
\begin{align}
    \mathbb{E}\left[\min\left\{\frac{\theta}{T_L},1\right\}\right] &= \mathbb{P}\left(\theta\leq T_L\right) \times \mathbb{E}\left[\frac{\theta}{T_L} \mid \theta\leq T_L\right] + \mathbb{P}\left(\theta > T_L\right) \times 1 \nonumber \\
    & = \frac{T_L}{\Theta} \times \frac{1}{2} + \left(1-\frac{T_L}{\Theta}\right) = 1 - \frac{T_L}{2\Theta},
\end{align}
where the last equality follows from the fact that $\theta$ is uniformly distributed over $\left[0,\Theta\right]$. With probability $1-\eta$, a liquidity trader arrives at $t=1$ and trades $\theta$. If $\theta>T_L$, then the liquidity trader consumes the entire pool and the $\LP$ receives the fee $\ell$ for each unit of liquidity posted. Conversely, if $\theta\leq T_L$, then the liquidity provider receives a share $\frac{q_i}{T_L}$ of the aggregate fees $\theta \ell$. With probability $\eta$, news occurs: from Lemma \ref{lem:t1}, if a liquidity providers reacts before the arbitrageur (with probability $\pi$) she either pays the gas fee $\Gamma$ and withdraws $q_i$ from the pool or does nothing and incurs a loss $q_i\left(\delta-\ell\right)$ on the subsequent arbitrage trade.

Alternatively, the $\LP$ can deposit liquidity on pool $H$ and earn expected profit
\begin{align}\label{eq:lp_H}
    \pi^\LP_H &= q_i \left(1-\eta\right) \mathbb{E}\left[\max\left\{0,\frac{\theta-T_L}{T_H}\right\}\right] h  \nonumber \\
    & = q_i \left(1-\eta\right)\left(1-\frac{T_L}{\Theta}\right) \frac{\Theta-T_L}{2 T_H} h,
\end{align}
where the second line follows from explicitly computing the expectation
\begin{align}
    \mathbb{E}\left[\max\left\{0,\frac{\theta-T_L}{T_H}\right\}\right] &= \mathbb{P}\left(\theta\leq T_L\right) \times 0 + \mathbb{P}\left(\theta > T_L\right) \times \frac{\frac{\Theta+T_L}{2}-T_L}{T_H} \nonumber \\
    & = \left(1-\frac{T_L}{\Theta}\right) \frac{\Theta-T_L}{2 T_H}.
\end{align}
If the liquidity trader demand is low enough, that is if $\theta\leq T_L$, then the entire trade is filled on pool $L$ and liquidity providers on $H$ earn nothing. However, if $\theta>T_L$, the residual liquidity demand $\theta-T_L$ is routed to pool $H$ and liquidity providers earn a share proportional to their deposit, i.e., $\frac{q_i}{T_H}$. If news occurs, $\LP$s on $H$ do not incur an adverse selection cost since from Lemma \ref{lem:t1} arbitrageurs do not submit orders to the high-fee pool.


Liquidity providers in the low-fee pool absorb a larger share of the uninformed order flow, since the $\LT$ order is first routed to pool $L$. On the other hand, they face adverse selection costs and may need to pay gas fees $\Gamma$ upon the realization of news to withdraw liquidity. At the same, $\LP$s in the high-fee pool face no adverse selection, receive a larger fee per unit traded, but volume is limited as they only fill the residual demand from uninformed $\LT$s after liquidity on the low-fee pool is exhausted. From equations \eqref{eq:lp_L} and \eqref{eq:lp_H}, liquidity provider $i$ chooses the low-fee pool $L$ if and only if
\begin{align}\label{eq:cost_comparison}
    \pi^\LP_L>\pi^\LP_H \Longleftrightarrow & q_i \left[\left(1-\eta\right) \frac{\ell T_H\left(2\Theta-T_L\right)-h \left(\Theta-T_L\right)^2}{2\Theta T_H}+\eta\left(1-\pi\right)\left(\ell-\delta\right)\right]- \nonumber \\
    &- \eta\pi\min\left\{\Gamma,q_i\left(1-f\right)\right\} > 0.
\end{align}
A salient implication of equation \eqref{eq:cost_comparison} is that $\LP$s with larger endowments are more likely to choose the low-fee pool, keeping liquidity shares constant. The rationale is that gas fees are a fixed cost, and larger $\LP$s are more likely to achieve economies of scale. The expected fee revenue scales linearly with a liquidity provider's share in the liquidity pool (proportional to $q_i$), better compensating $\LP$s for the gas fee paid upon news arrival at $t=1$. 

We follow \citet{KatzShapiro1985} and conjecture that there exists a marginal liquidity provider $\qmg$ such that all $\LP$s with $q_i>\qmg$ post liquidity on the low-fee pool and all $\LP$s with $q_i\leq \qmg$ choose the high-fee pool.\footnote{We note that there cannot be a ``reversed-sign'' equilibrium, where $\LP$s with $q_i\leq\qmg$ post liquidity on the low-fee pool and all $\LP$s with $q_i>\qmg$ choose the high-fee pool. To understand the rationale, we point out that for an $\LP$ with endowment $\tilde{q}<\qmg$, submitting liquidity to pool $L$ yields a lower expected revenue since
\begin{align*}
    \pi^\LP_L>\pi^\LP_H \Longleftrightarrow & \tilde{q} \left[\left(1-\eta\right) \frac{\ell T_H\left(2\Theta-T_L\right)-h \left(\Theta-T_L\right)^2}{2\Theta T_H}+\eta\left(1-\pi\right)\left(\ell-\delta\right)\right]- \nonumber \\
    &- \eta\pi\min\left\{\Gamma,\tilde{q}\left(1-f\right)\right\} <0.
\end{align*}
Therefore, it is optimal for the $\LP$ with endowment $\tilde{q}$ to post liquidity on the high-fee pool, which contradicts the conjectured equilibrium.  Importantly, since each $\LP$ is ``small'' relative to the aggregate mass of liquidity providers, individual deviations do not impact aggregate pool sizes $T_L$ and $T_H$.} The conjectured equilibrium pins down the pool sizes $T_L$ and $T_H$ as a function of the endowment for the marginal $\LP$:
\begin{align}\label{eq:liquidity_levels}
    T_L&=\int_{\qmg}^2 q_i \phi\left(q_i\right) \diff i = \log^{-1}\left(2\right) \left(2 - \qmg\right) \text{ and }\nonumber \\
    T_H&=\int_1^{\qmg}  q_i \phi\left(q_i\right) \diff i = \log^{-1}\left(2\right)\left(\qmg -1\right). 
\end{align}
From equations \eqref{eq:cost_comparison} and \eqref{eq:liquidity_levels} it follows that the expected profit difference between the low- and high-fee pools can be written as a linear decreasing function of the marginal $\LP$'s endowment, that is
\begin{equation}\label{eq:pi_diff}
    \pi^\LP_L-\pi^\LP_H = q_i \left[\frac{1}{2} \left(1-\eta\right) \left(1-\left(1-f\right)\qmg\right)\right] - \eta \min\left\{q_i\left(1-f\right),\Gamma\right\}.
\end{equation}
We search for fulfilled expectation equilibria \citep[following the definition of][]{KatzShapiro1985}, where the beliefs of $\LP$s at $t=0$ about the size of liquidity pools are consistent with the outcome of their choices. We solve \eqref{eq:pi_diff} on the support for $q_i$ -- the interval $\left[1,2\right]$ to obtain the $\LP$ reaction function
\begin{equation}\label{eq:reaction_main}
    \tilde{q}\left(\qmg\right)=\begin{cases}
    1, & \text{ for } \qmg \leq \frac{1-\eta\left(1+2\min\left\{\Gamma,1-f\right\}\right)}{\left(1-f\right)\left(1-\eta\right)}\\
    \frac{2\eta\Gamma}{ \left(1-\eta\right) \left(1-\left(1-f\right)\qmg\right)}, & \text{ for } \qmg \in \left(\frac{1-\eta\left(1+2\min\left\{\Gamma,1-f\right\}\right)}{\left(1-f\right)\left(1-\eta\right)}, \frac{1-\eta\left(1+\Gamma\right)}{\left(1-f\right)\left(1-\eta\right)}\right] \\
    2, & \text{ for } \qmg > \frac{1-\eta\left(1+\Gamma\right)}{\left(1-f\right)\left(1-\eta\right)}.
    \end{cases}
\end{equation}
In any fulfilled expectation equilibrium, the equilibrium endowment of the marginal $\LP$ is a fixed point of equation \eqref{eq:reaction_main}. Figure \ref{fig:reaction} plots the $\LP$ reaction function $\tilde{q}\left(\cdot\right)$ to graphically illustrate equilibrium formation for two parameter choices. Let $q^\star_1$ and $q^\star_2$ be the interior roots of the reaction function \eqref{eq:reaction_main}, that is the solutions of the quadratic form
\begin{equation}
    q-\frac{2\eta\Gamma}{ \left(1-\eta\right) \left(1-\left(1-f\right)q\right)}=0.
\end{equation}
In the top left panel, we illustrate a parameter combination for which are three equilibria, at $\qmg\in\left\{q^\star_1, q^\star_2, 2\right\}$. However, $q^\star_2$ is an unstable equilibrium -- a tipping point \citep[as in][]{Jullien2011} at which small perturbation in beliefs cause the $\LP$s to spiral away from the postulated equilibrium (we refer the reader to the proof of Proposition \ref{prop:equilibria} for a more formal discussion). Consequently, the stable interior equilibrium co-exists with an equilibrium in which all $\LP$s choose pool $H$; this is the case for $f\leq\frac{2}{3}$. The top right panel illustrates a parameter combination for which the stable interior equilibrium coexists with an equilibrium where all $\LP$s provide liquidity on the low-fee pool (for $f>\frac{2\eta}{1+\eta}$).  Finally, the bottom panel illustrates a parameter combination for which there is a unique and stable interior equilibrium at $\qmg=q^\star_1$. 

\begin{figure}[H]
\caption{\label{fig:reaction} Liquidity provider reaction function and equilibria}
\begin{minipage}[t]{1\columnwidth}%
\footnotesize
This figure illustrates equilibrium $\LP$ liquidity pool choices as fixed points of the reaction function $\tilde{q}\left(\qmg\right)=\qmg$. We consider three distinct cases for which a stable interior equilibrium may arise. Stable equilibria are marked with green circles, whereas unstable equilibria are market with magenta squares. Parameter values are $f=0.64$, $G=0.14$, $\eta=0.71$ (top left), $f=0.69$, $G=0.15$, $\eta=0.71$ (top right), $f=0.792$, $G=0.26$, $\eta=0.65$ (bottom).
\end{minipage}

\vspace{0.05in}

\begin{centering}
\includegraphics[width=\textwidth]{Figures/model_reaction_stable.png}
\par\end{centering}

\end{figure}


Proposition \ref{prop:equilibria} establishes conditions under which a fragmented equilibrium exists, wherein both liquidity pools have positive market share. 

\begin{prop}\label{prop:equilibria}
\begin{leftbar} \setlength{\parskip}{0ex}
A stable fragmented equilibrium, in which both liquidity pools have positive market share, exists for $\Gamma\in\left[\underline{\Gamma},\bar{\Gamma}\right)$, where
\begin{align}
    \underline{\Gamma}&=\max\left\{f\frac{1-\eta}{2\eta},\frac{1+\eta(2f-3)}{1-\eta}\right\} \text{ and }     \bar{\Gamma}=\begin{cases} \frac{1-\eta}{8\eta(1-f)} & f \leq 0.75 \\
                           \frac{(2f-1)(1-\eta)}{\eta} & f>0.75 \end{cases}.
\end{align}
The fragmented equilibrium is further unique if $f\in\left[\frac{2}{3},\frac{2\eta}{1+\eta}\right)$ and $\Gamma\in\left[f\frac{1-\eta}{2\eta},\frac{(2f-1)(1-\eta)}{\eta}\right)$. 
In any fragmented equilibrium, the token endowment of the marginal liquidity provider is 
\begin{equation}
    \qmg^\star=\frac{1}{2\left(1-f\right)}-\frac{1}{2\left(1-f\right)}\sqrt{1-\eta\frac{1+8\left(1-f\right)\Gamma}{1-\eta}},
\end{equation}
such that all liquidity providers with $q_i\leq \qmg^\star$ post liquidity on pool $H$, and all liquidity providers with $q_i> \qmg^\star$ post liquidity on pool $L$.
\end{leftbar}    
\end{prop}

Figure \ref{fig:region_gamma} highlights the parameter region where multiple liquidity pools coexist in equilibrium with positive market share.\footnote{We note that the interior equilibrium is not necessarily the unique one. For low fees on pool $L$ ($f\leq\frac{2}{3}$), the interior equilibrium coexists with a corner equilibrium where all traders choose platform $H$. Conversely, for $f>\frac{2\eta}{1+\eta}$, the interior equilibrium coexists with an equilibrium where all traders choose platform $L$.} In particular, an interior equilibrium for which both the $L$ and $H$ pool attract a positive market share emerges for moderate gas fee $\Gamma$ and a small enough difference between liquidity fees on the two pools (i.e., a large $f$). For low values of the gas fee ($\Gamma\leq\underline{\Gamma}$), managing liquidity is cheap: competition effects are strong and all $\LP$s post liquidity on the low-fee pool. For high values of the gas fee ($\Gamma>\bar{\Gamma}$), withdrawing liquidity upon the realization of news is prohibitively expensive and $\LP$s cluster on the high-fee pool where they are protected from adverse selection. For very large gas fees $\Gamma>2\left(1-f\right)$, no $\LP$ optimally reacts upon news -- in this case, multiple single-pool equilibria may emerge where liquidity either clusters on pool $L$ or on pool $H$. 

\begin{cor}\label{cor:monitoring}
\begin{leftbar} \setlength{\parskip}{0ex}
In any interior equilibrium, \emph{all} liquidity providers on $L$ withdraw liquidity upon news.
\end{leftbar}  
\end{cor}

Corollary \ref{cor:monitoring} establishes that there are no $\LP$s in a fragmented equilibrium that do not actively manage liquidity. All low-endowment $\LP$s for whom reacting upon news is not profitable provide liquidity on platform $H$. In contrast, on single-pool equilibria and for $\Gamma>1-f$, only a fraction of liquidity providers withdraw liquidity upon news. Empirically, we would expect a higher share of $\LP$s actively managing liquidity on pool $L$ when multiple pools co-exist in equilibrium than when all trading concentrates on pool $L$.

\begin{figure}[H]
\caption{\label{fig:region_gamma} Parameter regions for which a two-pool equilibrium exists}
\begin{minipage}[t]{1\columnwidth}%
\footnotesize
This figure illustrates the parameter regions for which a fragmented stable equilibrium emerges, in which both pools attract positive market share. The top panel focuses on the case where $\eta=0.65$. We further highlight (in red) the region for which the equilibrium is unique. In the bottom panel, we plot fragmented equilibrium regions for multiple values of $\eta$.
\end{minipage}

\vspace{0.05in}

\begin{centering}
\includegraphics[width=\textwidth]{Figures/region_interior.png}
\par\end{centering}

\end{figure}





% \begin{prop}\label{prop:equilibria}
% \begin{leftbar} \setlength{\parskip}{0ex}
% For ease of notation, we define and tabulate below three gas fee thresholds $\bar{\Gamma}_k$, $k\in\left\{1,2,3\right\}$.

% \begin{center}
%     \begin{tabular}{ccc}
%     \toprule
%     $\bar{\Gamma}_1$ & $\bar{\Gamma}_2$ & $\bar{\Gamma}_3$ \\
%     \cmidrule{1-3}
%     $f\frac{1-\eta}{2\eta}$     &  $\frac{\left(2f-1\right)\left(1-\eta\right)}{\eta}$ & $\frac{1-\eta}{8\left(1-f\right)\eta}$\\
%     \bottomrule
%     \end{tabular}
% \end{center}

% It follows there are has either one, two, or three stable fulfilled expectation equilibria at $t=0$, corresponding to the following $\LP$ liquidity pool choices:
% \begin{enumerate}
%     \item[(i)] An interior equilibrium with marginal $\LP$ characterized by endowment $\qmg^\star=q^\star_1$, such that all $\LP$s with endowment $q>q^\star_1$ add liquidity to the low-fee pool and the rest choose the high-fee pool. The equilibrium emerges for $f\in\left[\frac{1}{2},\frac{3}{4}\right)$ and $\Gamma\in\left(\bar{\Gamma}_1, \bar{\Gamma}_3\right]$ and $f>\frac{3}{4}$ and $\Gamma\in\left(\bar{\Gamma}_1, \bar{\Gamma}_2\right]$. Moreover, the interior equilibrium is unique for $f>\frac{2}{3}$ and $\Gamma\in\left(\bar{\Gamma}_1, \bar{\Gamma}_2\right]$.
%     \item[(ii)] A corner equilibrium where $\qmg^\star=1$, such that all $\LP$s post liquidity on the low-fee pool. The equilibrium emerges for $\Gamma\leq\bar{\Gamma}_1$ and is further unique if $f>\frac{1}{2}$ and $\Gamma\leq\min\left\{\bar{\Gamma}_1,\bar{\Gamma}_2\right\}$.
%     \item[(iii)] A corner equilibrium where $\qmg^\star=2$, such that all $\LP$s post liquidity on the high-fee pool. The equilibrium emerges for $\Gamma>\bar{\Gamma}_2$ and is further unique if $f>\frac{3}{4}$ and $\Gamma>\bar{\Gamma}_2$, $f>\frac{1}{2}$ and $\Gamma>\bar{\Gamma}_3$, or $f\leq\frac{1}{2}$ and $\Gamma>\bar{\Gamma}_1$.
% \end{enumerate}

% \end{leftbar}
% \end{prop}

% Proposition \ref{prop:equilibria} establishes existence conditions for each possible equilibrium. In particular, an interior equilibrium for which both the $L$ and $H$ pool attract a positive market share emerges for moderate gas fee $\Gamma$ and a small enough difference between liquidity fees on the two pools (i.e., a large $f$). The interior equilibrium is unique if the liquidity fees are close enough across the two pools. Figure \ref{fig:regions} highlights the parameter region where multiple liquidity pools coexist with positive market share. 

% The remaining results in Proposition \ref{prop:equilibria} are intuitive: a small gas fee $\Gamma$ reduces the $\LP$s' costs to manage stale liquidity upon news and stimulates competition on the low-fee pool. In other words, the cost of updating liquidity is lower than the opportunity cost of not capturing uninformed trades. In contrast, a large enough $\Gamma$ incentivizes liquidity providers to deposit tokens on the high-fee pool, since managing liquidity on pool $L$ is too costly. 

% \begin{figure}[H]
% \caption{\label{fig:regions} The emergence of two-pool equilibria}
% \begin{minipage}[t]{1\columnwidth}%
% \footnotesize
% This figure illustrates the emergence of two-pool equilibria for different values of the liquidity fee $f$ and gas fee $\Gamma$. We set the probability of informed trading at $\eta=0.85$. We highlight the parameter region for which a two-pool equilibria emerges and is unique (in red) as well as the region for which a two-pool equilibria emerges but is not unique (in blue). 
% \end{minipage}

% \vspace{0.05in}

% \begin{centering}
% \includegraphics[width=0.9\textwidth]{Figures/model_int_eq_region.png}
% \par\end{centering}

% \end{figure}

\subsection{Implications and empirical predictions}

In this section, we zoom in on the properties of the interior equilibrium, that is, the most interesting case featuring segmented liquidity across multiple pools. From Proposition \ref{prop:equilibria}, the only possible interior equilibrium in the liquidity provision game is for a marginal $\LP$ with endowment $\qmg=q_1^\star$.

\begin{pred}\label{pred:clienteles}
\emph{If an interior equilibrium exists where liquidity is segmented across multiple pools, the average liquidity deposit in the low-fee pool is larger than for the high-fee pool.}
\end{pred}

Prediction \ref{pred:clienteles} follows from the discussion in Section \ref{sec:liqprov}. Liquidity providers with large token endowments ($q_i>\qmg$) deposit them in the low-fee pool since they have stronger incentives to pay the gas fee and actively manage the liquidity. Conversely, $\LP$s with lower endowments ($q_i\leq\qmg$) gravitate towards the high-fee pool, accepting a lower trade probability in exchange for reducing adverse selection costs without active liquidity management and paying gas fees.

\begin{pred}\label{pred:updates}
\emph{Liquidity providers on the low-fee pool are more likely to actively manage liquidity.}
\end{pred}
\begin{pred}\label{pred:monitoring_shares}
\emph{Liquidity providers on the low-fee pool are more likely to actively manage liquidity in a fragmented market than in a consolidated market.}
\end{pred}

The two predictions follow from Corollary \ref{cor:monitoring}. In equilibrium, the $\LP$s on the low-fee pool update their liquidity upon news arrival to avoid adverse selection, unlike their counterparts on the high-fee pool. 


\begin{pred}\label{pred:comp_stat_Gamma}
\emph{The liquidity share of the low-fee pool $L$ decreases in the gas fee $\Gamma$.}
\end{pred}
\begin{pred}\label{pred:comp_stat_eta}
\emph{The liquidity share of the low-fee pool $L$ decreases in the probability of informed trading $\eta$.}
\end{pred}

Predictions \ref{pred:comp_stat_Gamma} and \ref{pred:comp_stat_eta} state that the low-fee pool becomes less attractive for liquidity providers if the gas fee increases (higher $\Gamma$) -- making active liquidity management less profitable -- or if the probability of informed trading is higher ($\eta$ increases) which leads to \emph{more frequent} liquidity management. Formally, we can show that $q_1^\star$ increases in both $\Gamma$ and $\eta$ -- leading to a lower value of $T_L^\star$:
\begin{align}
    \frac{\partial q_1^\star}{\partial \Gamma}&=\frac{2 \eta }{\sqrt{(1-\eta ) (\eta  (8 \Gamma  (f-1)-1)+1)}}>0 \text{ and } \nonumber \\
    \frac{\partial q_1^\star}{\partial \eta}&=\frac{2 \Gamma }{(1-\eta) \sqrt{(1-\eta ) (\eta  (8 \Gamma  (f-1)-1)+1)}}.
\end{align}

\begin{pred}\label{pred:trade_volume}
\emph{If an interior equilibrium exists, the trading volume share of the low-fee pool is higher than its liquidity share.}
\end{pred}
The intuition is that $\LP$s on the low-fee pool deposit large token quantities and they absorb a disproportionate amount of incoming trades -- it is possible that $\LP$s on the high-fee pool do not trade at all against incoming orders, despite providing positive liquidity in equilibrium. To formally see the result, we first note that there is no informed trade in equilibrium on either pool. The average $\LT$ trade size on the low-fee pool is
\begin{align}
    \mathbb{E}\left[\min\left\{\theta,T_L^\star\right\}\right]&=\mathbb{P}\left(\theta\leq T_L\right) \mathbb{E}\left[\theta\mid \theta<T_L^\star\right] + \left(1-\mathbb{P}\left(\theta\leq T_L\right)\right) T_L^\star \nonumber \\
    &= T_L^\star\log 2\frac{T_L^\star}{2} + \left(1-T_L^\star\log 2\right) T_L^\star= T_L^\star-\frac{\left(T_L^\star\right)^2}{2}\log 2.
\end{align}
The average $\LT$ trade size on the high-fee pool is
\begin{align}
    \mathbb{E}\left[\max\left\{0,\theta-T_L^\star\right\}\right]& = \left(1-\mathbb{P}\left(\theta\leq T_L\right)\right) \left(\mathbb{E}\left[\theta\mid \theta>T_L^\star\right]-T_L^\star\right)\nonumber \\
    &= \left(1-T_L^\star\log 2\right) \frac{\left(\log^{-1} 2-T_L^\star\right)}{2}=\frac{\log^{-1} 2}{2}-T_L^\star+\frac{\left(T_L^\star\right)^2}{2}\log 2.
\end{align}
We note that the trade share of pool $L$ is equal to $2T_L^\star\log 2-\left(T_L^\star\log 2\right)^2$ which is larger than its liquidity share $T_L^\star\log 2$ since $T_L^\star\log 2<1$. Figure \ref{fig:liqshares} illustrates this result.




\begin{figure}[H]
\caption{\label{fig:liqshares} Liquidity and volume shares}
\begin{minipage}[t]{1\columnwidth}%
\footnotesize
This figure illustrates the relative liquidity and trade volume on the two pools, as a function of the gas fee $\Gamma$. Parameters: $\eta=0.36$ and $f=0.8$.
\end{minipage}

\vspace{0.05in}

\begin{centering}
\includegraphics[width=0.9\textwidth]{Figures/model_compstatics.png}
\par\end{centering}

\end{figure}


\begin{pred}\label{pred:liq_shares}
\emph{The low-fee pool is larger than the high-fee pool (in terms of aggregate deposits) only if the gas fee is low enough, that is if}
\begin{equation}
    \Gamma < \Gamma^\star \equiv \frac{3 (3 f-1) (1-\eta)}{8 \eta }
\end{equation}
\end{pred}

From equation \eqref{eq:liquidity_levels}, if the marginal $\LP$ has endowment $q_1^\star$, then the equilibrium sizes of the two liquidity pools are, respectively,
\begin{align}
    T_L^\star&=\log^{-1}\left(2\right)\left[2- \frac{1}{2\left(1-f\right)} \left(1- \sqrt{1-\eta\frac{1+8\left(1-f\right)\Gamma}{1-\eta}}\right)\right] \text{ and } \nonumber \\
    T_H^\star&=\log^{-1}\left(2\right)\left[\frac{1}{2\left(1-f\right)} \left(1- \sqrt{1-\eta\frac{1+8\left(1-f\right)\Gamma}{1-\eta}}\right)-1\right].
\end{align}


Prediction \ref{pred:liq_shares} translates to stating that $T_L^\star>T_H^\star$, or equivalently to $q_1^\star\leq \frac{3}{2}$, where the latter inequality is true for any $\Gamma\leq\Gamma^\star$. Therefore, even though the low-fee pool attracts the $\LP$s with large token endowments, it is not necessarily the largest pool if the gas fee exceeds a certain threshold. 






==> Old/proofs.tex <==
\noindent \textbf{\large Proposition \ref{prop:equilibria}}
\begin{proof}

To account for kinks in the reaction function \eqref{eq:reaction_main} -- depending on the fraction of $\LP$s that optimally manage liquidity on platform $L$ -- we separately discuss three parameter regions: $\Gamma\leq 1-f$, $\Gamma\in\left(1-f, 2\left(1-f\right)\right]$, and $\Gamma>2\left(1-f\right)$, respectively.

\subsubsection*{Region \#1: $\Gamma\leq 1-f$}

We start by considering the case that $\Gamma\leq 1-f$: that is, it is optimal for any $\LP$ to react upon news arrival if they post liquidity on pool $L$.First, let $\bar{\Gamma}_1=f\frac{1-\eta}{2\eta}$. If $\Gamma<\bar{\Gamma}_1$, then from equation \eqref{eq:reaction_main} it follows that $\tilde{q}\left(1\right)=1$ and therefore $\qmg=1$ is a fixed point of the reaction function. That is, for $\Gamma<\bar{\Gamma}_1$ there is an equilibrium for which all $\LP$s choose to provide liquidity on the $L$ platform. 

Second, let $\bar{\Gamma}_2=\frac{\left(2f-1\right)\left(1-\eta\right)}{\eta}$. From \eqref{eq:reaction_main}, if $\Gamma\geq \bar{\Gamma}_2$ then $\tilde{q}\left(2\right)=2$, which implies that $\qmg=2$ is a fixed point and there is an equilibrium for which all $\LP$s choose to provide liquidity on the $H$ platform.

Third, we note that among possible interior equilibria, $q_1^\star$ increases in $\Gamma$ and $q_2^\star$ decreases in $\Gamma$. If $f\leq\frac{1}{2}$, then $q_1^\star<1$ and is not a feasible root. However, if $f>\frac{1}{2}$, then $q_1^\star\geq 1$ for $\Gamma\geq\bar{\Gamma}_1$. and $q_1^\star<2$ for $\Gamma<\bar{\Gamma}_2$. Similarly, if $f\leq\frac{1}{2}$, then $q_2^\star<2$ and $q_2^\star<1$ for $\Gamma>\bar{\Gamma}_1$. For $f>\frac{1}{2}$, $q_2^\star\geq 2$ for $\Gamma\leq\bar{\Gamma}_2$. However, for $f>\frac{3}{4}$, $q_2>2$ for all $\Gamma$ so it stops being a feasible equilibrium. Finally, the roots $q_1^\star$ and $q_2^\star$ are real if and only if $\Gamma\leq\bar{\Gamma}_3$ where $\bar{\Gamma}_3=\frac{1-\eta}{8\left(1-f\right)\eta}$. For any $f$ and $\eta$ in $\left[0,1\right] \times \left[0,1\right]$, $\bar{\Gamma}_3\geq \bar{\Gamma}_1$ (with equality for $f=\frac{1}{2}$) and $\bar{\Gamma}_3\geq \bar{\Gamma}_2$ (with equality for $f=\frac{3}{4}$). We analyze all possible cases sequentially.

\paragraph{Case \#1: Low fee on $L$ ($f\leq \frac{1}{2}$).} If $f\leq \frac{1}{2}$, then $\bar{\Gamma}_2\leq 0 < \bar{\Gamma}_1 < \bar{\Gamma}_3$. We distinguish between two potential regions for the gas fee $\Gamma$:
\begin{enumerate}
    \item[(i)] $\Gamma\leq\bar{\Gamma}_1$. For a low gas fee, $\qmg^\star=1$ is a fixed point of the reaction function and therefore an equilibrium. Since $\bar{\Gamma}_2<0$, then immediately $\Gamma>\bar{\Gamma}_2$ and therefore $\qmg^\star=2$ is also an equilibrium. From the intermediate value theorem, and monotonicity of $\tilde{q}\left(\cdot\right)$, there is another fixed point (i.e., interior equilibrium) at $q^\star_2$. However, this interior equilibrium if unstable. If we perturb the $\LP$s' beliefs such the expectation for the marginal $\LP$ endowment is $\qmg+\epsilon$, there is pressure to switch to the high-fee pool since $\tilde{q}\left(q^\prime\right)>q^\prime$ for any $q^\prime>q^\star_2$. The system spirals towards an equilibrium in which all $\LP$s provide liquidity on the high-fee pool. Conversely, if we perturb beliefs in the opposite direction ($\qmg-\epsilon$) there is pressure to switch to the low-fee pool.
    \item[(ii)] $\Gamma>\bar{\Gamma}_1$. For a larger gas fee, the only equilibrium is $\qmg^\star=2$, that is all $\LP$s provide liquidity on the high-fee pool. This is because $q=1$ is not a fixed point of the reaction function, and the interior roots $q^\star_1$ and $q^\star_2$ are either outside the $\left[1,2\right]$ interval or they are irrational. 
\end{enumerate}

\paragraph{Case \#2: Medium fee on $L$ (i.e., $f\in\left(\frac{1}{2},\frac{2}{3}\right]$).} If $f\in\left(\frac{1}{2},\frac{2}{3}\right]$, then $0<\bar{\Gamma}_2 < \bar{\Gamma}_1 < \bar{\Gamma}_3$. We distinguish between four potential regions for the gas fee $\Gamma$:
\begin{enumerate}
    \item[(i)] $\Gamma\leq\bar{\Gamma}_2$. From the discussion above, $\qmg^\star=1$ is an equilibrium since $\bar{\Gamma}_2\leq \bar{\Gamma}_1$ and $\qmg^\star=2$ is not. Further, $q^\star_1<1$ and $q^\star_2>2$: the only equilibrium is the one where all $\LP$s provide liquidity on the low-fee pool.
    \item[(ii)] $\Gamma\in\left(\bar{\Gamma}_2,\bar{\Gamma}_1\right]$. Both $\qmg^\star=1$ and $\qmg^\star=2$ are equilibria in this case. There is also third, unstable equilibrium at $q^\star_2<2$ since  $\Gamma>\bar{\Gamma}_2$. The remaining interior root is not a fixed point since $q^\star_1<1$ for $\Gamma<\bar{\Gamma}_1$.
    \item[(iii)] $\Gamma\in\left(\bar{\Gamma}_1,\bar{\Gamma}_3\right]$. There are two stable equilibria, an interior one at $q^\star_1>1$ (since $\Gamma>\bar{\Gamma}_1$) and at $\qmg^\star=2$. There is a third, unstable equilibrium at $q^\star_2$.
    \item[(iv)] $\Gamma>\bar{\Gamma}_3$. The unique equilibrium is for $\qmg^\star=2$. The interior roots $q^\star_{1,2}$ are not real numbers, and $\tilde{q}(1)>1$ such that $\qmg^\star=1$ is not an equilibrium. 
\end{enumerate}

\paragraph{Case \#3: Large fee on $L$ (i.e., $f\in\left(\frac{2}{3},\frac{3}{4}\right]$).} If  $f\in\left(\frac{2}{3},\frac{3}{4}\right]$, then $0<\bar{\Gamma}_1 < \bar{\Gamma}_2 < \bar{\Gamma}_3$. We distinguish again between four potential regions for the gas fee $\Gamma$:
\begin{enumerate}
    \item[(i)] $\Gamma\leq\bar{\Gamma}_1$. As in the low gas fee case for $f\in\left(\frac{1}{2},\frac{2}{3}\right]$, $\qmg^\star=1$ is an equilibrium since $\bar{\Gamma}_2\leq \bar{\Gamma}_1$ and $\qmg^\star=2$ is not. Further, $q^\star_1<1$ and $q^\star_2>2$: the only equilibrium is the one where all $\LP$s provide liquidity on the low-fee pool.
    \item[(ii)] $\Gamma\in\left(\bar{\Gamma}_1,\bar{\Gamma}_2\right]$. Neither $\qmg^\star=1$ and $\qmg^\star=2$ are equilibria in this case. There is an unique interior equilibrium at $q^\star_1<1$ since $\Gamma>\bar{\Gamma}_1$. The second root is out of bounds: that is,  $q^\star_2>2$ since $\Gamma<\bar{\Gamma}_2$.
    \item[(iii)] $\Gamma\in\left(\bar{\Gamma}_2,\bar{\Gamma}_3\right]$. There are two stable equilibria, an interior one at $q^\star_1>1$ (since $\Gamma>\bar{\Gamma}_1$) and at $\qmg^\star=2$. There is a third, unstable equilibrium at $q^\star_2<2$.
    \item[(iv)] $\Gamma>\bar{\Gamma}_3$. The unique equilibrium is for $\qmg^\star=2$. The interior roots $q^\star_{1,2}$ are not real numbers, and $\tilde{q}(1)>1$ such that $\qmg^\star=1$ is not an equilibrium. 
\end{enumerate}

\paragraph{Case \#4: Very large fee on $L$ (i.e., $f>\frac{3}{4}$).} The scenario where $f>\frac{3}{4}$ is similar to the one above, the  but $q_2>2$ for $\Gamma\in\left(\bar{\Gamma}_2,\bar{\Gamma}_3\right]$ so one possible equilibrium is no longer feasible. We distinguish between three potential regions for the gas fee $\Gamma$:
\begin{enumerate}
    \item[(i)] $\Gamma\leq\bar{\Gamma}_1$. As in the low gas fee case for $f\in\left(\frac{1}{2},\frac{2}{3}\right]$, $\qmg^\star=1$ is an equilibrium since $\bar{\Gamma}_2\leq \bar{\Gamma}_1$ and $\qmg^\star=2$ is not. Further, $q^\star_1<1$ and $q^\star_2>2$: the only equilibrium is the one where all $\LP$s provide liquidity on the low-fee pool.
    \item[(ii)] $\Gamma\in\left(\bar{\Gamma}_1,\bar{\Gamma}_2\right]$. Neither $\qmg^\star=1$ and $\qmg^\star=2$ are equilibria in this case. There is an unique interior equilibrium at $q^\star_1<1$ since $\Gamma>\bar{\Gamma}_1$. The second root is out of bounds: that is,  $q^\star_2>2$ since $\Gamma<\bar{\Gamma}_2$.
    \item[(iii)] $\Gamma>\bar{\Gamma}_2$. The unique equilibrium is for $\qmg^\star=2$. The interior roots $q^\star_{1,2}$ are not real numbers, and $\tilde{q}(1)>1$ such that $\qmg^\star=1$ is not an equilibrium. 
\end{enumerate}

\subsubsection*{Region \#2: $\Gamma\in\left(1-f, 2\left(1-f\right)\right]$}

For $\Gamma>1-f$, the reaction function \eqref{eq:reaction_main} becomes
\begin{equation}
    \tilde{q}\left(\qmg\right)=\begin{cases}
    1, & \text{ for } \qmg \leq \frac{1-\eta\left(1+2(1-f)\right)}{\left(1-f\right)\left(1-\eta\right)}\\
    \frac{2\eta\Gamma}{ \left(1-\eta\right) \left(1-\left(1-f\right)\qmg\right)}, & \text{ for } \qmg \in \left(\frac{1-\eta\left(1+2(1-f)\right)}{\left(1-f\right)\left(1-\eta\right)}, \frac{1-\eta\left(1+\Gamma\right)}{\left(1-f\right)\left(1-\eta\right)}\right] \\
    2, & \text{ for } \qmg > \frac{1-\eta\left(1+\Gamma\right)}{\left(1-f\right)\left(1-\eta\right)}.
    \end{cases}
\end{equation}
First, $\qmg=1$ is a fixed point and therefore an equilibrium of the liquidity provision game if and only if
\begin{equation}
    \frac{1-\eta\left(1+2(1-f)\right)}{\left(1-f\right)\left(1-\eta\right)}>1 \Longleftrightarrow f>\frac{2\eta}{1+\eta}.
\end{equation}
Second, as for the first gas fee region, $\qmg=2$ is an equilibrium if $\Gamma>\bar{\Gamma}_2$.  The existence condition for a stable equilibrium is:
\begin{equation}
1\leq\frac{1}{2\left(1-f\right)} - \frac{1}{2\left(1-f\right)}\sqrt{1-\eta\frac{1+8\left(1-f\right)\Gamma}{1-\eta}}<\frac{1-\eta\left(1+\Gamma\right)}{\left(1-f\right)\left(1-\eta\right)},
\end{equation}
which translates to $\Gamma\in\left[f\frac{1-\eta}{2\eta},\frac{(2f-1)(1-\eta)}{\eta}\right)$. However, the interior equilibrium is only unique for $f\leq\frac{2\eta}{1+\eta}$.

\subsubsection*{Region \#3: $\Gamma>2\left(1-f\right)$}
If $\Gamma>2\left(1-f\right)$, then no liquidity provider reacts upon news to remove liquidity since the gas fee is too high. The expected profit difference from submitting quotes on the low- and high- fee pool is therefore proportional to $q_i$:
\begin{equation}\label{eq:pi_diff_highG}
    \pi^\LP_L-\pi^\LP_H = q_i \left[\frac{1}{2} \left(1-\eta\right) \left(1-\left(1-f\right)\qmg\right) - \eta \left(1-f\right)\right],
\end{equation}
which is always positive if $\qmg\leq\frac{1-\eta\left(3-2f\right)}{\left(1-f\right)\left(1-\eta\right)}$ and negative otherwise. Therefore, either all liquidity providers choose the low-fee pool or all liquidity providers choose the high-fee pool. Depending on whether $\frac{1-\eta\left(3-2f\right)}{\left(1-f\right)\left(1-\eta\right)}\in\left[1,2\right]$ or not, the coordination game might have one or two equilibria, but with a single liquidity pool dominating the market.

\end{proof}

\noindent \textbf{\large Corollary \ref{cor:monitoring}}
\begin{proof}
    Generally, from \eqref{eq:pi_diff} and \eqref{eq:pi_diff_highG}, the expected profit difference from submitting quotes on the low- and high- fee pool is
\begin{equation}\label{eq:pi_diff_general}
    \pi^\LP_L-\pi^\LP_H = q_i \left[\frac{1}{2} \left(1-\eta\right) \left(1-\left(1-f\right)\qmg\right)\right] - \eta \min\left\{q_i\left(1-f\right),\Gamma\right\},
\end{equation}
where the latter term reflects whether is is optimal for an LP with endowment $q_i$ to monitor on pool $L$ or not.

\paragraph{Case 1: $\qmg<\frac{1-\eta\left(3-2f\right)}{\left(1-f\right)\left(1-\eta\right)}$.} In this case, it follows that
\begin{equation}
   \pi^\LP_L-\pi^\LP_H > q_i\left[\frac{1}{2} \left(1-\eta\right) \left(1-\left(1-f\right)\qmg\right) - \eta \left(1-f\right)\right]>0,
\end{equation}
and therefore it is optimal for all liquidity providers to choose pool $L$, leading to $\qmg^\star=1$ -- a corner equilibrium where all liquidity providers choose pool $L$.

\paragraph{Case 2: $\qmg>\frac{1-\eta\left(3-2f\right)}{\left(1-f\right)\left(1-\eta\right)}$.} In this case,  $\frac{1}{2} \left(1-\eta\right) \left(1-\left(1-f\right)\qmg\right) - \eta \left(1-f\right)<0$ and therefore for any $q_i\leq\frac{\Gamma}{1-f}$
\begin{equation}
   \pi^\LP_L-\pi^\LP_H > q_i\left[\frac{1}{2} \left(1-\eta\right) \left(1-\left(1-f\right)\qmg\right) - \eta \left(1-f\right)\right]<0,
\end{equation}
That is, all liquidity providers who do not optimally monitor their quotes choose to provide liquidity on the high-fee pool $H$. The marginal LP, if it exists, is the one for whom the expected profit on the high-fee and low-fee pool are equal, conditional on paying the gas fee to monitor their quotes:
\begin{equation}\label{eq:pi_diff_general}
    \pi^\LP_L-\pi^\LP_H = q_i \left[\frac{1}{2} \left(1-\eta\right) \left(1-\left(1-f\right)\qmg\right)\right] - \eta \Gamma  =0,
\end{equation}
which leads to the same fixed points $q_i=\qmg$ as in Proposition \ref{prop:equilibria}. 

% \subsection{A more general condition for interior equilibrium existence}

% Formally, the LP reaction function can be augmented as:
% \begin{equation}\label{eq:reaction}
%     \tilde{q}\left(\qmg\right)=\begin{cases}
%     1, & \text{ for } \qmg \leq \frac{1-\eta\left(1+2\min\left\{\Gamma,1-f\right\}\right)}{\left(1-f\right)\left(1-\eta\right)}\\
%     \frac{2\eta\Gamma}{ \left(1-\eta\right) \left(1-\left(1-f\right)\qmg\right)}, & \text{ for } \qmg \in \left(\frac{1-\eta\left(1+2\min\left\{\Gamma,1-f\right\}\right)}{\left(1-f\right)\left(1-\eta\right)}, \frac{1-\eta\left(1+\Gamma\right)}{\left(1-f\right)\left(1-\eta\right)}\right] \\
%     2, & \text{ for } \qmg > \frac{1-\eta\left(1+\Gamma\right)}{\left(1-f\right)\left(1-\eta\right)}.
%     \end{cases}
% \end{equation}
% The existence condition for a stable equilibrium is:
% \begin{equation}
%  \frac{1-\eta\left(1+2\min\left\{\Gamma,1-f\right\}\right)}{\left(1-f\right)\left(1-\eta\right)}<\frac{1}{2\left(1-f\right)} - \frac{1}{2\left(1-f\right)}\sqrt{1-\eta\frac{1+8\left(1-f\right)\Gamma}{1-\eta}}<\frac{1-\eta\left(1+\Gamma\right)}{\left(1-f\right)\left(1-\eta\right)},
% \end{equation}
% which translates to $\Gamma\in\left[\underline{\Gamma},\bar{\Gamma}\right)$, where
% \begin{align}
%     \underline{\Gamma}&=\max\left\{f\frac{1-\eta}{2\eta},\frac{1+\eta(2f-3)}{1-\eta}\right\} \text{ and } \nonumber \\
%     \bar{\Gamma}&=\begin{cases} \frac{1-\eta}{8\eta(1-f)} & f \leq 0.75 \\
%                            \frac{(2f-1)(1-\eta)}{\eta} & f>0.75 \end{cases}
% \end{align}


\end{proof}







==> Sections/comments.tex <==
What does this model give us?

\begin{enumerate}
  \item \textbf{Old prediction.} The liquidity market share of the low-fee pool  decreases in the gas fee $\Gamma$. \\
   \mz{Confirmed, since the market share of the low fee pool is $e^{-\frac{\max\left\{0,\qmg-q_h\right\}}{\lambda}}$ and $\qmg-q_h$ increases in $\Gamma$ in any fragmented equilibrium. }
  \item \textbf{Old prediction.} $\LP$s on the low-fee pool make larger liquidity deposits than $\LP$s on the high-fee pool.
    \mz{Confirmed.}
    \item \textbf{Old prediction.} The average trade size is higher on pool $H$ than on pool $L$. At the same time, trading volume is higher on pool $L$ than on pool $H$. \\
    \mz{Confirmed. Trades with low enough private values or news size only go to low-fee pool, if private value/news is high enough the trade goes on both pools.}
    \item \textbf{Old prediction.} The average liquidity deposit on both the low- and- high fee pool increases with gas costs.
    \mz{Likely confirmed, mechanism is very similar. First, the $\LP$s with the lowest endowments on pool $L$ switch to pool $H$. As a result, the average deposit on pool $L$ increases. Second, the $\LP$s with low endowments on pool $H$ may leave the market. }
    \item \textbf{Old prediction.} $\LP$s update liquidity more frequently on the low-fee than on the high-fee pool.\\
    \mz{Confirmed. Liquidity more likely to hit the bound on low fee pool.}
    \item \textbf{Old prediction.} A larger gas price leads to more frequent liquidity updates on the low-fee pool.\\
    \mz{\textbf{Not true} in the current model, the frequency of re-balancing does not depend on gas costs.}
    \item \textbf{New prediction.} Adverse selection cost is higher on the low fee pool than on the high fee pool. \\
    \mz{True in the data, we have the analysis.}
    \item \textbf{New prediction.} In a fragmented equilibrium, the liquidity yield must be higher on the low fee pool than on the high fee pool. \\
    \mz{True in the data, we have the analysis on liquidity yield.}
    \item Model has new, more realistic ingredients:
        \begin{itemize}
            \item Price impact on high- and low-fee pools.
            \item Adverse selection costs.
            \item A price range which is Uniswap v3-specific (but exogenous).
            \item A clear rationale for re-balancing (i.e., hit the price limit).
        \end{itemize}
    
\end{enumerate}}



==> Sections/introcp.tex <==
The way in which economic agents react to transaction costs affects the extent to which such costs are detrimental to  economic efficiency.  Or, as \citet{demsetz1968} puts it ``the question that is relevant for efficiency is whether or not the cost is appropriately economized.''  In this paper, we investigate a unique environment that allows us to investigate, theoretically and empirically, how explicit transactions costs affect liquidity supply.

We investigate liquidity provision on a decentralized exchange (Uniswap v3). Automated exchanges such as Uniswap present a unique laboratory to investigate how transaction costs affect the market for liquidity. While there are various new institutional details that animate these exchanges, for our purposes  two are economically important.   First, in automated exchanges, liquidity demand and supply can easily be distinguished:  users either post liquidity or initiate a trade.  So, we can isolate the effect of transactions costs on each side of the market for liquidity.  Second, prices are not set by market participants, but are automatically calculated as a function of liquidity demand and supply. Thus, costs are not directly passed from liquidity suppliers to demanders through prices. 



Briefly, Uniswap v3 allows liquidity suppliers and demanders to select into  trading places (called pools) that differ on transaction fees.  These proportional fees are paid by liquidity demanders and are the only source of remuneration to liquidity suppliers.  As noted, prices are calculated mechanically based on posted liquidity, so liquidity suppliers do not earn price impact. In addition, all participants pay a fixed transaction cost (called a ``gas fee'') to access the markets. Our theory and empirical work investigates the effect of different proportional fees and fixed fees on liquidity supply.

To do so, we present a simple model of liquidity supply in which there are two markets -- one has high fees, and one has low fees.  Consistent with the design of V3, liquidity suppliers  chose a market and then place their liquidity into a band around the current value of the asset. The posted liquidity is subject to a bonding curve and hence generates a price impact cost.  Liquidity suppliers have heterogeneous endowments, interpretable as different capital constraints --- low-endowment liquidity providers are akin to retail traders, whereas high-endowments stand in for large institutional investors or quantitative funds. Trade occurs against these positions either because a liquidity demander arrives who has experienced a liquidity shock or because the value of the asset has changed and an arbitrageur adversely selects the passive liquidity supply.  Collectively, the decisions of the liquidity demanders determine the payoff to the liquidity suppliers. After large private or common value trades, liquidity providers rebalance their positions; to do so liquidity providers incur a fixed cost (i.e., gas price) each time they update their position.

Traders demanding liquidity face two types of costs:  first, the fee associated with their chosen pool (low or high) and second, the price impact costs generated by the pool's bonding curve and supplied liquidity.  They route their orders to the low-fee pool which minimizes transaction costs. The high-fee pool executes the residual order flow from large traders who exhaust all liquidity at the cheaper venue. As a result, low-fee markets are actively traded and require frequent liquidity updates whereas high-fee pools have a longer liquidity update cycle since they absorb fewer trades.

We  establish conditions under which there is fragmentation or consolidation.  Specifically, even in this simple framework there is a robust parameter range in which liquidity does not naturally concentrate on one of the exchanges. Not only does liquidity fragment, but it differs in both use and type across the two markets.  That is, one exchange features liquidity provided by large suppliers while on the other smaller (retail) suppliers predominate. 

As we distinguish between liquidity demanders who are trading to exploit gains from trade and liquidity demanders who are arbitraging common value changes, we can decomposed returns to liquidity providers, and how that adverse selection is higher on the low fee pool.  Given that the low fee pool is populated with larger liquidity suppliers, this suggests that institutional traders bear price risk. 

Our paper also shows that fixed costs translate to significant economies of scale, which lead to market fragmentation and the emergence of liquidity provider clienteles. Specifically, our findings reveal that a small number of highly active large liquidity providers, potentially institutional investors and hedge funds, primarily trade against numerous small incoming trades on pools with low fees. In contrast, high-fee pools involve less frequent trading between a substantial number of capital-constrained passive liquidity providers (e.g., retail market makers) on one side and a few sizeable incoming orders on the other. The underlying economic mechanism is that smaller liquidity providers strategically trade off a lower execution probability against higher liquidity fee and less frequent fixed costs, such as gas fees.

Both pools can attract a positive market share if the gas price is large enough due to economies of scale. Liquidity providers trade off a higher revenue per unit of time in the low-fee pool (driven by the larger trading volume) against the additional gas cost required for active liquidity management. As a result, market maker clienteles emerge in equilibrium. Liquidity providers with large endowments gravitate towards low-fee markets, as they are best positioned to frequently update their position. In contrast, smaller market makers choose to passively provide liquidity on high-fee markets where they only trade against large orders being routed there. They optimally trade off a lower execution probability against higher fees per unit of volume and a lower liquidity management cost per unit of time. 


%{Our findings indicate that liquidity fragmentation can enhance market quality, as measured by a lower implementation shortfall --- a metric that combines both realized gains from trade as well as trading costs. In a single-pool market, selecting the optimal fee involves balancing these costs. A fee that is too low fails to attract liquidity providers with lower endowments, leading to unrealized gains. Conversely, a very high fee results in prohibitively high trading costs. A two-pool market with heterogeneous fees provides enhanced flexibility, offering two instruments to independently manage the two components of the implementation shortfall. The higher fee determines the marginal liquidity provider $\LP$ entering the market, and therefore the realized gains from trade. The lower fee pool, by attracting $\LP$ with larger endowments, can reduce transaction costs. We demonstrate that a two-pool fee structure can always be designed to yield a lower implementation shortfall compared to any single-pool arrangement.}


Uniswap v3 launched in May 2021 and quickly established itself as the leading decentralized exchange. Daily trading volume on Uniswap v3 typically exceeds US \$1 billion, whereas the total liquidity supply varies between US \$2-4 billion in our sample, across hundreds of cryptocurrencies. For major pairs such as Ether against USD stablecoins, Uniswap boasts twice or three times better liquidity than centralized exchanges such as Binance.\footnote{See \href{https://uniswap.org/blog/uniswap-v3-dominance}{The Dominance of Uniswap v3 Liquidity}; May 5, 2022.} 

The market design explicitly allows for fragmentation. Each asset pair to be traded on up to four liquidity pools that only differ in the compensation for liquidity providers: in particular, liquidity fees can be equal to 1, 5, 30, or 100 basis points and the corresponding tick sizes are 1, 10, 60, or 200 basis points. The liquidity pools are otherwise identical and, importantly, they share the common infrastructure of the Ethereum blockchain -- i.e., they are similarly impacted by variation in gas prices due to, say, network congestion. At launch, Uniswap Labs conjectured that trading and liquidity should consolidate in equilibrium on a single ``canonical'' pool for which the liquidity fee is just enough to compensate the marginal market maker for adverse selection and inventory costs. That is, activity in low-volatility pairs such as stablecoin-to-stablecoin trades should naturally gravitate to low fee liquidity pools, whereas speculative trading in more volatile pairs will consolidate on high fee markets.\footnote{See \emph{Flexible fees} paragraph at \url{https://uniswap.org/blog/uniswap-v3}; accessed September 14, 2022.}

Using the model for guidance, we analyze  more than 28 million interactions with Uniswap v3 liquidity pools -- that is, all liquidity updates and trades from the inception of v3 in May 2021 until July 2023. 
We first document  liquidity fragmentation in 32 out of 242 asset pairs in our sample, 
%AL why only 242 pairs?
which account for 95\% of liquidity committed to Uniswap v3 smart contracts and 93\% of trading volume. For each of the fragmented pairs, trading consolidates on two pools with adjacent fee levels: either 1 and 5 basis points (e.g., USDC-USDT), 5 and 30 basis points (ETH-USDC), or 30 and 100 basis points (USDC-CRV).

We then document that high-fee pools are on average larger -- with aggregate end-of-day liquidity of \$46.50 million relative to \$33.78 million, the average size of low-fee pools. Nevertheless, three quarters of daily trading volume executes on low-fee pools. In line with the model predictions, low-fee pools are more active as they capture many small trades. There are five times as many trades on low- than on high-fee pools (610 versus 110). However, the average trade on the high fee pool is twice as large: \$14,490 relative to \$6,340. Unsurprisingly, liquidity cycles -- measured as the time between the submission and update of posted liquidity -- are 20\% shorter on the highly active low-fee pool. 

We find robust evidence of liquidity supply clienteles across pools. The average liquidity deposit is 107.5\% larger on the low-fee pool, after controlling for daily volume and return volatility. At the same time, high-fee pools' market share is 21 percentage points higher. The results point to an asymmetric match between liquidity supply and demand: large liquidity suppliers are matched with small liquidity demanders on low-fee pools, whereas small liquidity suppliers trade with a few large orders on the high-fee pool. 

We then turn to the common fixed cost of accessing the market, or gas fees.  The degree of market fragmentation depends on the magnitude of gas costs on the Ethereum blockchain. In the model, a higher gas price leads to a shift in liquidity supply from the low- to the high-fee pool as active position management becomes relatively more costly for the marginal liquidity supplier. We find that a one standard deviation increase in gas prices corresponds to a 4.63 percentage points decrease in the low-fee pool market share, and a 29\% drop in liquidity inflows on days when gas costs are elevated. As liquidity suppliers  leave the low-fee pool, the time between position updates becomes 4.19\% shorter since incoming order flow depletes liquidity at a faster pace. The effect reinforces the expected gas cost difference between the two pools, and more liquidity suppliers switch to the high-fee venue.

Our paper is related to various literatures. 
The classical study of \citet{pagano1989trading} shows that if an asset is traded on two identical exchanges with equal transaction costs, in equilibrium market participants gravitate to a single exchange due to network effects. In practice, exchanges are rarely identical: fragmentation can emerge between fast and slow exchanges \citep{pagnotta2018competing, brocim:20} or between lit and dark markets \citep{Zhu2014}. In our model, fragmentation on decentralized exchanges is driven by variation in liquidity fees as well as different economies of scale due to heterogeneity in liquidity provider capital. We find that liquidity fragmentation driven by high gas fees implies larger transaction costs on incoming orders. We note that there is no time priority on decentralized exchanges, which clear in a pro rata fashion. On markets with time priority, \citet{FoucaultMenkveld2008} and \citet{Ohara2011market} find that market segmentation in equity markets improves liquidity (by allowing queue jumping) and price discovery.

Fixed costs for order submission are uncommon in traditional markets. However, in 2012, the Canadian regulator IIROC implemented an ``integrated fee model'' that charged traders for all messages sent to Canadian marketplaces. \citet{KorajczykMurphy2018} document that this measure disproportionately affected high-frequency traders, resulting in wider bid-ask spreads but lower implementation shortfall for large traders, possibly due to a reduction in back-running activity. Our study contributes additional insights by highlighting that the introduction of a fixed cost, even when applied across exchanges, can lead to market fragmentation.

We also relate to a rich literature on market fragmentation and differential fees. Closest to our paper, \citet{Battalio2016} and \citet{Cimon2021} study the trade-off between order execution risk and compensation for liquidity provision in the context of make-take fee exchanges. However, \citet{Battalio2016} specifically addresses the issue of the broker-customer agency problem, whereas our study focuses on liquidity providers who trade on their own behalf. In traditional securities markets, make-take fees are contingent on trade execution and proportional to the size of the order.  On the other hand, gas costs on decentralized exchanges are independent of order execution, highlighting the significance of economies of scale (lower proportional costs for larger liquidity provision orders) and dynamic liquidity cycles (managing the frequency of fixed cost payments). Strategic brokers in \citet{Cimon2021} provide liquidity alongside exogenous market-makers in a static setting. We complement this approach by modelling network externalities inherent in the coordination problem of heterogeneous liquidity suppliers. In our dynamic setup, this allows us to pin down the equilibrium duration of liquidity cycles and the relative importance of gas fixed costs.


Our paper relates to a nascent and fast-growing literature on the economics of decentralized exchanges. Many studies \citep[e.g.,][]{aoyagi2020,aoyagiito2021,park2022} focus on the economics of constant-function automated market makers, which do not allow liquidity providers to set price limits. In this restrictive environment, \citet{CapponiJia2021} argue that market makers have little incentives to update their position upon the arrival of news to avoid adverse selection, since pro-rata clearing gives an advantage to arbitrageurs. \citet{LeharParlour2021} solve for the equilibrium pool size in a setting where liquidity providers fully internalize information costs without rushing to withdraw positions at risk of being sniped. We argue that on exchanges that allow for limit or range orders, the cost of actively managing positions becomes a first-order concern, as liquidity suppliers need to re-set the price limits once posted liquidity no longer earns fees. Our empirical result on economies of scale echoes the argument in \citet{BarbonRanaldo2021}, who compare transaction costs on centralized and decentralized exchanges and find that high gas prices imply that the latter only become competitive for transactions over US\$100,000. \citet{HasbrouckRiveraSaleh2022} argue that liquidity suppliers require remuneration.  We complement the argument by stating that high fees might be \emph{necessary} for some liquidity providers to cover the fixed costs of managing their position. In line with our theoretical predictions, \citet{caparros2023blockchain} find that liquidity providers reposition their quotes more often on Uniswap V3 pools built on Polygon, which features substantially lower gas fees. Finally, \citet{Heimbach2023} document that after accounting for price impact, concentrated liquidity on Uniswap v3 pools results in increased returns for sophisticated participants but losses for retail traders. 


Despite higher gas costs, decentralized exchanges may hold advantages over centralized venues. \citet{han2022trust} demonstrate Uniswap frequently leads price discovery compared to centralized exchanges such as Binance, despite the latter having higher trading volume. \citet{capponi2023price} find that the fee paid traders to establish execution priority unveils their private information, and therefore contributes to price discovery. \citet{ASPRIS2021101845} argue that decentralized exchanges offer better security than their centralized counterparts since assets are never transferred to the custody of a third party such as an exchange wallet. In turn, \citet{BrolleyZoican2022b} make the point that decentralized exchanges may be able to reduce overall computational costs associated with latency arbitrage races, as they eliminate long-term co-location subscriptions.






==> Sections/introduction.tex <==
In 1971, Fischer Black explored the concept of computer-driven ``automated exchanges'' that could streamline intermediation in financial markets \citep{Black1971}. One important argument was that broadening the group of traders who provide liquidity would alleviate the limitations imposed by a specialist's inventory size. Over the following half-century, markets progressively moved in this direction, with the majority of exchanges now operating as limit order books, theoretically enabling any trader to supply liquidity. However, in practice, the rise of algorithmic and high-frequency trading made liquidity provision in limit order markets a technology-intensive affair, necessitating low-latency connectivity and active management of quotes. Some trader categories, such as retail investors, struggle to competitively supply liquidity in this environment.

Decentralized exchanges (DEXs), which function as fully automated trading platforms implemented as smart contracts on public blockchains, offer a novel passive liquidity supply mechanism which requires significantly fewer quote updates. Market makers can deposit and withdraw funds into a ``liquidity pool,'' and trade prices are determined by an Automated Market Maker algorithm \citep[see, e.g.,][]{park2022} as a function of the available funds in the pool. They receive compensation through liquidity fees, computed as a fixed percentage of trading volume charged to traders seeking immediate execution, as opposed to bid-ask spreads. Uniswap, the leading decentralized exchange, allows for the fragmentation of trading for each token pair across multiple pools with varying liquidity fees.  In Appendix \ref{sec:app-dex}, we discuss in depth the trading mechanics on Uniswap.

The passive nature of liquidity supply in DEXs was initially designed to minimize interactions with blockchain smart contracts, as these interactions incur gas costs to compensate the decentralized network for spent computational power. Nevertheless, passive liquidity supply is particularly well-suited for small retail liquidity providers, who face their own time and effort fixed costs. Can the mechanisms used by decentralized exchanges have a comparable impact on liquidity supply as ETFs had on transforming portfolio management in recent decades?

Our paper shows that fixed costs translate to significant economies of scale on decentralized exchanges, which lead to market fragmentation and the emergence of liquidity provider clienteles. Specifically, our findings reveal that a small number of highly active large liquidity providers, potentially institutional investors and hedge funds, primarily trade against numerous small incoming trades on pools with low fees. In contrast, high-fee pools involve less frequent trading between a substantial number of capital-constrained passive liquidity providers (e.g., retail market makers) on one side and a few sizeable incoming orders on the other. The underlying economic mechanism is that smaller liquidity providers strategically trades off a lower execution probability against higher liquidity fee and less frequent fixed costs, such as gas fees.

Our first contribution is a theoretical model of liquidity provision on decentralized exchanges. A continuum of liquidity providers ($\LP$s) choose to deposit their token endowments in either a high- or a low-fee pool; that is, they \emph{mint} liquidity. The liquidity providers have heterogeneous token endowments, which map to different capital constraints --- low-endowment $\LP$s are akin to retail traders, whereas high-endowment $\LP$s may stand in for large institutional investors or quantitative funds. Further, liquidity providers incur a fixed cost (i.e., gas price) each time they update their position.

Traders demanding liquidity route their orders first to the low-fee pool to minimize transaction costs. The high-fee pool executes the residual order flow from large traders who exhaust all liquidity at the cheaper venue. As a result, low-fee markets are actively traded and require frequent liquidity updates whereas high-fee pools have a longer liquidity update cycle since they absorb fewer trades. 

Both pools can attract a positive market share if the gas price is large enough due to economies of scale. Liquidity providers trade off a higher revenue per unit of time in the low-fee pool (driven by the larger trading volume) against the additional gas cost required for active liquidity management. As a result, market maker clienteles emerge in equilibrium. Liquidity providers with large endowments gravitate towards low-fee markets, as they are best positioned to frequently update their position. In contrast, smaller market makers choose to passively provide liquidity on high-fee markets where they only trade against large orders being routed there. They optimally trade off a lower execution probability against higher fees per unit of volume and a lower liquidity management cost per unit of time. 

Using the model for guidance, we analyze a data set comprising of more than 28 million interactions with Uniswap v3 liquidity pools -- that is, all liquidity updates and trades from May 2021 until July 2023. Uniswap v3 launched in May 2021 and quickly established itself as the leading decentralized exchange. Daily trading volume on Uniswap v3 typically exceeds US \$1 billion, whereas the total liquidity supply varies between US \$2-4 billion in our sample, across hundreds of cryptocurrencies. For major pairs such as Ether against USD stablecoins, Uniswap boasts twice or three times better liquidity than centralized exchanges such as Binance.\footnote{See \href{https://uniswap.org/blog/uniswap-v3-dominance}{The Dominance of Uniswap v3 Liquidity}; May 5, 2022.} 

The market design explicitly allows for fragmentation. Each asset pair to be traded on up to four liquidity pools that only differ in the compensation for liquidity providers: in particular, liquidity fees can be equal to 1, 5, 30, or 100 basis points and the corresponding tick sizes are 1, 10, 60, or 200 basis points. The liquidity pools are otherwise identical and, importantly, they share the common infrastructure of the Ethereum blockchain -- i.e., they are similarly impacted by variation in gas prices due to, say, network congestion. At launch, Uniswap Labs conjectured that trading and liquidity should consolidate in equilibrium on a single ``canonical'' pool for which the liquidity fee is just enough to compensate the marginal market maker for adverse selection and inventory costs. That is, activity in low-volatility pairs such as stablecoin-to-stablecoin trades should naturally gravitate to low fee liquidity pools, whereas speculative trading in more volatile pairs will consolidate on high fee markets.\footnote{See \emph{Flexible fees} paragraph at \url{https://uniswap.org/blog/uniswap-v3}; accessed September 14, 2022.}

We document significant liquidity fragmentation in 32 out of 242 asset pairs in our sample, which account for 95\% of liquidity committed to Uniswap v3 smart contracts and 93\% of trading volume. For each of the fragmented pairs, trading consolidates on two pools with adjacent fee levels: either 1 and 5 basis points (e.g., USDC-USDT), 5 and 30 basis points (ETH-USDC), or 30 and 100 basis points (USDC-CRV).

High-fee pools are on average larger -- with aggregate end-of-day liquidity of \$46.50 million relative to \$33.78 million, the average size of low-fee pools. Nevertheless, three quarters of daily trading volume executes on low-fee pools. In line with the model predictions, low-fee pools are more active as they capture many small trades. There are five times as many trades on low- than on high-fee pools (610 versus 110). However, the average trade on the high fee pool is twice as large: \$14,490 relative to \$6,340. Unsurprisingly, liquidity cycles -- measured as the time between the submission and update of an order -- are 20\% shorter on the highly active low-fee pool. 

We find evidence of market maker clienteles across pools. The average liquidity deposit is 107.5\% larger on the low-fee pool, after controlling for daily volume and return volatility. At the same time, high-fee pools' market share is 21 percentage points higher. The results point to an asymmetric match between liquidity supply and demand: large $\LP$s are matched with small trader on low-fee pools, whereas small $\LP$s trade with a few large orders on the high-fee pool. 

The degree of market fragmentation depends on the magnitude of gas costs on the Ethereum blockchain. In the model, a higher gas price leads to a shift in liquidity supply from the low- to the high-fee pool as active position management becomes relatively more costly for the marginal $\LP$. We find that a one standard deviation increase in gas prices corresponds to a 4.63 percentage points decrease in the low-fee pool market share, and a 29\% drop in liquidity inflows on days when gas costs are elevated. As $\LP$s leave the low-fee pool, the time between position updates becomes 4.19\% shorter since incoming order flow depletes liquidity at a faster pace. The effect reinforces the expected gas cost difference between the two pools, leading to more $\LP$s switching to the high-fee venue.

Our paper relates to a nascent and fast-growing literature on the economics of decentralized exchanges. Many studies \citep[e.g.,][]{aoyagi2020,aoyagiito2021,park2022} focus on the economics of constant-function automated market makers, which do not allow liquidity providers to set price limits. In this restrictive environment, \citet{CapponiJia2021} argue that market makers have little incentives to update their position upon the arrival of news to avoid adverse selection, since pro-rata clearing gives an advantage to arbitrageurs. \citet{LeharParlour2021} solve for the equilibrium pool size in a setting where liquidity providers fully internalize information costs without rushing to withdraw positions at risk of being sniped. We argue that on exchanges that allow for limit or range orders, the cost of actively managing positions becomes a first-order concern, as $\LP$s need to re-set the price limits once posted liquidity no longer earns fees. Our empirical result on economies of scale echoes the argument in \citet{BarbonRanaldo2021}, who compare transaction costs on centralized and decentralized exchanges and find that high gas prices imply that the latter only become competitive for transactions over US\$100,000. \citet{HasbrouckRiveraSaleh2022} argue that higher liquidity fees on decentralized exchanges stimulate liquidity supply and lead to an increase in the equilibrium trading volume. We complement the argument by stating that high fees might be \emph{necessary} for some liquidity providers to cover the fixed costs of managing their position. In line with our theoretical predictions, \citet{caparros2023blockchain} find that liquidity providers reposition their quotes more often on Uniswap V3 pools built on Polygon, which features substantially lower gas fees. Finally, \citet{Heimbach2023} document that after accounting for price impact, concentrated liquidity on Uniswap v3 pools results in increased returns for sophisticated participants but losses for retail traders. 


Despite higher gas costs, decentralized exchanges may hold advantages over centralized venues. \citet{han2022trust} demonstrate Uniswap frequently leads price discovery compared to centralized exchanges such as Binance, despite the latter having higher trading volume. \citet{capponi2023price} find that the fee paid traders to establish execution priority unveils their private information, and therefore contributes to price discovery. \citet{ASPRIS2021101845} argue that decentralized exchanges offer better security than their centralized counterparts since assets are never transferred to the custody of a third party such as an exchange wallet. In turn, \citet{BrolleyZoican2022b} make the point that decentralized exchanges may be able to reduce overall computational costs associated with latency arbitrage races, as they eliminate long-term co-location subscriptions.

We also relate to a rich literature on market fragmentation and differential fees. Closest to our paper, \citet{Battalio2016} and \citet{Cimon2021} study the trade-off between order execution risk and compensation for liquidity provision in the context of make-take fee exchanges. However, \citet{Battalio2016} specifically addresses the issue of the broker-customer agency problem, whereas our study focuses on liquidity providers who trade on their own behalf. In traditional securities markets, make-take fees are contingent on trade execution and proportional to the size of the order.  On the other hand, gas costs on decentralized exchanges are independent of order execution, highlighting the significance of economies of scale (lower proportional costs for larger liquidity provision orders) and dynamic liquidity cycles (managing the frequency of fixed cost payments). Strategic brokers in \citet{Cimon2021} examines strategic brokers who provide liquidity alongside exogenous market-makers in a static setting. We complement this approach by modelling network externalities inherent in the coordination problem of heterogeneous liquidity suppliers. In our dynamic setup, this allows us to pin down the equilibrium duration of liquidity cycles and the relative importance of gas fixed costs.

Fixed costs for order submission are uncommon in traditional markets. However, in 2012, the Canadian regulator IIROC implemented an ``integrated fee model'' that charged traders for all messages sent to Canadian marketplaces. \citet{KorajczykMurphy2018} document that this measure disproportionately affected high-frequency traders, resulting in wider bid-ask spreads but lower implementation shortfall for large traders, possibly due to a reduction in back-running activity. Our study contributes additional insights by highlighting that the introduction of a fixed cost, even when applied across exchanges, can lead to market fragmentation.

The classical study of \citet{pagano1989trading} shows that if an asset is traded on two identical exchanges with equal transaction costs, in equilibrium market participants gravitate to a single exchange due to network effects. In practice, exchanges are rarely identical: fragmentation can emerge between fast and slow exchanges \citep{pagnotta2018competing, brocim:20} or between lit and dark markets \citep{Zhu2014}. In our model, fragmentation on decentralized exchanges is driven by variation in liquidity fees as well as different economies of scale due to heterogeneity in liquidity provider capital. We find that liquidity fragmentation driven by high gas fees implies larger transaction costs on incoming orders. We note that there is no time priority on decentralized exchanges, which clear in a pro rata fashion. On markets with time priority, \citet{FoucaultMenkveld2008} and \citet{Ohara2011market} find that market segmentation in equity markets improves liquidity (by allowing queue jumping) and price discovery.


==> Sections/model_CP_AMM.tex <==
\paragraph{Asset and trading enviroment.} Consider a continuous time model of trade in a single token $\T$ with expected value $v_t>0$. The asset is traded in two liquidity pools in which token trade occurs against a num\'{e}raire asset (cash). Prices in both pools satisfy a constant product bonding curve, as common in practice. So, for a pool with $T$ tokens and $N$ of the num\'{e}raire good, 
\begin{equation}\label{eq:bond_curve}
    T \times N = \text{constant}.
\end{equation}
To purchase $\Delta T$ tokens, a traders needs to add 
\begin{align}
    \Delta N & = \frac{T \times N}{T - \Delta T} - N \\
    & = \frac{v T^2}{T-\Delta T}-v T \nonumber
\end{align}
units of cash to the pool, where the last equality follows from the pool trading at the fair price, that is $N=v \times T$.

Fees are levied on liquidity takers  as a fraction of the value of the trade and distributed pro rata to liquidity providers.  The pools have different fees.  One pool charges a low fee, and one pool charges a high fee which we denote $\ell$ and $h$ respectively. Specifically, to purchase $\Delta T$ units of the token on the low fee pool, the total cost to a taker is
\begin{equation}
    \Delta N \left(1+\ell\right) = v T \left(1+\ell\right)\left(\frac{T}{T-\Delta T}-1\right),
\end{equation}
while the liquidity providers receive a fee revenue equal to $\Delta N \ell$.

In addition, consistent with gas costs on Ethereum,  liquidity providers incur a fixed execution cost $\Gamma>0$ to interact with the market.  

\paragraph{Liquidity providers.}  Liquidity providers ($\LP$) differ in their endowments of the token. Each provider $i$ can supply at most $q_i$  of the token, where $q_i$ follows a distribution $\varphi\left(q\right)$ between $\left[\underline{q},\overline{q}\right]$ tokens. \mz{This can be defined later, or left general?}

\paragraph{Traders.} Traders arrive at the market as a Poisson process with unit intensity. Upon arrival, with probability $\eta$ there is news: i.e., the common asset value increases to $v\left(1+\tilde{\theta}_\text{news}\right)$. In this case, the incoming trader is an arbitrageur ($\A$). With probability $1-\eta$, a liquidity trader ($\LT$) receives a positive shock to their private value $v\left(1+\tilde{\theta}_\text{private}\right)$. 

The two shocks are independently and identically distributed: with probability $\alpha$ the shock is $\theta_b$ and with probability $1-\alpha$ the shock is $\theta_s$, with
\begin{equation}
    \theta_b > h > \theta_s > l.
\end{equation}
Private value trades are immediately reversed by arbitrageurs, whereas common value trades are not and trigger costly re-balancing by liquidity providers.

Figure \ref{fig:timing_revised} illustrates the timing of the model.

\begin{figure}[H]
    \centering
\begin{tikzpicture}
    % Draw the vertical lines
    \draw[|->, thick] (0,0) -- (15.75,0);
    \draw[|->, thick] (0,1.5) -- (15.75,1.5);

    \node at (15.75,0.5) {Pool H};
    \node at (15.75, 2) {Pool L};

    \node[align=left] at (1.5, 0.75) {$\LP$s deposit $q_i$ \\ in pool $k\in\left\{L,H\right\}$};

    \draw[->,blue] (1,2)--(1,1.5);
    \node[blue, align=center] at (1,2.4) {Type $\theta_s$ \\ LT};

    \draw[->,blue] (2.5,2)--(2.5,1.5);
    \node[blue, align=center] at (2.5,2.4) {Type $\theta_s$ \\ LT};

    \draw[->,blue,thick] (4,2)--(4,1.5);
    \draw[->,blue,thick] (4,1.5)--(4,0);
    \node[blue, align=center] at (4,2.4) {\bfseries Type $\theta_b$ \\ LT};

    \draw[dotted,thick,red] (4.5,1.5) -- (4.5, 0);
    \node[red, align=left] at (5,0.75) {News \\ $\theta_s$}; 

    \draw[->,red] (6,2)--(6,1.5);
    \node[red, align=left] at (6,2.4) {$\A$ trades \\ on pool $L$};

    \draw[->,thick](8,2)--(8,1.5);
    \node[align=center] at (8,2.4) {$\LP$ rebalance \\ on pool $L$};

    \draw[->,blue,thick] (9.75,2)--(9.75,1.5);
    \draw[->,blue,thick] (9.75,1.5)--(9.75,0);
    \node[blue, align=center] at (9.75,2.4) {\bfseries Type $\theta_b$ \\ LT};


    \draw[->,blue] (11,2)--(11,1.5);
    \node[blue, align=center] at (11,2.4) {Type $\theta_s$ \\ LT};

    \draw[dotted,thick,red] (11.25,1.5) -- (11.25, 0);
    \node[red, align=left] at (11.75,0.75) {News: \\ $\theta_b$}; 

    \draw[->,red] (12.5,2)--(12.5,1.5);
    \draw[->,red] (12.5,1.5)--(12.5,0);
    \node[red, align=left] at (12.5,2.6) {\textbf{A} trades \\ on both \\ pools};

    \draw[->,thick](14.75,2)--(14.75,1.5);
    \draw[->,thick](14.75,1.5)--(14.75,0);
    \node[align=left] at (14.75,2.6) {$\LP$ rebalance \\ on both \\ pools};

    
\end{tikzpicture}
    \caption{Model timing}
    \label{fig:timing_revised}
\end{figure} 

\subsection{Equilibrium}

Consider the general case of a trader with valuation $v\left(1+\tilde{\theta}\right)$ -- that can be either a private or common value shock. The optimal trade quantity on a pool with liquidity supply $T_k$ and fee $f_k$ solves:
\begin{equation}
    \max_\tau v\left(1+\tilde{\theta}\right) \tau - \left(1+\ell\right)\left(\frac{v T_k^2}{T_k-\tau}-v T_k\right),
\end{equation}
which leads to the optimal trade quantity
\begin{equation}
    \tau^\star= v T_k \max\left\{0,\left(1-\sqrt{\frac{1+f_k}{1+\tilde{\theta}}}\right)\right\}.
\end{equation}
The total revenue for liquidity providers is
\begin{equation}
    f_k\left(\frac{v T_k^2}{T_k-\tau^\star}-v T_k\right)=f_k T_k v \left(\sqrt{\frac{1+\tilde{\theta}}{1+f_k}}-1\right).
\end{equation}
Since the revenue is prorated across all $\LP$ at rates $\frac{q_i}{T_k}$, the revenue for liquidity provider $i$ is proportional to their endoment:
\begin{equation}
    q_i\text{Revenue}\left(f_k,\tilde{\theta}\right)=q_i f_k v \left(\sqrt{\frac{1+\tilde{\theta}}{1+f_k}}-1\right)
\end{equation}

==> Sections/model_advsel.tex <==

\subsection{Model primitives}

Consider the following model of trade in a single token, \textbf{T}, over three periods $t\in\left\{0,1,2\right\}$.  The expected value of the token, $v>0$, is common knowledge.  Three risk neutral trader types consummate trade in this market: a continuum of liquidity providers ($\LP$s), a continuum of liquidity takers ($\LT$s), and informed arbitrageurs ($\A$s). Trade occurs either because arbitrageurs profit from fundamental value changes (\emph{news}) or because liquidity providers and takers have heterogeneous private values for the asset. In particular, liquidity providers have no private value for the token, while liquidity takers value the token at $v\left(1+{\cal I}\Delta\right)$.  Here  $\Delta>0$ are the gains from trade and ${\cal I}$ is an indicator that takes on the value of $1$ if the taker buys and $-1$ if the taker sells.

Liquidity providers differ in their endowments of the token. At $t=0$, each provider $i$ can supply at most $q_i$  of the token, where $q_i$ follows a truncated Pareto distribution on $\left[1,Q\right]$.  So, 
\begin{equation}\label{eq:density}
    \varphi\left(q\right)=\Big(\frac{Q}{Q-1}\Big) \frac{1}{q^2} \; \; \text{ for } q\in\left[1,Q\right].
\end{equation}

\noindent The right skew of the Pareto distribution captures the idea that there are many  low-endowment liquidity providers such as retail traders, but few high-capital $\LP$s such as sophisticated quantitative funds.   Heterogeneity in $\LP$ size is captured by $Q$, where a larger $Q$ naturally corresponds to a larger dispersion of endowments. Given the endowment distribution, collectively $\LP$s  supply at most
\begin{equation}
   S  =   \int_1^Q q \varphi\left(q\right) \diff q = \frac{Q}{Q-1} \log Q
\end{equation}
tokens. 

At $t=1$, two types of exogenous events can occur. With probability $\eta<1$, the common value of the token changes to $v+\sigma$ (good news) or to $v-\sigma$ (bad news); good and bad news are equally likely. Conversely, with probability $\left(1-\eta\right)$ a liquidity trader ($\LT$) receives a private value shock and needs to trade $\tilde{\theta}$ units of the token, where $\tilde{\theta}\sim\text{Uniform}\left[0,\Theta\right]$. The liquidity trader is equally likely to buy or sell the token. We assume the $\LT$s private value is large enough to cover transaction costs on either liquidity pool.

Liquidity demanders and suppliers can interact in two liquidity pools in which token trade occurs against a num\'{e}raire asset (cash).   We assume that the terms of trade are fixed, so that all trades occur at the expected value of the token, $v$. We do this by assuming prices in both pools satisfy a linear bonding curve, so there is no price impact of trade.\footnote{In practice, most decentralized exchanges use convex bonding curves, for example constant product pricing.} So, for a pool with $T$ tokens and $N$ of the num\'{e}raire good, 
\begin{equation}\label{eq:bond_curve}
    vT + N = \text{constant}.
\end{equation}

Fees are levied on liquidity takers  as a fraction of the value of the trade and distributed pro rata to liquidity providers.  The pools have different fees.  One pool charges a low fee, and one pool charges a high fee which we denote $\ell$ and $h$ respectively.  Specifically, to purchase $\tau$ units of the token on the low fee pool, the total cost to a taker is $\tau\left(v+\ell\right)$. The $\LP$s  in the pool receive $\tau\ell$ in fees. 
 

In addition, consistent with gas costs on Ethereum,  any interaction with a liquidity pool (for example, trading or managing liquidity)  incurs a fixed execution cost $\Gamma>0$. 
It is important to note that 
gas fees on decentralized exchanges differ from trading fees on traditional exchanges.  First, they are not set by individual exchanges to compete with each other, but are a common transaction cost \emph{across} trading venues. Second, they are levied on a per-order rather than per-share basis: this implies economies of scale for larger orders. Third, there is significant time variation in gas fees which will allow us to identify the impact of transaction costs on liquidity pool market shares.\footnote{Empirical properties of gas fees are exhibited in \citet{LeharParlour2021}, while \citet{CapponiJia2021}, consider traders who affect the gas price.} 

To ensure that both small and large liquidity traders participate in the market, we assume that the gains from trade are larger than the aggregate transaction cost, including the pool fee and the gas price. 
To rule out trivial cases, we further assume that $Q\ell-\Gamma>0$. The condition ensures that there are at least some liquidity providers who can earn positive expected profit on the low fee pool.

% \paragraph{Assets.} Consider a three-period economy, where time is indexed by $t\in\left\{0,1,2\right\}$. There are two assets, a risky token $\T$ and a riskless num\'{e}raire $\C$. At $t=2$, the risky token $\T$ pays a stochastic dividend $\tilde{v}$ (denominated in units of $\C$). At the start of the game, the expected token value is $\mathbb{E}_0 \tilde{v}=v>1$. 

% \cp{Why dividend as opposed to terminal value?  Why is one token riskless?  Why isn't this just a relative price?}

% The asset $\C$ stands in for cryptocurrencies typically used as num\'{e}raire on decentralized exchanges -- for example Ether (the native currency of the Ethereum blockchain) or stablecoins such as Tether or USD~Coin. The num\'{e}raire pays a risk-free rate of return $r$, which we normalize to zero without loss of generality.

% \cp{I think the para above can just be nuked.}

% \paragraph{Trading environment.} The risky token is traded on two liquidity pools: $L$ (a low-fee pool) and $H$ (a high-fee pool). \cp{The type of fee has not been defined, i.e., fixed, proportional.} The asset quantities in each pool $k\in\left\{L,K\right\}$ must satisfy at all times the following linear bonding curve:
% \begin{equation}\label{eq:bond_curve}
%     v \T_k + \C_k = \text{constant}.
% \end{equation}
% The bonding curve \eqref{eq:bond_curve} implies that the token price is constant and equal to $v$ units of the num\'{e}raire, since $-\frac{\diff T}{\diff C}=v$.\footnote{In practice, most decentralized exchanges use convex bonding curve, for example constant product pricing. While the choice of bonding curve is of first order importance for liquidity demanders who need to split trades to optimize price impact, we argue it is less important for liquidity suppliers. For tractability, we assume a linear bonding curve which implies that liquidity traders only care about pool fees -- the focus of our model. In a richer model with convex pricing, we would expect to see relatively more fragmentation since minimzing price impact might require further splitting trades.} To fix intuition behind the mechanics of the market, suppose a trader wishes to buy $t$ units of the token. This reduces the token amount in the pool to $\T_k-t$. In return, the trader needs to add $\Delta$ units of the num\'{e}raire, where $\Delta$ is such that the new asset quantities remain on the bonding curve, that is:
% \begin{equation}
%     v \left(\T_k-t\right) + \left(\C_k+\Delta\right) = v \T_k + \C_k,
% \end{equation}
% which is equivalent to having $\Delta = v t$. The slope of the bonding curve is equal to the expected value of the asset to ensure there are no arbitrage opportunities at the start of the game. 

% The two liquidity pools charge different fees on liquidity-removing trades. Fees are expressed in units of num\'{e}raire and are distributed to all liquidity providers in a given pool, proportional to the amount of liquidity provided.  The low-fee pool $L$ charges a fee of $f~\C$ where $f<1$, and the high-fee pool $H$ charges a fee of $1~\C$ per token traded. That is, to purchase $t$ units of the token on the $L$ pool, the total cost of an investor is $t\left(v+f\right)$.

% \cp{I'm not sure that the notation is fabulous. Maybe $\ell$ and $h$. Everything will be in terms of $h-\ell$.} \mz{Agreed. What's really key here is the relation between the fees and the size of news.}

\paragraph{Events.} At $t=1$, two types of exogenous events can occur. With probability $\eta<1$, the common value of the token changes to $v+1$ (good news) or to $v-1$ (bad news); good and bad news are equally likely. With probability $\left(1-\eta\right)$ -- that is if news does not occur -- a liquidity trader ($\LT$) receives a private value shock and needs to trade $\tilde{\theta}$ units of the token, where $\tilde{\theta}\sim\text{Uniform}\left[0,\log^{-1}\left(2\right)\right]$. The liquidity trader is equally likely to buy or sell the token. We assume the $\LT$s private value is large enough to cover transaction costs on either liquidity pool.

\cp{This upper bound is ugly. How far can one go with a generic upper bound....The uniform is already quite specific. Also, up and down by an amount $\delta$?.  Maybe for each parameterization find the private value assumption needed.} \mz{The upper bound was chosen to match the aggregate liquidity provision (in an earlier version I had both the upper bound \& aggregate liquidity normalized to one). If $\theta$ can be higher than that, it weakens competition between $\LP$s: if everyone's liquidity executed for sure, then $\LP$s prefer the high-fee pool. So I set the upper bound such that there's always someone who does not get executed.}

\paragraph{Liquidity providers and arbitrageurs.} In addition to liquidity traders, the token is traded by two types of agents: risk-neutral liquidity providers ($\LP$) and arbitrageurs ($\A$). There is a continuum of liquidity providers indexed by $i$, endowed with heterogeneous amounts of the token $T$. Liquidity provider $i$ is endowed with $q_i$ units of the token. Following \citet{KhomynPutninsZoican2022}, we assume that $q_i$ is distributed with density
\begin{equation}\label{eq:density}
    \phi\left(q\right)=\log^{-1}\left(2\right)\frac{1}{q},\text{ for }q\in\left[1,2\right].
\end{equation}
The choice of density ensures that the aggregate token endowment of liquidity providers $\T_\text{agg}$ is normalized to a constant, since
\begin{equation}\label{eq:aggliq}
    \T_\text{agg}=\int_1^2 q_i \phi\left(q_i\right)\diff q_i = \log^{-1} \left(2\right).
\end{equation}
Further, the density is chosen to match key features of the empirical distribution of $\LP$s: there are many low-endowment liquidity providers (e.g., retail traders) and a long tail of high-capital investors who provide liquidity to decentralized exchange -- for example, quantitative institutional investors. Figure \ref{fig:distribution} illustrates the theoretical distribution of $\LP$s endowments.


\cp{Does something like a pareto distribution work or have their liquidity supply as 1+ RV drawn from an exponential?}
\mz{I am not sure. The point here was to have market shares that are linear in the marginal trader's $\qmg$ -- otherwise we don't get a closed form when solving for the fulfilled expectation equilibrium. To have linear market shares, I need $q_i\phi(q_i)$ to be a constant, which means $\phi(\cdot)$ needs to be proportional to $\frac{1}{q_i}$. The ugly log constant term just ensures the density integrates out to one.

$\int_1^{\qmg} q_i \phi\left(q_i\right)\diff q_i = a + b \qmg $}

\begin{figure}[H]
\caption{\label{fig:distribution} Liquidity provider endowment (scaled) $q_i$}
\begin{minipage}[t]{1\columnwidth}%
\footnotesize
This figure illustrates the probability density of liquidity provider token endowments, $\phi\left(\cdot\right)$, as defined in equation \eqref{eq:density}.
\end{minipage}

\vspace{0.05in}

\begin{centering}
\includegraphics[width=0.8\textwidth]{Figures/model_density.png}
\par\end{centering}

\end{figure}

The arbitrageurs $\A$ are risk-neutral speculative traders as in \citet{Budish2015TheResponse} or \citet{Menkveld2017NeedLiquidity}, and have zero private value for the token. Upon observing a common value innovation, arbitrageurs can submit a trade against liquidity providers if (i) liquidity is being offered at a stale price and (ii) it is profitable to take liquidity after taking into account gas costs and pool fees.

\cp{Every arbitrageur since the 1980s has been risk neutral and profit maximizing.  I don't think this warrants citations. }

\paragraph{Gas fee (order execution cost).} Orders submitted at $t=1$ to trade against pool liquidity or to withdraw existing liquidity incur a fixed execution cost $\Gamma>0$. The execution cost can be interpreted as the gas price on the Ethereum blockchain as in \citet{CapponiJia2021}. In contrast to \citet{CapponiJia2021}, we assume traders on the decentralized exchanges are price takers on the gas market and their orders do not impact the gas cost. A natural interpretation is that message volume at any time in a particular asset pair traded on decentralized exchanges is small relative to the aggregate transaction flow on the entire blockchain.

Gas fees on decentralized exchanges differ from trading fees on traditional exchanges in a number of ways. First, they are not set by individual exchanges to compete with each other, but are a common transaction cost \emph{across} exchanges. Second, they are levied on a per-order rather than per-share basis: this implies economies of scale for larger orders. Third, there is significant time variation in gas fees which allows us to better empirically identify the impact of transaction costs on liquidity pool market shares.

\paragraph{Timing.} Figure \ref{fig:timing} summarizes the sequence of events at each time $t$. At $t=0$, liquidity providers arrive at the market and choose to deposit their tokens (and corresponding num\'{e}raire) on either the high- or low-fee liquidity pool. At $t=1$, an exogenous trigger event happens: either news, that is a common value innovation, or a private value shock to liquidity traders. With probability $1-\eta$, a liquidity trader arrives and trades a random quantity $\tilde{\theta}$. Conversely, with probability $\eta$, news arrives which moves the asset value to either $v+1$ or $v-1$. In this case, liquidity providers have a first-mover advantage: they can pay the fixed gas fee $\Gamma$ and withdraw liquidity from the pool to avoid being adversely selected. Following the $\LP$s' choice, arbitrageurs may trade in the direction of the news if profitable to do so. Finally, at $t=2$ all payoffs are realized. 

\begin{figure}[H]
\caption{\label{fig:timing} \textbf{Model timing}}

\vspace{0.1in}
\begin{centering}
\includegraphics[width=0.9\textwidth]{Figures/timing_dex_v2.pdf}
\par\end{centering}

\end{figure}

\cp{Useful to have a variable that captures the extent to which LP can withdraw?  Something like an attention variable. After a news event, they can probabilistically withdraw liquidity if optimal. }

\subsection{Equilibrium \label{sec:eq}}

We solve the game by backward induction. First, we discuss the optimal strategy of arbitrageurs and liquidity traders at $t=1$, taking equilibrium liquidity provision as given. Next, we solve for the optimal liquidity pool choices of $\LP$s at $t=0$. 

\subsubsection{Optimal strategies at \texorpdfstring{$t=1$}{t=1}}

The linear pricing curve ensures that the liquidity trader $\LT$ always trades at the fundamental token value $v$, regardless of the trade size. In contrast to markets with convex bonding curves as described in \citet{LeharParlour2021} or \citet{CapponiJia2021}, there is no price impact on the constant price market. In turn, this implies there is no impermanent loss for liquidity providers following a liquidity trader arrival, and also that no subsequent arbitrage trade is needed to restore prices to the fundamental value. However, even in the absence of price impact, the liquidity trader needs to take into account the liquidity fee difference across the two pools. 

Let $T^\star_L$ and $T^\star_H$ be the equilibrium supply of tokens on liquidity pools $L$ and $H$, respectively. To minimize trading cost, the liquidity trader first submits an order on the low-fee pool. If liquidity on pool $L$ is sufficient to accommodate the demand, that is if $\theta\leq T^\star_L$, then the $\LT$ executes its entire order on $L$. Conversely, if $\theta>T^\star_L$, the liquidity trader exhaust the liquidity supply on $L$ and trades the residual quantity $\theta-T^\star_L$ against liquidity on pool $H$. From equation \eqref{eq:aggliq}, the aggregate liquidity supply is $T^\star_L+T^\star_H=\log^{-1}\left(2\right)$. Since $\theta<\log^{-1}\left(2\right)$, the liquidity trader executes her entire order with probability one and incurs a net cost of $f \times T_L^\star + 1 \times T_H^\star$.
\cp{Where is the gas fee?  How does that work here?} \mz{The implicit assumption is that liquidity traders have a very large private value for $\theta$ units of the asset such that they are willing to pay two gas fees if needed.}

If news occurs and $\LP$s do not withdraw liquidity from the pool, arbitrageurs can trade in the direction on the news to obtain a gross profit of $1~\C$ per token traded (i.e., the size of the news). Concretely, upon good news an arbitrageur deposits $q_{\text{arb},k} v$ units of num\'{e}raire into liquidity pool $k$ and removes $q_{\text{arb},k}$ tokens with a value of $q_{\text{arb},k} \left(v+1\right)$. Further, the arbitrageurs pays the pool fee $f_k$ and the gas fee equal to $\Gamma \diff i$. The net profit from trading $q_{\text{arb},k}$ on liquidity pool $k$ is therefore:
\begin{equation}\label{eq:pi_arb}
    \Pi_\A = q_{\text{arb},k}\left(1-f_k\right)-\Gamma \diff i>0.
\end{equation}
Since the arbitrageur can trade against a mass of liquidity providers and pay an infinitesimal gas price,  $\A$ optimally removes the entire liquidity from pool $L$. However, since the fee on pool $H$ is equal to the size of the news, the arbitrageur never consumes liquidity from pool $H$ for any positive gas fee. The mechanism is similar to the one in \citet{FoucaultMoinasTheissen2007}, where the size of news and the tick size are such that arbitrageurs consume only the liquidity at the best bid or ask. 

\cp{This is worth discussing.  a) Would it make sense to have some sort of inventory costs for arbitrageurs?  This would prevent them from draining one pool completely.  b) Also, why is it important to have no adverse selection on the high fee pool? It would be interesting to have lower, but not no AS.}  \mz{No AS on the high-fee pool is more of a normalization than anything else to simplify the exposition and monitoring choices. Under Christine's notation, it boils down to $\ell<\delta<h$. We can also have $\ell<h<\delta$ (AS on both pools), but I'm not sure if it adds much to consider both cases separately. }

% \begin{ass}\label{ass:gamma}
% \begin{leftbar} \setlength{\parskip}{0ex}
% The gas fee is low enough such that it does not prevent arbitrageurs from trading on any opportunities, that is $\Gamma < 1-f$.
% \end{leftbar}
% \end{ass}

% Assumption \ref{ass:gamma} guarantees that the arbitrageur profit as defined in \eqref{eq:pi_arb} is always positive on liquidity pool $L$, as long as the pool is non-empty. That is, arbitrageurs are willing to trade upon news even if only the lowest-endowment $\LP$ with $\tau_i=\log\left(2\right) \times 1 \diff i$ submits liquidity on pool $L$. Further, since the arbitrageur profit increases in the quantity traded, $\A$ optimally removes the entire liquidity from pool $L$. Finally, since the fee on pool $H$ is equal to the size of the news, the arbitrageur never consumes liquidity from pool $H$ for any positive gas fee. The mechanism is similar to the one in \citet{FoucaultMoinasTheissen2007}, where the size of news and the tick size are such that arbitrageurs consume only the liquidity at the best bid or ask. 

When do liquidity providers withdraw their liquidity? On pool $H$, withdrawing is never optimal since the fee is high enough to deter arbitrageurs which implies adverse selection risk is zero. On pool $L$, liquidity providers with endowment $q_i$ compare the adverse selection cost and the gas fee and withdraw liquidity upon news if and only if
\begin{equation}
    q_i \left(1-f\right)>\Gamma.
\end{equation}
Lemma \ref{lem:t1} summarizes the optimal strategies for all agents at $t=1$.

\begin{lem}\label{lem:t1}
\begin{leftbar} \setlength{\parskip}{0ex}
At $t=1$, the optimal strategies are as follows:
\begin{enumerate}
    \item[(i)] a liquidity trader with a private value shock of size $\theta$ trades $\min\left\{T_L^\star,\theta\right\}$ on pool $L$ and $\max\left\{0,T_L^\star-\theta\right\}$ on pool $H$.
    \item[(ii)] upon news arrival, liquidity providers on pool $L$ pay the gas price and withdraw their liquidity if $\Gamma\leq q_i \left(1-f\right)$. In contrast, liquidity providers on pool $H$ do not attempt to withdraw liquidity upon news.
    \item[(iii)] upon news, arbitrageurs buy (sell) on pool $L$ an amount of tokens equal to the size of the pool. The arbitrageurs does not trade on pool $H$.
\end{enumerate}

\end{leftbar}
\end{lem}

\subsubsection{Liquidity provision at \texorpdfstring{$t=0$}{t=0} \label{sec:liqprov}}

We turn next to the liquidity providers' choice of pool at $t=0$. Let $T_L$ and $T_H$ denote the size of liquidity pools $L$ and $H$, expressed in token units. The expected profit of an $\LP$ with endowment $q_i$ posting liquidity on pool $L$ is
\begin{align}\label{eq:lp_L}
    \pi^\LP_L &= q_i \left(1-\eta\right)\mathbb{E}\left[\min\left\{\frac{\theta}{T_L},1\right\}\right] f  - \eta \min\left\{\Gamma, q_i\left(1-f\right)\right\} \nonumber \\
    &=q_i \left[\left(1-\eta\right)\left(1 - \log 2\frac{T_L}{2}\right) f\right] -\eta \min\left\{\Gamma, q_i\left(1-f\right)\right\},
\end{align}
since
\begin{align}
    \mathbb{E}\left[\min\left\{\frac{\theta}{T_L},1\right\}\right] &= \mathbb{P}\left(\theta\leq T_L\right) \times \mathbb{E}\left[\frac{\theta}{T_L} \mid \theta\leq T_L\right] + \mathbb{P}\left(\theta > T_L\right) \times 1 \nonumber \\
    & = T_L \log 2 \times \frac{1}{2} + \left(1-T_L \log 2\right) = 1 - \log 2\frac{T_L}{2},
\end{align}
where the last equality follows from the fact that $\theta$ is uniformly distributed over $\left[0,\log^{-1} 2\right]$. With probability $1-\eta$, a liquidity trader arrives at $t=1$ and trades $\theta$. If $\theta>T_L$, then the liquidity trader consumes the entire pool and the $\LP$ receives the fee $f$ for each unit of liquidity posted. Conversely, if $\theta\leq T_L$, then the liquidity provider receives a share $\frac{q_i}{T_L}$ of the aggregate fees $\theta f$. With probability $\eta$, news occurs: from Lemma \ref{lem:t1}, the liquidity provider either pays the gas fee $\Gamma$ and withdraws $q_i$ from the pool or does nothing and incurs a loss $q_i\left(1-f\right)$ on the subsequent arbitrage trade.

Alternatively, the $\LP$ can deposit liquidity on pool $H$ and earn expected profit
\begin{align}\label{eq:lp_H}
    \pi^\LP_H &= q_i \left(1-\eta\right) \mathbb{E}\left[\max\left\{0,\frac{\theta-T_L}{T_H}\right\}\right] \nonumber \\
    & = q_i \left(1-\eta\right) \left(1-T_L \log 2\right) \frac{1-T_L \log 2}{2 T_H \log 2},
\end{align}
where the second line follows from explicitly computing the expectation
\begin{align}
    \mathbb{E}\left[\max\left\{0,\frac{\theta-T_L}{T_H}\right\}\right] &= \mathbb{P}\left(\theta\leq T_L\right) \times 0 + \mathbb{P}\left(\theta > T_L\right) \times \frac{\frac{\log^{-1} 2+T_L}{2}-T_L}{T_H} \nonumber \\
    & = \left(1-T_L \log 2\right) \frac{1-T_L \log 2}{2 T_H \log 2}.
\end{align}
If the liquidity trader demand is low enough, that is if $\theta\leq T_L$, then the entire trade is filled on pool $L$ and liquidity providers on $H$ earn nothing. However, if $\theta>T_L$, the residual liquidity demand $\theta-T_L$ is routed to pool $H$ and liquidity providers earn a share proportional to their deposit, i.e., $\frac{q_i}{T_H}$. If news occurs, $\LP$s on $H$ do not incur an adverse selection cost since from Lemma \ref{lem:t1} arbitrageurs do not submit orders to the high-fee pool.


Liquidity providers in the low-fee pool absorb a larger share of the uninformed order flow, since the $\LT$ order is first routed to pool $L$. On the other hand, they face adverse selection costs and may need to pay gas fees $\Gamma$ upon the realization of news to withdraw liquidity. At the same, $\LP$s in the high-fee pool face no adverse selection, receive a larger fee per unit traded, but volume is limited as they only fill the residual demand from uninformed $\LT$s after liquidity on the low-fee pool is exhausted. From equations \eqref{eq:lp_L} and \eqref{eq:lp_H}, liquidity provider $i$ chooses the low-fee pool $L$ if and only if
\begin{equation}\label{eq:cost_comparison}
    \pi^\LP_L>\pi^\LP_H \Longleftrightarrow q_i \frac{\left(1-\eta\right)\left(\left(1-T_L \log 2\right)^2-f T_H \log 2 \left(2-T_L\log 2\right)\right)}{2\log2 T_H} - \eta\min\left\{\Gamma,q_i\left(1-f\right)\right\} > 0.
\end{equation}
A salient implication of equation \eqref{eq:cost_comparison} is that $\LP$s with larger endowments are more likely to choose the low-fee pool, keeping liquidity shares constant. The rationale is that gas fees are a fixed cost, and larger $\LP$s are more likely to achieve economies of scale. The expected fee revenue scales linearly with a liquidity provider's share in the liquidity pool (proportional to $q_i$), better compensating $\LP$s for the gas fee paid upon news arrival at $t=1$. 

We follow \citet{KatzShapiro1985} and conjecture that there exists a marginal liquidity provider $\qmg$ such that all $\LP$s with $q_i>\qmg$ post liquidity on the low-fee pool and all $\LP$s with $q_i\leq \qmg$ choose the high-fee pool.\footnote{We note that there cannot be a ``reversed-sign'' equilibrium, where $\LP$s with $q_i\leq\qmg$ post liquidity on the low-fee pool and all $\LP$s with $q_i>\qmg$ choose the high-fee pool. To understand the rationale, we point out that for an $\LP$ with endowment $\tilde{q}<\qmg$, submitting liquidity to pool $L$ yields a lower expected revenue since
\begin{equation*}
    \pi^\LP_L-\pi^\LP_H=\tilde{q} \frac{\left(1-\eta\right)\left(\left(1-T_L\right)^2-f T_H \left(2-T_L\right)\right)}{2T_H} - \eta\min\left\{\Gamma,q_i\left(1-f\right)\right\} < 0.
\end{equation*}
Therefore, it is optimal for the $\LP$ with endowment $\tilde{q}$ to post liquidity on the high-fee pool, which contradicts the conjectured equilibrium.  Importantly, since each $\LP$ is ``small'' relative to the aggregate mass of liquidity providers, individual deviations do not impact aggregate pool sizes $T_L$ and $T_H$.} The conjectured equilibrium pins down the pool sizes $T_L$ and $T_H$ as a function of the endowment for the marginal $\LP$:
\begin{align}\label{eq:liquidity_levels}
    T_L&=\int_{\qmg}^2 q_i \phi\left(q_i\right) \diff i = \log^{-1}\left(2\right) \left(2 - \qmg\right) \text{ and }\nonumber \\
    T_H&=\int_1^{\qmg}  q_i \phi\left(q_i\right) \diff i = \log^{-1}\left(2\right)\left(\qmg -1\right). 
\end{align}
From equations \eqref{eq:cost_comparison} and \eqref{eq:liquidity_levels} it follows that the expected profit difference between the low- and high-fee pools can be written as a linear decreasing function of the marginal $\LP$'s endowment, that is
\begin{equation}\label{eq:pi_diff}
    \pi^\LP_L-\pi^\LP_H = q_i \left[\frac{1}{2} \left(1-\eta\right) \left(1-\left(1-f\right)\qmg\right)\right] - \eta \min\left\{q_i\left(1-f\right),\Gamma\right\}.
\end{equation}
We search for fulfilled expectation equilibria \citep[following the definition of][]{KatzShapiro1985}, where the beliefs of $\LP$s at $t=0$ about the size of liquidity pools are consistent with the outcome of their choices. We solve \eqref{eq:pi_diff} on the support for $q_i$ -- the interval $\left[1,2\right]$ to obtain the $\LP$ reaction function
\begin{equation}\label{eq:reaction_main}
    \tilde{q}\left(\qmg\right)=\begin{cases}
    1, & \text{ for } \qmg \leq \frac{1-\eta\left(1+2\min\left\{\Gamma,1-f\right\}\right)}{\left(1-f\right)\left(1-\eta\right)}\\
    \frac{2\eta\Gamma}{ \left(1-\eta\right) \left(1-\left(1-f\right)\qmg\right)}, & \text{ for } \qmg \in \left(\frac{1-\eta\left(1+2\min\left\{\Gamma,1-f\right\}\right)}{\left(1-f\right)\left(1-\eta\right)}, \frac{1-\eta\left(1+\Gamma\right)}{\left(1-f\right)\left(1-\eta\right)}\right] \\
    2, & \text{ for } \qmg > \frac{1-\eta\left(1+\Gamma\right)}{\left(1-f\right)\left(1-\eta\right)}.
    \end{cases}
\end{equation}
In any fulfilled expectation equilibrium, the equilibrium endowment of the marginal $\LP$ is a fixed point of equation \eqref{eq:reaction_main}. Figure \ref{fig:reaction} plots the $\LP$ reaction function $\tilde{q}\left(\cdot\right)$ to graphically illustrate equilibrium formation for two parameter choices. Let $q^\star_1$ and $q^\star_2$ be the interior roots of the reaction function \eqref{eq:reaction_main}, that is the solutions of the quadratic form
\begin{equation}
    q-\frac{2\eta\Gamma}{ \left(1-\eta\right) \left(1-\left(1-f\right)q\right)}=0.
\end{equation}
In the top left panel, we illustrate a parameter combination for which are three equilibria, at $\qmg\in\left\{q^\star_1, q^\star_2, 2\right\}$. However, $q^\star_2$ is an unstable equilibrium -- a tipping point \citep[as in][]{Jullien2011} at which small perturbation in beliefs cause the $\LP$s to spiral away from the postulated equilibrium (we refer the reader to the proof of Proposition \ref{prop:equilibria} for a more formal discussion). Consequently, the stable interior equilibrium co-exists with an equilibrium in which all $\LP$s choose pool $H$; this is the case for $f\leq\frac{2}{3}$. The top right panel illustrates a parameter combination for which the stable interior equilibrium coexists with an equilibrium where all $\LP$s provide liquidity on the low-fee pool (for $f>\frac{2\eta}{1+\eta}$).  Finally, the bottom panel illustrates a parameter combination for which there is a unique and stable interior equilibrium at $\qmg=q^\star_1$. 

\begin{figure}[H]
\caption{\label{fig:reaction} Liquidity provider reaction function and equilibria}
\begin{minipage}[t]{1\columnwidth}%
\footnotesize
This figure illustrates equilibrium $\LP$ liquidity pool choices as fixed points of the reaction function $\tilde{q}\left(\qmg\right)=\qmg$. We consider three distinct cases for which a stable interior equilibrium may arise. Stable equilibria are marked with green circles, whereas unstable equilibria are market with magenta squares. Parameter values are $f=0.64$, $G=0.14$, $\eta=0.71$ (top left), $f=0.69$, $G=0.15$, $\eta=0.71$ (top right), $f=0.792$, $G=0.26$, $\eta=0.65$ (bottom).
\end{minipage}

\vspace{0.05in}

\begin{centering}
\includegraphics[width=\textwidth]{Figures/model_reaction_stable.png}
\par\end{centering}

\end{figure}


Proposition \ref{prop:equilibria} establishes conditions under which a fragmented equilibrium exists, wherein both liquidity pools have positive market share. 

\begin{prop}\label{prop:equilibria}
\begin{leftbar} \setlength{\parskip}{0ex}
A stable fragmented equilibrium, in which both liquidity pools have positive market share, exists for $\Gamma\in\left[\underline{\Gamma},\bar{\Gamma}\right)$, where
\begin{align}
    \underline{\Gamma}&=\max\left\{f\frac{1-\eta}{2\eta},\frac{1+\eta(2f-3)}{1-\eta}\right\} \text{ and }     \bar{\Gamma}=\begin{cases} \frac{1-\eta}{8\eta(1-f)} & f \leq 0.75 \\
                           \frac{(2f-1)(1-\eta)}{\eta} & f>0.75 \end{cases}.
\end{align}
The fragmented equilibrium is further unique if $f\in\left[\frac{2}{3},\frac{2\eta}{1+\eta}\right)$ and $\Gamma\in\left[f\frac{1-\eta}{2\eta},\frac{(2f-1)(1-\eta)}{\eta}\right)$. 
In any fragmented equilibrium, the token endowment of the marginal liquidity provider is 
\begin{equation}
    \qmg^\star=\frac{1}{2\left(1-f\right)}-\frac{1}{2\left(1-f\right)}\sqrt{1-\eta\frac{1+8\left(1-f\right)\Gamma}{1-\eta}},
\end{equation}
such that all liquidity providers with $q_i\leq \qmg^\star$ post liquidity on pool $H$, and all liquidity providers with $q_i> \qmg^\star$ post liquidity on pool $L$.
\end{leftbar}    
\end{prop}

Figure \ref{fig:region_gamma} highlights the parameter region where multiple liquidity pools coexist in equilibrium with positive market share.\footnote{We note that the interior equilibrium is not necessarily the unique one. For low fees on pool $L$ ($f\leq\frac{2}{3}$), the interior equilibrium coexists with a corner equilibrium where all traders choose platform $H$. Conversely, for $f>\frac{2\eta}{1+\eta}$, the interior equilibrium coexists with an equilibrium where all traders choose platform $L$.} In particular, an interior equilibrium for which both the $L$ and $H$ pool attract a positive market share emerges for moderate gas fee $\Gamma$ and a small enough difference between liquidity fees on the two pools (i.e., a large $f$). For low values of the gas fee ($\Gamma\leq\underline{\Gamma}$), managing liquidity is cheap: competition effects are strong and all $\LP$s post liquidity on the low-fee pool. For high values of the gas fee ($\Gamma>\bar{\Gamma}$), withdrawing liquidity upon the realization of news is prohibitively expensive and $\LP$s cluster on the high-fee pool where they are protected from adverse selection. For very large gas fees $\Gamma>2\left(1-f\right)$, no $\LP$ optimally reacts upon news -- in this case, multiple single-pool equilibria may emerge where liquidity either clusters on pool $L$ or on pool $H$. 

\begin{cor}\label{cor:monitoring}
\begin{leftbar} \setlength{\parskip}{0ex}
In any interior equilibrium, \emph{all} liquidity providers on $L$ withdraw liquidity upon news.
\end{leftbar}  
\end{cor}

Corollary \ref{cor:monitoring} establishes that there are no $\LP$s in a fragmented equilibrium that do not actively manage liquidity. All low-endowment $\LP$s for whom reacting upon news is not profitable provide liquidity on platform $H$. In contrast, on single-pool equilibria and for $\Gamma>1-f$, only a fraction of liquidity providers withdraw liquidity upon news. Empirically, we would expect a higher share of $\LP$s actively managing liquidity on pool $L$ when multiple pools co-exist in equilibrium than when all trading concentrates on pool $L$.

\begin{figure}[H]
\caption{\label{fig:region_gamma} Parameter regions for which a two-pool equilibrium exists}
\begin{minipage}[t]{1\columnwidth}%
\footnotesize
This figure illustrates the parameter regions for which a fragmented stable equilibrium emerges, in which both pools attract positive market share. The top panel focuses on the case where $\eta=0.65$. We further highlight (in red) the region for which the equilibrium is unique. In the bottom panel, we plot fragmented equilibrium regions for multiple values of $\eta$.
\end{minipage}

\vspace{0.05in}

\begin{centering}
\includegraphics[width=\textwidth]{Figures/region_interior.png}
\par\end{centering}

\end{figure}





% \begin{prop}\label{prop:equilibria}
% \begin{leftbar} \setlength{\parskip}{0ex}
% For ease of notation, we define and tabulate below three gas fee thresholds $\bar{\Gamma}_k$, $k\in\left\{1,2,3\right\}$.

% \begin{center}
%     \begin{tabular}{ccc}
%     \toprule
%     $\bar{\Gamma}_1$ & $\bar{\Gamma}_2$ & $\bar{\Gamma}_3$ \\
%     \cmidrule{1-3}
%     $f\frac{1-\eta}{2\eta}$     &  $\frac{\left(2f-1\right)\left(1-\eta\right)}{\eta}$ & $\frac{1-\eta}{8\left(1-f\right)\eta}$\\
%     \bottomrule
%     \end{tabular}
% \end{center}

% It follows there are has either one, two, or three stable fulfilled expectation equilibria at $t=0$, corresponding to the following $\LP$ liquidity pool choices:
% \begin{enumerate}
%     \item[(i)] An interior equilibrium with marginal $\LP$ characterized by endowment $\qmg^\star=q^\star_1$, such that all $\LP$s with endowment $q>q^\star_1$ add liquidity to the low-fee pool and the rest choose the high-fee pool. The equilibrium emerges for $f\in\left[\frac{1}{2},\frac{3}{4}\right)$ and $\Gamma\in\left(\bar{\Gamma}_1, \bar{\Gamma}_3\right]$ and $f>\frac{3}{4}$ and $\Gamma\in\left(\bar{\Gamma}_1, \bar{\Gamma}_2\right]$. Moreover, the interior equilibrium is unique for $f>\frac{2}{3}$ and $\Gamma\in\left(\bar{\Gamma}_1, \bar{\Gamma}_2\right]$.
%     \item[(ii)] A corner equilibrium where $\qmg^\star=1$, such that all $\LP$s post liquidity on the low-fee pool. The equilibrium emerges for $\Gamma\leq\bar{\Gamma}_1$ and is further unique if $f>\frac{1}{2}$ and $\Gamma\leq\min\left\{\bar{\Gamma}_1,\bar{\Gamma}_2\right\}$.
%     \item[(iii)] A corner equilibrium where $\qmg^\star=2$, such that all $\LP$s post liquidity on the high-fee pool. The equilibrium emerges for $\Gamma>\bar{\Gamma}_2$ and is further unique if $f>\frac{3}{4}$ and $\Gamma>\bar{\Gamma}_2$, $f>\frac{1}{2}$ and $\Gamma>\bar{\Gamma}_3$, or $f\leq\frac{1}{2}$ and $\Gamma>\bar{\Gamma}_1$.
% \end{enumerate}

% \end{leftbar}
% \end{prop}

% Proposition \ref{prop:equilibria} establishes existence conditions for each possible equilibrium. In particular, an interior equilibrium for which both the $L$ and $H$ pool attract a positive market share emerges for moderate gas fee $\Gamma$ and a small enough difference between liquidity fees on the two pools (i.e., a large $f$). The interior equilibrium is unique if the liquidity fees are close enough across the two pools. Figure \ref{fig:regions} highlights the parameter region where multiple liquidity pools coexist with positive market share. 

% The remaining results in Proposition \ref{prop:equilibria} are intuitive: a small gas fee $\Gamma$ reduces the $\LP$s' costs to manage stale liquidity upon news and stimulates competition on the low-fee pool. In other words, the cost of updating liquidity is lower than the opportunity cost of not capturing uninformed trades. In contrast, a large enough $\Gamma$ incentivizes liquidity providers to deposit tokens on the high-fee pool, since managing liquidity on pool $L$ is too costly. 

% \begin{figure}[H]
% \caption{\label{fig:regions} The emergence of two-pool equilibria}
% \begin{minipage}[t]{1\columnwidth}%
% \footnotesize
% This figure illustrates the emergence of two-pool equilibria for different values of the liquidity fee $f$ and gas fee $\Gamma$. We set the probability of informed trading at $\eta=0.85$. We highlight the parameter region for which a two-pool equilibria emerges and is unique (in red) as well as the region for which a two-pool equilibria emerges but is not unique (in blue). 
% \end{minipage}

% \vspace{0.05in}

% \begin{centering}
% \includegraphics[width=0.9\textwidth]{Figures/model_int_eq_region.png}
% \par\end{centering}

% \end{figure}

\subsection{Implications and empirical predictions}

In this section, we zoom in on the properties of the interior equilibrium, that is, the most interesting case featuring segmented liquidity across multiple pools. From Proposition \ref{prop:equilibria}, the only possible interior equilibrium in the liquidity provision game is for a marginal $\LP$ with endowment $\qmg=q_1^\star$.

\begin{pred}\label{pred:clienteles}
\emph{If an interior equilibrium exists where liquidity is segmented across multiple pools, the average liquidity deposit in the low-fee pool is larger than for the high-fee pool.}
\end{pred}

Prediction \ref{pred:clienteles} follows from the discussion in Section \ref{sec:liqprov}. Liquidity providers with large token endowments ($q_i>\qmg$) deposit them in the low-fee pool since they have stronger incentives to pay the gas fee and actively manage the liquidity. Conversely, $\LP$s with lower endowments ($q_i\leq\qmg$) gravitate towards the high-fee pool, accepting a lower trade probability in exchange for reducing adverse selection costs without active liquidity management and paying gas fees.

\begin{pred}\label{pred:updates}
\emph{Liquidity providers on the low-fee pool are more likely to actively manage liquidity.}
\end{pred}
\begin{pred}\label{pred:monitoring_shares}
\emph{Liquidity providers on the low-fee pool are more likely to actively manage liquidity in a fragmented market than in a consolidated market.}
\end{pred}

The two predictions follow from Corollary \ref{cor:monitoring}. In equilibrium, the $\LP$s on the low-fee pool update their liquidity upon news arrival to avoid adverse selection, unlike their counterparts on the high-fee pool. 


\begin{pred}\label{pred:comp_stat_Gamma}
\emph{The liquidity share of the low-fee pool $L$ decreases in the gas fee $\Gamma$.}
\end{pred}
\begin{pred}\label{pred:comp_stat_eta}
\emph{The liquidity share of the low-fee pool $L$ decreases in the probability of informed trading $\eta$.}
\end{pred}

Predictions \ref{pred:comp_stat_Gamma} and \ref{pred:comp_stat_eta} state that the low-fee pool becomes less attractive for liquidity providers if the gas fee increases (higher $\Gamma$) -- making active liquidity management less profitable -- or if the probability of informed trading is higher ($\eta$ increases) which leads to \emph{more frequent} liquidity management. Formally, we can show that $q_1^\star$ increases in both $\Gamma$ and $\eta$ -- leading to a lower value of $T_L^\star$:
\begin{align}
    \frac{\partial q_1^\star}{\partial \Gamma}&=\frac{2 \eta }{\sqrt{(1-\eta ) (\eta  (8 \Gamma  (f-1)-1)+1)}}>0 \text{ and } \nonumber \\
    \frac{\partial q_1^\star}{\partial \eta}&=\frac{2 \Gamma }{(1-\eta) \sqrt{(1-\eta ) (\eta  (8 \Gamma  (f-1)-1)+1)}}.
\end{align}

\begin{pred}\label{pred:trade_volume}
\emph{If an interior equilibrium exists, the trading volume share of the low-fee pool is higher than its liquidity share.}
\end{pred}
The intuition is that $\LP$s on the low-fee pool deposit large token quantities and they absorb a disproportionate amount of incoming trades -- it is possible that $\LP$s on the high-fee pool do not trade at all against incoming orders, despite providing positive liquidity in equilibrium. To formally see the result, we first note that there is no informed trade in equilibrium on either pool. The average $\LT$ trade size on the low-fee pool is
\begin{align}
    \mathbb{E}\left[\min\left\{\theta,T_L^\star\right\}\right]&=\mathbb{P}\left(\theta\leq T_L\right) \mathbb{E}\left[\theta\mid \theta<T_L^\star\right] + \left(1-\mathbb{P}\left(\theta\leq T_L\right)\right) T_L^\star \nonumber \\
    &= T_L^\star\log 2\frac{T_L^\star}{2} + \left(1-T_L^\star\log 2\right) T_L^\star= T_L^\star-\frac{\left(T_L^\star\right)^2}{2}\log 2.
\end{align}
The average $\LT$ trade size on the high-fee pool is
\begin{align}
    \mathbb{E}\left[\max\left\{0,\theta-T_L^\star\right\}\right]& = \left(1-\mathbb{P}\left(\theta\leq T_L\right)\right) \left(\mathbb{E}\left[\theta\mid \theta>T_L^\star\right]-T_L^\star\right)\nonumber \\
    &= \left(1-T_L^\star\log 2\right) \frac{\left(\log^{-1} 2-T_L^\star\right)}{2}=\frac{\log^{-1} 2}{2}-T_L^\star+\frac{\left(T_L^\star\right)^2}{2}\log 2.
\end{align}
We note that the trade share of pool $L$ is equal to $2T_L^\star\log 2-\left(T_L^\star\log 2\right)^2$ which is larger than its liquidity share $T_L^\star\log 2$ since $T_L^\star\log 2<1$. Figure \ref{fig:liqshares} illustrates this result.




\begin{figure}[H]
\caption{\label{fig:liqshares} Liquidity and volume shares}
\begin{minipage}[t]{1\columnwidth}%
\footnotesize
This figure illustrates the relative liquidity and trade volume on the two pools, as a function of the gas fee $\Gamma$. Parameters: $\eta=0.36$ and $f=0.8$.
\end{minipage}

\vspace{0.05in}

\begin{centering}
\includegraphics[width=0.9\textwidth]{Figures/model_compstatics.png}
\par\end{centering}

\end{figure}


\begin{pred}\label{pred:liq_shares}
\emph{The low-fee pool is larger than the high-fee pool (in terms of aggregate deposits) only if the gas fee is low enough, that is if}
\begin{equation}
    \Gamma < \Gamma^\star \equiv \frac{3 (3 f-1) (1-\eta)}{8 \eta }
\end{equation}
\end{pred}

From equation \eqref{eq:liquidity_levels}, if the marginal $\LP$ has endowment $q_1^\star$, then the equilibrium sizes of the two liquidity pools are, respectively,
\begin{align}
    T_L^\star&=\log^{-1}\left(2\right)\left[2- \frac{1}{2\left(1-f\right)} \left(1- \sqrt{1-\eta\frac{1+8\left(1-f\right)\Gamma}{1-\eta}}\right)\right] \text{ and } \nonumber \\
    T_H^\star&=\log^{-1}\left(2\right)\left[\frac{1}{2\left(1-f\right)} \left(1- \sqrt{1-\eta\frac{1+8\left(1-f\right)\Gamma}{1-\eta}}\right)-1\right].
\end{align}


Prediction \ref{pred:liq_shares} translates to stating that $T_L^\star>T_H^\star$, or equivalently to $q_1^\star\leq \frac{3}{2}$, where the latter inequality is true for any $\Gamma\leq\Gamma^\star$. Therefore, even though the low-fee pool attracts the $\LP$s with large token endowments, it is not necessarily the largest pool if the gas fee exceeds a certain threshold. 




==> Sections/model_rebalance.tex <==
Consider the following continuous time model of trade in a single token, \textbf{T}.  The expected value of the token, $v>0$, is common knowledge.  Two risk neutral trader types consummate trade in this market: a continuum of liquidity providers ($\LP$s) and a continuum of liquidity takers ($\LT$s). Trade occurs because 
  market participants have heterogeneous private values for the asset. In particular, liquidity providers have no private value for the token, while liquidity takers value the token at $v\left(1+{\cal I}\Delta\right)$.  Here  $\Delta>0$ are the gains from trade and ${\cal I}$ is an indicator that takes on the value of $1$ if the taker buys and $-1$ if the taker sells. In what follows for expositional simplicity, as in \citet{foucault2013liquidity}, we focus on a one sided market in which liquidity takers act as buyers. 
 
 Liquidity providers differ in their endowments of the token. Each provider $i$ can supply at most $q_i$  of the token, where $q_i$ follows a truncated Pareto distribution on $\left[1,Q\right]$.  So, 
\begin{equation}\label{eq:density}
    \varphi\left(q\right)=\Big(\frac{Q}{Q-1}\Big) \frac{1}{q^2} \; \; \text{ for } q\in\left[1,Q\right].
\end{equation}

\noindent The right skew of the Pareto distribution captures the idea that there are many  low-endowment liquidity providers such as retail traders, but few high-capital $\LP$s such as sophisticated quantitative funds.   Heterogeneity in $\LP$ size is captured by $Q$, where a larger $Q$ naturally corresponds to a larger dispersion of endowments. Given the endowment distribution, collectively $\LP$s  supply at most
\begin{equation}
   S  =   \int_1^Q q \varphi\left(q\right) \diff q = \frac{Q}{Q-1} \log Q
\end{equation}
tokens. 

\begin{comment}

Figure \ref{fig:distribution} illustrates the theoretical distribution of $\LP$s endowments for $Q\in\left\{3,4\right\}$. 

\begin{figure}[H]
\caption{\label{fig:distribution} Liquidity provider endowment $q_i$}
\begin{minipage}[t]{1\columnwidth}%
\footnotesize
This figure illustrates the probability density of liquidity provider token endowments, $\varphi\left(\cdot\right)$, as defined in equation \eqref{eq:density} for $Q\in\left\{3,4\right\}$.
\end{minipage}

\vspace{0.05in}

\begin{centering}
\includegraphics[width=0.8\textwidth]{Figures/model_density.png}
\par\end{centering}

\end{figure} 

\end{comment}


There are two types of liquidity takers: small and large. Small $\LT$s  arrive at the market at constant rate $\theta \diff t$, and each demand one unit of the token. The large $\LT$ arrival time follows a Poisson process with rate $\lambda>0$. Conditional on arrival, a large $\LT$ demands $\Theta$ units of the token, where $\Theta>S$. That is,  the large $\LT$ liquidity demand exceeds the maximum liquidity supply.  Let $D_t$ denote aggregate liquidity demand.  Then,  
\begin{equation}
    \diff D_t = \theta \diff t + \Theta \diff J_t\left(\lambda\right),
\end{equation}
where $J_t\left(\lambda\right)$ is the Poisson arrival process.

Liquidity demanders and suppliers can interact in two liquidity pools in which token trade occurs against a num\'{e}raire asset (cash).   We assume that the terms of trade are fixed, so that all trades occur at the expected value of the token, $v$. We do this by assuming prices in both pools satisfy a linear bonding curve, so there is no price impact of trade.\footnote{In practice, most decentralized exchanges use convex bonding curves, for example constant product pricing.} So, for a pool with $T$ tokens and $N$ of the num\'{e}raire good, 
\begin{equation}\label{eq:bond_curve}
    vT + N = \text{constant}.
\end{equation}
%  It is well known that price impact costs can lead to order splitting and fragmentation. Fixing the terms of trade allows us to focus on how fees affect liquidity supply. 
%  \mz{I think this assumption is actually harmless. Small LTs have no mass, and therefore no price impact. Large LTs have to consume all available liquidity anyway. The one thing that the assumption buys us is that we do not need arbitrageurs to restore the price after a large trader or a sufficiently long sequence of small traders.}
% %\cp{Is it obvious that the equilibrium effect of price impact costs lead to OS and F?  We might need a cite or two here. }

We note in passing that allowing for a bonding curve for which trades have price impact (such as a constant product function) would not materially affect our results. This is because small LTs have no mass, and therefore no price impact, whereas large LTs need to consume all available liquidity. It is well known that price impact costs can lead to order splitting and fragmentation. Fixing the terms of trade allows us to focus on how fees affect liquidity supply. 

Fees are levied on liquidity takers  as a fraction of the value of the trade and distributed pro rata to liquidity providers.  The pools have different fees.  One pool charges a low fee, and one pool charges a high fee which we denote $\ell$ and $h$ respectively.  Specifically, to purchase $\tau$ units of the token on the low fee pool, the total cost to a taker is $\tau\left(v+\ell\right)$. The $\LP$s  in the pool receive $\tau\ell$ in fees. 
 

In addition, consistent with gas costs on Ethereum,  any interaction with a liquidity pool (for example, trading or managing liquidity)  incurs a fixed execution cost $\Gamma>0$. 
It is important to note that 
gas fees on decentralized exchanges differ from trading fees on traditional exchanges.  First, they are not set by individual exchanges to compete with each other, but are a common transaction cost \emph{across} trading venues. Second, they are levied on a per-order rather than per-share basis: this implies economies of scale for larger orders. Third, there is significant time variation in gas fees which will allow us to identify the impact of transaction costs on liquidity pool market shares.\footnote{Empirical properties of gas fees are exhibited in \citet{LeharParlour2021}, while \citet{CapponiJia2021}, consider traders who affect the gas price.} 

To ensure that both small and large liquidity traders participate in the market, we assume that the gains from trade are larger than the aggregate transaction cost, including the pool fee and the gas price. 
To rule out trivial cases, we further assume that $Q\ell-\Gamma>0$. The condition ensures that there are at least some liquidity providers who can earn positive expected profit on the low fee pool.

\begin{ass} The gains from trade are sufficiently large so that all liquidity takers participate in the market, and the fixed costs are sufficiently low so that both pools can attract liquidity. 

\begin{enumerate} 
\item [i.] Gains from trade are sufficiently large $\Delta > h + \frac{\Gamma}{v}$.
\item [ii.] The low fee pool can attract liquidity $Q\ell-\Gamma>0$
\end{enumerate}
\end{ass}


We follow \citet{foucault2013liquidity} and partition the continuous timeline into \emph{liquidity cycles}. A liquidity cycle starts with an empty pool (zero liquidity offered) which triggers $\LP$ token deposits and ends when incoming trades deplete the liquidity supply. The first liquidity cycle starts at $t=0$, and  the sequence of events within a cycle is as follows:  each liquidity provider deposits their token into the high fee pool or the low fee pool and pays the gas cost $\Gamma$, or withdraw from the market. The $\LP$s do not interact with the pool again until the their liquidity is consumed at some random time $\tilde{\tau}$ and the next cycle begins. Figure \ref{fig:timing} illustrates the model timing.



\begin{figure}[H]
\caption{\label{fig:timing} \textbf{Model timing}}

\vspace{0.1in}
\begin{centering}
\includegraphics[width=\textwidth]{Figures/timing_dex_rebalance_v1.pdf}
\par\end{centering}

\end{figure}

\subsection{Discussion \label{sec:model_discussion}}
% \mz{Not 100\% sure where best to place this. A natural place is immediately after the model primitives, to convince a reader our assumptions are reasonable.}

Our model is clearly stylized. First, we assume a linear bonding curve, meaning trades do not have price impact. In reality, decentralized exchanges like Uniswap V3 use convex bonding curves, such as ``constant product'' functions, for which larger trades generate higher price impact. Akin to how limit order markets operate, the price impact of a trade decreases in the liquidity available on high- and low-fee pools, and can therefore vary over time. Second, a linear bonding curve implies that all trades execute at the same price, precluding the need to model the market makers' choice of a price range for providing concentrated liquidity.

Our assumptions significantly streamline the analysis, enabling us to highlight the key economic trade-offs related to the cost structure of liquidity supply. In practice, small orders in both low- and high-fee markets typically have a minimal price impact. Therefore, we assume without loss of generality that small orders are routed to the low fee pool. Large orders, which have a more substantial price impact, are strategically routed in practice across high- and low-fee pools for optimal execution. Figure \ref{fig:routing} offer empirical support for this claim. Using liquidity snapshot data from Kaiko, we compute the optimal routing strategy for trades of different sizes. We show that while small trades are almost fully routed to low-fee pools, large trades are optimally split between low- and high-fee pools.

\begin{figure}[H]
\caption{\label{fig:routing} Optimal order routing on Uniswap v3 pools}
\begin{minipage}[t]{1\columnwidth}%
\footnotesize
This figure displays the optimal order split for purchasing ETH using USDC across various trade sizes, on USDC-WETH Uniswap v3 pools with liquidity fees of 5 and 30 basis points. Order execution is optimized to minimize trading costs, encompassing both price impact and liquidity fees. We use liquidity distribution snapshots data from Kaiko, and focus on the last Ethereum block of each day from May 4, 2021, to July 15, 2023.
\end{minipage}

\vspace{0.05in}

\begin{centering}
\includegraphics[width=\textwidth]{Figures/Empirics_202308/optimal_routing.png}
\par\end{centering}

\end{figure}

Large orders in our model also trade on both pools. For simplicity, we assume they are routed sequentially across markets: first on the low- and then on the high-fee pool. Further, we assume that the large trader depletes liquidity in the high fee pool. This assumption mirrors the modelling approach in \citet{foucault2013liquidity}, where a limit order book cycles between ``empty'' and ``full'' states.  
The economic mechanism we aim to illustrate is that due to the routing of liquidity demand across pools, market makers in high-fee pools need to adjust their liquidity less frequently than those in low-fee pools, resulting in reduced fixed costs over time.

We streamlined liquidity demand in our model to better focus on the effect of fixed and variable costs on liquidity supply. A richer model with realistic price impact functions would need to account for the optimal order splitting across pools with different liquidity fees. This would add mathematical complexity to the model without necessarily bringing new insight on the economics of liquidity supply. Similar to the theoretical literature on limit order markets \citep{Parlour1998,Foucault1999,rocsu2009dynamic}, restrictive assumptions are required to obtain analytical solutions.  Our approach ensures a tractable framework that produces clear predictions to direct our empirical analysis. 




\subsection{Equilibrium}\label{sec:liqprov}

First, consider the liquidity traders' decisions. Faced with pool sizes of $\mathcal{L}_\ell$ and $\mathcal{L}_h$ in the low and high pool respectively, they choose the pool which minimizes their trading costs.  Conditional on trading, the small liquidity takers choose the $\ell$ fee pool.  Thus, small traders arrive at the $\ell$ fee pool at rate $\theta$, and each trade one unit.  By assumption the large liquidity taker wants to trade more than the posted liquidity and exhausts both pools.  Thus, liquidity is consumed on the low fee pool at rate $\frac{\theta}{\mathcal{L}_\ell} \diff t$, while liquidity is only consumed on the high fee pool if a large trader arrives. Once each pool is empty, liquidity providers refill it and restart the cycle. Let $d_k, k=\ell,h$ denote the duration of a liquidity cycle on the low and high pool respectively. Then, the expected duration of a cycle on the low fee pool is 
\begin{align}
    d_\ell &=e^{-\lambda \frac{\LL}{\theta}} \frac{\LL}{\theta}+\int_{0}^{\frac{\LL}{\theta}} t\lambda e^{-\lambda t}\diff t =\frac{1}{\lambda}-\frac{1}{\lambda}e^{-\frac{\LL}{\theta}\lambda},
    \end{align}
\noindent while the expected duration on a high fee pool is $d_h=\frac{1}{\lambda}.$  Thus,


\begin{lem}\label{lem:duration}
 \setlength{\parskip}{0ex}
The expected duration of a liquidity cycle is shorter in the low fee pool than the high feel pool. Or, $d_\ell<d_h$.
\end{lem}

Lemma \ref{lem:duration} is intuitive.  A liquidity cycle on the high fee pool only ends with the arrival of a large trader.   Conversely, a liquidity cycle on the low fee pool ends either because a large liquidity taker arrived or the cumulative small liquidity trader orders exhaust the pool. 

Notice that the low fee pool provides liquidity for a large share of the order flow, as both small and large $\LT$s trade there. However, the liquidity providers on that pool earn a low fee per traded unit. Additionally, as the expected cycle duration is shorter, they need to manage their liquidity more often, which leads to larger gas costs per unit of time. Liquidity providers face a choice between the low and high fee pool or not participating in the market. Thus, an \LP of size $q_i$ chooses between:

\begin{equation}\label{eq:optimal_pool}
  \max \Big[\frac{q_i \ell - \Gamma}{d_\ell} , \; \frac{q_i h -\Gamma}{d_h}, \; 0\Big].
\end{equation}

\noindent First, consider the choice between pools.  Rearranging Equation \ref{eq:optimal_pool}, liquidity provider $i$ chooses the low-fee pool  if and only if
\begin{equation}\label{eq:cost_comparison}
    \left(d_h \ell - d_\ell h\right) q_i> \Gamma \left(d_h-d_\ell\right).
\end{equation}

Equation \ref{eq:cost_comparison} highlights the tradeoff between the expected fee revenue per unit time and the fixed cost of accessing the market. 
If $\frac{h}{d_h}>\frac{\ell}{d_\ell}$,  then  the expected liquidity fee per unit of time on the high fee pool is larger than that of the low fee pool, and  the left hand side of Equation \ref{eq:cost_comparison} is negative.  From Lemma \ref{lem:duration}, the expected duration is higher on the high fee pool and the right hand side is always positive.  In this case,  all liquidity providers choose the high fee pool.
The more natural case to consider is if $\frac{h}{d_h}<\frac{\ell}{d_\ell}$ so that 
 liquidity providers face a trade-off between a higher liquidity fee per unit of time on the low fee pool against lower gas costs on the high fee pool. Clearly, the larger a liquidity providers' endowment, the more important is the fee revenue.  We have

 \begin{lem}\label{lem:sort} For any liquidity pools, $\{\mathcal{L}_\ell, \mathcal{L}_h\}$, for which $\frac{h}{d_h}<\frac{\ell}{d_\ell}$, if a liquidity provider of size $q$ prefers the low fee pool, then any liquidity provider with a larger endowment,  $\widetilde{q}>q$, also prefers the low fee pool.
 \end{lem}

 Now consider the choice of participating in the market.  An agent  only provides liquidity if she is able to break even on the high-fee pool -- that is, if her endowment $q_i$ is large enough. The participation constraint follows from equation \eqref{eq:optimal_pool}:
\begin{equation}\label{eq:pc}
    q_i h - \Gamma \geq 0.
\end{equation}

Define $\underline{q}=\frac{\Gamma}{h}$.  Recall, that the lower bound of the Pareto distribution is 1.  Thus, if $\frac{\Gamma}{h}>1$,  all $\LP$s with $q_i>\underline{q}$ enter the market, and the marginal entrant earns zero expected profit. Conversely, if $\frac{\Gamma}{h}\leq 1$,  liquidity provision is not competitive; all $\LP$s enter the market and earn strictly positive profits.
 
 

Following Lemma \ref{lem:sort}, let $\qmg$  be the threshold endowment such that all $\LP$s with $q_i>\qmg$ post liquidity on the low-fee pool and all $\LP$s with $q_i\leq \qmg$ choose the high-fee pool. 
This allows us to characterize pool sizes
$\LL$ and $\LH$ as a function of the endowment for the marginal $\LP$:
\begin{align}\label{eq:liquidity_levels}
    \LL&=\int_{\qmg}^Q q_i \varphi\left(q_i\right) \diff i = \frac{Q}{Q-1}\left(\log Q - \log \qmg \right)  \text{ and }\nonumber \\
    \LH&=\int_{\underline{q}}^{\qmg}  q_i \varphi\left(q_i\right) \diff i = \frac{Q}{Q-1}\left(\log \qmg - \log \underline{q}\right)
\end{align}
From equations \eqref{eq:cost_comparison} through \eqref{eq:liquidity_levels} it follows that the expected profit difference between the low- and high-fee pools can be written as an increasing function of the marginal $\LP$'s endowment, that is
\begin{align}\label{eq:pi_diff}
    \pi_\ell-\pi_h &=\frac{1}{\lambda d_h d_\ell}\left[\exp\left(-\frac{\lambda}{\theta} \LL\right) \underbrace{\left(q_i h - \Gamma\right)}_{>0} - q_i\left(h-\ell\right)\right] \nonumber \\
        &=\frac{1}{\lambda d_h d_\ell}\left[\qmg^{\frac{\lambda}{\theta}\frac{Q}{Q-1}} \times Q^{-\frac{\lambda}{\theta}\frac{Q}{Q-1}} \underbrace{\left(q_i h - \Gamma\right)}_{>0}- q_i\left(h-\ell\right)\right]. 
\end{align}
 Proposition \ref{prop:equilibria} characterizes the equilibrium liquidity provision.

\begin{prop}\label{prop:equilibria}
%\begin{leftbar} \setlength{\parskip}{0ex}
%\emph{(Fragmentation)} 
\begin{enumerate}
    \item [i.]
If $\frac{h-l}{h} Q^{\frac{\lambda}{\theta}\frac{Q}{Q-1}}<1$ and $\frac{\Gamma}{h}<1-\frac{h-l}{h} Q^{\frac{\lambda}{\theta}\frac{Q}{Q-1}}$, then  all $\LP$s deposit liquidity on the low fee pool. 
\item[ii.]If $\Gamma>Q\ell$, then all $\LP$s deposit liquidity on the high fee pool. 
\item [iii.] Otherwise, there exists a unique fragmented equilibrium characterized by marginal trader $\qmg^\star$ which solves
\begin{equation}\label{eq:mg_eq}
    \qmg^\star = \Gamma \frac{\qmg^{\frac{\lambda}{\theta}\frac{Q}{Q-1}} \times Q^{-\frac{\lambda}{\theta}\frac{Q}{Q-1}}}{h\left[\qmg^{\frac{\lambda}{\theta}\frac{Q}{Q-1}} \times Q^{-\frac{\lambda}{\theta}\frac{Q}{Q-1}}\right]-\left(h-\ell\right)} \in \left[\underline{q},Q\right]
\end{equation}
such that all $\LP$s with $q_i\leq \qmg^\star$ deposit liquidity in the high fee pool and all $\LP$s with $q_i>\qmg^\star$ choose the low fee pool.
\end{enumerate}
%\end{leftbar}    
\end{prop}

Figure \ref{fig:region_equilibrium} illustrates the equilibrium regions in Proposition \ref{prop:equilibria}. If the gas price is low and $\LP$s are homogeneous (low $\Gamma$ and $Q$), then all liquidity providers choose the low fee pool because  managing liquidity is relatively cheap. If more high-endowment $\LP$s enter the market (i.e., there is an increase in $Q$) the more liquidity is posted the low fee pool.  Keeping the $\LT$ arrival rate fixed, a larger pool depletes more slowly and thus the liquidity cycle on the pool becomes longer. As a consequence, the liquidity fee per unit of time on pool $L$ drops and smaller $\LP$s switch to the high-fee pool. As a result, liquidity becomes fragmented across the two pools. 

\begin{figure}[H]
\caption{\label{fig:region_equilibrium} Fragmented and single-pool equilibria}
\begin{minipage}[t]{1\columnwidth}%
\footnotesize
This figure plots the existence conditions for a fragmented market equilibrium, as described in Proposition \ref{prop:equilibria}, for various values of gas cost ($\Gamma$) on the y-axis and liquidity endowment $Q$ on the x-axis. Parameter values: $h=1$, $\ell=0.75$, $\lambda=0.5$ $\theta=0.66$.
\end{minipage}

\vspace{0.05in}

\begin{centering}
\includegraphics[width=\textwidth]{Figures/equilibrium_existence.png}
\par\end{centering}

\end{figure}

An equilibrium in which all liquidity consolidates on the high fee pool is only sustainable for very high gas costs $\Gamma>Q\ell$. In this case,  none of the $\LP$s breaks even on pool $L$. For intermediate values of gas price, both pools co-exist  with positive market share.

Proposition \ref{cor:comp_stat_ms} establishes comparative statics for the two pools' liquidity market shares. From equation \eqref{eq:liquidity_levels}, we can compute the liquidity market share of the low-fee pool at the beginning of each cycle as
\begin{equation}
w_\ell=\frac{\LL}{\LL+\LH}=\frac{\log Q - \log \qmg^\star}{\log Q - \log \underline{q}}.
\end{equation}

\begin{prop}\label{cor:comp_stat_ms}
%\begin{leftbar} \setlength{\parskip}{0ex}
 In equilibrium, the market share of the low fee pool $w_\ell$
\begin{itemize}
    \item[i.] decreases in the gas cost ($\Gamma$), the arrival rate of large trades ($\lambda$), and the fee on pool $H$ (h).
    \item[ii.] increases in the fee on pool $L$ ($\ell$) and the arrival rate of small trades ($\theta$)
\end{itemize}
%\end{leftbar}    
\end{prop}

The results in Proposition \ref{cor:comp_stat_ms} are intuitive. The market share of the low fee pool increases if the fee gap $h-\ell$ is narrower, since this reduces $\LP$ incentives to switch to the high-fee pool. If the small $\LT$ arrival rate is large, then liquidity cycles in the low-fee pool are shorter, increasing the revenue per unit of time and consequently the market share of pool $L$. Conversely, if large trades arrive more often (high $\lambda$), then the high fee pool attracts a higher share of incoming order flow and becomes more appealing for liquidity providers.

Figure \ref{fig:liqshares} shows that the market share of the low fee pool (weakly) decreases in the gas cost $\Gamma$. A larger gas price increases the costs of active liquidity management, everything else equal, and incentivizes smaller $\LP$s to switch from the low fee pool to the high fee pool, since the latter has a lower turnover. For $\Gamma\leq h$, any increase in gas costs leads to a \emph{redistribution} of liquidity from one pool to another; the aggregate liquidity across both pools is constant since all $\LP$s participate in the market.

\begin{figure}[H]
\caption{\label{fig:liqshares} Liquidity shares and gas costs}
\begin{minipage}[t]{1\columnwidth}%
\footnotesize
This figure illustrates the equilibrium liquidity market shares (left panel) and absolute liquidity deposits on the two pools (right panel), as a function of the gas fee $\Gamma$. Parameter values: $h=1$, $\ell=0.75$, $\lambda=0.5$, $\theta=0.66$, $Q=3$, and $\Gamma=1$.
\end{minipage}

\vspace{0.05in}

\begin{centering}
\includegraphics[width=\textwidth]{Figures/mkt_share_gas.png}
\par\end{centering}

\end{figure}

If gas prices increase beyond a threshold ($\Gamma>h$), then the aggregate liquidity falls since $\LP$s with $q_i<\frac{\Gamma}{h}$ are shut out of the market. Both the low and high fee pool experience a decrease in liquidity deposits. However, the liquidity drop is sharper for the low fee pool which further depresses its market share.

\subsection{Pool fragmentation and market quality}


In our model, liquidity takers incur two main costs beyond gas prices: pool fees, which represent the cost of taking liquidity, as well as foregone gains from trade if liquidity providers do not fully participate in the market. To integrate these costs into a single measure of market quality, we use an \emph{implementation shortfall} metric, following \citet{Perold_1988}. If the asset is traded on a sequence of pools, where $f_k$ and $\mathcal{L}_k$ represent the fees and liquidity deposits on pool $k$, respectively, the implementation shortfall (IS) for a large $\LT$ is defined as
\begin{equation}\label{eq:IS_general}
    \text{IS}\left(\left\{f_k\right\}_k\right)=\underbrace{\sum_k f_k \mathcal{L}_k}_\text{trading fees} + \underbrace{\Delta \left(\Theta - \sum_k \mathcal{L}_k\right)}_\text{unrealized gains},
\end{equation}
where $\Theta - \sum_k \mathcal{L}_k$ is the difference between the $\LT$ trading demand and the cumulative liquidity available across all pools, and  $\Delta$ is  the per-unit gains from trade.

Suppose an asset is traded on a single pool that imposes a liquidity fee $f$. From equation \eqref{eq:IS_general} it follows that the implementation shortfall on this pool is:
\begin{align}
    \text{IS}\left(\left\{f\right\}\right)&= f \int_{\frac{\Gamma}{f}}^{Q}  q_i \varphi\left(q_i\right) \diff i + \Delta \left(\Theta - \int_{\frac{\Gamma}{f}}^{Q}  q_i \varphi\left(q_i\right) \diff i\right).
\end{align}
Here, the magnitude of the liquidity fee drives the trade-off between the participation of liquidity providers (\(\LP\)) and trading costs. A lower fee \( f \) results in fewer \(\LP\)s offering liquidity, leading to increased unrealized gains. In contrast, a higher fee increases trading costs, potentially outweighing the benefits of increased \(\LP\) participation. 

The trade-off is illustrated in the left panel of Figure \ref{fig:is}. The optimal fee \( f^\star \) that minimizes the single-pool implementation shortfall is equal to \( f^\star = g W^{-1}\left({\rm e}\frac{g Q}{\Gamma }\right) \), where \( W(\cdot) \) represents the Lambert function.

\begin{prop}\label{prop:optimality}
For any single-pool fee $f\geq 0$, there exists a set of fees \( \{h, \ell\} \) for a two-pool fragmented market, where \( h = f \) and \( h > \ell \), that guarantees an equal or reduced implementation shortfall in a fragmented market compared to the single-pool market. \\ Furthermore, when $f>\frac{\Gamma}{Q}$, the fee structure \( \{h, \ell\} \) can be chosen to ensure a strictly lower implementation shortfall in the fragmented market.
\end{prop}


Proposition \ref{prop:optimality} suggests that fragmentation with multiple fee levels improves market quality. Specifically, it is always possible to devise a fee structure in a fragmented market that yields a (weakly) lower implementation shortfall than a single-fee market. The logic is as follows: First, the highest fee in the fragmented market is set equal to the single pool fee, ensuring that the marginal $\LP$ participating the market is the same across both scenarios (i.e., the $\LP$ with endowment $\underline{q}=\frac{\Gamma}{f}$). This condition guarantees the same level of realized gains from trade in fragmented and non-fragmented markets. Second, a lower fee is then chosen for another pool to attract liquidity providers with higher token endowments, resulting in lower trading costs. This combination of reduced trading costs and unchanged gains from trade leads to a lower implementation shortfall in a fragmented market. 

\begin{figure}[H]
\caption{\label{fig:is} Implementation shortfall and market structure}
\begin{minipage}[t]{1\columnwidth}%
\footnotesize
The left panel plots the implementation shortfall for large liquidity traders on a single pool, as a function of the pool fee $f$. The right panel plots the implementation shortfall for large liquidity traders on both single and fragmented pools as a function of the gas cost $\Gamma$. The single pool fee is set to the optimal level $f^\star$, whereas the fragmented pool fee menu is set to $\left(h,\ell\right)=\left(f^\star, \frac{1}{2}f^\star\right)$.
\end{minipage}

\vspace{0.05in}

\begin{centering}

\includegraphics[width=\textwidth]{Figures/Empirics_202308/implementation_shortfall.png}


\par\end{centering}

\end{figure}

\begin{cor}\label{cor:optimality}
There exists a fee menu in a two-pool fragmented market structure that achieves an equal or lower implementation shortfall than on any single-fee pool configuration. Further, the fee menu can be chosen to achieve strictly lower implementation shortfall in fragmented markets if $f^\star=g W^{-1}\left({\rm e}\frac{g Q}{\Gamma }\right)>\frac{\Gamma}{Q}$.
\end{cor}

Corollary \ref{cor:optimality} emerges as a particular case of Proposition \ref{prop:optimality}, with the assumption that the single-pool operates at its optimal fee level. In essence, if a fragmented fee structure can be designed to achieve a lower implementation shortfall compared to an arbitrary single-pool fee, then a fee structure that dominates the optimally set single-pool fee achieves a lower implementation shortfall than any single-fee pool. 

The right panel of Figure \ref{fig:is} illustrates the scenario where the lower fee in a fragmented market is set to half the optimal fee of a single pool, denoted as \( \ell = \frac{1}{2}f^\star \). When gas prices are sufficiently low, $\LP$s with large endowments choose to provide liquidity on the low-fee pool, leading to reduced trading costs and, consequently, a lower implementation shortfall. As gas prices increase, the implementation shortfall rises in both single-pool and fragmented markets, primarily because more $\LP$s are priced out which results in higher unrealized gains. Additionally, the shortfall increases more rapidly with rising gas prices in the fragmented market as $\LP$s switch over from the low- to the high-fee pool --- that is, the result in Proposition \ref{cor:comp_stat_ms}. At very high gas prices, all $\LP$s converge in the high-fee pool, effectively collapsing the fragmented market into a single pool with the optimal fee level.








\subsection{Model implications and empirical predictions}

\begin{pred}\label{pred:comp_stat_Gamma}
The liquidity market share of the low-fee pool  decreases in the gas fee $\Gamma$.
\end{pred}

Prediction \ref{pred:comp_stat_Gamma} follows directly from Proposition \ref{cor:comp_stat_ms} and Figure \ref{fig:liqshares}. A higher gas price increases the fixed cost of active liquidity management, particularly so for smaller liquidity providers. In response, $\LP$s with lower endowments migrate to the high-fee pool  where they trade less often. 

\begin{pred}\label{pred:clienteles}
$\LP$s on the low-fee pool make larger liquidity deposits than $\LP$s on the high-fee pool.
\end{pred}

Prediction \ref{pred:clienteles} follows from the equilibrium discussion in Section \ref{sec:liqprov}. Liquidity providers with large token endowments ($q_i>\qmg$) deposit them in the low-fee pool since they are better positioned to actively manage liquidity due to economies of scale. $\LP$s with lower endowments ($q_i\leq\qmg$) either stay out of the market or choose pool $H$ which allows them to offer liquidity in a more passive manner.

\begin{figure}[H]
\caption{\label{fig:theory_liqsupply} Liquidity supply on fragmented markets}
\begin{minipage}[t]{1\columnwidth}%
\footnotesize
This figure illustrates equilibrium liquidity supply on a fragmented market. We simulate 100,000 liquidity endowments from the truncated Pareto distribution in \eqref{eq:density}. The top panel illustrates the simulated distributions: $\LP$s to the left (right) of the marginal trader $\qmg^\star$ provide liquidity on pool $H$ (pool $L$, respectively). The bottom left panel shows the gap in average liquidity deposits for $\LP$s participating on the two pools. The bottom right panel shows the gap in the number of $\LP$s participating on the two pools. Parameter values: $h=1$, $\ell=0.75$, $\lambda=0.5$, $\theta=0.66$, $Q=3$, and $\Gamma=1$.
\end{minipage}

\vspace{0.05in}

\begin{centering}
\includegraphics[width=\textwidth]{Figures/liquidity_supply.png}
\par\end{centering}

\end{figure}

Figure \ref{fig:theory_liqsupply} illustrates this prediction through a Monte Carlo simulation. We plot the equilibrium liquidity supply decisions of 100,000 $\LP$s with endowments drawn from density \eqref{eq:density} and $Q=3$. The top panel highlights three groups of liquidity providers: low-endowment $\LP$s (in green) that are being rationed out of the market due to high gas cost, medium-endowment $\LP$s (blue) that deposit liquidity on pool $H$, and high-endowment $\LP$s (orange) that choose the low-fee pool $L$. 



\begin{pred}\label{pred:trade_size_volume}
The average trade size is higher on pool $H$ than on pool $L$. At the same time, trading volume is higher on pool $L$ than on pool $H$.
\end{pred}

Next, Prediction \ref{pred:trade_size_volume} deals with differences between incoming trades on the two liquidity pools. For a wide range of model parameters, incoming order flow on the low fee pool consists of a large number of small trades, and occasional large trades. In contrast, there are few trades on the high fee pool, but they are all relatively large. The model can therefore reconcile two apparently conflicting patterns: one liquidity pool captures most of the trading volume, while the largest trades are executed on the competitor. Figure \ref{fig:theory_trade} illustrates the prediction through a Monte Carlo simulation of the model.


\begin{figure}[H]
\caption{\label{fig:theory_trade} Trade volume and trade size on fragmented markets}
\begin{minipage}[t]{1\columnwidth}%
\footnotesize
The left panel illustrates the average trading volume per unit of time in both pools, using 100,000 Monte Carlo simulations with a discrete time increment of $\Delta t=0.1$. The right panel illustrates the average trade size on a given liquidity pool, conditional on having a non-zero volume in the discrete time interval $\Delta t$. If a large liquidity trader arrives, it depletes both pools -- i.e., she trades amounts $\LL$ and $\LH$ on the low- and high-fee pools, respectively. Parameter values: $h=1$, $\ell=0.75$, $\lambda=0.5$, $\theta=0.66$, $Q=3$, and $\Gamma=1$.
\end{minipage}

\vspace{0.05in}

\begin{centering}
\includegraphics[width=\textwidth]{Figures/trade_volumesize.png}
\par\end{centering}

\end{figure}


\begin{pred}\label{pred:clienteles_cs}
The average liquidity deposit on both the low- and- high fee pool increases with gas costs.
\end{pred}

An increase in the gas cost $\Gamma$ has two effects: first, the $\LP$s with the lowest endowments on pool $L$ switch to pool $H$. As a result, the average deposit on pool $L$ increases. Second, the $\LP$s with low endowments on pool $H$ may leave the market. Both channels translate to a higher average deposit on pool $H$, which experiences an inflow (outflow) of relatively high (low) endowment $LP$ following an increase in gas costs.



The bottom left panel highlights the clientele effect: that is, the average deposit is higher on pool $L$. Due to the skew of the Pareto distribution, however, there are more $\LP$ accounts active on pool $H$ than on pool $L$ for a wide range of parameter values.



\begin{pred}\label{pred:updates}
$\LP$s update liquidity more frequently on the low-fee than on the high-fee pool.
\end{pred}

Prediction \ref{pred:updates} is a consequence of Lemma \ref{lem:duration}. Liquidity cycles on pool $L$ are shorter than on pool $H$, since $\LP$s on the low-fee pool trade against both small and large orders, rather than only against large orders on the high-fee pool. Consequently, we expect $\LP$s on pool $L$ to actively manage their liquidity positions.


\begin{pred}\label{pred:updates_gas}
A larger gas price leads to more frequent liquidity updates on the low-fee pool.
\end{pred}
An increase in gas price leads to some $\LP$s switching from the low- to the high-fee pool. As a result, liquidity supply on the low-fee pool drops, leading to a shorter cycle as incoming order flow depletes the pool at a faster pace.



==> Sections/sketch_model_AS.tex <==
\paragraph{Asset.} Consider a continuous time model of trade in a single token $\T$ with expected value $v_t>0$. Common value innovations (``news'') arrive as Poisson process with rate $\eta>0$. News is equally likely to be positive or negative. The absolute size of news is uniformly distributed between $\left[0,\sigma\right]$.\footnote{\mz{I added a distribution of news sizes so there is more arbitrage activity on low-fee pools than on high-fee pools. I.e., arbitrageurs go to the low-fee pool only if $\ell\leq\text{news size}<h$.}} Three risk-neutral trader types trade in this market: a continuum of liquidity providers ($\LP$s), a continuum of liquidity takers ($\LT$s), and arbitrageurs ($\A$). 

\paragraph{Trading environment.} Traders can interact in two liquidity pools in which token trade occurs against a num\'{e}raire asset (cash).   We assume that the terms of trade are fixed, so that all trades occur at the expected value of the token, $v$. We do this by assuming prices in both pools satisfy a linear bonding curve, so there is no price impact of trade.\footnote{In practice, most decentralized exchanges use convex bonding curves, for example constant product pricing.} So, for a pool with $T$ tokens and $N$ of the num\'{e}raire good, 
\begin{equation}\label{eq:bond_curve}
    vT + N = \text{constant}.
\end{equation}
Fees are levied on liquidity takers  as a fraction of the value of the trade and distributed pro rata to liquidity providers.  The pools have different fees.  One pool charges a low fee, and one pool charges a high fee which we denote $\ell$ and $h$ respectively.  Specifically, to purchase $\tau$ units of the token on the low fee pool, the total cost to a taker is $\tau\left(v+\ell\right)$. The $\LP$s  in the pool receive $\tau\ell$ in fees. In addition, consistent with gas costs on Ethereum,  liquidity providers incur a fixed execution cost $\Gamma>0$ to interact with the market.

\paragraph{Liquidity providers.}  Liquidity providers ($\LP$) differ in their endowments of the token. Each provider $i$ can supply at most $q_i$  of the token, where $q_i$ follows a log-uniform distribution on $\left[1,Q\right]$.  So, 
\begin{equation}\label{eq:density}
    \varphi\left(q\right)=\Big(\frac{1}{\log{Q}}\Big) \frac{1}{q} \; \; \text{ for } q\in\left[1,Q\right].
\end{equation}

\noindent The right skew of the log-uniform distribution captures the idea that there are many  low-endowment liquidity providers such as retail traders, but few high-capital $\LP$s such as sophisticated quantitative funds.   Heterogeneity in $\LP$ size is captured by $Q$, where a larger $Q$ naturally corresponds to a larger dispersion of endowments. Given the endowment distribution, collectively $\LP$s  supply at most
\begin{equation}
   S  =   \int_1^Q q \varphi\left(q\right) \diff q = \frac{Q-1}{\log Q} 
\end{equation}
tokens. 

\paragraph{Liquidity takers.} Liquidity takers ($\LT$) arrive at the market following a Poisson process with unit rate.\footnote{\mz{This is WLOG, since what matters is the ratio between news and $\LT$ arrival rates, which can be controlled through $\eta$.}} \mz{The $\LT$s arrive in pairs, that is a buyer followed by an symmetrical seller.} The assumption captures ``reversal arbitrage'' as in \citet{LeharParlour2021} without the need to explicitly model price impact: that is, the pool remains balanced upon the arrival of uninformed trade flow and no rebalancing is required.

There are two types of liquidity takers: small and large. Small $\LT$s represent a fraction $1-\lambda$ of liquidity traders. Small $\LT$s have a private value $\delta\in\left[\ell,h\right)$ such that they trade on low-fee pools but not high-fee pools. Conditional on arrival, the demand from small $\LT$s is uniformly distributed between $\left[0,\theta\right]$. Large $\LT$s represent a fraction $\lambda$ of liquidity traders and have a private value $\Delta>h$ for the asset. Conditional on arrival, a large $\LT$ demands $\Theta$ units of the token, where $\Theta>S$.


\paragraph{Arbitrageurs.} Arbitrageurs trade on common value innovations by depleting the liquidity pools as long as the size of news is larger than the pool fee. Unlike liquidity trades, arbitrageur trades are not reversed and trigger costly re-balancing from liquidity providers.

Figure \ref{fig:timing_revised} illustrates the timing of the model.

\begin{figure}[H]
    \centering
\begin{tikzpicture}
    % Draw the vertical lines
    \draw[|->, thick] (0,0) -- (15.75,0);
    \draw[|->, thick] (0,1.5) -- (15.75,1.5);

    \node at (15.75,0.5) {Pool H};
    \node at (15.75, 2) {Pool L};

    \node[align=left] at (1.5, 0.75) {$\LP$s deposit $q_i$ \\ in pool $k\in\left\{L,H\right\}$};

    \draw[->,blue] (1,2)--(1,1.5);
    \node[blue, align=center] at (1,2.4) {Small \\ LT};

    \draw[->,blue] (2.5,2)--(2.5,1.5);
    \node[blue, align=center] at (2.5,2.4) {Small \\ LT};

    \draw[->,blue,thick] (4,2)--(4,1.5);
    \draw[->,blue,thick] (4,1.5)--(4,0);
    \node[blue, align=center] at (4,2.4) {\bfseries Large \\ \bfseries LT};

    \draw[dotted,thick,red] (4.5,1.5) -- (4.5, 0);
    \node[red, align=left] at (5.25,0.75) {News \\ $\tilde{\sigma}\in\left(\ell,h\right)$}; 

    \draw[->,red] (6,2)--(6,1.5);
    \node[red, align=left] at (6,2.4) {$\A$ trades \\ on pool $L$};

    \draw[->,thick](8,2)--(8,1.5);
    \node[align=center] at (8,2.4) {$\LP$ rebalance \\ on pool $L$};

    \draw[->,blue,thick] (9.75,2)--(9.75,1.5);
    \draw[->,blue,thick] (9.75,1.5)--(9.75,0);
    \node[blue, align=center] at (9.75,2.4) {\bfseries Large \\ \bfseries LT};


    \draw[->,blue] (10.75,2)--(10.75,1.5);
    \node[blue, align=center] at (10.75,2.4) {Small \\ LT};

    \draw[dotted,thick,red] (11.25,1.5) -- (11.25, 0);
    \node[red, align=center] at (11.75,0.75) {News \\ $\tilde{\sigma}>h$}; 

    \draw[->,red] (12.5,2)--(12.5,1.5);
    \draw[->,red] (12.5,1.5)--(12.5,0);
    \node[red, align=left] at (12.5,2.6) {\textbf{A} trades \\ on both \\ pools};

    \draw[->,thick](14.75,2)--(14.75,1.5);
    \draw[->,thick](14.75,1.5)--(14.75,0);
    \node[align=left] at (14.75,2.6) {$\LP$ rebalance \\ on both \\ pools};

    
\end{tikzpicture}
    \caption{Model timing}
    \label{fig:timing_revised}
\end{figure}

\subsection{Equilibrium}\label{sec:liqprov}

First, consider the liquidity traders' decisions. Faced with pool sizes of $\mathcal{L}_\ell$ and $\mathcal{L}_h$ in the low and high pool respectively, they choose the pool which minimizes their trading costs. Since small traders' private value is between $\ell$ and $h$, they only trade on the low-fee pool. If their demand $\tilde{\theta}$ is lower than the available liquidity in the pool, their trade is executed in full. Otherwise, they exhaust the low fee pool and the trade size is rationed. The fraction of the low-fee pool that is consumed after the arrival of a small $\LT$ is:
\begin{equation}
    \mathbb{E}\left[\min\left\{\frac{\tilde{\theta}}{\LL},1\right\}\right]=1-\frac{\LL}{2\theta}.
\end{equation}
By assumption the large liquidity taker wants to trade more than the posted liquidity and exhausts both pools. \mz{Once a liquidity trader executes the trade, a reversal arbitrage trade of same size and opposite direction restores the original state of the pool.}

Second, consider the trading decisions of arbitrageurs. If the size of news $\tilde{\sigma}\geq h$, then arbitrageurs obtain positive profit on both pools since $\tilde{\sigma}-h>0$ and $\tilde{\sigma}-\ell>0$. They exhaust liquidity on both pools in the direction of the trade. Since the trade is motivated by information, there is no reversal arbitrage trade and liquidity providers need to re-balance at cost $\Gamma$. However, if $\tilde{\sigma}\in\left[\ell,h\right)$, then arbitrageurs trade only on the low-fee pool. Finally, if $\tilde{\sigma}<\ell$, then arbitrageurs do not trade upon the realization of news.

Let $d_k, k=\ell,h$ denote the duration of a re-balancing cycle on the low and high pool respectively. Then, the expected duration of a cycle on the low fee pool is 
\begin{align}
    d_\ell &= \eta \left(1-\frac{\ell}{\sigma}\right),
    \end{align}
\noindent while the expected duration on a high fee pool is $d_h=\eta \left(1-\frac{h}{\sigma}\right).$  Thus,


\begin{lem}\label{lem:duration}
 \setlength{\parskip}{0ex}
The expected duration of a liquidity cycle is shorter in the low fee pool than the high fee pool. Or, $d_\ell<d_h$.
\end{lem}

==> slides/slides-cp.tex <==

\input{preamble}
\setbeamertemplate{itemize item}{\textbullet}
% Define a boolean parameter
\newboolean{longtalk}
\setboolean{longtalk}{false} % Set to 'true' to show the slides, 'false' to hide them


\newcommand{\takeaways}{
\begin{itemize}
\item Decentralized exchanges are designed for \emph{passive} liquidity provision.
\item Fixed costs to participate in markets lead to different economies of scale for heterogeneous \textbf{LP}s.
\item If fragmented: high-fee pools tend to have lower execution, lower liquidity yields and higher adverse selection cost.
\item But, fragmentation can be efficient.
\end{itemize}

\begin{center}
\begin{tabular}{ll}
\toprule
Low-fee pools & High-fee pools \\
\cmidrule{1-2}
High trading volume & Low trading volume \\
Low aggregate liquidity & High aggregate liquidity \\
Few, large \textbf{LP}s & Many, small \textbf{LP}s \\
Short liquidity cycles & Large liquidity cycles \\
\bottomrule
\end{tabular}
\end{center}

}

\begin{document}



\title{Fragmentation and Optimal Liquidity Supply on Decentralized Exchanges} 
\author[Lehar, Parlour, Zoican]{Alfred Lehar, Christine A. Parlour, and Marius Zoican}

\date{March 2024}

\institute[U Toronto]{Haskayne School of Business, University of Calgary \and Haas School of Business, UC Berkeley \and Rotman School of Management,  University of Toronto}

\begin{frame}[noframenumbering]
\titlepage
\end{frame}

\begin{frame}\frametitle{This paper}
\begin{itemize}
\item Use design of  an automated market maker (AMM) to study:
\medskip
\begin{itemize}
\item[\textbullet] Effect of fixed and variable costs on liquidity supply
\smallskip
\item[\textbullet] Find that fragmented liquidity can be beneficial
\end{itemize}
\bigskip
\item Why study an AMM?
\begin{enumerate}
\item They process a large volume of transactions.
\smallskip
\item They seem to provide more liquidity than centralized limit order markets.
\smallskip
\item As real world assets (RWA) move to tokenization models, trading may migrate.
\smallskip
\item Costs/benefits to supplying liquidity is cleaner to observe than in centralized markets.
\end{enumerate}

\end{itemize}


\end{frame}

\begin{frame}{Decentralized exchanges (DEX) trade}
    \begin{center}
        \includegraphics[width=\textwidth]{Figures/dex-volume-monthly.png}
    \end{center}
\end{frame}

\begin{frame}{DEX have substantial liquidity (at least in major pairs)}
    \begin{center}
        \includegraphics[width=\textwidth]{Figures/chartkaiko.png}
    \end{center}
\end{frame}


\begin{frame}\frametitle{Uniswap - Details}
\begin{itemize}
\item UniSwap is a decentralized protocol originally on the Ethereum Blockchain
\item Uniswap comprises tens of thousands of liquidity pools
\begin{itemize}
\item[\textbullet] Each pool has two assets -- all trades are swaps
\end{itemize}
\bigskip
\item There are three versions of Uniswap (v1,v2,v3)
\medskip
\item Features common to all versions:
\begin{itemize}
\item[\textbullet] Agents choose to supply or demand liquidity
\item[\textbullet] Transaction prices are automatically calculated as a function of liquidity demand and supply.
\item[\textbullet] Only payoff for liquidity supplier is a \% fee paid by the liquidity demander.
\end{itemize}
\medskip
\item Unique to v3
\begin{itemize}
\item[\textbullet] Variable fees:  Each asset pair can trade in 1, 5, 30 or 100bps pools.
\item[\textbullet] Concentrated liquidity:  Liquidity suppliers can choose the price range over which they supply liquidity 
\end{itemize}
\end{itemize}
\end{frame}


\begin{frame}\frametitle{Uniswap -- Liquidity Provision v2 \\ A Pool with Ethereum ``E'' and a token ``T''}

\begin{minipage}{0.35\textwidth}%
\begin{tikzpicture}
\draw(0,1) circle(0.5in);
\draw[thick,dashed](-1.15,0.45)--(1.15,0.45);
\draw(0,1) node[above]{E};
\draw(0,0.35) node[below]{T};
\end{tikzpicture}
\end{minipage} %
\begin{minipage}{0.55\textwidth}%
\begin{itemize}
\item Liquidity suppliers deposit Eth and T

\medskip
\item Liquidity demander who buys the token, removes it from the pool and deposits Eth.
\item Liquidity demander who sells the token, adds it to the pool and withdraws Eth.

\bigskip
\item Liquidity demanders pay a fixed, proportional fee which is passed through to the liquidity suppliers.

\end{itemize}
\end{minipage}

\end{frame}




\begin{frame}\frametitle{Price Impact to sell $\Delta_T$ tokens}
\begin{minipage}{0.25 \textwidth}
\begin{tikzpicture}[scale=0.35]
\draw[thick,->] (0,0)-- (15,0);
\draw[thick,->] (0,0) -- (0,10);
\draw (0,8) node[left]{Eth};
\draw(10,0) node[below]{Token};
\draw[dotted,red, thick](0,5)--(4,5);
\draw[dotted,red,thick](4,5)--(4,0);
\draw (0,5) node[left]{$E_0$};
\draw (4,0) node[below]{$T_0$};
\draw(6,0) node[below]{$ T_1$};
\draw(5,-1.5) node[below] {$\Delta_T$}; 
\draw[dotted,blue,thick](6,0)--(6,3.9);
\draw[dotted,blue,thick](0,3.9)--(6,3.9);
\draw(0,3.9) node[left]{$E_1$};
\draw plot[smooth] coordinates {(2,10)  (4,5) (12,1.9)};
\end{tikzpicture}
\end{minipage}
\begin{minipage}{0.2\textwidth}
\hspace{1in}
\end{minipage}
\begin{minipage}{0.45 \textwidth}
\begin{itemize}
\item For negligible quantities, the exchange between Eth and the Token is E/T
\item For larger trades, the exchange rate is determined by a ``bonding curve.''
\item For given $E$ and $T$, so $ET=k$: \end{itemize}
\begin{eqnarray*}
(E + \Delta_E)(T+\Delta_T) = k
\end{eqnarray*}
\begin{itemize}
\item As more liquidity is supplied, bonding curve shifts out.
\end{itemize}
\end{minipage}
\end{frame}

\begin{frame}{Unique to v3:  Concentrated Liquidity}
\begin{itemize}
    \item On Uniswap v3, liquidity providers can specify price limits on their positions.
    \item If the current pool price (e.g., ``midpoint'') is outside the range, the position does not earn fees.
    \item $\rightarrow$ incentive to re-price the position to capture fees.
\end{itemize}
    \begin{center}
        \includegraphics[width=\textwidth]{Figures/uniswapv3_positions.png}
    \end{center}
\end{frame}

\begin{frame}
\frametitle{Managing liquidity on DEX is costly}
\begin{center}
   \includegraphics[width=\textwidth]{Figures/usp3_mechanism.eps}
\end{center}
\end{frame}

\begin{frame}{Fixed cost of supplying liquidity (gas fee) on Uniswap v3}
    \begin{center}
        \includegraphics[width=\textwidth]{Figures/gas_timeline.png}
    \end{center}
\end{frame}




\ifthenelse{\boolean{longtalk}}{
\begin{frame}{Liquidity Provision on a DEX}

\bigskip

    \begin{enumerate}
    \item Unique laboratory to study how transaction costs affect the market for liquidity.
        \item DEX  designed for \textbf{passive} liquidity provision. \vspace{0.05in}
        %\item ``\emph{Set-it-and-forget-it}'' liquidity: i.e., what ETFs did for portfolio management. \vspace{0.05in}
        \item On v3 actively managing liquidity is costly:
            \begin{enumerate}
                \item \emph{gas price} from interacting with Ethereum blockchain. \vspace{0.05in}
                \item \emph{time/effort} to monitoring the position.
            \end{enumerate}
        \vspace{0.05in}
        %\item Economies of scale: small liquidity providers face higher relative costs.\vspace{0.05in}
         
    \end{enumerate}
    \medskip

    
    \end{frame} }

% \begin{frame}{Decentralized exchanges $\approx$ 20\% of crypto trading volume}
%     \begin{center}
%         \includegraphics[width=\textwidth]{Figures/dex-volume-monthly.png}
%     \end{center}
% \end{frame}







\begin{frame}\frametitle{Results}

\vspace{0.1in}

\begin{alertblock}{Theory and  evidence of LP ``clienteles'' based on their scale:}
\bigskip

\begin{enumerate}
    \item Small LPs are more passive, have  lower fill rates but get high fees. 
    \bigskip
    \item Large LPs are more active, have higher fill rates but get low fees.
    \bigskip
    \item This segmentation can be efficient
\end{enumerate}


\end{alertblock}

\end{frame}

%\section{Model}

\begin{frame}{Model}

\begin{block}{Asset and markets.} \begin{itemize}
    \item Token with expected value $v$ trades on two liquidity pools with fees $h>\ell>0$.
    \item Fixed cost $\Gamma>0$ of interacting with the pool (e.g., gas fee).
\end{itemize}
\end{block}

\begin{block}{Liquidity providers (\textbf{LP})}

 \begin{tabular}{cl}  
     \begin{tabular}{l}
            \parbox{0.35\linewidth}{%  change the parbox width as appropriate
                \begin{itemize}
        \item Risk-neutral;
        \item Token endowments $q_i$; \item $q_i$ follows a bounded Pareto distribution:
        \begin{equation*}\label{eq:density}
    \varphi\left(q\right)=\Big(\frac{Q}{Q-1}\Big) \frac{1}{q^2}.
    \end{equation*}
    \end{itemize}}
       \end{tabular}
    &\begin{tabular}{c}
            \includegraphics[width=8.5cm]{Figures/model_density.png}
        \end{tabular}  
   \end{tabular}

\end{block}

\end{frame}



\begin{frame}{Timeline}

\begin{block}{Liquidity takers (\textbf{LT}).} Two types of $\textbf{LT}$: 
\begin{enumerate}
    \item \emph{small} $\textbf{LT}$ arrive at constant rate $\theta \diff t$ and optimally go to the low-fee pool first ($\ell$). 
    \item \emph{large} $\textbf{LT}$ demand $\Theta$ token units and arrive as Poisson process $J_t\left(\lambda\right)$. \\ They are exogenously large enough to consume all liquidity on $\ell$ and $h$ pools.
\end{enumerate}
\end{block}
\vspace{0.1in}
    \begin{center}
        \includegraphics[width=\textwidth]{Figures/timing_dex_rebalance.eps}
    \end{center}


\end{frame}

\begin{frame}\frametitle{Prices}
\begin{itemize}
\item We assume a linear bonding curve -- prices occur at $v$.
\bigskip
\item Traditionally, a spread compensates market makers for adverse selection \\ (``insider trading") \vspace{0.1in}
\item In these markets 
\begin{enumerate}
    \item liquidity providers do not post or earn a spread
    \item as these are assets with no cash flows, unclear what form adverse selection takes
    \item no clear ``value" benchmarks as off chain assets have a different use value. 
\end{enumerate}
\end{itemize}

    
\end{frame}



\begin{frame}{The liquidity provider problem}
\begin{itemize}
\item ${\color{red} d_k}$ is the endogenous liquidity cycle duration, which $\nearrow$ in aggregate liquidity:
\begin{eqnarray*}
d_h & = & \frac{1}{\lambda}\\
    d_\ell&=&\frac{1}{\lambda}-\frac{1}{\lambda}\exp\left(-\frac{\LL}{\theta}\lambda\right) 
\end{eqnarray*}
where $\LL$ is the aggregate liquidity on the low-fee pool.
\medskip
 \item Liquidity providers choose pool $k^\star$ to maximize expected profit per unit of time:
\begin{equation*}
\label{eq:optimal_pool}
    k^\star\left(q_i\right) = \arg\max_{\left\{\ell,h,\emptyset\right\}}   \Big[\frac{q_i \ell - \Gamma}{d_\ell} , \; \frac{q_i h -\Gamma}{d_h}, \; \emptyset\Big].
\end{equation*}
\item Trade-off between:
\begin{enumerate}
   \item higher liquidity fee per unit of time in low fee pools, and 
    \item lower rebalancing cost in high-fee pools.
\end{enumerate}
\end{itemize}
\end{frame}

\begin{frame}{Equilibrium}
\begin{itemize}
\item There is a threshold endowment $\qmg$ such that all $\LP$s with $q_i>\qmg$ post liquidity on the low-fee pool and all $\LP$s with $q_i\leq \qmg$ choose the high-fee pool. 
\begin{align*}\label{eq:liquidity_levels}
    \LL&=\int_{\qmg}^Q q_i \varphi\left(q_i\right) \diff i = \frac{Q}{Q-1}\left(\log Q - \log \qmg \right)  \text{ and }\nonumber \\
    \LH&=\int_{\underline{q}}^{\qmg}  q_i \varphi\left(q_i\right) \diff i = \frac{Q}{Q-1}\left(\log \qmg - \log \underline{q}\right)
\end{align*}
\end{itemize}
\bigskip
\begin{center}
\begin{tikzpicture}[scale= 0.5]
    \draw[thick] (0,0)--(15,0);
    \draw[thick] (10,0)--(10,1);
    \draw[thick] (15,0)--(15,1);
    \draw[thick] (0,0)--(0,1);
    \draw[thick] (5,0)--(5,1);
    \draw[thick] node[below]{$1$};
    \draw[thick] (5,0) node[below]{$\underline q$};
    \draw[thick] (10,0) node[below]{$q_t$};
    \draw[thick] (15,0) node[below]{Q};
    \draw[thick] (2.5,0) node[above]{out};
    \draw[thick] (7.5,0) node[above]{high};
    \draw[thick] (12.5,0) node[above]{low};
\end{tikzpicture}
\end{center}
\end{frame}

\begin{frame}{High-fee pools attract small liquidity providers}
    \begin{center}
        \includegraphics[width=\textwidth]{Figures/liquidity_supply.png}
    \end{center}
\end{frame}

%
\begin{frame}{Trading volume and liquidity in equilibrium}
    \begin{center}
        \includegraphics[width=\textwidth]{Figures/trade_volumesize.png}
    \end{center}
\end{frame}

\ifthenelse{\boolean{longtalk}}{%
\begin{frame}{Equilibrium regions}
    \begin{center}
        \includegraphics[width=\textwidth]{Figures/equilibrium_existence.png}
    \end{center}
\end{frame}
}
\ifthenelse{\boolean{longtalk}}{
\begin{frame}\frametitle{Evaluating the fragmented liquidity}
\begin{itemize}
\item LP participates if $q_if>\Gamma$, or fee greater than fixed cost.
\bigskip
\item Shortfall for the large liquidity trader:
\end{itemize}
\begin{eqnarray*}
\underbrace{\sum_k f_k {\cal L}_k}_{\mbox{trading fees}} + \underbrace{\Delta \left( \Theta - \sum_k{\cal L}_k\right)}_{\mbox{unrealized gains from trade}}
\end{eqnarray*}
\begin{itemize}
\item Higher fee: 
\begin{itemize}
    \item more posted liquidity, more gains from trade
    \item higher trading fees for trader
    \end{itemize}
\item Optimal fee for single pool

\medskip
\item For any single fee pool, a fragmented pool exists that improves the large trader's shortfall
\begin{itemize}
    \item Set high pool fee equal to optimal fee of single pool $\to$ at least a good
    \item Add a low fee pool to reduce trading fees
\end{itemize}
\end{itemize}
\end{frame} }


% \begin{frame}{Time-series predictions}
% \begin{enumerate}
%     \item The liquidity market share of low-fee pool $\searrow$ in gas fee.
%     \item Average 
% \end{enumerate}
% \end{frame}

%\section{Empirical findings}

\begin{frame}{Data}
\begin{itemize}
    \item Data from Uniswap v3 Subgraph on all trades, liquidity deposits and withdrawals from May 4, 2021 until July 15, 2023, including traders' wallet addresses. \vspace{0.1in}
    \item Gas cost is the average of the lowest daily 1000 gas prices for mint events. \vspace{0.1in}
    \item Focus on economically sizeable pools:
    \begin{enumerate}
        \item active in more than 100 days within the sample;
        \item 500+ liquidity events throughout the sample;
        \item average daily liquidity balance $>$US\$100,000;
        \item $>$1\% of volume for a traded pair.
    \end{enumerate} \vspace{0.1in}
    \item We obtain 274 pools in 242 asset pairs:
    \begin{enumerate}
        \item aggregate daily volume of US\$~1.12bn;
        \item end-of-sample aggregate liquidity US\$~2.53bn.
        \item account for 86.04\% of all Uniswap v3 interactions.
    \end{enumerate}
\end{itemize}
\end{frame}

\begin{frame}{Uniswap v3 pairs can be traded in 1, 5, 30, or 100 bps fee pools}
\begin{itemize}
    \item 32 fragmented pools collectively account for 95\% of committed liquidity and 93\% of traded volume
    \item Trading concentrates on adjacent fee levels e.g.:  USDC/USDT 1-5bps, ETH/USDC 5-30bps, USDC-CRV 30-100bps
\end{itemize}
\bigskip
\begin{enumerate}
    \item Significant fragmentation across different-fee pools for the same pair.
    \item Low-fee pools are more actively traded, but high-fee pools are deeper.
    \begin{center}
        \includegraphics[width=0.9\textwidth]{Figures/sumstat_TVL_volume.png}
    \end{center}
%\item We show that fixed transaction costs partly drive this effect.
\end{enumerate}
\end{frame}

\begin{frame}{Liquidity clienteles: high fee pools feature many small \textbf{LP}s.}
    \begin{center}
        \includegraphics[width=\textwidth]{Figures/sumstat_mint_trade.png}
        \includegraphics[width=\textwidth]{Figures/sumstat_wallets.png}
    \end{center}
\end{frame}


\ifthenelse{\boolean{longtalk}}{
\begin{frame}{Low-fee pools: Larger mints, fewer LP wallets, many small trades.\\ (Mints and Trades in log USD)}
\begin{center}


\scalebox{0.76}{
\begin{tabular}{lccccccc}
\toprule
 & \multicolumn{1}{c}{Mint size} &  \multicolumn{1}{c}{Trade size} & \multicolumn{1}{c}{Volume} & \multicolumn{1}{c}{\# Trades}  & \multicolumn{1}{c}{\# Wallets} & \multicolumn{1}{c}{Liquidity yield} & \multicolumn{1}{c}{Price range} \\
 & (1) & (2) & (3) & (4) & (5) & (6) & (7) \\
\rowcolor{red!20} 
$ d_\text{low-fee}$ & 0.73*** & -0.30*** & 0.89*** & 1.02*** & -3.40*** & 2.03*** & -0.18*** \\
\rowcolor{red!20}
 & (12.27) & (-10.05) & (14.23) & (32.95) & (-5.00) & (3.60) & (-41.84) \\
Gas price $\times$ $ d_\text{low-fee}$ & 0.37*** & 0.08*** & -0.03 & -0.22*** & -3.00*** & 3.57** & -0.00 \\
 & (4.96) & (3.75) & (-0.95) & (-7.29) & (-3.43) & (2.30) & (-0.47) \\
Gas price $\times$ $ d_\text{high-fee}$ & 0.58*** & 0.17*** & 0.24*** & 0.07** & -2.89*** & 5.57*** & -0.03*** \\
 & (7.52) & (8.81) & (5.95) & (2.46) & (-3.15) & (2.83) & (-4.65) \\
Volume & 0.37*** & 0.16*** & 0.43*** & 0.20*** & 1.22*** & 1.01 & -0.01** \\
 & (8.68) & (21.38) & (15.27) & (13.85) & (6.56) & (0.81) & (-2.56) \\
Total value locked & -0.16 & 0.11*** & 0.23** & -0.01 & -1.86 & -13.42 & -0.02 \\
 & (-1.30) & (3.54) & (1.99) & (-0.18) & (-0.99) & (-1.09) & (-0.99) \\
Volatility & -0.04 & -0.01 & -0.07 & 0.01 & -0.09 & 1.18** & 0.02*** \\
 & (-1.11) & (-1.34) & (-1.38) & (0.88) & (-1.03) & (2.21) & (3.98) \\
Constant & 1.88*** & 1.64*** & 5.27*** & 3.26*** & 10.12*** & 10.01*** & 0.59*** \\
 & (58.27) & (111.47) & (168.58) & (209.84) & (28.65) & (26.04) & (184.91) \\
Observations & 21,000 & 36,059 & 36,059 & 40,288 & 40,288 & 40,252 & 24,058 \\
 R-squared & 0.26 & 0.53 & 0.55 & 0.52 & 0.37 & 0.09 & 0.42 \\ \hline
\bottomrule
\end{tabular}
}
\end{center}
\end{frame} }

\ifthenelse{\boolean{longtalk}}{
\begin{frame}{$\Uparrow$ gas cost of liquidity management:  mid-size LPs switch to $h$ fee pool\\Small LPs leave the pools}
    \begin{center}
        \includegraphics[width=\textwidth]{Figures/mkt_share_gas.png}
    \end{center}
\end{frame} }



\ifthenelse{\boolean{longtalk}}{
\begin{frame}{Do gas prices move market shares?}
\begin{center}
    

\scalebox{0.82}{
\begin{tabular}{lccc@{\hskip 0.3in}ccc}
\toprule
 & \multicolumn{3}{c}{Liquidity market share (\%)} & \multicolumn{3}{c}{Volume market share (\%)} \\ 
 \cmidrule{1-7}
\rowcolor{red!20} $ d_\text{low-fee}$ & -20.92*** & -20.92*** & -20.92*** & 24.62*** & 24.63*** & 24.62*** \\
 & (-27.42) & (-27.41) & (-27.42) & (20.55) & (20.56) & (20.55) \\
\rowcolor{red!20} Gas price $\times$ $ d_\text{low-fee}$ & -4.63*** & -4.62*** & -4.63*** & -6.52*** & -6.52*** & -6.52*** \\
 & (-7.32) & (-7.32) & (-7.32) & (-5.92) & (-5.92) & (-5.92) \\
Gas price & 2.31*** & 2.31*** & 2.31*** & 3.63*** & 3.61*** & 3.61*** \\
 & (7.32) & (7.32) & (7.32) & (7.33) & (7.30) & (7.26) \\
Volume & 0.00 & 0.00 & 0.00 & -0.19** & -0.20** & -0.19** \\
 & (0.65) & (1.33) & (0.65) & (-2.54) & (-2.61) & (-2.50) \\
Total value locked & -0.00 & -0.00 &  & 0.58 & 0.58 &  \\
 & (-0.58) & (-0.06) &  & (1.44) & (1.44) &  \\
Volatility & -0.29 &  & -0.29 & -1.15*** &  & -1.15*** \\
 & (-0.90) &  & (-0.90) & (-2.74) &  & (-2.74) \\
Constant & 60.45*** & 60.46*** & 60.45*** & 41.96*** & 41.99*** & 41.96*** \\
 & (158.00) & (158.46) & (158.00) & (69.99) & (70.22) & (70.02) \\
Observations & 40,288 & 40,288 & 40,288 & 36,059 & 36,059 & 36,059 \\
 R-squared & 0.10 & 0.10 & 0.10 & 0.13 & 0.13 & 0.13 \\ \hline
\bottomrule
\end{tabular}



}
\end{center}
\end{frame}
}


\ifthenelse{\boolean{longtalk}}{
\begin{frame}{Liquidity flows and gas prices}
\begin{center}
    

\scalebox{0.77}{
\begin{tabular}{lcccccc}
\toprule
 & \multicolumn{3}{c}{Daily mints (log US\$)} &  \multicolumn{3}{c}{$\text{Prob}\left(\text{at least one mint}\right)$} \\
\cmidrule{1-7}
$ d_\text{low-fee}$ & 0.15* & 0.16** & 0.15* & 1.33* & 1.30* & 1.33* \\
 & (1.94) & (2.03) & (1.94) & (1.82) & (1.85) & (1.82) \\
\cellcolor{LRed}Gas price $\times$ $ d_\text{low-fee}$ & \cellcolor{LRed} -0.36*** & \cellcolor{LRed}-0.36*** & \cellcolor{LRed}-0.39*** & \cellcolor{LRed}-7.60*** & \cellcolor{LRed}-7.63*** & \cellcolor{LRed}-5.68*** \\
 & (-6.66) & (-6.43) & (-5.22) & (-9.36) & (-9.09) & (-8.22) \\
\cellcolor{LRed}Gas price $\times$ $ d_\text{high-fee}$ & \cellcolor{LRed} 0.03 & \cellcolor{LRed} 0.00 & \cellcolor{LRed} & \cellcolor{LRed}-\cellcolor{LRed}1.92*** & \cellcolor{LRed}-2.14*** & \cellcolor{LRed} \\
 & (0.33) & (0.00) &  & (-2.74) & (-2.85) &  \\
Trade volume (pair) & 0.45*** & 0.44*** & 0.45*** & 1.19 & 1.17 & 1.19 \\
 & (7.16) & (7.04) & (7.16) & (1.33) & (1.25) & (1.33) \\
Pool size (pair) & -0.45*** & -0.52*** & -0.45*** & -5.31** & -5.56** & -5.31** \\
 & (-2.75) & (-3.34) & (-2.75) & (-2.43) & (-2.52) & (-2.43) \\
Volatility & 0.02 &  & 0.02 & 1.50* &  & 1.50* \\
 & (0.73) &  & (0.73) & (1.80) &  & (1.80) \\
Gas price &  &  & 0.03 &  &  & -1.92*** \\
 &  &  & (0.33) &  &  & (-2.74) \\
Constant & 0.55 & 1.14 & 0.55 & 81.06*** & 82.73*** & 81.06*** \\
 & (0.60) & (1.36) & (0.60) & (6.12) & (5.72) & (6.12) \\
Observations & 20,454 & 21,097 & 20,454 & 21,097 & 20,454 & 20,454 \\
 R-squared & 0.51 & 0.51 & 0.51 & 0.61 & 0.62 & 0.62 \\ \hline
\bottomrule
\end{tabular}
}
\end{center}
\end{frame}
}

\begin{frame}{Re-balancing cycles}
\includegraphics[width=0.9\textwidth]{Figures/time_elapsed_distribution.png}
\includegraphics[width=0.9\textwidth]{Figures/out_of_range_distribution.png}
\end{frame}

\ifthenelse{\boolean{longtalk}}{

\begin{frame}{Gas price $\uparrow$ $\Rightarrow$ Liquidity supply on $L$ $\downarrow$ $\Rightarrow$ Re-balancing frequency $\uparrow$}
\begin{center}
    

\scalebox{0.78}{
\begin{tabular}{lcccccc}
\toprule
 & \multicolumn{3}{c}{Mint-burn time} & \multicolumn{3}{c}{Burn-mint time} \\
\cmidrule{1-7}
\rowcolor{red!20}
$ d_\text{low-fee}$ & -99.74*** & -100.17*** & -104.09*** & -157.95*** & -159.71*** & -159.69*** \\
 & (-8.86) & (-8.94) & (-9.22) & (-10.59) & (-10.81) & (-10.80) \\
\rowcolor{red!20} 
Gas price $\times$ $ d_\text{low-fee}$ & -16.65** & -15.41* & -15.80** & -11.29 & 2.95 & 2.94 \\
 & (-2.13) & (-1.98) & (-2.02) & (-1.65) & (0.40) & (0.39) \\
Gas price $\times$ $ d_\text{high-fee}$ & -14.44** & -13.42* & -13.98* & -10.52* & 1.96 & 1.95 \\
 & (-2.04) & (-1.89) & (-1.96) & (-1.69) & (0.32) & (0.32) \\
Volume &  & -5.87 & -7.45 &  & -24.84*** & -24.82*** \\
 &  & (-1.15) & (-1.41) &  & (-4.10) & (-4.09) \\
Total value locked &  & -53.17* & -51.72* &  & -12.71 & -12.71 \\
 &  & (-1.70) & (-1.66) &  & (-0.52) & (-0.52) \\
Volatility &  & -2.11*** & -2.26*** &  & -2.99*** & -2.98*** \\
 &  & (-2.75) & (-2.86) &  & (-3.36) & (-3.36) \\
Position out-of-range &  &  & 37.09*** &  &  & -1.53 \\
 &  &  & (6.43) &  &  & (-0.22) \\
Constant & 497.18*** & 497.00*** & 479.22*** & 248.00*** & 250.13*** & 250.47*** \\
 & (91.65) & (90.60) & (82.13) & (29.91) & (30.27) & (30.32) \\
Observations & 405,586 & 405,584 & 405,584 & 265,848 & 265,848 & 265,848 \\
 R-squared & 0.82 & 0.82 & 0.82 & 0.37 & 0.37 & 0.37 \\ \hline
\bottomrule
\end{tabular}
}
\end{center}
\end{frame}
}

\ifthenelse{\boolean{longtalk}}{%
\begin{frame}{Is order flow on high-fee pools more toxic?}

\begin{block}{``Impermanent loss"}
    \begin{itemize}
        \item A measure of adverse selection cost
        \item Negative return from providing liquidity as opposed to marking to market.
    \end{itemize}
\end{block}

\begin{block}{Example}
    \begin{itemize}
        \item At $t=0$, LP deposits 1 ETH and 3000 USDC (fair price).
        \item At $t=1$, value jumps to ETH/USDC 3500:
            \begin{enumerate}
                \item An arbitrageur optimally purchases ETH to bring price in line.
                \item New LP holdings: 0.92 ETH and 3240 USDC.  {\color{red} \textbf{Value:} $V_\text{pos}=\$6,480.74$.}
                \item Counterfactual (holding) value if not providing liquidity: {\color{red} \textbf{Value:} $V_\text{hold}=\$6,500$}.
            \end{enumerate}
       
        \begin{equation*}
    \text{Impermanent Loss}=\frac{V_\text{hold}-V_\text{pos}}{V_\text{hold}}=29 \text{ bps}.
        \end{equation*}
    \end{itemize}
\end{block}
    
\end{frame}
}

\ifthenelse{\boolean{longtalk}}{%
\begin{frame}{Low-fee pool LPs: adverse selection costs $\downarrow$ (controlling for activity)}
\begin{center}
    

\scalebox{0.75}{
\begin{tabular}{lcccccccc}
\toprule
& \multicolumn{8}{c}{Impermanent loss for a liquidity position with range $\left[\frac{p}{\alpha}, \alpha p\right]$ around price $p$} \\
\cmidrule{1-9} 
& \multicolumn{2}{c}{$\alpha=1.01$} & \multicolumn{2}{c}{$\alpha=1.05$} & \multicolumn{2}{c}{$\alpha=1.10$} & \multicolumn{2}{c}{$\alpha=1.25$} \\
\cmidrule{1-9}
$ d_\text{low-fee}$ & 2.59*** & -1.38 & 1.08*** & -1.85** & 0.71*** & -1.56** & 0.37** & -1.09* \\
 & (11.26) & (-1.57) & (5.72) & (-2.28) & (4.28) & (-2.18) & (2.58) & (-1.98) \\
Gas price &  & 4.75*** &  & 3.68*** &  & 2.72*** &  & 1.55*** \\
 &  & (3.97) &  & (3.96) &  & (3.86) &  & (3.42) \\
Trade count &  & 4.82*** &  & 3.56*** &  & 2.78*** &  & 1.79*** \\
 &  & (4.59) &  & (3.71) &  & (3.30) &  & (2.83) \\
Volume &  & 3.03*** &  & 1.19*** &  & 0.60** &  & 0.22 \\
 &  & (7.00) &  & (3.87) &  & (2.45) &  & (1.25) \\
Total value locked &  & 0.43 &  & 1.78 &  & 2.02 &  & 1.83 \\
 &  & (0.16) &  & (0.79) &  & (1.05) &  & (1.38) \\
Volatility &  & 6.98*** &  & 6.65** &  & 6.39** &  & 6.06** \\
 &  & (2.69) &  & (2.59) &  & (2.51) &  & (2.40) \\
Constant & 15.52*** & 15.87*** & 7.37*** & 7.65*** & 4.63*** & 4.87*** & 2.45*** & 2.66*** \\
 & (134.72) & (103.02) & (77.84) & (60.07) & (55.47) & (43.73) & (34.58) & (29.33) \\
Observations & 40,250 & 40,248 & 40,250 & 40,248 & 40,250 & 40,248 & 40,250 & 40,248 \\
 R-squared & 0.17 & 0.23 & 0.09 & 0.15 & 0.06 & 0.11 & 0.03 & 0.08 \\ \hline
\bottomrule
\end{tabular}
}
\end{center}
\end{frame}}
% {\begin{frame}{Is order flow on high-fee pools more toxic?}
% \begin{center}
    

% \scalebox{0.75}{
% \begin{tabular}{lcccccccc}
% \toprule
% & \multicolumn{8}{c}{Impermanent loss for a liquidity position with range $\left[\frac{p}{\alpha}, \alpha p\right]$ around price $p$} \\
% \cmidrule{1-9} 
% & \multicolumn{2}{c}{$\alpha=1.01$} & \multicolumn{2}{c}{$\alpha=1.05$} & \multicolumn{2}{c}{$\alpha=1.10$} & \multicolumn{2}{c}{$\alpha=1.25$} \\
% \cmidrule{1-9}
% $ d_\text{low-fee}$ & 2.59*** & -1.38 & 1.08*** & -1.85** & 0.71*** & -1.56** & 0.37** & -1.09* \\
%  & (11.26) & (-1.57) & (5.72) & (-2.28) & (4.28) & (-2.18) & (2.58) & (-1.98) \\
% Gas price &  & 4.75*** &  & 3.68*** &  & 2.72*** &  & 1.55*** \\
%  &  & (3.97) &  & (3.96) &  & (3.86) &  & (3.42) \\
% Trade count &  & 4.82*** &  & 3.56*** &  & 2.78*** &  & 1.79*** \\
%  &  & (4.59) &  & (3.71) &  & (3.30) &  & (2.83) \\
% Volume &  & 3.03*** &  & 1.19*** &  & 0.60** &  & 0.22 \\
%  &  & (7.00) &  & (3.87) &  & (2.45) &  & (1.25) \\
% Total value locked &  & 0.43 &  & 1.78 &  & 2.02 &  & 1.83 \\
%  &  & (0.16) &  & (0.79) &  & (1.05) &  & (1.38) \\
% Volatility &  & 6.98*** &  & 6.65** &  & 6.39** &  & 6.06** \\
%  &  & (2.69) &  & (2.59) &  & (2.51) &  & (2.40) \\
% Constant & 15.52*** & 15.87*** & 7.37*** & 7.65*** & 4.63*** & 4.87*** & 2.45*** & 2.66*** \\
%  & (134.72) & (103.02) & (77.84) & (60.07) & (55.47) & (43.73) & (34.58) & (29.33) \\
% Observations & 40,250 & 40,248 & 40,250 & 40,248 & 40,250 & 40,248 & 40,250 & 40,248 \\
%  R-squared & 0.17 & 0.23 & 0.09 & 0.15 & 0.06 & 0.11 & 0.03 & 0.08 \\ \hline
% \bottomrule
% \end{tabular}
% }
% \end{center}
% \end{frame}}

% \begin{frame}{Returns and costs from liquidity provision}

% Liquidity yield is computed as in \citet{augustin2022reaching}:
% \begin{equation}\label{eq:liq_yield}
%     \text{Liquidity yield}=\text{liquidity fee}_i \times \frac{\text{Volume}_{i,t}}{\text{TVL}_{i,t-1}},
% \end{equation}

%     \begin{center}
%         \includegraphics[width=\textwidth]{Figures/lyield_IL.png}
%     \end{center}
% \end{frame}


\begin{frame}{Conclusion}
    \takeaways
\end{frame}






\appendix
\begin{frame}<beamer:0> [noframenumbering]
\bibliographystyle{jf}
\bibliography{references}
\end{frame}


\end{document}

==> slides/slides-mz-short.tex <==

\input{preamble}
\setbeamertemplate{itemize item}{\textbullet}
% Define a boolean parameter
\newboolean{longtalk}
\setboolean{longtalk}{false} % Set to 'true' to show the slides, 'false' to hide them


\newcommand{\takeaways}{
\begin{itemize}
\item Decentralized exchanges are designed for \emph{passive} liquidity provision.
\item Fixed costs to participate in markets lead to different economies of scale for heterogeneous \textbf{LP}s.
\item If fragmented: high-fee pools tend to have lower execution, lower liquidity yields and higher adverse selection cost.
\item But, fragmentation can be efficient.
\end{itemize}

\begin{center}
\begin{tabular}{ll}
\toprule
Low-fee pools & High-fee pools \\
\cmidrule{1-2}
High trading volume & Low trading volume \\
Low aggregate liquidity & High aggregate liquidity \\
Few, large \textbf{LP}s & Many, small \textbf{LP}s \\
Short liquidity cycles & Large liquidity cycles \\
\bottomrule
\end{tabular}
\end{center}

}

\begin{document}



\title{Fragmentation and Optimal Liquidity Supply \\ on Decentralized Exchanges} 
\author[Lehar, Parlour, Zoican]{Alfred Lehar, Christine A. Parlour, and Marius Zoican}

\date{March 2024}

\institute[U Toronto]{Haskayne School of Business, University of Calgary \and Haas School of Business, UC Berkeley \and Rotman School of Management,  University of Toronto}

\begin{frame}[noframenumbering]
\titlepage
\end{frame}

\begin{frame}\frametitle{This paper}
\begin{itemize}
\item Use design of  an automated market maker (AMM) to study:
\medskip
\begin{itemize}
\item[\textbullet] Effect of fixed and variable costs on liquidity supply
\smallskip
\item[\textbullet] Find that fragmented liquidity can be beneficial
\end{itemize}
\bigskip
\item Why study an AMM?
\begin{enumerate}
\item They process a large volume of transactions.
\smallskip
\item They seem to provide more liquidity than centralized limit order markets.
\smallskip
\item As real world assets (RWA) move to tokenization models, trading may migrate.
\smallskip
\item Costs/benefits to supplying liquidity is cleaner to observe than in centralized markets.
\end{enumerate}

\end{itemize}


\end{frame}

\begin{frame}{Decentralized exchanges (DEX) trade}
    \begin{center}
        \includegraphics[width=\textwidth]{Figures/dex-volume-monthly.png}
    \end{center}
\end{frame}

\begin{frame}{DEX have substantial liquidity (at least in major pairs)}
    \begin{center}
        \includegraphics[width=\textwidth]{Figures/chartkaiko.png}
    \end{center}
\end{frame}


\begin{frame}\frametitle{Uniswap - Details}
\begin{itemize}
\item UniSwap is a decentralized protocol originally on the Ethereum Blockchain
\item Uniswap comprises tens of thousands of liquidity pools
\begin{itemize}
\item[\textbullet] Each pool has two assets -- all trades are swaps
\end{itemize}
\bigskip
\item There are three versions of Uniswap (v1,v2,v3)
\medskip
\item Features common to all versions:
\begin{itemize}
\item[\textbullet] Agents choose to supply or demand liquidity
\item[\textbullet] Transaction price is automatic function of liquidity demand and supply.
\item[\textbullet] Only payoff for liquidity supplier is a \% fee paid by the liquidity demander.
\end{itemize}
\medskip
\item Unique to v3
\begin{itemize}
\item[\textbullet] Variable fees:  Each asset pair can trade in 1, 5, 30 or 100bps pools.
\item[\textbullet] Concentrated liquidity:  Liquidity suppliers can choose the price range over which they supply liquidity 
\end{itemize}
\end{itemize}
\end{frame}


\begin{frame}\frametitle{Uniswap -- Liquidity Provision v2 \\ A Pool with Ethereum ``E'' and a token ``T''}

\begin{minipage}{0.35\textwidth}%
\begin{tikzpicture}
\draw(0,1) circle(0.5in);
\draw[thick,dashed](-1.15,0.45)--(1.15,0.45);
\draw(0,1) node[above]{E};
\draw(0,0.35) node[below]{T};
\end{tikzpicture}
\end{minipage} %
\begin{minipage}{0.55\textwidth}%
\begin{itemize}
\item Liquidity suppliers deposit Eth and T

\medskip
\item Liquidity demander who buys the token, removes it from the pool and deposits Eth.
\item Liquidity demander who sells the token, adds it to the pool and withdraws Eth.

\bigskip
\item Liquidity demanders pay a fixed, proportional fee which is passed through to the liquidity suppliers.

\end{itemize}
\end{minipage}

\end{frame}




\begin{frame}\frametitle{Price Impact to sell $\Delta_T$ tokens}
\begin{minipage}{0.25 \textwidth}
\begin{tikzpicture}[scale=0.35]
\draw[thick,->] (0,0)-- (15,0);
\draw[thick,->] (0,0) -- (0,10);
\draw (0,8) node[left]{Eth};
\draw(10,0) node[below]{Token};
\draw[dotted,red, thick](0,5)--(4,5);
\draw[dotted,red,thick](4,5)--(4,0);
\draw (0,5) node[left]{$E_0$};
\draw (4,0) node[below]{$T_0$};
\draw(6,0) node[below]{$ T_1$};
\draw(5,-1.5) node[below] {$\Delta_T$}; 
\draw[dotted,blue,thick](6,0)--(6,3.9);
\draw[dotted,blue,thick](0,3.9)--(6,3.9);
\draw(0,3.9) node[left]{$E_1$};
\draw plot[smooth] coordinates {(2,10)  (4,5) (12,1.9)};
\end{tikzpicture}
\end{minipage}
\begin{minipage}{0.2\textwidth}
\hspace{1in}
\end{minipage}
\begin{minipage}{0.45 \textwidth}
\begin{itemize}
\item For negligible quantities, the exchange between Eth and the Token is E/T
\item For larger trades, the exchange rate is determined by a ``bonding curve.''
\item For given $E$ and $T$, so $ET=k$: \end{itemize}
\begin{eqnarray*}
(E + \Delta_E)(T+\Delta_T) = k
\end{eqnarray*}
\begin{itemize}
\item As more liquidity is supplied, bonding curve shifts out.
\end{itemize}
\end{minipage}
\end{frame}

\begin{frame}{Unique to v3:  Concentrated Liquidity}
\begin{itemize}
    \item On Uniswap v3, liquidity providers can specify price limits on their positions.
    \item If the current pool price (e.g., ``midpoint'') is outside the range, the position does not earn fees.
    \item $\rightarrow$ incentive to re-price the position to capture fees.
\end{itemize}
    \begin{center}
        \includegraphics[width=\textwidth]{Figures/uniswapv3_positions.png}
    \end{center}
\end{frame}

\begin{frame}
\frametitle{Managing liquidity on DEX is costly}
\begin{center}
   \includegraphics[width=\textwidth]{Figures/usp3_mechanism.eps}
\end{center}
\end{frame}

\begin{frame}{Fixed cost of supplying liquidity (gas fee) on Uniswap v3}
    \begin{center}
        \includegraphics[width=\textwidth]{Figures/gas_timeline.png}
    \end{center}
\end{frame}




\ifthenelse{\boolean{longtalk}}{
\begin{frame}{Liquidity Provision on a DEX}

\bigskip

    \begin{enumerate}
    \item Unique laboratory to study how transaction costs affect the market for liquidity.
        \item DEX  designed for \textbf{passive} liquidity provision. \vspace{0.05in}
        %\item ``\emph{Set-it-and-forget-it}'' liquidity: i.e., what ETFs did for portfolio management. \vspace{0.05in}
        \item On v3 actively managing liquidity is costly:
            \begin{enumerate}
                \item \emph{gas price} from interacting with Ethereum blockchain. \vspace{0.05in}
                \item \emph{time/effort} to monitoring the position.
            \end{enumerate}
        \vspace{0.05in}
        %\item Economies of scale: small liquidity providers face higher relative costs.\vspace{0.05in}
         
    \end{enumerate}
    \medskip

    
    \end{frame} }

% \begin{frame}{Decentralized exchanges $\approx$ 20\% of crypto trading volume}
%     \begin{center}
%         \includegraphics[width=\textwidth]{Figures/dex-volume-monthly.png}
%     \end{center}
% \end{frame}







\begin{frame}\frametitle{Results}

\vspace{0.1in}

\begin{alertblock}{Theory and  evidence of LP ``clienteles'' based on their scale:}
\bigskip

\begin{enumerate}
    \item Small LPs are more passive, have  lower fill rates but get high fees. 
    \bigskip
    \item Large LPs are more active, have higher fill rates but get low fees.
    \bigskip
    \item This segmentation can be efficient
\end{enumerate}


\end{alertblock}

\end{frame}

%\section{Model}

\begin{frame}{Model}

\begin{block}{Asset and markets.} \begin{itemize}
    \item Token with expected value $v$ trades on two liquidity pools with fees $h>\ell>0$.
    \item Fixed cost $\Gamma>0$ of interacting with the pool (e.g., gas fee).
\end{itemize}
\end{block}

\begin{block}{Liquidity providers (\textbf{LP})}

 \begin{tabular}{cl}  
     \begin{tabular}{l}
            \parbox{0.35\linewidth}{%  change the parbox width as appropriate
                \begin{itemize}
        \item Risk-neutral;
        \item Token endowments $q_i$; \item $q_i$ follows a bounded Pareto distribution:
        \begin{equation*}\label{eq:density}
    \varphi\left(q\right)=\Big(\frac{Q}{Q-1}\Big) \frac{1}{q^2}.
    \end{equation*}
    \end{itemize}}
       \end{tabular}
    &\begin{tabular}{c}
            \includegraphics[width=8.5cm]{Figures/model_density.png}
        \end{tabular}  
   \end{tabular}

\end{block}

\end{frame}



\begin{frame}{Timeline}

\begin{block}{Liquidity takers (\textbf{LT}).} Two types of $\textbf{LT}$: 
\begin{enumerate}
    \item \emph{small} $\textbf{LT}$ arrive at constant rate $\theta \diff t$ and optimally go to the low-fee pool first ($\ell$). 
    \item \emph{large} $\textbf{LT}$ demand $\Theta$ token units and arrive as Poisson process $J_t\left(\lambda\right)$. \\ They are exogenously large enough to consume all liquidity on $\ell$ and $h$ pools.
\end{enumerate}
\end{block}
\vspace{0.1in}
    \begin{center}
        \includegraphics[width=\textwidth]{Figures/timing_dex_rebalance.eps}
    \end{center}


\end{frame}

\begin{frame}\frametitle{Prices}
\begin{itemize}
\item We assume a linear bonding curve -- prices occur at $v$.
\bigskip
\item Traditionally, a spread compensates market makers for adverse selection (``insider trading")
\item In these markets 
\begin{enumerate}
    \item liquidity providers do not post or earn a spread
    \item as these are assets with no cash flows, unclear what form adverse selection takes
    \item no clear ``value" benchmarks as off chain assets have a different use value. 
\end{enumerate}
\end{itemize}

    
\end{frame}



\begin{frame}{The liquidity provider problem}
\begin{itemize}
\item ${\color{red} d_k}$ is the endogenous liquidity cycle duration, which $\nearrow$ in aggregate liquidity:
\begin{eqnarray*}
d_h & = & \frac{1}{\lambda}\\
    d_\ell&=&\frac{1}{\lambda}-\frac{1}{\lambda}\exp\left(-\frac{\LL}{\theta}\lambda\right) 
\end{eqnarray*}
where $\LL$ is the aggregate liquidity on the low-fee pool.
\medskip
 \item Liquidity providers choose pool $k^\star$ to maximize expected profit per unit of time:
\begin{equation*}
\label{eq:optimal_pool}
    k^\star\left(q_i\right) = \arg\max_{\left\{\ell,h,\emptyset\right\}}   \Big[\frac{q_i \ell - \Gamma}{d_\ell} , \; \frac{q_i h -\Gamma}{d_h}, \; \emptyset\Big].
\end{equation*}
\item Trade-off between:
\begin{enumerate}
   \item higher liquidity fee per unit of time in low fee pools, and 
    \item lower rebalancing cost in high-fee pools.
\end{enumerate}
\end{itemize}
\end{frame}

\begin{frame}{Equilibrium}
\begin{itemize}
\item There is a threshold endowment $\qmg$ such that all $\LP$s with $q_i>\qmg$ post liquidity on the low-fee pool and all $\LP$s with $q_i\leq \qmg$ choose the high-fee pool. 
\begin{align*}\label{eq:liquidity_levels}
    \LL&=\int_{\qmg}^Q q_i \varphi\left(q_i\right) \diff i = \frac{Q}{Q-1}\left(\log Q - \log \qmg \right)  \text{ and }\nonumber \\
    \LH&=\int_{\underline{q}}^{\qmg}  q_i \varphi\left(q_i\right) \diff i = \frac{Q}{Q-1}\left(\log \qmg - \log \underline{q}\right)
\end{align*}
\end{itemize}
\bigskip
\begin{center}
\begin{tikzpicture}[scale= 0.5]
    \draw[thick] (0,0)--(15,0);
    \draw[thick] (10,0)--(10,1);
    \draw[thick] (15,0)--(15,1);
    \draw[thick] (0,0)--(0,1);
    \draw[thick] (5,0)--(5,1);
    \draw[thick] node[below]{$1$};
    \draw[thick] (5,0) node[below]{$\underline q$};
    \draw[thick] (10,0) node[below]{$q_t$};
    \draw[thick] (15,0) node[below]{Q};
    \draw[thick] (2.5,0) node[above]{out};
    \draw[thick] (7.5,0) node[above]{high};
    \draw[thick] (12.5,0) node[above]{low};
\end{tikzpicture}
\end{center}
\end{frame}

% \begin{frame}{High-fee pools attract small liquidity providers}
%     \begin{center}
%         \includegraphics[width=\textwidth]{Figures/liquidity_supply.png}
%     \end{center}
% \end{frame}

%
% \begin{frame}{Trading volume and liquidity in equilibrium}
%     \begin{center}
%         \includegraphics[width=\textwidth]{Figures/trade_volumesize.png}
%     \end{center}
% \end{frame}
\begin{frame}\frametitle{Evaluating the fragmented liquidity}

\begin{block}{Full participation benchmark}
    \begin{itemize}
        \item \textbf{LP} $i$ participates if $q_if>\Gamma$, or fee greater than fixed cost.
        \item Maximal {\bf LP} participation if fee=fixed cost.
        \item Difficult to implement; also costly for liquidity takers
    \end{itemize}
\end{block}

\begin{block}{Implementation shortfall benchmark \citep{perold1988}}
\begin{minipage}{0.55\textwidth}%
\begin{itemize}
\item Shortfall for the large liquidity trader:
\end{itemize}
\begin{eqnarray*}
\underbrace{\sum_k f_k {\cal L}_k}_{\mbox{trading fees}} + \underbrace{\Delta \left( \Theta - \sum_k{\cal L}_k\right)}_{\mbox{unrealized gains from trade}}
\end{eqnarray*}    
\begin{minipage}{0.1\textwidth}%
\end{minipage}
\end{minipage}
\begin{minipage}{0.4\textwidth}%
    \includegraphics[width=\textwidth]{Figures/Empirics_202308/implementation_shortfall_left.png}
\end{minipage}

\end{block}


\end{frame}

\begin{frame}{Fragmented liquidity leads to lower implementation shortfall}

\begin{block}{Proposition}
From any single fee pool, you can find a fragmented pool that reduces the large trader's implementation shortfall.
\end{block}

\begin{enumerate}
    \medskip
\item Set the high fee equal to the single-pool fee: $h=f$ (same {\bfseries LP} participation).
\item Introduce a lower fee pool $\ell<h$ such that large {\bfseries LP} migrate there.
\end{enumerate}

\begin{center}
    \includegraphics[width=\textwidth]{Figures/Empirics_202308/implementation_shortfall_right.png}
\end{center}

\end{frame}

\ifthenelse{\boolean{longtalk}}{%
\begin{frame}{Equilibrium regions}
    \begin{center}
        \includegraphics[width=\textwidth]{Figures/equilibrium_existence.png}
    \end{center}
\end{frame}
}
\ifthenelse{\boolean{longtalk}}{
\begin{frame}\frametitle{Evaluating the fragmented liquidity}
\begin{itemize}
\item LP participates if $q_if>\Gamma$, or fee greater than fixed cost.
\bigskip
\item Shortfall for the large liquidity trader:
\end{itemize}
\begin{eqnarray*}
\underbrace{\sum_k f_k {\cal L}_k}_{\mbox{trading fees}} + \underbrace{\Delta \left( \Theta - \sum_k{\cal L}_k\right)}_{\mbox{unrealized gains from trade}}
\end{eqnarray*}
\begin{itemize}
\item Higher fee: 
\begin{itemize}
    \item more posted liquidity, more gains from trade
    \item higher trading fees for trader
    \end{itemize}
\item Optimal fee for single pool

\medskip
\item For any single fee pool, a fragmented pool exists that improves the large trader's shortfall
\begin{itemize}
    \item Set high pool fee equal to optimal fee of single pool $\to$ at least a good
    \item Add a low fee pool to reduce trading fees
\end{itemize}
\end{itemize}
\end{frame} }


% \begin{frame}{Time-series predictions}
% \begin{enumerate}
%     \item The liquidity market share of low-fee pool $\searrow$ in gas fee.
%     \item Average 
% \end{enumerate}
% \end{frame}

%\section{Empirical findings}

\begin{frame}{Data}
\begin{itemize}
    \item Data from Uniswap v3 Subgraph on all trades, liquidity deposits and withdrawals from May 4, 2021 until July 15, 2023, including traders' wallet addresses. \vspace{0.1in}
    \item Gas cost is the average of the lowest daily 1000 gas prices for mint events. \vspace{0.1in}
    \item Focus on economically sizeable pools:
    \begin{enumerate}
        \item active in more than 100 days within the sample;
        \item 500+ liquidity events throughout the sample;
        \item average daily liquidity balance $>$US\$100,000;
        \item $>$1\% of volume for a traded pair.
    \end{enumerate} \vspace{0.1in}
    \item We obtain 274 pools in 242 asset pairs:
    \begin{enumerate}
        \item aggregate daily volume of US\$~1.12bn;
        \item end-of-sample aggregate liquidity US\$~2.53bn.
        \item account for 86.04\% of all Uniswap v3 interactions.
    \end{enumerate}
\end{itemize}
\end{frame}

\begin{frame}{Uniswap v3 pairs can be traded in 1, 5, 30, or 100 bps fee pools}
\begin{itemize}
    \item 32 fragmented pools collectively account for 95\% of committed liquidity and 93\% of traded volume
    \item Trading concentrates on adjacent fee levels e.g.:  USDC/USDT 1-5bps, ETH/USDC 5-30bps, USDC-CRV 30-100bps
\end{itemize}
\bigskip
\begin{enumerate}
    \item Significant fragmentation across different-fee pools for the same pair.
    \item Low-fee pools are more actively traded, but high-fee pools are deeper.
    \begin{center}
        \includegraphics[width=0.9\textwidth]{Figures/sumstat_TVL_volume.png}
    \end{center}
%\item We show that fixed transaction costs partly drive this effect.
\end{enumerate}
\end{frame}

\begin{frame}{Liquidity clienteles: high fee pools feature many small \textbf{LP}s.}
    \begin{center}
        \includegraphics[width=\textwidth]{Figures/sumstat_mint_trade.png}
        \includegraphics[width=\textwidth]{Figures/sumstat_wallets.png}
    \end{center}
\end{frame}


\ifthenelse{\boolean{longtalk}}{
\begin{frame}{Low-fee pools: Larger mints, fewer LP wallets, many small trades.\\ (Mints and Trades in log USD)}
\begin{center}


\scalebox{0.76}{
\begin{tabular}{lccccccc}
\toprule
 & \multicolumn{1}{c}{Mint size} &  \multicolumn{1}{c}{Trade size} & \multicolumn{1}{c}{Volume} & \multicolumn{1}{c}{\# Trades}  & \multicolumn{1}{c}{\# Wallets} & \multicolumn{1}{c}{Liquidity yield} & \multicolumn{1}{c}{Price range} \\
 & (1) & (2) & (3) & (4) & (5) & (6) & (7) \\
\rowcolor{red!20} 
$ d_\text{low-fee}$ & 0.73*** & -0.30*** & 0.89*** & 1.02*** & -3.40*** & 2.03*** & -0.18*** \\
\rowcolor{red!20}
 & (12.27) & (-10.05) & (14.23) & (32.95) & (-5.00) & (3.60) & (-41.84) \\
Gas price $\times$ $ d_\text{low-fee}$ & 0.37*** & 0.08*** & -0.03 & -0.22*** & -3.00*** & 3.57** & -0.00 \\
 & (4.96) & (3.75) & (-0.95) & (-7.29) & (-3.43) & (2.30) & (-0.47) \\
Gas price $\times$ $ d_\text{high-fee}$ & 0.58*** & 0.17*** & 0.24*** & 0.07** & -2.89*** & 5.57*** & -0.03*** \\
 & (7.52) & (8.81) & (5.95) & (2.46) & (-3.15) & (2.83) & (-4.65) \\
Volume & 0.37*** & 0.16*** & 0.43*** & 0.20*** & 1.22*** & 1.01 & -0.01** \\
 & (8.68) & (21.38) & (15.27) & (13.85) & (6.56) & (0.81) & (-2.56) \\
Total value locked & -0.16 & 0.11*** & 0.23** & -0.01 & -1.86 & -13.42 & -0.02 \\
 & (-1.30) & (3.54) & (1.99) & (-0.18) & (-0.99) & (-1.09) & (-0.99) \\
Volatility & -0.04 & -0.01 & -0.07 & 0.01 & -0.09 & 1.18** & 0.02*** \\
 & (-1.11) & (-1.34) & (-1.38) & (0.88) & (-1.03) & (2.21) & (3.98) \\
Constant & 1.88*** & 1.64*** & 5.27*** & 3.26*** & 10.12*** & 10.01*** & 0.59*** \\
 & (58.27) & (111.47) & (168.58) & (209.84) & (28.65) & (26.04) & (184.91) \\
Observations & 21,000 & 36,059 & 36,059 & 40,288 & 40,288 & 40,252 & 24,058 \\
 R-squared & 0.26 & 0.53 & 0.55 & 0.52 & 0.37 & 0.09 & 0.42 \\ \hline
\bottomrule
\end{tabular}
}
\end{center}
\end{frame} }

\ifthenelse{\boolean{longtalk}}{
\begin{frame}{$\Uparrow$ gas cost of liquidity management:  mid-size LPs switch to $h$ fee pool\\Small LPs leave the pools}
    \begin{center}
        \includegraphics[width=\textwidth]{Figures/mkt_share_gas.png}
    \end{center}
\end{frame} }



\ifthenelse{\boolean{longtalk}}{
\begin{frame}{Do gas prices move market shares?}
\begin{center}
    

\scalebox{0.82}{
\begin{tabular}{lccc@{\hskip 0.3in}ccc}
\toprule
 & \multicolumn{3}{c}{Liquidity market share (\%)} & \multicolumn{3}{c}{Volume market share (\%)} \\ 
 \cmidrule{1-7}
\rowcolor{red!20} $ d_\text{low-fee}$ & -20.92*** & -20.92*** & -20.92*** & 24.62*** & 24.63*** & 24.62*** \\
 & (-27.42) & (-27.41) & (-27.42) & (20.55) & (20.56) & (20.55) \\
\rowcolor{red!20} Gas price $\times$ $ d_\text{low-fee}$ & -4.63*** & -4.62*** & -4.63*** & -6.52*** & -6.52*** & -6.52*** \\
 & (-7.32) & (-7.32) & (-7.32) & (-5.92) & (-5.92) & (-5.92) \\
Gas price & 2.31*** & 2.31*** & 2.31*** & 3.63*** & 3.61*** & 3.61*** \\
 & (7.32) & (7.32) & (7.32) & (7.33) & (7.30) & (7.26) \\
Volume & 0.00 & 0.00 & 0.00 & -0.19** & -0.20** & -0.19** \\
 & (0.65) & (1.33) & (0.65) & (-2.54) & (-2.61) & (-2.50) \\
Total value locked & -0.00 & -0.00 &  & 0.58 & 0.58 &  \\
 & (-0.58) & (-0.06) &  & (1.44) & (1.44) &  \\
Volatility & -0.29 &  & -0.29 & -1.15*** &  & -1.15*** \\
 & (-0.90) &  & (-0.90) & (-2.74) &  & (-2.74) \\
Constant & 60.45*** & 60.46*** & 60.45*** & 41.96*** & 41.99*** & 41.96*** \\
 & (158.00) & (158.46) & (158.00) & (69.99) & (70.22) & (70.02) \\
Observations & 40,288 & 40,288 & 40,288 & 36,059 & 36,059 & 36,059 \\
 R-squared & 0.10 & 0.10 & 0.10 & 0.13 & 0.13 & 0.13 \\ \hline
\bottomrule
\end{tabular}



}
\end{center}
\end{frame}
}


\ifthenelse{\boolean{longtalk}}{
\begin{frame}{Liquidity flows and gas prices}
\begin{center}
    

\scalebox{0.77}{
\begin{tabular}{lcccccc}
\toprule
 & \multicolumn{3}{c}{Daily mints (log US\$)} &  \multicolumn{3}{c}{$\text{Prob}\left(\text{at least one mint}\right)$} \\
\cmidrule{1-7}
$ d_\text{low-fee}$ & 0.15* & 0.16** & 0.15* & 1.33* & 1.30* & 1.33* \\
 & (1.94) & (2.03) & (1.94) & (1.82) & (1.85) & (1.82) \\
\cellcolor{LRed}Gas price $\times$ $ d_\text{low-fee}$ & \cellcolor{LRed} -0.36*** & \cellcolor{LRed}-0.36*** & \cellcolor{LRed}-0.39*** & \cellcolor{LRed}-7.60*** & \cellcolor{LRed}-7.63*** & \cellcolor{LRed}-5.68*** \\
 & (-6.66) & (-6.43) & (-5.22) & (-9.36) & (-9.09) & (-8.22) \\
\cellcolor{LRed}Gas price $\times$ $ d_\text{high-fee}$ & \cellcolor{LRed} 0.03 & \cellcolor{LRed} 0.00 & \cellcolor{LRed} & \cellcolor{LRed}-\cellcolor{LRed}1.92*** & \cellcolor{LRed}-2.14*** & \cellcolor{LRed} \\
 & (0.33) & (0.00) &  & (-2.74) & (-2.85) &  \\
Trade volume (pair) & 0.45*** & 0.44*** & 0.45*** & 1.19 & 1.17 & 1.19 \\
 & (7.16) & (7.04) & (7.16) & (1.33) & (1.25) & (1.33) \\
Pool size (pair) & -0.45*** & -0.52*** & -0.45*** & -5.31** & -5.56** & -5.31** \\
 & (-2.75) & (-3.34) & (-2.75) & (-2.43) & (-2.52) & (-2.43) \\
Volatility & 0.02 &  & 0.02 & 1.50* &  & 1.50* \\
 & (0.73) &  & (0.73) & (1.80) &  & (1.80) \\
Gas price &  &  & 0.03 &  &  & -1.92*** \\
 &  &  & (0.33) &  &  & (-2.74) \\
Constant & 0.55 & 1.14 & 0.55 & 81.06*** & 82.73*** & 81.06*** \\
 & (0.60) & (1.36) & (0.60) & (6.12) & (5.72) & (6.12) \\
Observations & 20,454 & 21,097 & 20,454 & 21,097 & 20,454 & 20,454 \\
 R-squared & 0.51 & 0.51 & 0.51 & 0.61 & 0.62 & 0.62 \\ \hline
\bottomrule
\end{tabular}
}
\end{center}
\end{frame}
}

\begin{frame}{Re-balancing cycles}
\includegraphics[width=0.9\textwidth]{Figures/time_elapsed_distribution.png}
\includegraphics[width=0.9\textwidth]{Figures/out_of_range_distribution.png}
\end{frame}

\ifthenelse{\boolean{longtalk}}{

\begin{frame}{Gas price $\uparrow$ $\Rightarrow$ Liquidity supply on $L$ $\downarrow$ $\Rightarrow$ Re-balancing frequency $\uparrow$}
\begin{center}
    

\scalebox{0.78}{
\begin{tabular}{lcccccc}
\toprule
 & \multicolumn{3}{c}{Mint-burn time} & \multicolumn{3}{c}{Burn-mint time} \\
\cmidrule{1-7}
\rowcolor{red!20}
$ d_\text{low-fee}$ & -99.74*** & -100.17*** & -104.09*** & -157.95*** & -159.71*** & -159.69*** \\
 & (-8.86) & (-8.94) & (-9.22) & (-10.59) & (-10.81) & (-10.80) \\
\rowcolor{red!20} 
Gas price $\times$ $ d_\text{low-fee}$ & -16.65** & -15.41* & -15.80** & -11.29 & 2.95 & 2.94 \\
 & (-2.13) & (-1.98) & (-2.02) & (-1.65) & (0.40) & (0.39) \\
Gas price $\times$ $ d_\text{high-fee}$ & -14.44** & -13.42* & -13.98* & -10.52* & 1.96 & 1.95 \\
 & (-2.04) & (-1.89) & (-1.96) & (-1.69) & (0.32) & (0.32) \\
Volume &  & -5.87 & -7.45 &  & -24.84*** & -24.82*** \\
 &  & (-1.15) & (-1.41) &  & (-4.10) & (-4.09) \\
Total value locked &  & -53.17* & -51.72* &  & -12.71 & -12.71 \\
 &  & (-1.70) & (-1.66) &  & (-0.52) & (-0.52) \\
Volatility &  & -2.11*** & -2.26*** &  & -2.99*** & -2.98*** \\
 &  & (-2.75) & (-2.86) &  & (-3.36) & (-3.36) \\
Position out-of-range &  &  & 37.09*** &  &  & -1.53 \\
 &  &  & (6.43) &  &  & (-0.22) \\
Constant & 497.18*** & 497.00*** & 479.22*** & 248.00*** & 250.13*** & 250.47*** \\
 & (91.65) & (90.60) & (82.13) & (29.91) & (30.27) & (30.32) \\
Observations & 405,586 & 405,584 & 405,584 & 265,848 & 265,848 & 265,848 \\
 R-squared & 0.82 & 0.82 & 0.82 & 0.37 & 0.37 & 0.37 \\ \hline
\bottomrule
\end{tabular}
}
\end{center}
\end{frame}
}

\ifthenelse{\boolean{longtalk}}{%
\begin{frame}{Is order flow on high-fee pools more toxic?}

\begin{block}{``Impermanent loss"}
    \begin{itemize}
        \item A measure of adverse selection cost
        \item Negative return from providing liquidity as opposed to marking to market.
    \end{itemize}
\end{block}

\begin{block}{Example}
    \begin{itemize}
        \item At $t=0$, LP deposits 1 ETH and 3000 USDC (fair price).
        \item At $t=1$, value jumps to ETH/USDC 3500:
            \begin{enumerate}
                \item An arbitrageur optimally purchases ETH to bring price in line.
                \item New LP holdings: 0.92 ETH and 3240 USDC.  {\color{red} \textbf{Value:} $V_\text{pos}=\$6,480.74$.}
                \item Counterfactual (holding) value if not providing liquidity: {\color{red} \textbf{Value:} $V_\text{hold}=\$6,500$}.
            \end{enumerate}
       
        \begin{equation*}
    \text{Impermanent Loss}=\frac{V_\text{hold}-V_\text{pos}}{V_\text{hold}}=29 \text{ bps}.
        \end{equation*}
    \end{itemize}
\end{block}
    
\end{frame}
}

\ifthenelse{\boolean{longtalk}}{%
\begin{frame}{Low-fee pool LPs: adverse selection costs $\downarrow$ (controlling for activity)}
\begin{center}
    

\scalebox{0.75}{
\begin{tabular}{lcccccccc}
\toprule
& \multicolumn{8}{c}{Impermanent loss for a liquidity position with range $\left[\frac{p}{\alpha}, \alpha p\right]$ around price $p$} \\
\cmidrule{1-9} 
& \multicolumn{2}{c}{$\alpha=1.01$} & \multicolumn{2}{c}{$\alpha=1.05$} & \multicolumn{2}{c}{$\alpha=1.10$} & \multicolumn{2}{c}{$\alpha=1.25$} \\
\cmidrule{1-9}
$ d_\text{low-fee}$ & 2.59*** & -1.38 & 1.08*** & -1.85** & 0.71*** & -1.56** & 0.37** & -1.09* \\
 & (11.26) & (-1.57) & (5.72) & (-2.28) & (4.28) & (-2.18) & (2.58) & (-1.98) \\
Gas price &  & 4.75*** &  & 3.68*** &  & 2.72*** &  & 1.55*** \\
 &  & (3.97) &  & (3.96) &  & (3.86) &  & (3.42) \\
Trade count &  & 4.82*** &  & 3.56*** &  & 2.78*** &  & 1.79*** \\
 &  & (4.59) &  & (3.71) &  & (3.30) &  & (2.83) \\
Volume &  & 3.03*** &  & 1.19*** &  & 0.60** &  & 0.22 \\
 &  & (7.00) &  & (3.87) &  & (2.45) &  & (1.25) \\
Total value locked &  & 0.43 &  & 1.78 &  & 2.02 &  & 1.83 \\
 &  & (0.16) &  & (0.79) &  & (1.05) &  & (1.38) \\
Volatility &  & 6.98*** &  & 6.65** &  & 6.39** &  & 6.06** \\
 &  & (2.69) &  & (2.59) &  & (2.51) &  & (2.40) \\
Constant & 15.52*** & 15.87*** & 7.37*** & 7.65*** & 4.63*** & 4.87*** & 2.45*** & 2.66*** \\
 & (134.72) & (103.02) & (77.84) & (60.07) & (55.47) & (43.73) & (34.58) & (29.33) \\
Observations & 40,250 & 40,248 & 40,250 & 40,248 & 40,250 & 40,248 & 40,250 & 40,248 \\
 R-squared & 0.17 & 0.23 & 0.09 & 0.15 & 0.06 & 0.11 & 0.03 & 0.08 \\ \hline
\bottomrule
\end{tabular}
}
\end{center}
\end{frame}}
% {\begin{frame}{Is order flow on high-fee pools more toxic?}
% \begin{center}
    

% \scalebox{0.75}{
% \begin{tabular}{lcccccccc}
% \toprule
% & \multicolumn{8}{c}{Impermanent loss for a liquidity position with range $\left[\frac{p}{\alpha}, \alpha p\right]$ around price $p$} \\
% \cmidrule{1-9} 
% & \multicolumn{2}{c}{$\alpha=1.01$} & \multicolumn{2}{c}{$\alpha=1.05$} & \multicolumn{2}{c}{$\alpha=1.10$} & \multicolumn{2}{c}{$\alpha=1.25$} \\
% \cmidrule{1-9}
% $ d_\text{low-fee}$ & 2.59*** & -1.38 & 1.08*** & -1.85** & 0.71*** & -1.56** & 0.37** & -1.09* \\
%  & (11.26) & (-1.57) & (5.72) & (-2.28) & (4.28) & (-2.18) & (2.58) & (-1.98) \\
% Gas price &  & 4.75*** &  & 3.68*** &  & 2.72*** &  & 1.55*** \\
%  &  & (3.97) &  & (3.96) &  & (3.86) &  & (3.42) \\
% Trade count &  & 4.82*** &  & 3.56*** &  & 2.78*** &  & 1.79*** \\
%  &  & (4.59) &  & (3.71) &  & (3.30) &  & (2.83) \\
% Volume &  & 3.03*** &  & 1.19*** &  & 0.60** &  & 0.22 \\
%  &  & (7.00) &  & (3.87) &  & (2.45) &  & (1.25) \\
% Total value locked &  & 0.43 &  & 1.78 &  & 2.02 &  & 1.83 \\
%  &  & (0.16) &  & (0.79) &  & (1.05) &  & (1.38) \\
% Volatility &  & 6.98*** &  & 6.65** &  & 6.39** &  & 6.06** \\
%  &  & (2.69) &  & (2.59) &  & (2.51) &  & (2.40) \\
% Constant & 15.52*** & 15.87*** & 7.37*** & 7.65*** & 4.63*** & 4.87*** & 2.45*** & 2.66*** \\
%  & (134.72) & (103.02) & (77.84) & (60.07) & (55.47) & (43.73) & (34.58) & (29.33) \\
% Observations & 40,250 & 40,248 & 40,250 & 40,248 & 40,250 & 40,248 & 40,250 & 40,248 \\
%  R-squared & 0.17 & 0.23 & 0.09 & 0.15 & 0.06 & 0.11 & 0.03 & 0.08 \\ \hline
% \bottomrule
% \end{tabular}
% }
% \end{center}
% \end{frame}}

% \begin{frame}{Returns and costs from liquidity provision}

% Liquidity yield is computed as in \citet{augustin2022reaching}:
% \begin{equation}\label{eq:liq_yield}
%     \text{Liquidity yield}=\text{liquidity fee}_i \times \frac{\text{Volume}_{i,t}}{\text{TVL}_{i,t-1}},
% \end{equation}

%     \begin{center}
%         \includegraphics[width=\textwidth]{Figures/lyield_IL.png}
%     \end{center}
% \end{frame}


\begin{frame}{Conclusion}
    \takeaways
\end{frame}






\appendix
\begin{frame}<beamer:0> [noframenumbering]
\bibliographystyle{jf}
\bibliography{references}
\end{frame}


\end{document}

==> slides/slides_al.tex <==

\input{preamble}
\setbeamertemplate{itemize item}{\textbullet}
% Define a boolean parameter
\newboolean{longtalk}
\setboolean{longtalk}{true} % Set to 'true' to show the slides, 'false' to hide them


\newcommand{\takeaways}{
\begin{itemize}
\item Decentralized exchanges are designed for \emph{passive} liquidity provision.
\item Fixed costs to participate in markets lead to different economies of scale for heterogeneous \textbf{LP}s.
\item If fragmented: high-fee pools tend to have lower execution, lower liquidity yields and higher adverse selection cost.
\item But, fragmentation can be efficient.
\end{itemize}

\begin{center}
\begin{tabular}{ll}
\toprule
Low-fee pools & High-fee pools \\
\cmidrule{1-2}
High trading volume & Low trading volume \\
Low aggregate liquidity & High aggregate liquidity \\
Few, large \textbf{LP}s & Many, small \textbf{LP}s \\
Short liquidity cycles & Large liquidity cycles \\
\bottomrule
\end{tabular}
\end{center}

}

\begin{document}



\title{Fragmentation and Optimal Liquidity Supply on Decentralized Exchanges} 
\author[Lehar, Parlour, Zoican]{Alfred Lehar, Christine A. Parlour, and Marius Zoican}

\date{Feb 2024}

\institute[U Toronto]{Haskayne School of Business, University of Calgary \and Haas School of Business, UC Berkeley \and Rotman School of Management,  University of Toronto}

\begin{frame}[noframenumbering]
\titlepage
\end{frame}

\begin{frame}\frametitle{This paper}
\begin{itemize}
\item Use design of  an automated market maker (AMM) to study:
\medskip
\begin{itemize}
\item[\textbullet] Effect of fixed and variable costs on liquidity supply
\smallskip
\item[\textbullet] Fragmented liquidity can be beneficial
\end{itemize}
\bigskip
\item Why study an AMM?
\begin{enumerate}
\item They process a large volume of transactions.
\smallskip
\item They seem to provide more liquidity than centralized limit order markets.
\smallskip
\item As real world assets (RWA) move to tokenization models, trading may migrate.
\smallskip
\item Costs/benefits to supplying liquidity is cleaner to observe than in centralized markets.
\end{enumerate}

\end{itemize}


\end{frame}

\begin{frame}{Decentralized exchanges (DEX) trade}
    \begin{center}
        \includegraphics[width=\textwidth]{Figures/dex-volume-monthly.png}
    \end{center}
\end{frame}

\begin{frame}{DEX have substantial liquidity (at least in major pairs)}
    \begin{center}
        \includegraphics[width=\textwidth]{Figures/chartkaiko.png}
    \end{center}
\end{frame}


\begin{frame}\frametitle{Uniswap - Details}
\begin{itemize}
\item UniSwap is a decentralized protocol originally on the Ethereum Blockchain
\item Uniswap comprises tens of thousands of liquidity pools
\begin{itemize}
\item[\textbullet] Each pool has two assets -- all trades are swaps
\end{itemize}
\bigskip
\item There are three versions of Uniswap (v1,v2,v3)
\medskip
\item Features common to all versions:
\begin{itemize}
\item[\textbullet] Agents choose to supply or demand liquidity
\item[\textbullet] Transaction prices automatically calculated as a function of liquidity demand and supply.
\item[\textbullet] Only payoff for liquidity supplier is a \% fee paid by the liquidity demander.
\end{itemize}
\medskip
\item Unique to v3
\begin{itemize}
\item[\textbullet] Variable fees:  Each asset pair can trade in 1, 5, 30 or 100bps pools.
\item[\textbullet] Concentrated liquidity:  Liquidity suppliers can choose the price range over which they supply liquidity 
\end{itemize}
\end{itemize}
\end{frame}


\begin{frame}\frametitle{Uniswap -- Liquidity Provision v2 \\ A Pool with Ethereum ``E'' and a token ``T''}

\begin{minipage}{0.35\textwidth}%
\begin{tikzpicture}
\draw(0,1) circle(0.5in);
\draw[thick,dashed](-1.15,0.45)--(1.15,0.45);
\draw(0,1) node[above]{E};
\draw(0,0.35) node[below]{T};
\end{tikzpicture}
\end{minipage} %
\begin{minipage}{0.55\textwidth}%
\begin{itemize}
\item Liquidity suppliers deposit Eth and T

\medskip
\item Liquidity demander who buys the token, removes it from the pool and deposits Eth.
\item Liquidity demander who sells the token, adds it to the pool and withdraws Eth.

\bigskip
\item Liquidity demanders pay a fixed, proportional fee which is passed through to the liquidity suppliers.

\end{itemize}
\end{minipage}

\end{frame}




\begin{frame}\frametitle{Price Impact to sell $\Delta_T$ tokens}
\begin{minipage}{0.25 \textwidth}
\begin{tikzpicture}[scale=0.35]
\draw[thick,->] (0,0)-- (15,0);
\draw[thick,->] (0,0) -- (0,10);
\draw (0,8) node[left]{Eth};
\draw(10,0) node[below]{Token};
\draw[dotted,red, thick](0,5)--(4,5);
\draw[dotted,red,thick](4,5)--(4,0);
\draw (0,5) node[left]{$E_0$};
\draw (4,0) node[below]{$T_0$};
\draw(6,0) node[below]{$ T_1$};
\draw(5,-1.5) node[below] {$\Delta_T$}; 
\draw[dotted,blue,thick](6,0)--(6,3.9);
\draw[dotted,blue,thick](0,3.9)--(6,3.9);
\draw(0,3.9) node[left]{$E_1$};
\draw plot[smooth] coordinates {(2,10)  (4,5) (12,1.9)};
\end{tikzpicture}
\end{minipage}
\begin{minipage}{0.2\textwidth}
\hspace{1in}
\end{minipage}
\begin{minipage}{0.45 \textwidth}
\begin{itemize}
\item For negligible quantities, the exchange between Eth and the Token is E/T
\item For larger trades, the exchange rate is determined by a ``bonding curve.''
\item For given $E$ and $T$, so $ET=k$: \end{itemize}
\begin{eqnarray*}
(E + \Delta_E)(T+\Delta_T) = k
\end{eqnarray*}
\begin{itemize}
\item As more liquidity is supplied, bonding curve shifts out.
\end{itemize}
\end{minipage}
\end{frame}

\begin{frame}{Unique to v3:  Concentrated Liquidity}
\begin{itemize}
    \item On Uniswap v3, liquidity providers can specify price limits on their positions.
    \item If the current pool price (e.g., ``midpoint'') is outside the range, the position does not earn fees.
    \item $\rightarrow$ incentive to re-price the position to capture fees.
\end{itemize}
    \begin{center}
        \includegraphics[width=\textwidth]{Figures/uniswapv3_positions.png}
    \end{center}
\end{frame}

\begin{frame}
\frametitle{Managing liquidity on DEX is costly}
\begin{center}
   \includegraphics[width=\textwidth]{Figures/usp3_mechanism.eps}
\end{center}
\end{frame}

\begin{frame}{Fixed cost of supplying liquidity (gas fee) on Uniswap v3}
    \begin{center}
        \includegraphics[width=\textwidth]{Figures/gas_timeline.png}
    \end{center}
\end{frame}





\begin{frame}{Liquidity Provision on a DEX}

\bigskip

    \begin{enumerate}
    \item Unique laboratory to study how transaction costs affect the market for liquidity.
        \item DEX  designed for \textbf{passive} liquidity provision. \vspace{0.05in}
        %\item ``\emph{Set-it-and-forget-it}'' liquidity: i.e., what ETFs did for portfolio management. \vspace{0.05in}
        \item On v3 actively managing liquidity is costly:
            \begin{enumerate}
                \item \emph{gas price} from interacting with Ethereum blockchain. \vspace{0.05in}
                \item \emph{time/effort} to monitoring the position.
            \end{enumerate}
        \vspace{0.05in}
        %\item Economies of scale: small liquidity providers face higher relative costs.\vspace{0.05in}
         
    \end{enumerate}
    \medskip

\citet{demsetz1968}: ``the question that is relevant for efficiency is whether or not the cost is appropriately economized.''  

    
    \end{frame}

% \begin{frame}{Decentralized exchanges $\approx$ 20\% of crypto trading volume}
%     \begin{center}
%         \includegraphics[width=\textwidth]{Figures/dex-volume-monthly.png}
%     \end{center}
% \end{frame}







\begin{frame}\frametitle{Results}

\vspace{0.1in}

\begin{alertblock}{Theory and  evidence of LP ``clienteles'' based on their scale:}
\bigskip

\begin{enumerate}
    \item Small LPs are more passive, have  lower fill rates but get high fees. 
    \item Large LPs are more active, have higher fill rates but get low fees.
    \item This segmentation can be efficient
\end{enumerate}


\end{alertblock}

\end{frame}

\begin{frame}{Related literature}
We contribute to: \vspace{0.1in}
    \begin{itemize}
       \item  a growing literature on decentralized exchanges \citep{LeharParlour2021, caparros2023blockchain, augustin2022reaching, kp2023dex, capponi2023price, CapponiJia2021, BarbonRanaldo2021, HasbrouckRiveraSaleh2022}. \vspace{0.1in}
       \item the literature on optimal routing for retail orders \citep{Battalio2016,Cimon2021, FoucaultMenkveld2008}. \vspace{0.1in}
       \item the literature on make/take fees on  liquidity provision \citep{foucault2013liquidity, YaoYe2018,LiWangYe2021}
       
    \end{itemize}
\end{frame}


%\section{Model}

\begin{frame}{Model}

\begin{block}{Asset and markets.} \begin{itemize}
    \item Token with expected value $v$ trades on two liquidity pools with fees $h>\ell>0$.
    \item Fixed cost $\Gamma>0$ of interacting with the pool (e.g., gas fee).
\end{itemize}
\end{block}

\begin{block}{Liquidity providers (\textbf{LP})}

 \begin{tabular}{cl}  
     \begin{tabular}{l}
            \parbox{0.35\linewidth}{%  change the parbox width as appropriate
                \begin{itemize}
        \item Risk-neutral;
        \item Token endowments $q_i$; \item $q_i$ follows a bounded Pareto distribution:
        \begin{equation*}\label{eq:density}
    \varphi\left(q\right)=\Big(\frac{Q}{Q-1}\Big) \frac{1}{q^2}.
    \end{equation*}
    \end{itemize}}
       \end{tabular}
    &\begin{tabular}{c}
            \includegraphics[width=8.5cm]{Figures/model_density.png}
        \end{tabular}  
   \end{tabular}

\end{block}

\end{frame}



\begin{frame}{Timeline}

\begin{block}{Liquidity takers (\textbf{LT}).} Two types of $\textbf{LT}$: 
\begin{enumerate}
    \item \emph{small} $\textbf{LT}$ arrive at constant rate $\theta \diff t$ and optimally go to the low-fee pool first ($\ell$). 
    \item \emph{large} $\textbf{LT}$ demand $\Theta$ token units and arrive as Poisson process $J_t\left(\lambda\right)$. \\ They are exogenously large enough to consume all liquidity on $\ell$ and $h$ pools.
\end{enumerate}
\end{block}
\vspace{0.1in}
    \begin{center}
        \includegraphics[width=\textwidth]{Figures/timing_dex_rebalance.eps}
    \end{center}


\end{frame}

\begin{frame}\frametitle{Prices}
\begin{itemize}
\item We assume a linear bonding curve -- prices occur at $v$.
\bigskip
\item Traditionally, a spread compensates market makers for adverse selection (``insider trading")
\item In these markets 
\begin{enumerate}
    \item liquidity providers do not post or earn a spread
    \item as these are assets with no cash flows, unclear what form adverse selection takes
    \item no clear ``value" benchmarks as off chain assets have a different use value. 
\end{enumerate}
\end{itemize}

    
\end{frame}



\begin{frame}{The liquidity provider problem}
\begin{itemize}
\item ${\color{red} d_k}$ is the endogenous liquidity cycle duration, which $\nearrow$ in aggregate liquidity:
\begin{eqnarray*}
d_h & = & \frac{1}{\lambda}\\
    d_\ell&=&\frac{1}{\lambda}-\frac{1}{\lambda}\exp\left(-\frac{\LL}{\theta}\lambda\right) 
\end{eqnarray*}
where $\LL$ is the aggregate liquidity on the low-fee pool.
\medskip
 \item Liquidity providers choose pool $k^\star$ to maximize expected profit per unit of time:
\begin{equation*}
\label{eq:optimal_pool}
    k^\star\left(q_i\right) = \arg\max_{\left\{\ell,h,\emptyset\right\}}   \Big[\frac{q_i \ell - \Gamma}{d_\ell} , \; \frac{q_i h -\Gamma}{d_h}, \; \emptyset\Big].
\end{equation*}
\item Trade-off between:
\begin{enumerate}
   \item higher liquidity fee per unit of time in low fee pools, and 
    \item lower rebalancing cost in high-fee pools.
\end{enumerate}
\end{itemize}
\end{frame}

\begin{frame}{Equilibrium}
\begin{itemize}
\item There is a threshold endowment $\qmg$ such that all $\LP$s with $q_i>\qmg$ post liquidity on the low-fee pool and all $\LP$s with $q_i\leq \qmg$ choose the high-fee pool. 
\begin{align*}\label{eq:liquidity_levels}
    \LL&=\int_{\qmg}^Q q_i \varphi\left(q_i\right) \diff i = \frac{Q}{Q-1}\left(\log Q - \log \qmg \right)  \text{ and }\nonumber \\
    \LH&=\int_{\underline{q}}^{\qmg}  q_i \varphi\left(q_i\right) \diff i = \frac{Q}{Q-1}\left(\log \qmg - \log \underline{q}\right)
\end{align*}
\end{itemize}
\bigskip
\begin{center}
\begin{tikzpicture}[scale= 0.5]
    \draw[thick] (0,0)--(15,0);
    \draw[thick] (10,0)--(10,1);
    \draw[thick] (15,0)--(15,1);
    \draw[thick] (0,0)--(0,1);
    \draw[thick] (5,0)--(5,1);
    \draw[thick] node[below]{$1$};
    \draw[thick] (5,0) node[below]{$\underline q$};
    \draw[thick] (10,0) node[below]{$q_t$};
    \draw[thick] (15,0) node[below]{Q};
    \draw[thick] (2.5,0) node[above]{out};
    \draw[thick] (7.5,0) node[above]{high};
    \draw[thick] (12.5,0) node[above]{low};
\end{tikzpicture}
\end{center}
\end{frame}

\begin{frame}{High-fee pools attract small liquidity providers}
    \begin{center}
        \includegraphics[width=\textwidth]{Figures/liquidity_supply.png}
    \end{center}
\end{frame}

\ifthenelse{\boolean{longtalk}}{%
\begin{frame}{Trading volume and liquidity in equilibrium}
    \begin{center}
        \includegraphics[width=\textwidth]{Figures/trade_volumesize.png}
    \end{center}
\end{frame}}

\ifthenelse{\boolean{longtalk}}{%
\begin{frame}{Equilibrium regions}
    \begin{center}
        \includegraphics[width=\textwidth]{Figures/equilibrium_existence.png}
    \end{center}
\end{frame}
}

\begin{frame}\frametitle{Evaluating the fragmented liquidity}
\begin{itemize}
\item LP participates if $q_if>\Gamma$, or fee greater than fixed cost.
\item Maximal {\bf LP} participation if fee=fixed cost.
\item Difficult to implement
\bigskip
\item Shortfall for the large liquidity trader:
\end{itemize}
\begin{eqnarray*}
\underbrace{\sum_k f_k {\cal L}_k}_{\mbox{trading fees}} + \underbrace{\Delta \left( \Theta - \sum_k{\cal L}_k\right)}_{\mbox{unrealized gains from trade}}
\end{eqnarray*}
\begin{itemize}

\medskip
\item From any single fee pool, you can find a fragmented pool that improves the large trader's shortfall
\item Set $f=h$, and introduce a lower fee pool.
\end{itemize}

\end{frame}


% \begin{frame}{Time-series predictions}
% \begin{enumerate}
%     \item The liquidity market share of low-fee pool $\searrow$ in gas fee.
%     \item Average 
% \end{enumerate}
% \end{frame}

%\section{Empirical findings}

\begin{frame}{Data}
\begin{itemize}
    \item Data from Uniswap v3 Subgraph on all trades, liquidity deposits and withdrawals from May 4, 2021 until July 15, 2023, including traders' wallet addresses. \vspace{0.1in}
    \item Gas cost is the average of the lowest daily 1000 gas prices for mint events. \vspace{0.1in}
    \item Focus on economically sizeable pools:
    \begin{enumerate}
        \item active in more than 100 days within the sample;
        \item 500+ liquidity events throughout the sample;
        \item average daily liquidity balance $>$US\$100,000;
        \item $>$1\% of volume for a traded pair.
    \end{enumerate} \vspace{0.1in}
    \item We obtain 274 pools in 242 asset pairs:
    \begin{enumerate}
        \item aggregate daily volume of US\$~1.12bn;
        \item end-of-sample aggregate liquidity US\$~2.53bn.
        \item account for 86.04\% of all Uniswap v3 interactions.
    \end{enumerate}
\end{itemize}
\end{frame}

\begin{frame}{Uniswap v3 pairs can be traded in 1, 5, 30, or 100 bps fee pools}
\begin{itemize}
    \item 32 fragmented pools collectively account for 95\% of committed liquidity and 93\% of traded volume
    \item Trading concentrates on adjacent fee levels e.g.:  USDC/USDT 1-5bps, ETH/USDC 5-30bps, USDC-CRV 30-100bps
\end{itemize}
\bigskip
\begin{enumerate}
    \item Significant fragmentation across different-fee pools for the same pair.
    \item Low-fee pools are more actively traded, but high-fee pools are deeper.
    \begin{center}
        \includegraphics[width=0.9\textwidth]{Figures/sumstat_TVL_volume.png}
    \end{center}
%\item We show that fixed transaction costs partly drive this effect.
\end{enumerate}
\end{frame}

\begin{frame}{Liquidity clienteles: high fee pools feature many small \textbf{LP}s.}
    \begin{center}
        \includegraphics[width=\textwidth]{Figures/sumstat_mint_trade.png}
        \includegraphics[width=\textwidth]{Figures/sumstat_wallets.png}
    \end{center}
\end{frame}

\begin{frame}{Low-fee pools: Larger mints, fewer LP wallets, many small trades.\\ (Mints and Trades in log USD)}
\begin{center}


\scalebox{0.76}{
\begin{tabular}{lccccccc}
\toprule
 & \multicolumn{1}{c}{Mint size} &  \multicolumn{1}{c}{Trade size} & \multicolumn{1}{c}{Volume} & \multicolumn{1}{c}{\# Trades}  & \multicolumn{1}{c}{\# Wallets} & \multicolumn{1}{c}{Liquidity yield} & \multicolumn{1}{c}{Price range} \\
 & (1) & (2) & (3) & (4) & (5) & (6) & (7) \\
\rowcolor{red!20} 
$ d_\text{low-fee}$ & 0.73*** & -0.30*** & 0.89*** & 1.02*** & -3.40*** & 2.03*** & -0.18*** \\
\rowcolor{red!20}
 & (12.27) & (-10.05) & (14.23) & (32.95) & (-5.00) & (3.60) & (-41.84) \\
Gas price $\times$ $ d_\text{low-fee}$ & 0.37*** & 0.08*** & -0.03 & -0.22*** & -3.00*** & 3.57** & -0.00 \\
 & (4.96) & (3.75) & (-0.95) & (-7.29) & (-3.43) & (2.30) & (-0.47) \\
Gas price $\times$ $ d_\text{high-fee}$ & 0.58*** & 0.17*** & 0.24*** & 0.07** & -2.89*** & 5.57*** & -0.03*** \\
 & (7.52) & (8.81) & (5.95) & (2.46) & (-3.15) & (2.83) & (-4.65) \\
Volume & 0.37*** & 0.16*** & 0.43*** & 0.20*** & 1.22*** & 1.01 & -0.01** \\
 & (8.68) & (21.38) & (15.27) & (13.85) & (6.56) & (0.81) & (-2.56) \\
Total value locked & -0.16 & 0.11*** & 0.23** & -0.01 & -1.86 & -13.42 & -0.02 \\
 & (-1.30) & (3.54) & (1.99) & (-0.18) & (-0.99) & (-1.09) & (-0.99) \\
Volatility & -0.04 & -0.01 & -0.07 & 0.01 & -0.09 & 1.18** & 0.02*** \\
 & (-1.11) & (-1.34) & (-1.38) & (0.88) & (-1.03) & (2.21) & (3.98) \\
Constant & 1.88*** & 1.64*** & 5.27*** & 3.26*** & 10.12*** & 10.01*** & 0.59*** \\
 & (58.27) & (111.47) & (168.58) & (209.84) & (28.65) & (26.04) & (184.91) \\
Observations & 21,000 & 36,059 & 36,059 & 40,288 & 40,288 & 40,252 & 24,058 \\
 R-squared & 0.26 & 0.53 & 0.55 & 0.52 & 0.37 & 0.09 & 0.42 \\ \hline
\bottomrule
\end{tabular}
}
\end{center}
\end{frame}

\begin{frame}{$\Uparrow$ gas $\Uparrow$ cost of liquidity management:  Smaller LPs switch to $h$ fee pool}
    \begin{center}
        \includegraphics[width=\textwidth]{Figures/mkt_share_gas.png}
    \end{center}
\end{frame}




\begin{frame}{Do gas prices move market shares?}
\begin{center}
    

\scalebox{0.82}{
\begin{tabular}{lccc@{\hskip 0.3in}ccc}
\toprule
 & \multicolumn{3}{c}{Liquidity market share (\%)} & \multicolumn{3}{c}{Volume market share (\%)} \\ 
 \cmidrule{1-7}
\rowcolor{red!20} $ d_\text{low-fee}$ & -20.92*** & -20.92*** & -20.92*** & 24.62*** & 24.63*** & 24.62*** \\
 & (-27.42) & (-27.41) & (-27.42) & (20.55) & (20.56) & (20.55) \\
\rowcolor{red!20} Gas price $\times$ $ d_\text{low-fee}$ & -4.63*** & -4.62*** & -4.63*** & -6.52*** & -6.52*** & -6.52*** \\
 & (-7.32) & (-7.32) & (-7.32) & (-5.92) & (-5.92) & (-5.92) \\
Gas price & 2.31*** & 2.31*** & 2.31*** & 3.63*** & 3.61*** & 3.61*** \\
 & (7.32) & (7.32) & (7.32) & (7.33) & (7.30) & (7.26) \\
Volume & 0.00 & 0.00 & 0.00 & -0.19** & -0.20** & -0.19** \\
 & (0.65) & (1.33) & (0.65) & (-2.54) & (-2.61) & (-2.50) \\
Total value locked & -0.00 & -0.00 &  & 0.58 & 0.58 &  \\
 & (-0.58) & (-0.06) &  & (1.44) & (1.44) &  \\
Volatility & -0.29 &  & -0.29 & -1.15*** &  & -1.15*** \\
 & (-0.90) &  & (-0.90) & (-2.74) &  & (-2.74) \\
Constant & 60.45*** & 60.46*** & 60.45*** & 41.96*** & 41.99*** & 41.96*** \\
 & (158.00) & (158.46) & (158.00) & (69.99) & (70.22) & (70.02) \\
Observations & 40,288 & 40,288 & 40,288 & 36,059 & 36,059 & 36,059 \\
 R-squared & 0.10 & 0.10 & 0.10 & 0.13 & 0.13 & 0.13 \\ \hline
\bottomrule
\end{tabular}



}
\end{center}
\end{frame}



\begin{frame}{Liquidity flows and gas prices}
\begin{center}
    

\scalebox{0.77}{
\begin{tabular}{lcccccc}
\toprule
 & \multicolumn{3}{c}{Daily mints (log US\$)} &  \multicolumn{3}{c}{$\text{Prob}\left(\text{at least one mint}\right)$} \\
\cmidrule{1-7}
$ d_\text{low-fee}$ & 0.15* & 0.16** & 0.15* & 1.33* & 1.30* & 1.33* \\
 & (1.94) & (2.03) & (1.94) & (1.82) & (1.85) & (1.82) \\
\cellcolor{LRed}Gas price $\times$ $ d_\text{low-fee}$ & \cellcolor{LRed} -0.36*** & \cellcolor{LRed}-0.36*** & \cellcolor{LRed}-0.39*** & \cellcolor{LRed}-7.60*** & \cellcolor{LRed}-7.63*** & \cellcolor{LRed}-5.68*** \\
 & (-6.66) & (-6.43) & (-5.22) & (-9.36) & (-9.09) & (-8.22) \\
\cellcolor{LRed}Gas price $\times$ $ d_\text{high-fee}$ & \cellcolor{LRed} 0.03 & \cellcolor{LRed} 0.00 & \cellcolor{LRed} & \cellcolor{LRed}-\cellcolor{LRed}1.92*** & \cellcolor{LRed}-2.14*** & \cellcolor{LRed} \\
 & (0.33) & (0.00) &  & (-2.74) & (-2.85) &  \\
Trade volume (pair) & 0.45*** & 0.44*** & 0.45*** & 1.19 & 1.17 & 1.19 \\
 & (7.16) & (7.04) & (7.16) & (1.33) & (1.25) & (1.33) \\
Pool size (pair) & -0.45*** & -0.52*** & -0.45*** & -5.31** & -5.56** & -5.31** \\
 & (-2.75) & (-3.34) & (-2.75) & (-2.43) & (-2.52) & (-2.43) \\
Volatility & 0.02 &  & 0.02 & 1.50* &  & 1.50* \\
 & (0.73) &  & (0.73) & (1.80) &  & (1.80) \\
Gas price &  &  & 0.03 &  &  & -1.92*** \\
 &  &  & (0.33) &  &  & (-2.74) \\
Constant & 0.55 & 1.14 & 0.55 & 81.06*** & 82.73*** & 81.06*** \\
 & (0.60) & (1.36) & (0.60) & (6.12) & (5.72) & (6.12) \\
Observations & 20,454 & 21,097 & 20,454 & 21,097 & 20,454 & 20,454 \\
 R-squared & 0.51 & 0.51 & 0.51 & 0.61 & 0.62 & 0.62 \\ \hline
\bottomrule
\end{tabular}
}
\end{center}
\end{frame}

\begin{frame}{Re-balancing cycles}
\includegraphics[width=0.9\textwidth]{Figures/time_elapsed_distribution.png}
\includegraphics[width=0.9\textwidth]{Figures/out_of_range_distribution.png}
\end{frame}



\begin{frame}{Gas price $\uparrow$ $\Rightarrow$ Liquidity supply on $L$ $\downarrow$ $\Rightarrow$ Re-balancing frequency $\uparrow$}
\begin{center}
    

\scalebox{0.78}{
\begin{tabular}{lcccccc}
\toprule
 & \multicolumn{3}{c}{Mint-burn time} & \multicolumn{3}{c}{Burn-mint time} \\
\cmidrule{1-7}
\rowcolor{red!20}
$ d_\text{low-fee}$ & -99.74*** & -100.17*** & -104.09*** & -157.95*** & -159.71*** & -159.69*** \\
 & (-8.86) & (-8.94) & (-9.22) & (-10.59) & (-10.81) & (-10.80) \\
\rowcolor{red!20} 
Gas price $\times$ $ d_\text{low-fee}$ & -16.65** & -15.41* & -15.80** & -11.29 & 2.95 & 2.94 \\
 & (-2.13) & (-1.98) & (-2.02) & (-1.65) & (0.40) & (0.39) \\
Gas price $\times$ $ d_\text{high-fee}$ & -14.44** & -13.42* & -13.98* & -10.52* & 1.96 & 1.95 \\
 & (-2.04) & (-1.89) & (-1.96) & (-1.69) & (0.32) & (0.32) \\
Volume &  & -5.87 & -7.45 &  & -24.84*** & -24.82*** \\
 &  & (-1.15) & (-1.41) &  & (-4.10) & (-4.09) \\
Total value locked &  & -53.17* & -51.72* &  & -12.71 & -12.71 \\
 &  & (-1.70) & (-1.66) &  & (-0.52) & (-0.52) \\
Volatility &  & -2.11*** & -2.26*** &  & -2.99*** & -2.98*** \\
 &  & (-2.75) & (-2.86) &  & (-3.36) & (-3.36) \\
Position out-of-range &  &  & 37.09*** &  &  & -1.53 \\
 &  &  & (6.43) &  &  & (-0.22) \\
Constant & 497.18*** & 497.00*** & 479.22*** & 248.00*** & 250.13*** & 250.47*** \\
 & (91.65) & (90.60) & (82.13) & (29.91) & (30.27) & (30.32) \\
Observations & 405,586 & 405,584 & 405,584 & 265,848 & 265,848 & 265,848 \\
 R-squared & 0.82 & 0.82 & 0.82 & 0.37 & 0.37 & 0.37 \\ \hline
\bottomrule
\end{tabular}
}
\end{center}
\end{frame}

\ifthenelse{\boolean{longtalk}}{%
\begin{frame}{Is order flow on high-fee pools more toxic?}

\begin{block}{``Impermanent loss"}
    \begin{itemize}
        \item A measure of adverse selection cost
        \item Negative return from providing liquidity as opposed to marking to market.
    \end{itemize}
\end{block}

\begin{block}{Example}
    \begin{itemize}
        \item At $t=0$, LP deposits 1 ETH and 3000 USDC (fair price).
        \item At $t=1$, value jumps to ETH/USDC 3500:
            \begin{enumerate}
                \item An arbitrageur optimally purchases ETH to bring price in line.
                \item New LP holdings: 0.92 ETH and 3240 USDC.  {\color{red} \textbf{Value:} $V_\text{pos}=\$6,480.74$.}
                \item Counterfactual (holding) value if not providing liquidity: {\color{red} \textbf{Value:} $V_\text{hold}=\$6,500$}.
            \end{enumerate}
       
        \begin{equation*}
    \text{Impermanent Loss}=\frac{V_\text{hold}-V_\text{pos}}{V_\text{hold}}=29 \text{ bps}.
        \end{equation*}
    \end{itemize}
\end{block}
    
\end{frame}
}

\ifthenelse{\boolean{longtalk}}{%
\begin{frame}{Low-fee pool LPs: adverse selection costs $\downarrow$ (controlling for activity)}
\begin{center}
    

\scalebox{0.75}{
\begin{tabular}{lcccccccc}
\toprule
& \multicolumn{8}{c}{Impermanent loss for a liquidity position with range $\left[\frac{p}{\alpha}, \alpha p\right]$ around price $p$} \\
\cmidrule{1-9} 
& \multicolumn{2}{c}{$\alpha=1.01$} & \multicolumn{2}{c}{$\alpha=1.05$} & \multicolumn{2}{c}{$\alpha=1.10$} & \multicolumn{2}{c}{$\alpha=1.25$} \\
\cmidrule{1-9}
$ d_\text{low-fee}$ & 2.59*** & -1.38 & 1.08*** & -1.85** & 0.71*** & -1.56** & 0.37** & -1.09* \\
 & (11.26) & (-1.57) & (5.72) & (-2.28) & (4.28) & (-2.18) & (2.58) & (-1.98) \\
Gas price &  & 4.75*** &  & 3.68*** &  & 2.72*** &  & 1.55*** \\
 &  & (3.97) &  & (3.96) &  & (3.86) &  & (3.42) \\
Trade count &  & 4.82*** &  & 3.56*** &  & 2.78*** &  & 1.79*** \\
 &  & (4.59) &  & (3.71) &  & (3.30) &  & (2.83) \\
Volume &  & 3.03*** &  & 1.19*** &  & 0.60** &  & 0.22 \\
 &  & (7.00) &  & (3.87) &  & (2.45) &  & (1.25) \\
Total value locked &  & 0.43 &  & 1.78 &  & 2.02 &  & 1.83 \\
 &  & (0.16) &  & (0.79) &  & (1.05) &  & (1.38) \\
Volatility &  & 6.98*** &  & 6.65** &  & 6.39** &  & 6.06** \\
 &  & (2.69) &  & (2.59) &  & (2.51) &  & (2.40) \\
Constant & 15.52*** & 15.87*** & 7.37*** & 7.65*** & 4.63*** & 4.87*** & 2.45*** & 2.66*** \\
 & (134.72) & (103.02) & (77.84) & (60.07) & (55.47) & (43.73) & (34.58) & (29.33) \\
Observations & 40,250 & 40,248 & 40,250 & 40,248 & 40,250 & 40,248 & 40,250 & 40,248 \\
 R-squared & 0.17 & 0.23 & 0.09 & 0.15 & 0.06 & 0.11 & 0.03 & 0.08 \\ \hline
\bottomrule
\end{tabular}
}
\end{center}
\end{frame}}
{\begin{frame}{Is order flow on high-fee pools more toxic?}
\begin{center}
    

\scalebox{0.75}{
\begin{tabular}{lcccccccc}
\toprule
& \multicolumn{8}{c}{Impermanent loss for a liquidity position with range $\left[\frac{p}{\alpha}, \alpha p\right]$ around price $p$} \\
\cmidrule{1-9} 
& \multicolumn{2}{c}{$\alpha=1.01$} & \multicolumn{2}{c}{$\alpha=1.05$} & \multicolumn{2}{c}{$\alpha=1.10$} & \multicolumn{2}{c}{$\alpha=1.25$} \\
\cmidrule{1-9}
$ d_\text{low-fee}$ & 2.59*** & -1.38 & 1.08*** & -1.85** & 0.71*** & -1.56** & 0.37** & -1.09* \\
 & (11.26) & (-1.57) & (5.72) & (-2.28) & (4.28) & (-2.18) & (2.58) & (-1.98) \\
Gas price &  & 4.75*** &  & 3.68*** &  & 2.72*** &  & 1.55*** \\
 &  & (3.97) &  & (3.96) &  & (3.86) &  & (3.42) \\
Trade count &  & 4.82*** &  & 3.56*** &  & 2.78*** &  & 1.79*** \\
 &  & (4.59) &  & (3.71) &  & (3.30) &  & (2.83) \\
Volume &  & 3.03*** &  & 1.19*** &  & 0.60** &  & 0.22 \\
 &  & (7.00) &  & (3.87) &  & (2.45) &  & (1.25) \\
Total value locked &  & 0.43 &  & 1.78 &  & 2.02 &  & 1.83 \\
 &  & (0.16) &  & (0.79) &  & (1.05) &  & (1.38) \\
Volatility &  & 6.98*** &  & 6.65** &  & 6.39** &  & 6.06** \\
 &  & (2.69) &  & (2.59) &  & (2.51) &  & (2.40) \\
Constant & 15.52*** & 15.87*** & 7.37*** & 7.65*** & 4.63*** & 4.87*** & 2.45*** & 2.66*** \\
 & (134.72) & (103.02) & (77.84) & (60.07) & (55.47) & (43.73) & (34.58) & (29.33) \\
Observations & 40,250 & 40,248 & 40,250 & 40,248 & 40,250 & 40,248 & 40,250 & 40,248 \\
 R-squared & 0.17 & 0.23 & 0.09 & 0.15 & 0.06 & 0.11 & 0.03 & 0.08 \\ \hline
\bottomrule
\end{tabular}
}
\end{center}
\end{frame}}

\begin{frame}{Returns and costs from liquidity provision}

Liquidity yield is computed as in \citet{augustin2022reaching}:
\begin{equation}\label{eq:liq_yield}
    \text{Liquidity yield}=\text{liquidity fee}_i \times \frac{\text{Volume}_{i,t}}{\text{TVL}_{i,t-1}},
\end{equation}

    \begin{center}
        \includegraphics[width=\textwidth]{Figures/lyield_IL.png}
    \end{center}
\end{frame}


\begin{frame}{Conclusion}
    \takeaways
\end{frame}






\appendix
\begin{frame}<beamer:0> [noframenumbering]
\bibliographystyle{jf}
\bibliography{references}
\end{frame}


\end{document}

==> slides/slides_mz.tex <==

\input{preamble}
\setbeamertemplate{itemize item}{\textbullet}
% Define a boolean parameter
\newboolean{longtalk}
\setboolean{longtalk}{true} % Set to 'true' to show the slides, 'false' to hide them


\newcommand{\takeaways}{
\begin{itemize}
\item Decentralized exchanges are designed for \emph{passive} liquidity provision.
\item Fixed costs to participate in markets lead to different economies of scale for heterogeneous \textbf{LP}s.
\item If fragmented: high-fee pools tend to have lower execution, lower liquidity yields and higher adverse selection cost.
\item But, fragmentation can be efficient.
\end{itemize}

\begin{center}
\begin{tabular}{ll}
\toprule
Low-fee pools & High-fee pools \\
\cmidrule{1-2}
High trading volume & Low trading volume \\
Low aggregate liquidity & High aggregate liquidity \\
Few, large \textbf{LP}s & Many, small \textbf{LP}s \\
Short liquidity cycles & Large liquidity cycles \\
\bottomrule
\end{tabular}
\end{center}

}

\begin{document}



\title[Liquidity fragmentation on decentralized exchanges]{Fragmentation and optimal liquidity supply \\ on decentralized exchanges}
\author[Lehar, Parlour, Zoican]{Alfred Lehar, Christine A. Parlour, and Marius Zoican}

\date{May 2024}

\institute[U Toronto]{Haskayne School of Business, University of Calgary \and Haas School of Business, UC Berkeley \and Rotman School of Management,  University of Toronto}

\begin{frame}[noframenumbering]
\titlepage
\end{frame}

\begin{frame}{Decentralized exchanges (DEX) trade}
    \begin{center}
        \includegraphics[width=0.97\textwidth]{Figures/dex-volume-monthly.png}
    \end{center}
\end{frame}

\begin{frame}{DEX can provide better liquidity than centralized exchanges}
    \begin{center}
        \includegraphics[width=\textwidth]{Figures/chartkaiko.png}
    \end{center}
\end{frame}

\begin{frame}\frametitle{What do we do?}
\begin{itemize}
\item Use the design of  an automated market maker (AMM) as a laboratory: 
\medskip
\begin{itemize}
\item[\textbullet] Study the effect of fixed and variable costs on liquidity supply
\smallskip
\item[\textbullet] Argue fragmented liquidity can be beneficial to capture passive liquidity supply. 
\end{itemize}
\bigskip
\item Why study an AMM?
\smallskip
\begin{enumerate}
\item They process a large volume of transactions.
\smallskip
\item They seem to provide more liquidity than centralized limit order markets.
\smallskip
\item As real world assets (RWA) move to tokenization models, trading may migrate.
\smallskip
\item Costs/benefits to supplying liquidity is cleaner to observe than in centralized markets.
\end{enumerate}
\end{itemize}
\end{frame}

\begin{frame}\frametitle{Uniswap - Details}
\begin{itemize}
\item UniSwap is a decentralized protocol originally on the Ethereum Blockchain.
\begin{itemize}
\item[\textbullet] Each pool has two assets -- all trades are swaps
\end{itemize}
\bigskip
\item There are three versions of Uniswap (v1,v2,v3)
\medskip
\item Features common to all versions:
\begin{itemize}
\item[\textbullet] Agents choose to supply or demand liquidity
\item[\textbullet] Trade prices automatically calculated as a function of liquidity demand and supply.
\item[\textbullet] Only payoff for liquidity supplier is a \% fee paid by the liquidity demander.
\end{itemize}
\medskip
\item Unique to v3
\begin{itemize}
\item[\textbullet] Variable fees:  Each asset pair can trade in 1, 5, 30 or 100bps pools.
\item[\textbullet] Concentrated liquidity:  Liquidity suppliers can choose the price range over which they supply liquidity 
\end{itemize}
\end{itemize}
\end{frame}


% \begin{frame}\frametitle{Uniswap -- Liquidity Provision v2 \\ A Pool with Ethereum ``E'' and a token ``T''}

% \begin{minipage}{0.35\textwidth}%
% \begin{tikzpicture}
% \draw(0,1) circle(0.5in);
% \draw[thick,dashed](-1.15,0.45)--(1.15,0.45);
% \draw(0,1) node[above]{E};
% \draw(0,0.35) node[below]{T};
% \end{tikzpicture}
% \end{minipage} %
% \begin{minipage}{0.55\textwidth}%
% \begin{itemize}
% \item Liquidity suppliers deposit Eth and T

% \medskip
% \item Liquidity demander who buys the token, removes it from the pool and deposits Eth.
% \item Liquidity demander who sells the token, adds it to the pool and withdraws Eth.

% \bigskip
% \item Liquidity demanders pay a fixed, proportional fee which is passed through to the liquidity suppliers.

% \end{itemize}
% \end{minipage}

% \end{frame}


\begin{frame}{Unique to v3:  Concentrated Liquidity}
\begin{itemize}
    \item On Uniswap v3, liquidity providers can specify price limits on their positions.
    \item If the current pool price (e.g., ``midpoint'') is outside the range, the position does not earn fees.
    \item $\rightarrow$ incentive to re-price the position to capture fees.
\end{itemize}
    \begin{center}
        \includegraphics[width=\textwidth]{Figures/uniswapv3_positions.png}
    \end{center}
\end{frame}

\begin{frame}{Fixed cost of adjusting liquidity (gas fee) on Uniswap v3}
    \begin{center}
        \includegraphics[width=\textwidth]{Figures/Empirics_202308/gas_timeline.png}
    \end{center}
\end{frame}


\begin{frame}\frametitle{Price impact to purchase $\tau$ tokens}

\begin{minipage}{0.25 \textwidth}
\begin{tikzpicture}[scale=0.25]
\draw[thick,->] (0,0)-- (15,0);
\draw[thick,->] (0,0) -- (0,10);
\draw (0,9) node[left]{Numeraire};
\draw(10,0) node[below]{Token};
\draw[dotted,red, thick](0,5)--(1.7,5);
\draw[dotted,red,thick](1.7,5)--(1.7,0);
\draw (0,1.7) node[left]{$n_0$};
\draw (1.7,0) node[below]{$T_1$};
\draw(5,0) node[below]{$ T_0$};
\draw(5,-1.5) node[below] {$\Delta_T$}; 
\draw[dotted,blue,thick](5,0)--(5,1.7);
\draw[dotted,blue,thick](0,1.7)--(5,1.7);
\draw(0,5) node[left]{$n_1$};
\draw plot[smooth] coordinates {(12,0)  (4,2) (0,8)};
\end{tikzpicture}
\end{minipage}
\begin{minipage}{0.15\textwidth}
\hspace{1in}
\end{minipage}
\begin{minipage}{0.5 \textwidth}
\begin{itemize}
\item For $ \tau\rightarrow 0$ the exchange between Eth and the Token is $\frac{N}{T}=v$.
\item For larger trades, the exchange rate is determined by a ``bonding curve.''
\end{itemize}
\end{minipage}

\begin{itemize}
\item For given $N$ and $T$, if liquidity is provided across prices $\left[\frac{v}{(1+r)^2},v(1+r)^2\right]$, you need to deposit $n\left(\tau\right)$ in the pool to remove $\tau$ tokens: \end{itemize}
\begin{eqnarray*}
    \underbrace{\left(T_k-\tau+\frac{L_k}{\sqrt{v}\left(1+r\right)}\right)}_\text{virtual token reserves}\underbrace{\left(T_k v + n\left(\tau\right) +  L_k\frac{\sqrt{v}}{1+r}\right)}_\text{virtual numeraire reserves}=L_k^2.
\end{eqnarray*}
\begin{itemize}
\item As more liquidity is supplied ($L_k \nearrow$), bonding curve shifts out.
\end{itemize}
\end{frame}

% \begin{frame}
% \frametitle{Managing liquidity on DEX is costly}
% \begin{center}
%    \includegraphics[width=\textwidth]{Figures/usp3_mechanism.eps}
% \end{center}
% \end{frame}


\begin{frame}{Liquidity Provision on a DEX}

\bigskip

    \begin{enumerate}
    \item Unique laboratory to study how transaction costs affect the market for liquidity. \vspace{0.05in}
        \item DEX  designed for \textbf{passive} liquidity provision. \vspace{0.05in}
        \item ``\emph{Set-it-and-forget-it}'' liquidity: i.e., what ETFs did for portfolio management. \vspace{0.05in}
        \item On v3 actively managing liquidity is costly:
            \begin{enumerate}
                \item \emph{gas price} from interacting with Ethereum blockchain. \vspace{0.05in}
                \item \emph{time/effort} to monitoring the position.
            \end{enumerate}
        \vspace{0.05in}
        \item How do passive liquidity suppliers manage adverse selection? \vspace{0.05in}
        %\item Economies of scale: small liquidity providers face higher relative costs.\vspace{0.05in}
         
    \end{enumerate}
    \medskip

\citet{demsetz1968}: ``the question that is relevant for efficiency is whether or not the cost is appropriately economized.''  

    
    \end{frame}

\begin{frame}{Related literature}
We contribute to: \vspace{0.1in}
    \begin{itemize}
       \item  a growing literature on decentralized exchanges \citep{LeharParlour2021, caparros2023blockchain, augustin2022reaching, kp2023dex, capponi2023price, CapponiJia2021, BarbonRanaldo2021, HasbrouckRiveraSaleh2022}. \vspace{0.1in}
       \item the literature on optimal routing for retail orders \citep{Battalio2016,Cimon2021, FoucaultMenkveld2008}. \vspace{0.1in}
       \item the literature on make/take fees on  liquidity provision \citep{foucault2013liquidity, YaoYe2018,LiWangYe2021}
       
    \end{itemize}
\end{frame}


\begin{frame}\frametitle{Results}

\vspace{0.1in}

\begin{alertblock}{Theory and  evidence of LP ``clienteles'' based on their scale:}
\bigskip

\begin{enumerate}
    \item Small LPs are more passive: fill rates $\downarrow$, but adverse selection \& rebalancing cost $\downarrow$. 
    \item Large LPs are more active: fill rates $\uparrow$, but adverse selection \& rebalancing cost $\uparrow$. 
    \item This segmentation can be efficient
\end{enumerate}


\end{alertblock}

\end{frame}

% \begin{frame}{Related literature}
% We contribute to: \vspace{0.1in}
%     \begin{itemize}
%        \item  a growing literature on decentralized exchanges \citep{LeharParlour2021, caparros2023blockchain, augustin2022reaching, kp2023dex, capponi2023price, CapponiJia2021, BarbonRanaldo2021, HasbrouckRiveraSaleh2022}. \vspace{0.1in}
%        \item the literature on optimal routing for retail orders \citep{Battalio2016,Cimon2021, FoucaultMenkveld2008}. \vspace{0.1in}
%        \item the literature on make/take fees on  liquidity provision \citep{foucault2013liquidity, YaoYe2018,LiWangYe2021}
       
%     \end{itemize}
% \end{frame}

\begin{frame}{Model}
\begin{block}{Asset and markets.} \begin{itemize}
    \item Token with expected value $v_t$ trades on two liquidity pools with fees $h>\ell>0$.
    \item Fixed cost $\Gamma>0$ of interacting with the pool (e.g., gas fee).
\end{itemize}
\end{block}

\begin{block}{Liquidity providers (\textbf{LP})}
\begin{itemize}
\item Risk-neutral
\item Post liquidity on at most one pool between prices $\frac{v_t}{\left(1+r\right)^2}$ and $v_t\left(1+r\right)^2$.
\item Token endowments $q_i$; $q_i$ follows an exponential distribution with scale $\lambda$.
\end{itemize}
\end{block}

\begin{block}{Liquidity takers}
\begin{itemize}
    \item Value shock $v\left(1+\tilde{\delta}\right)$, where $\tilde{\delta}$ has density $\phi\left(\delta\right)=\frac{1}{2\Delta \sqrt{1+\delta}} \; \; \text{ for } \delta\in\left[0,\Delta^2-1\right]$.
    \item With rate $\eta$, shock is {\color{red} common value} (news). Aggressive orders are arbitrageurs \textbf{A}. 
    \item Otherwise, shock is {\color{blue} private value}. Aggressive orders are liquidity traders \textbf{LT}.
\end{itemize}
\end{block}

\end{frame}

\begin{frame}{Optimal trade size: minimize price impact and fees}

\begin{equation*}\label{eq:optimal_trade_size}
    \tau^\star\left(\delta\right)=T_k\min\left\{1,\frac{1+r}{r}\max\left\{0,1-\sqrt{\frac{1+f_k}{1+\delta}}\right\}\right\}.
\end{equation*}


    \small
    \begin{tikzpicture}[scale=0.86]
    % Draw the vertical lines
    \draw[|->, thick] (0,0) -- (15.75,0);
    \draw[|->, thick] (0,1.5) -- (15.75,1.5);

    \node at (15.75,0.5) {Pool H};
    \node at (15.75, 2) {Pool L};

    \node[align=left] at (1.5, 0.75) {$\LP$s deposit $q_i$ \\ in pool $k\in\left\{L,H\right\}$};

    \draw[->,blue] (1,2)--(1,1.5);
    \node[blue, align=center] at (1,2.4) {Small \\ LT};

    \draw[->,blue] (2.5,2)--(2.5,1.5);
    \node[blue, align=center] at (2.5,2.4) {Small \\ LT};

    \draw[->,blue,thick] (4,2)--(4,1.5);
    \draw[->,blue,thick] (4,1.5)--(4,0);
    \node[blue, align=center] at (4,2.4) {\bfseries Large \\ \bfseries LT};

    \draw[dotted,thick,red] (4.5,1.5) -- (4.5, 0);
    \node[red, align=left] at (5.25,0.75) {News \\ $\tilde{\delta}\in\left(\ell,h\right)$}; 

    \draw[->,red] (6,2)--(6,1.5);
    \node[red, align=left] at (6,2.4) {\textbf{A} trades \\ on pool $L$};

    \draw[->,thick](8,2)--(8,1.5);
    \node[align=center] at (8,2.4) {$\LP$ rebalance \\ on pool $L$};

    \draw[->,blue,thick] (9.75,2)--(9.75,1.5);
    \draw[->,blue,thick] (9.75,1.5)--(9.75,0);
    \node[blue, align=center] at (9.75,2.4) {\bfseries Large \\ \bfseries LT};


    \draw[->,blue] (10.75,2)--(10.75,1.5);
    \node[blue, align=center] at (10.75,2.4) {Small \\ LT};

    \draw[dotted,thick,red] (11.25,1.5) -- (11.25, 0);
    \node[red, align=center] at (11.75,0.75) {News \\ $\tilde{\delta}>h$}; 

    \draw[->,red] (12.5,2)--(12.5,1.5);
    \draw[->,red] (12.5,1.5)--(12.5,0);
    \node[red, align=left] at (12.5,2.6) {\textbf{A} trades \\ on both \\ pools};

    \draw[->,thick](14.75,2)--(14.75,1.5);
    \draw[->,thick](14.75,1.5)--(14.75,0);
    \node[align=left] at (14.75,2.6) {$\LP$ rebalance \\ on both \\ pools};

    
\end{tikzpicture}

\begin{itemize}
    \item Liquidity trades are immediately reversed by arbitrageurs \citep{LeharParlour2021}; \vspace{0.1in}
    \item News trades have permanent price impact. \vspace{0.1in}
    \item Large news trades ($\delta>(1+f_k)(1+r)^2-1$) exhaust available liquidity supply \\ $\Rightarrow$ costly re-balancing by \textbf{LP}s. \vspace{0.1in}
\end{itemize}

\end{frame}

\begin{frame}{Optimal order routing in practice}
    \begin{center}
        \includegraphics[width=\textwidth]{Figures/Empirics_202308/optimal_routing.png}
    \end{center}
\end{frame}



\begin{frame}{Liquidity provider' choice}
Choose pool to maximize expected profit:
\begin{equation*}
    \max_{f\in\left\{\ell,h,\emptyset\right\}} q_i \left[\left(1-\eta\right) \mathcal{L}\left(f\right)-\eta \mathcal{A}\left(f\right)\right]-\eta \Gamma\left(1-\frac{\sqrt{1+f}\left(1+r\right)}{\Delta}\right),
\end{equation*}
where
\begin{itemize}
    \item $\mathcal{L}\left(f\right)$: liquidity yield on pool with fee $f$;
    \item $\mathcal{A}\left(f\right)$: adverse selection on pool with fee $f$;\vspace{0.1in}
\end{itemize}

    \begin{centering}
    \includegraphics[width=\textwidth]{slides/Figures/liqrev_advsel_may2024_narrow.png}
    \par\end{centering}
\end{frame}

\begin{frame}{Equilibrium regions}
    \begin{centering}
    \includegraphics[width=\textwidth]{../Figures/eq_regions_may2024}
    \par\end{centering}
\end{frame}

\begin{frame}{Fragmented equilibrium}
\begin{itemize}
\item $\LP$s with endowment $\underline{q}_h$ do not supply liquidity.
\item There is a threshold endowment $\qmg$ such that all $\LP$s with $q_i>\qmg$ post liquidity on the low-fee pool and all $\LP$s with $q_i\leq \qmg$ choose the high-fee pool. Market share:
\begin{equation*}
w_\ell=\frac{\exp\left(-\frac{\qmg-\underline{q}_h}{\lambda}\right)\left(\qmg+\lambda\right)}{\underline{q}_h+\lambda} \leq 1,
\end{equation*}
\end{itemize}
\bigskip
% \begin{center}
% \begin{tikzpicture}[scale= 0.5]
%     \draw[thick] (0,0)--(15,0);
%     \draw[thick] (10,0)--(10,1);
%     \draw[thick] (15,0)--(15,1);
%     \draw[thick] (0,0)--(0,1);
%     \draw[thick] (5,0)--(5,1);
%     \draw[thick] node[below]{$1$};
%     \draw[thick] (5,0) node[below]{$\underline q$};
%     \draw[thick] (10,0) node[below]{$q_t$};
%     \draw[thick] (15,0) node[below]{Q};
%     \draw[thick] (2.5,0) node[above]{out};
%     \draw[thick] (7.5,0) node[above]{high};
%     \draw[thick] (12.5,0) node[above]{low};
% \end{tikzpicture}
% \end{center}
    \begin{centering}
    \includegraphics[width=\textwidth]{slides/Figures/clienteles_may2024}
    \par\end{centering}
\end{frame}


\begin{frame}{Gas cost and liquidity supply}
    \begin{centering}
    \includegraphics[width=\textwidth]{../Figures/mkt_share_gas_may2024}
    \par\end{centering}
\end{frame}

\begin{frame}\frametitle{Evaluating the fragmented liquidity}
\begin{block}{Proposition}
From any single fee pool, you can find a fragmented pool that increases the expected gains from trade, $\mathbb{E}\sum_k \delta T_k \tau^\star_k$.
\end{block}

\begin{enumerate}
    \medskip
\item Set the high fee equal to the single-pool fee: $h=f$ (same {\bfseries LP} participation).
\item Introduce a lower fee pool $\ell<h$ such that large {\bfseries LP} migrate there.
\bigskip
\end{enumerate}
    \begin{centering}
    \includegraphics[width=\textwidth]{slides/Figures/gft_may2024.png}
    \par\end{centering}
\end{frame}


\begin{frame}{Data}
\begin{itemize}
    \item Data from Uniswap v3 Subgraph on all trades, liquidity deposits and withdrawals from May 4, 2021 until July 15, 2023, including traders' wallet addresses. \vspace{0.1in}
    \item Gas cost is the average of the lowest daily 1000 gas prices for mint events. \vspace{0.1in}
    \item Focus on economically sizeable pools:
    \begin{enumerate}
        \item active in more than 100 days within the sample;
        \item 500+ liquidity events throughout the sample;
        \item average daily liquidity balance $>$US\$100,000;
        \item $>$1\% of volume for a traded pair.
    \end{enumerate} \vspace{0.1in}
    \item We obtain 274 pools in 242 asset pairs:
    \begin{enumerate}
        \item aggregate daily volume of US\$~1.12bn;
        \item end-of-sample aggregate liquidity US\$~2.53bn.
        \item account for 86.04\% of all Uniswap v3 interactions.
    \end{enumerate}
\end{itemize}
\end{frame}

\begin{frame}{Uniswap v3 pairs can be traded in 1, 5, 30, or 100 bps fee pools}
\begin{itemize}
    \item 32 fragmented pools collectively account for 95\% of committed liquidity and 93\% of traded volume
    \item Trading concentrates on adjacent fee levels e.g.:  \\ USDC/USDT 1-5bps, ETH/USDC 5-30bps, USDC-CRV 30-100bps
\end{itemize}
\bigskip
\begin{enumerate}
    \item Significant fragmentation across different-fee pools for the same pair.
    \item Low-fee pools are more actively traded, but high-fee pools are deeper.
    \begin{center}
        \includegraphics[width=0.9\textwidth]{Figures/sumstat_TVL_volume.png}
    \end{center}
%\item We show that fixed transaction costs partly drive this effect.
\end{enumerate}
\end{frame}

\begin{frame}{Liquidity clienteles: high fee pools feature many small \textbf{LP}s.}
    \begin{center}
        \includegraphics[width=\textwidth]{Figures/sumstat_mint_trade.png}
        \includegraphics[width=\textwidth]{Figures/sumstat_wallets.png}
    \end{center}
\end{frame}

\begin{frame}{Low-fee pools: Larger mints, fewer LP wallets, many small trades.\\ (Mints and Trades in log USD)}
\begin{center}


\scalebox{0.73}{
\begin{tabular}{lccccccc}
\toprule
 & \multicolumn{1}{c}{Mint size} &  \multicolumn{1}{c}{Trade size} & \multicolumn{1}{c}{Volume} & \multicolumn{1}{c}{\# Trades}  & \multicolumn{1}{c}{\# Wallets} & \multicolumn{1}{c}{Liquidity yield} & \multicolumn{1}{c}{Price range} \\
 & (1) & (2) & (3) & (4) & (5) & (6) & (7) \\
\rowcolor{red!20} 
$ d_\text{low-fee}$ & 0.73*** & -0.30*** & 0.89*** & 1.02*** & -3.40*** & 2.03*** & -0.18*** \\
\rowcolor{red!20}
 & (12.27) & (-10.05) & (14.23) & (32.95) & (-5.00) & (3.60) & (-41.84) \\
Gas price $\times$ $ d_\text{low-fee}$ & 0.37*** & 0.08*** & -0.03 & -0.22*** & -3.00*** & 3.57** & -0.00 \\
 & (4.96) & (3.75) & (-0.95) & (-7.29) & (-3.43) & (2.30) & (-0.47) \\
Gas price $\times$ $ d_\text{high-fee}$ & 0.58*** & 0.17*** & 0.24*** & 0.07** & -2.89*** & 5.57*** & -0.03*** \\
 & (7.52) & (8.81) & (5.95) & (2.46) & (-3.15) & (2.83) & (-4.65) \\
Volume & 0.37*** & 0.16*** & 0.43*** & 0.20*** & 1.22*** & 1.01 & -0.01** \\
 & (8.68) & (21.38) & (15.27) & (13.85) & (6.56) & (0.81) & (-2.56) \\
Total value locked & -0.16 & 0.11*** & 0.23** & -0.01 & -1.86 & -13.42 & -0.02 \\
 & (-1.30) & (3.54) & (1.99) & (-0.18) & (-0.99) & (-1.09) & (-0.99) \\
Volatility & -0.04 & -0.01 & -0.07 & 0.01 & -0.09 & 1.18** & 0.02*** \\
 & (-1.11) & (-1.34) & (-1.38) & (0.88) & (-1.03) & (2.21) & (3.98) \\
Constant & 1.88*** & 1.64*** & 5.27*** & 3.26*** & 10.12*** & 10.01*** & 0.59*** \\
 & (58.27) & (111.47) & (168.58) & (209.84) & (28.65) & (26.04) & (184.91) \\
Observations & 21,000 & 36,059 & 36,059 & 40,288 & 40,288 & 40,252 & 24,058 \\
 R-squared & 0.26 & 0.53 & 0.55 & 0.52 & 0.37 & 0.09 & 0.42 \\ \hline
\bottomrule
\end{tabular}
}
\end{center}
\end{frame}


\begin{frame}{Do gas prices move market shares?}
\begin{center}
    

\scalebox{0.82}{
\begin{tabular}{lccc@{\hskip 0.3in}ccc}
\toprule
 & \multicolumn{3}{c}{Liquidity market share (\%)} & \multicolumn{3}{c}{Volume market share (\%)} \\ 
 \cmidrule{1-7}
\rowcolor{red!20} $ d_\text{low-fee}$ & -20.92*** & -20.92*** & -20.92*** & 24.62*** & 24.63*** & 24.62*** \\
 & (-27.42) & (-27.41) & (-27.42) & (20.55) & (20.56) & (20.55) \\
\rowcolor{red!20} Gas price $\times$ $ d_\text{low-fee}$ & -4.63*** & -4.62*** & -4.63*** & -6.52*** & -6.52*** & -6.52*** \\
 & (-7.32) & (-7.32) & (-7.32) & (-5.92) & (-5.92) & (-5.92) \\
Gas price & 2.31*** & 2.31*** & 2.31*** & 3.63*** & 3.61*** & 3.61*** \\
 & (7.32) & (7.32) & (7.32) & (7.33) & (7.30) & (7.26) \\
Volume & 0.00 & 0.00 & 0.00 & -0.19** & -0.20** & -0.19** \\
 & (0.65) & (1.33) & (0.65) & (-2.54) & (-2.61) & (-2.50) \\
Total value locked & -0.00 & -0.00 &  & 0.58 & 0.58 &  \\
 & (-0.58) & (-0.06) &  & (1.44) & (1.44) &  \\
Volatility & -0.29 &  & -0.29 & -1.15*** &  & -1.15*** \\
 & (-0.90) &  & (-0.90) & (-2.74) &  & (-2.74) \\
Constant & 60.45*** & 60.46*** & 60.45*** & 41.96*** & 41.99*** & 41.96*** \\
 & (158.00) & (158.46) & (158.00) & (69.99) & (70.22) & (70.02) \\
Observations & 40,288 & 40,288 & 40,288 & 36,059 & 36,059 & 36,059 \\
 R-squared & 0.10 & 0.10 & 0.10 & 0.13 & 0.13 & 0.13 \\ \hline
\bottomrule
\end{tabular}



}
\end{center}
\end{frame}



\begin{frame}{Liquidity flows and gas prices}
\begin{center}
    

\scalebox{0.77}{
\begin{tabular}{lcccccc}
\toprule
 & \multicolumn{3}{c}{Daily mints (log US\$)} &  \multicolumn{3}{c}{$\text{Prob}\left(\text{at least one mint}\right)$} \\
\cmidrule{1-7}
$ d_\text{low-fee}$ & 0.43*** & 0.43*** & 0.43*** & 1.38* & 1.37* & 1.38* \\
 & (6.07) & (6.07) & (6.07) & (1.71) & (1.71) & (1.71) \\
\rowcolor{LRed} Gas price $\times$ $ d_\text{low-fee}$ & -0.35*** & -0.35*** & -0.46*** & -6.02*** & -6.01*** & -4.58*** \\
\rowcolor{LRed} & (-8.50) & (-8.50) & (-7.14) & (-9.13) & (-9.13) & (-6.76) \\
\rowcolor{LRed} Gas price $\times$ $ d_\text{high-fee}$ & 0.11** & 0.11** &  & -1.43** & -1.43** &  \\
\rowcolor{LRed} & (2.15) & (2.15) &  & (-2.57) & (-2.57) &  \\
Volume & 0.26*** & 0.26*** & 0.26*** & 0.96*** & 0.96*** & 0.96*** \\
 & (14.78) & (14.77) & (14.78) & (3.93) & (3.93) & (3.93) \\
Total value locked & -0.07 & -0.07 & -0.07 & 1.47 & 1.47 & 1.47 \\
 & (-0.78) & (-0.78) & (-0.78) & (1.01) & (1.00) & (1.01) \\
Volatility & -0.01 &  & -0.01 & 0.26 &  & 0.26 \\
 & (-0.68) &  & (-0.68) & (0.59) &  & (0.59) \\
Gas price &  &  & 0.11** &  &  & -1.43** \\
 &  &  & (2.15) &  &  & (-2.57) \\
Constant & 2.61*** & 2.61*** & 2.61*** & 51.44*** & 51.43*** & 51.44*** \\
 & (73.46) & (73.49) & (73.46) & (126.67) & (127.28) & (126.67) \\
Observations & 40,288 & 40,288 & 40,288 & 40,288 & 40,288 & 40,288 \\
 R-squared & 0.47 & 0.47 & 0.47 & 0.28 & 0.28 & 0.28 \\ \hline
\bottomrule
\end{tabular}
}
\end{center}
\end{frame}

\begin{frame}{$\LP$s rebalance more often on low-fee pools}
\includegraphics[width=0.9\textwidth]{Figures/time_elapsed_distribution.png}
\includegraphics[width=0.9\textwidth]{Figures/out_of_range_distribution.png}
\end{frame}


\ifthenelse{\boolean{longtalk}}{%
\begin{frame}{Adverse selection and liquidity yield on decentralized pools}

\begin{block}{Loss-versus-rebalancing \citep{zhang2023amm}}
    \begin{itemize}
        \item A measure of adverse selection cost. For each swap $j$, we compute:
            \begin{eqnarray*}
                \text{LVR}_{j}=\underbrace{d_j}_{\substack{\text{swap}\\\text{direction}}} \times \underbrace{\Delta x_j}_{\substack{\text{swap}\\\text{quantity}}} (p_{\text{swap},j}-\underbrace{p^\prime_j}_{\substack{\text{benchmark}\\\text{price}}})
            \end{eqnarray*}
        \item Benchmark prices: 
            \begin{enumerate}
                \item Pool price immediately after swap: captures {\color{blue} temporary} \& {\color{red} permanent} price impact.
                \item Pool price at 1 hour after swap: captures only {\color{red} permanent} price impact. 
            \end{enumerate}
    \end{itemize}
\end{block}

\begin{block}{Liquidity yield}
 Liquidity yield is computed as in \citet{augustin2022reaching}:
\begin{equation}\label{eq:liq_yield}
    \text{Liquidity yield}=\text{liquidity fee}_i \times \frac{\text{Volume}_{i,t}}{\text{TVL}_{i,t-1}},
\end{equation}   
\end{block}
\end{frame}
}

\ifthenelse{\boolean{longtalk}}{%
\begin{frame}{Low-fee pools have higher adverse selection cost}
\begin{center}

\begin{itemize}
    \item Higher LVR on low-fee pools \citep{milionis2023automated}
    \item Similar deviations from Binance prices among low- and high-fee pools.
\end{itemize}

\medskip

\scalebox{0.67}{
\begin{tabular}{lcccccccc}
\toprule
& \multicolumn{2}{c}{LVR (1h horizon)} & \multicolumn{2}{c}{LVR (after swap)} & \multicolumn{2}{c}{Impermanent loss} & \multicolumn{2}{c}{CEX price deviation} \\
& \multicolumn{2}{c}{Permanent price impact} & \multicolumn{2}{c}{Total price impact} \\
\cmidrule{1-9} 
 & (1) & (2) & (3) & (4) & (5) & (6) & (7) & (8)  \\
\cmidrule{1-9}
\rowcolor{LRed} $ d_\text{low-fee}$ & 6.39*** & 6.39*** & 29.78*** & 29.67*** & 1.08*** & 1.13*** & 0.06 & 0.04 \\
\rowcolor{LRed} & (16.57) & (17.05) & (14.86) & (14.95) & (5.72) & (6.18) & (1.51) & (1.33) \\
Gas price $\times$ $ d_\text{low-fee}$ &  & -0.75** &  & 3.51** &  & -0.01 &  & 0.08 \\
 &  & (-2.05) &  & (2.10) &  & (-0.05) &  & (1.09) \\
Gas price &  & 2.61*** &  & 6.16** &  & 3.71*** &  & -0.03 \\
 &  & (2.74) &  & (2.53) &  & (3.76) &  & (-0.28) \\
Volume &  & 3.22*** &  & 8.67*** &  & 1.81*** &  & 0.22*** \\
 &  & (8.15) &  & (6.61) &  & (6.22) &  & (4.74) \\
Total value locked &  & 0.53 &  & -2.12 &  & 1.93 &  & -0.39*** \\
 &  & (0.14) &  & (-0.34) &  & (0.74) &  & (-4.05) \\
Volatility &  & 1.85*** &  & 4.23*** &  & 6.69** &  & 1.04*** \\
 &  & (2.87) &  & (3.17) &  & (2.61) &  & (3.51) \\
Constant & 7.85*** & 7.86*** & 8.88*** & 8.97*** & 7.37*** & 7.51*** & 0.60*** & 0.67*** \\
 & (40.71) & (36.89) & (8.87) & (8.88) & (77.84) & (61.32) & (30.71) & (35.75) \\
Observations & 40,302 & 40,288 & 40,302 & 40,288 & 40,250 & 40,248 & 5,207 & 5,207 \\
 R-squared & 0.14 & 0.15 & 0.09 & 0.10 & 0.09 & 0.11 & 0.10 & 0.11 \\ \hline
\bottomrule
\end{tabular}

}
\end{center}
\end{frame}}
{\begin{frame}{Is order flow on high-fee pools more toxic?}
\begin{center}
    

\scalebox{0.75}{
\begin{tabular}{lcccccccc}
\toprule
& \multicolumn{8}{c}{Impermanent loss for a liquidity position with range $\left[\frac{p}{\alpha}, \alpha p\right]$ around price $p$} \\
\cmidrule{1-9} 
& \multicolumn{2}{c}{$\alpha=1.01$} & \multicolumn{2}{c}{$\alpha=1.05$} & \multicolumn{2}{c}{$\alpha=1.10$} & \multicolumn{2}{c}{$\alpha=1.25$} \\
\cmidrule{1-9}
 $ d_\text{low-fee}$ & \cellcolor{red!20} 2.59*** & -1.38 & 1.08*** & -1.85** & 0.71*** & -1.56** & 0.37** & -1.09* \\
 & (11.26) & (-1.57) & (5.72) & (-2.28) & (4.28) & (-2.18) & (2.58) & (-1.98) \\
Gas price &  & 4.75*** &  & 3.68*** &  & 2.72*** &  & 1.55*** \\
 &  & (3.97) &  & (3.96) &  & (3.86) &  & (3.42) \\
Trade count &  & 4.82*** &  & 3.56*** &  & 2.78*** &  & 1.79*** \\
 &  & (4.59) &  & (3.71) &  & (3.30) &  & (2.83) \\
Volume &  & 3.03*** &  & 1.19*** &  & 0.60** &  & 0.22 \\
 &  & (7.00) &  & (3.87) &  & (2.45) &  & (1.25) \\
Total value locked &  & 0.43 &  & 1.78 &  & 2.02 &  & 1.83 \\
 &  & (0.16) &  & (0.79) &  & (1.05) &  & (1.38) \\
Volatility &  & 6.98*** &  & 6.65** &  & 6.39** &  & 6.06** \\
 &  & (2.69) &  & (2.59) &  & (2.51) &  & (2.40) \\
Constant & 15.52*** & 15.87*** & 7.37*** & 7.65*** & 4.63*** & 4.87*** & 2.45*** & 2.66*** \\
 & (134.72) & (103.02) & (77.84) & (60.07) & (55.47) & (43.73) & (34.58) & (29.33) \\
Observations & 40,250 & 40,248 & 40,250 & 40,248 & 40,250 & 40,248 & 40,250 & 40,248 \\
 R-squared & 0.17 & 0.23 & 0.09 & 0.15 & 0.06 & 0.11 & 0.03 & 0.08 \\ \hline
\bottomrule
\end{tabular}
}
\end{center}
\end{frame}}

\begin{frame}{Price impact \& liquidity yield across fragmented pools}

    \begin{center}
        \includegraphics[width=\textwidth]{Figures/Empirics_202308/lvr.png}
    \end{center}
\end{frame}

\begin{frame}{Conclusion}
    \takeaways
\end{frame}




\appendix
\begin{frame}<beamer:0> [noframenumbering]
\bibliographystyle{jf}
\bibliography{references}
\end{frame}


\end{document}
